On regularity of maximal distance minimizers

We study the properties of sets $\Sigma$ which are the solutions of the maximal distance minimizer problem, id est of sets having the minimal length (one-dimensional Hausdorff measure) over the class of closed connected sets $\Sigma \subset \mathbb{R}^2$ satisfying the inequality $\max_{y \in M} dist(y,\Sigma) \leq r$ for a given compact set $M \subset \mathbb{R}^2$ and some given $r > 0$. Such sets can be considered as the shortest networks of radiating cables arriving to each customer (from the set $M$ of customers) at a distance at most $r$. In this work it is proved that each maximal distance minimizer is a union of finite number of simple curves, having one-sided tangents at each point. Moreover the angle between these rays at each point of a maximal distance minimizer is greater or equal to $2\pi/3$. It shows that a maximal distance minimizer is isotopic to a finite Steiner tree even for a "bad" compact $M$, which differs it from a solution of the Steiner problem (there exists an example of a Steiner tree with an infinite number of branching points). Also we classify the behavior of a minimizer in a neighbourhood of an arbitrary point of $\Sigma$. In fact, all the results are proved for more general class of local minimizer, id est sets which are optimal in a neighbourhood of its arbitrary point.

==> 2_5examples.tex <==
\section{Полная классификация локального поведения $\Sigma$. Примеры} \label{ex}

Напомним, что $\Sigma$ является минимайзером функционала максимального расстояния для плоского компакта $M$.
Нас интересует вопрос о поведении множества $\Sigma$ в окрестности точки $x \in \Sigma$.
Из доказательства Теоремы~\ref{mainT1} следует полная классификация вариантов локального поведения $\Sigma$. Мы приведем примеры для каждого из возможных вариантов.% На рисунках заданные множества $M$ обозначаются зеленым цветом, энергетические точки минимайзера $\Sigma$ --- красным, остальные точки множества %$\Sigma$ --- фиолетовым. 

Обычно достаточно сложно доказать, что конкретное множество $\Sigma$ является минимайзером для конкретного $M$. На иллюстрации~\ref{horseFig} множество $M$ --- окружность радиуса $R > r$, а множество $\Sigma$ --- объединение дуги окружности радиуса $R-r$ и двух отрезков касательных к этой окружности. Миранда, Степанов и Паолини~\cite{mir} предположили, что $\Sigma$ --- минимайзер для $M$. 
Доказательство того, что множество $\Sigma$ является минимайзером при условии $R > 4.98r$, можно найти в работе~\cite{cherkashin2015horseshoe}.

Стоит отметить, что если $M$ является конечным множеством точек, то существует простой критерий: связное множество $\Sigma$ является минимайзером для $M$ и числа $r>0$, если выполняется неравенство $\H(\Sigma) \leq \H(St(M))-r \sharp{M}$, где $\sharp{M}$ --- количество элементов множества $M$, а $St(M)$ --- связное множество с наименьшей длиной, содержащее все точки $M$ (иначе говоря,  произвольное дерево Штейнера для множества $M$). Несложно также заметить, что строгое неравенство в этом выражении невозможно. Этот критерий показывает, что в примерах на Рис.~\ref{X2},~\ref{X1ill},~\ref{X2non120} множество $\Sigma$ действительно минимайзер. 

Из Теорем~\ref{mainT1} и~\ref{persp} следует Теорема о классификации локального поведения минимайзера в произвольной точке.

\begin{theorem2}

Пусть $\Sigma$ --- минимайзер максимального расстояния, содержащий хотя бы две точки. Тогда
\begin{enumerate}
\item  Если $x \in S_\Sigma$, то найдется такое $\varepsilon > 0$, что $\Sigma \cap B_{\varepsilon}(x)$ является одним из двух множеств:
%(см свойства минимайзеров~\ref{g})
\begin{enumerate}
\item отрезком %, и в этом случае точка $x$ имеет порядок $2$ 
 (точка $S$ на Рис.~\ref{horseFig},~\ref{X2},~\ref{ElimX},~\ref{X1ill},~\ref{X2non120});
\item правильной треногой %, и в этом случае точка $x$ имеет порядок $3$ 
 (точка $F$ на Рис.~\ref{X1ill}).
\end{enumerate} 

\item Если $x \in X_\Sigma$, то найдется такое $\varepsilon > 0$, что $\Sigma \cap B_{\varepsilon}(x)$ является одним из двух множеств:
%(cм Утверждение~\ref{discr_str}) 
\begin{enumerate}
\item отрезком с концом в $x$ %, то есть точка $x$ имеет порядок $1$
 (точка $D$ на Рис.~\ref{horseFig},~\ref{X2},~\ref{ElimX},~\ref{X1ill},~\ref{X2non120});
\item объединением двух отрезков с концами в $x$ и углом большим (точка $E$ на Рис.~\ref{X2non120} и Рис.~\ref{ElimX}) или равным (точка $E$ на Рис.~\ref{X2}) $2\pi/3$, между ними.%, и в этом случае точка $x$ имеет порядок $2$.
\end{enumerate}


\item  Если $x \in E_\Sigma$, то найдется такое $\varepsilon > 0$, что $\Sigma \cap B_{\varepsilon}(x)$ является одним из двух множеств:
\begin{enumerate}
\item дугой с концом в $x$, имеющей в этой точке одностороннюю касательную. % (в этом случае точка $x$ имеет порядок $1$).
При этом точка $x$ может
\begin{enumerate}
\item являться предельной точкой множества $X_\Sigma$ (точка $G$ на Рис.~\ref{ElimX});
\item не являться предельной точкой множества $X_\Sigma$ (точка $G$ на Рис.~\ref{E1}).
\end{enumerate}

\item объединением двух отрезков дуг с концами в $x$, имеющих в этой точке односторонние касательные с углом, не меньшим $2\pi/3$, между ними %; в этом случае %точка $x$ имеет порядок $2$ 
 (точки $H_1$ и $H_2$ на Рис.~\ref{horseFig} и точка $H_2$ на Рис.~\ref{E1}).
\end{enumerate}
\end{enumerate}

\end{theorem2}


\input{pictures/horseshoe}
\input{pictures/X2}
\input{pictures/ElimX}
\input{pictures/X1ill}
\input{pictures/X2non120}
\input{pictures/E1}

%\begin{figure}[H]
%\begin{subfigure}[width=0.25\linewidth]
%\input{pictures/horseshoe}
%\end{subfigure}
%\begin{subfigure}[width=0.25\linewidth]
%\input{pictures/horseshoe}
%\end{subfigure}
%\end{figure}

%https://ru.wikipedia.org/wiki/%D0%92%D0%BF%D0%BE%D0%BB%D0%BD%D0%B5_%D0%BD%D0%B5%D1%81%D0%B2%D1%8F%D0%B7%D0%BD%D0%BE%D0%B5_%D0%BF%D1%80%D0%BE%D1%81%D1%82%D1%80%D0%B0%D0%BD%D1%81%D1%82%D0%B2%D0%BE
%https://ru.wikipedia.org/wiki/%D0%92%D0%BF%D0%BE%D0%BB%D0%BD%D0%B5_%D0%BD%D0%B5%D1%81%D0%B2%D1%8F%D0%B7%D0%BD%D0%BE%D0%B5_%D0%BF%D1%80%D0%BE%D1%81%D1%82%D1%80%D0%B0%D0%BD%D1%81%D1%82%D0%B2%D0%BE

Приведем пример ``плохого'' множества $M$:
\begin{example}
Пусть $M$ --- компактное вполне несвязное множество, дерево Штейнера для которого обладает бесконечным числом точек степени 3. 
Явный пример такого множества $M$ был построен в работе~\cite{paolini2015example}.
В то же время из результатов анонсируемой статьи следует, что для любого числа $r < \diam M$ минимайзер будет содержать конечное число точек ветвления. 
\end{example}



%Интересно может ли быть не прямолинейный отрезок
%\input{pictures/X2}

==> e_2_5examples.tex <==
\section{Classification of minimizer's local behavior. Examples.} \label{ex}

Recall, that $\Sigma$ is a maximal distance minimizer for a flat compact $M$. We are interested in the behavior of the set $\Sigma$ near $x \in \Sigma$.
 
Usually it is not easy to prove that a certain set is a minimizer. At the figure~\ref{horseFig} the set $M$ is a circle of radius $R > r$. The set $\Sigma$, depicted at the figure is a union of an arc of the circumference of radius $R-r$ and two segments tangent to this circumference. One can find the proof of the fact that $\Sigma$ is a minimizer in the case $R>5r$ in the work~\cite{cherkashin2015horseshoe}.

Note that if $M$ is a finite set of points there is an easy criterion: a connected set $\Sigma$ is a minimizer for a set $M$ and a number $r>0$, if the inequality $\H(\Sigma) \leq \H(St(M))-r \sharp{M}$ holds, where $\sharp{M}$ is a quantity of elements of set $M$, and $St(M)$ is an arbitrary Steiner set for $M$. It is easy to show that strong inequality can not be true. This criterion shows that at Fig.~\ref{X2},~\ref{X1ill},~\ref{X2non120} the set $\Sigma$ is a minimizer. 

Theorems~\ref{mainT1} and~\ref{persp} imply the classification of all possibilities for the local behavior of $\Sigma$. We will give an example for each possible case.

%Из Теорем~\ref{mainT1} и~\ref{persp} следует Теорема о классификации %локального поведения минимайзера в произвольной точке.

\begin{theorem2}

Let $\Sigma$ be a maximal distance minimizer contaning at least two point. Then 
\begin{enumerate}
\item  If $x \in S_\Sigma$, there exists such $\varepsilon > 0$, that $\Sigma \cap B_{\varepsilon}(x)$ coincides with one of two sets: 
\begin{enumerate}
\item a segment %, и в этом случае точка $x$ имеет порядок $2$ 
 (point $S$ at Fig.~\ref{horseFig},~\ref{X2},~\ref{ElimX},~\ref{X1ill},~\ref{X2non120});
\item a regular tripod  %, и в этом случае точка $x$ имеет порядок $3$ 
 (point $F$ at Fig.~\ref{X1ill}).
\end{enumerate} 

 If $x \in X_\Sigma$, there exists such $\varepsilon > 0$ that $\Sigma \cap B_{\varepsilon}(x)$  coincides with one of two sets:
\begin{enumerate}
\item a segment with an end at $x$ (point $D$ at Fig.~\ref{horseFig},~\ref{X2},~\ref{ElimX},~\ref{X1ill},~\ref{X2non120});
\item a union of two segments with common end at $x$ and an angle greater (point $E$ at Fig.~\ref{X2non120}) or equal (point $E$ at Fig.~\ref{X2}) to $2\pi/3$ between them.  
\end{enumerate}
\item  For $x \in E_\Sigma$  there exists such $\varepsilon > 0$ that $\Sigma \cap B_{\varepsilon}(x)$ coincides with one of two sets:
\begin{enumerate}
\item an arc with an end at $x$ having in this point a one-sided tangent line. Herewith $x$ can 
\begin{enumerate}
\item be a limit of points from  $X_\Sigma$ (point $G$ at Fig.~\ref{ElimX});
\item not be a limit of points from $X_\Sigma$ (point $G$ at Fig.~\ref{E1}).
\end{enumerate}

\item a union of two arcs with a common end at the point $x$, having in this point the one-sided tangent lines with angle greater or equal to $2\pi/3$ between them (points $H_1$ and $H_2$ at Fig.~\ref{horseFig} and point $H_2$ at Fig.~\ref{E1}).
\end{enumerate}
\end{enumerate}

\end{theorem2}


\input{e_shortparts/horseshoe}
\input{e_shortparts/X2}
\input{e_shortparts/ElimX}
\input{e_shortparts/X1ill}
\input{e_shortparts/X2non120}
\input{e_shortparts/E1}

Let us give an example of a ``bad'' set $M$:
%Приведем пример ``плохого'' множества $M$:
\begin{example}
Let $M$ be a totally disconnected compact set such that the unique Steiner tree connecting it has an infinite number branching points. An explicit example of such a set was constructed in the work~\cite{paolini2015example}. The results of the announced work imply that for each number $r < \diam M$ the minimizers will contain only a finite number of branching points. 
\end{example}



%Интересно может ли быть не прямолинейный отрезок
%\input{pictures/X2}

==> parts/new_proofs.tex <==
%\section{Доказательства и технические утверждения}
\subsection{Technical statements and proofs of some lemmas}
\label{new_proofs}
%%\color{blue}
%\begin{definition}
%Let $\bar x\in E_\Sigma$ and $\varepsilon>0$. Then let us define a set 
%\[
%U(\bar{x},\varepsilon) \defeq \left \{ y\in M | \dist(y, \overline{B_{\varepsilon}(\bar{x})})\leq r, \dist(y, \Sigma \setminus \overline{B_{\varepsilon}(\bar{x})})> r \right \}.
%\]
%\end{definition}
%\begin{remark}

%Let $x\in E_\Sigma$ and let $(ix]$ be an energetic ray. If $(ix]$ is one-orientated energetic ray then there exists such $\rho>0$ that for every $\bar x \in E_\Sigma \cap B_\rho(x)$ for sufficiently small $\varepsilon>0$ the set $U(\bar{x},\varepsilon)$ is located in the same half-plane bounded by $ (ix) $ \color{red}(the one into which the edge is orientated).\color{black} %понятно ли учитывая определки?

 % If an energetic ray $(ix]$ is two-orientated for each $\bar x$ either exist such   $\varepsilon>0$, that the set $U(\bar{x},\varepsilon)$ is located in one half-plane bounded by $ (ix) $
  %   or in both half-planes there exist different points $ y (\bar {x}) \in M$ corresponding to $ \bar{x} $. 

%\end{remark}
%\color{black}


Теперь приступим к доказательству Леммы~\ref{alm}. %НАДО СДЕЛАТЬ ОТДЕЛЬНОЙ ЛЕММОЙ

\begin{proof}
%Предположим противное утверждению Леммы: то есть найдется такое $c>0$, что для каждого $\rho>0$ найдется $\bar x \in %B_\rho(x) \setminus \{x\}$ такой, что $|g(\bar x)|>c$. То есть выполняется неравенство:  
%\begin{itemize}
%\item [(i)] $|\pi/2-\angle((s\bar x),(ix))|>c$, если $\bar x \in X_\Sigma$, $\oord_x\Sigma=1$ и $[s\bar x] \subset %\Sigma$;
%\item [(ii)]$|\angle((s\bar{x}], (ix))-\angle( (ix),(t\bar{x}])|>c$,  если $\bar x \in X_\Sigma$, $\oord_x\Sigma=2$ и %$([s\bar x] \cup [t \bar x]) \subset \Sigma$;
%\item [(iii)]$\max \left( \big| \pi- \angle(m(\bar{x}),n(\bar{x})) \big| , \angle(m(\bar{x}),(ix)) \right)>c$, если %$\bar x \in E_\Sigma$, где лучи $m(\bar x)$ и $n(\bar x)$ определены в формулировке Леммы.
%\end{itemize}
Сначала мы докажем вспомогательные утверждения (A), (B) и (C), а после последовательно каждый из пунктов Леммы.

%Мы сначала докажем вспомогательное утверждение, из которого будет следовать пункт~\ref{__1}. После этого докажем %вспомогательное утверждение, которое будет использовано в доказательстве невозможности пункта (ii) и разборе случая %$\oord_x\Sigma =2$. Невозможность пункта (iii) получается автоматически, а вот доказательство того, что $\Sigma \cap %B_\varepsilon(\bar x)$  случае $\oord_x\Sigma =2$ является объединением двух дуг, лежащих в некоторых псевдоконусах, %потребует усилий.
\begin{enumerate}
\item [(А)] \label{W}
Для произвольного $x\in E_\Sigma$  для каждого $c>0$ существует такое $\rho>0$, что для $\bar{x} \in B_\rho(x) \setminus \{ x\}$ такого, что $\oordball_{\bar x}\Sigma=1$ для каждого такого $\varepsilon<\min(|\bar x x|, \rho-|\bar x x|)$, что $\sharp(\partial B_{\varepsilon}(\bar x) \cap \Sigma)=1$, для $s^\varepsilon \defeq \partial B_{\varepsilon}(\bar x) \cap \Sigma$ выполняется $|\angle ((s^\varepsilon \bar x), (ix))-\pi/2|<c$. Иными словами, покажем, что $|\angle ((s^\varepsilon \bar x), (ix))-\pi/2|=o_\rho(1)$. %Заметим, что из этого будет следовать одно из двух утверждений пункта~\ref{__1} Леммы, а именно что в случае $\bar{x}\in X_\Sigma$ и $\oord_{\bar x}\Sigma=\oordball_{\bar x}\Sigma=1$ отрезок $[s\bar x] \subset \Sigma$ почти перпендикулярен $(ix)$
\begin{proof}
%[вспомогательного утверждения А]
Предположим противное, то есть что существует %не зависящая от $\rho>0$
константа $c>0$, такая что для каждого $\rho>0$ найдется $\bar{x} \in B_\rho(x) \setminus \{ x\}$ и такое $\varepsilon>0$, что $B_{\varepsilon_0}(\bar x) \subset B_\rho(x)$ и  $|\angle ((s_0\bar x), (ix))-\frac{\pi}{2}| > c$ для $s_0 \defeq \partial B_{\varepsilon_0}(\bar x) \cap \Sigma $.  Пусть тогда $w^0$ --- основание перпендикуляра, опущенного из $s_0$ на прямую, параллельную $(ix)$ и проходящую через $\bar x$: $(w^0\bar x)\ ||\ (ix)$ и $(w^0s_0) \perp (ix)$. Тогда определим множество $S \ni w^0$  как в Лемме~\ref{Losiu} для $w=w^0$. Тогда длина этого множества $\H(S)=o_\rho(1)\varepsilon_0$, . В то же время 
\[
|w^0s_0|=\sin \angle([s_0\bar x],(ix]) \cdot |s_0\bar x|= \cos c |s_0\bar x| < (1 - \frac{c^2}{2}) \varepsilon_0
\]
для достаточно малого $c$.
При этом $\H(\Sigma \cap B_{\varepsilon_0}(\bar x)) \geq \varepsilon_0$. Таким образом, \[
\H(\Sigma \setminus  B_{\varepsilon_0}(\bar x) \cup [s_0w^0] \cup S)\leq \H(\Sigma)-\varepsilon_0+\left(1-\frac{c^2}{2}\right)\varepsilon_0+o_\rho(1)\varepsilon_0<\H(\Sigma).
\]
Таким образом, $\Sigma \setminus  B_{\varepsilon_0}(\bar x) \cup [s_lw^l] \cup S$ является связным множеством с длиной меньшей и энергией, не большей, чем у $\Sigma$. Противоречие с оптимальностью $\Sigma$ завершает доказательство.
\end{proof}
\item [(B)]
Пусть $x \in E_\Sigma$. Тогда для достаточно малого $\rho>0$ для каждого $\bar x \in G_\Sigma \cap B_\rho(\Sigma)\setminus \{ x\}$, имеющего порядок $\oordball_{\bar x}\Sigma = 2$, найдется такое $\varepsilon>0$, что для каждой  $u \in \Sigma \cap B_\varepsilon(\bar x)$ выполняется $\angle((u \bar x),(ix)) \neq \pi/2$. Иными словами, если $\bar x \in G_\Sigma \cap B_\rho(\Sigma)\setminus \{ x\}$ имеет порядок $\oord_{\bar x}\Sigma = 2$, то не существует бесконечной последовательности точек $u_m\in \Sigma$, сходящейся к $\bar x$, таких что $\angle((u_m\bar x),(ix))=\pi/2$.
\label{QuQuQu}

\begin{proof}
Пусть $\{\varepsilon_l\}$ -- убывающая к нулю последовательность таких чисел, что $\sharp (\partial B_{\varepsilon_l}(\bar x) \cap \Sigma )=2$, а $\varepsilon_1 < \min (\rho, \rho-|\bar x x|)$. Обозначим  $s^l, t^l \defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$. 

Ясно, что угол $\angle s^l\bar xt^l > \frac{2\pi}{3} - o_\rho(1)$: в противном случае замена $\Sigma \setminus B_\varepsilon(\bar x) \cup St(s^l,t^l,\bar x) \cup S$, где $S \ni \bar x$ --- множество, определенное в Лемме~\ref{Losiu} для точки $w=\bar x$, а $St(s^l,t^l,\bar x)$ --- дерево Штейнера, соединяющее точки $s^l$, $t^l$ и $\bar x$, имело бы не большую энергию и строго меньшую длину, чем множество $\Sigma$.

С другой стороны $B_r(y(\bar x)) \cap \Sigma = \emptyset$ и $|\angle ((y(x)x),(ix)) - \pi/2| =o_\rho(1)$ ввиду пункта~3 доказательства леммы~\ref{Losiu}.
Тогда $\angle ((s^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ и $\angle ((t^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$.


Предположим противное утверждению пункта: что существует такая последовательность $u_l$. Тогда при достаточно малом $\rho$ для любого $l$ выполняется 
\[
\sharp (\Sigma \cap \partial B_{|\bar x u_l|}(\bar x))\geq 3.
\]

Заметим теперь, что для каждого $\varepsilon_l$ верно
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)=2\varepsilon_l+o_\rho(1)\varepsilon.
\label{1000}
\end{equation}
Формула~\eqref{1000} верна ввиду Леммы~\ref{Losiu}: в противном случае, можно было бы заменить $\Sigma$ на связное множество $\Sigma \setminus B_{\varepsilon_l}(\bar x) \cup [\bar xs^l]\cup [\bar x t^l]\cup S$, где $S$ определено в Лемме~\ref{Losiu} при $w=\bar x$, и получить противоречие с оптимальностью $\Sigma$. 
Можно считать, что 
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)<2\varepsilon_l \left (1+\frac{1}{36}\right).
\label{1010}
\end{equation}

Теперь заметим, что можно считать, что 
\begin{equation}
\frac{\varepsilon_l}{\varepsilon_{l+1}}\leq \frac{18}{17}.
\label{1030}
\end{equation}
Пусть не так, тогда найдется $\varepsilon_l$ такое, что $\sharp \left( \partial B_{\varepsilon_l}(\bar x)\cap \Sigma
\right) \geq 3$ для каждого $\varepsilon \in [\frac{17\varepsilon_l}{18},\varepsilon_l[$. Но тогда, ввиду неравенства коплощади,
\[
\H(\Sigma \cap B_{\varepsilon_l}(\bar x))\geq \H(\Sigma \cap B_{\frac{17\varepsilon_l}{18}}(\bar x)) +\H(\Sigma \cap (B_{\varepsilon_l}(\bar x) \setminus  B_{\frac{17\varepsilon_l}{18}}(\bar x))\geq 2\varepsilon_l\left(1+\frac{1}{36}\right),
\]
что противоречит (\ref{1010}).

Рассмотрим произвольную точку $u_m$ из последовательности $\{u_l\}$. Выберем такой номер $l$, что 
\begin{equation}
0<\varepsilon_l-|\bar xu_m|\leq \frac{1}{18}\varepsilon_l.
\label{1040}
\end{equation}
Такое $\varepsilon_l$ существует ввиду формулы~\eqref{1030}. Также можно полагать, что для каждого $\delta \in ]|\bar x u_m|, \varepsilon_l[$ выполняется $\sharp \left( \partial B_{\delta}(\bar x)\cap \Sigma
\right) \geq 3$.
Пусть \[\gamma \defeq \max_{s \in \Sigma \cap \overline B_{\varepsilon_l}: \sharp (B_{|\bar x s|}(\bar x) \cap \Sigma) <3)} \angle{ixs}.\] Тогда $\gamma\leq \frac{\pi}{3}+ o_\rho(1)$.
Пусть $q$ --- компонента связности $\Sigma \setminus \Lambda ((ix),\gamma)$, содержащая $u_m$.
Тогда 
\[
\H(q) \geq \dist (u_m, \Lambda((ix),\gamma))=\cos \gamma |u_m \bar x|\geq \frac{|u_m \bar x|}{3}.
\]
Заметим, что, ввиду неравенства коплощади для $\Sigma \setminus q$, верно
\begin{multline}
\H(\Sigma \cap \overline B_{\varepsilon_l}) = \H(q)+\H(\Sigma \cap \overline B_{\varepsilon_l}\setminus q ) \geq \H(q)+2\varepsilon_l\geq  \frac{|u_m \bar x|}{3} +2\varepsilon_l \geq \varepsilon_l (\frac{17}{18*3}+2),
 \end{multline}
где последнее неравенство верно ввиду~\eqref{1040}. Получили противоречие с~\eqref{1010}.
\end{proof}
\item [(C)] Пусть обозначениях леммы $\oordball_x \Sigma =2$ и пусть $(s \bar x]$ и $(t \bar x]$ --- касательные для компонент связности $\Sigma \setminus \bar x$ в точке $\bar x$. Тогда найдется такое $\rho$, что $|(\angle (s \bar x], (ix] - (\angle (t \bar x], (ix]| <c$.
Иными словами $|(\angle (s \bar x], (ix] - (\angle (t \bar x], (ix]| = o_\rho(1)$.
\begin{proof}
Предположим противное: что найдется число $c>0$, такое что 
\[
\eta \defeq \angle((s\bar x], (ix))-\angle( (ix),(t\bar x]) \geq c
\]
для сколь угодно малого $\rho$.
Пусть $\varepsilon< \min (\rho-|\bar x x|, |\bar x x|)$ такой, что $\sharp( \partial B_\varepsilon(\bar x) \cap \Sigma) =2$. Обозначим $T, S \defeq \partial B_\varepsilon(\bar x)  \cap \Sigma$. Тогда 
\begin{equation}
\angle ((T \bar x],(t\bar x))=o_\rho(1) \mbox{ и } \angle ((S \bar x],(s\bar x))  =o_\rho(1).
\label{ZAQ}
\end{equation}
Пусть $l$ --- прямая, проходящая через точку $\bar x$ и параллельная $(ix)$. Отразим отрезок $[T \bar x]$ относительно $l$. Пусть $T'$ --- образ точки $T$ при этом отображении. 
Тогда $|T'\bar x|=\varepsilon$ и
\[
|S \bar x|+|T \bar x|=|S\bar x|+|T' \bar x|=2\varepsilon.
\]
В то же время по теореме косинусов для $\Delta S\bar xT'$
\[
|ST'|^2 = |S\bar x|^2+|\bar xT'|^2-2|S\bar x||\bar x T'|\cos \angle S\bar xT'=2\varepsilon^2(1-\cos (\eta+o_\rho(1))),
\]
поскольку
\[
\angle S\bar xT'=\pi+\angle((T\bar x], (ix))-\angle( (ix),(S\bar x]),\]
то есть ввиду~\eqref{ZAQ}   
\[
\angle S\bar xT'=\pi+\angle((t\bar x], (ix))-\angle( (ix),(s\bar x])+o_\rho(1)=\pi+\angle((t\bar x], (ix))-\angle( (ix),(s\bar x])+o_\rho(1)=\pi=\eta+o_\rho(1).
\] 
%а $\angle S\bar xT'=\angle s \bar x t+o_\rho(1)=\pi-\eta+o_\rho(1)$.


Таким образом, при достаточно малом $\rho$,
\[
|S\bar x|+|T'\bar x|-|ST'|> c_2\varepsilon,
\]
где $c_2 > 0$ --- константа, зависящая только от $\eta$.

Пусть теперь точка $d \defeq [ST']\cap l$. Тогда $\angle((Sd], (ix))=\angle( (ix),(T'd])$ и 
%\begin{equation*}
\[(|S\bar x|+|T\bar x|)-(|Sd|+|dT|)= 2\varepsilon - |ST'|>c_2\varepsilon.\]
%\end{equation*}

Ввиду Леммы~\ref{Losiu} для $w=d$ найдется связное множество $S \ni d$ такое, что $\H(S)<c_2/2\varepsilon$, а $F_M(\Sigma \setminus B_\varepsilon(\bar x) \cup S)\leq F_M(\Sigma)$. Тогда связное множество $\Sigma \setminus ([S\bar x]\cup[T\bar x]) \cup S \cup [sd] \cup [td]$ при достаточно малом $\rho$ будет лучше $\Sigma$, поскольку имеет не большую энергию и строго меньшую длину.
%не превосходящую $\H(\Sigma)-c_2\varepsilon+ \H(S)<\H(\Sigma)$. 
Полученное противоречие с оптимальностью $\Sigma$ завершает доказательство пункта.
\end{proof}

\begin{corollary}
В ввиду леммы~\ref{angles2} верно $\angle s\bar xt \geq \frac{2\pi}{3}$ и 
\[
\angle((s\bar x], (ix))=\angle( (ix),(t\bar x] )+ o_\rho(1)\leq \frac{\pi}{6}+ o_\rho(1).
\] 
\label{__2c}
\end{corollary}

\item Теперь докажем, что 
%для произвольного $x \in E_\Sigma$ найдется такое $\rho>0$, что для каждого $\bar x \in B_\rho(\Sigma)\setminus \{ %x\}$, 
порядок $\oord_{\bar x}\Sigma = 1$ влечет  $\bar x\in X_\Sigma$. 
\label{QQ}
Предположим противное: пусть $\bar x \in E_\Sigma \cap B_\rho(x) \setminus x$. 
% Энергетическое ребро или ребра, к которым они сходятся, должны лежать на прямой, почти параллельной $(ix]$ ввиду %Следствия~\ref{alm_parr}.  
%\end{itemize}


Ввиду Леммы~\ref{ordball_} достаточно разобрать только следующие случаи:
\begin{itemize}
\item [(а)] Случай $\oordball_{\bar x}\Sigma=2$.
Пусть $\{\varepsilon_l\}$ -- убывающая к нулю последовательность таких чисел, что $\sharp (\partial B_{\varepsilon_l}(\bar x) \cap \Sigma )=2$, а $\varepsilon_1 < \min (\rho, \rho-|\bar x x|)$. Обозначим  $s^l, t^l \defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$. 

Как было показано в п. (B), верно $\angle ((s^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ и $\angle ((t^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$.%, то есть
%\begin{equation}
%s^l, t^l \in \Lambda((ix), \pi/3+o_\rho(1)).
%\label{LLL}
%\end{equation}


Тогда ввиду единичного порядка $\oord_{\bar x}(\Sigma)=1$, существует также сходящаяся к $\bar x$ последовательность точек $\{ u_l\}$ таких, что \[\angle\left((u_l\bar x),(ix)\right)=\frac{\pi}{2}.\] 
Противоречие с п.~(B).


\item [(б)] Случай $\oordball_{\bar x}\Sigma=1$. 

Пусть $\varepsilon_l>0$ --- последовательность стремящихся к нулю чисел таких, что $\sharp (\partial B_{\varepsilon_l}(\bar x) \cap \Sigma )=1$, а $s_l\defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$. Тогда ввиду~(A) $(s_l\bar x)$ почти перпендикулярно $(ix)$:
\begin{equation}
\left|\angle \left((s_l\bar x), (ix)\right)-\frac{\pi}{2}\right| =o_\rho(1).
\label{99}
\end{equation}
Заметим теперь, что для каждого $\varepsilon_l$ верно
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)=\varepsilon_l+o_\rho(1)\varepsilon.
\label{100}
\end{equation}

Формула~\eqref{100} верна ввиду Леммы~\ref{Losiu}: в противном случае можно было бы заменить $\Sigma$ на связное множество $\Sigma \setminus B_{\varepsilon_l}(\bar x) \cup [\bar xs_l]\cup S$, где $S$ определено в Лемме~\ref{Losiu} при $w=\bar x$, и получить противоречие с оптимальностью $\Sigma$. 

Можно считать, что 
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)<\varepsilon_l \left(1+\frac{1}{18}\right).
\label{101}
\end{equation}
Теперь заметим, что тогда
\begin{equation}
\frac{\varepsilon_l}{\varepsilon_{l+1}}\leq \frac{18}{17}.
\label{103}
\end{equation}
Пусть не так, тогда найдется $\varepsilon_l$ такое, что $\sharp ( \partial B_{\varepsilon_l}(\bar x)\cap \Sigma)\geq 2$ для каждого $\varepsilon \in [\frac{17\varepsilon_l}{18},\varepsilon_l[$. Но тогда, ввиду неравенства коплощади
\[
\H \left(\Sigma \cap B_{\varepsilon_l}(\bar x)\right)\geq \H \left(\Sigma \cap B_{\frac{17\varepsilon_l}{18}}(\bar x)\right) +\H \left(\Sigma \cap B_{\varepsilon_l}(\bar x) \setminus  B_{\frac{17\varepsilon_l}{18}}(\bar x)\right)\geq \varepsilon_l \left (1+\frac{1}{18} \right),
\]
что противоречит~\eqref{101}.
Заметим, что поскольку $\bar x$ имеет ребро, которое, ввиду Следствия~\ref{alm_parr} $o_\rho(1)$-почти параллельно $(ix)$, существует последовательность энергетических точек $\{x_l\}$, сходящихся к $\bar x$ таких, что $\angle ((x_l\bar x], (ix]) =o_\rho(1)+o_{|x_l\bar x|}(1)$. Ввиду наличия у $\bar x$ ребра, существования последовательности $\{ s_l \}$ и единичного порядка $\oord{\bar x}(\Sigma)=1$ существует также сходящаяся к $\bar x$ последовательность точек $\{ u_l\}\subset \Sigma$ таких, что $\angle \left((u_l\bar x),(ix)\right) = \frac{\pi}{4}$.

Рассмотрим произвольную точку $u_m$ из этой последовательности. Выберем такой номер $l$, что 
\begin{equation}
0<\varepsilon_l-|\bar xu_m|\leq \frac{1}{18}\varepsilon_l.
\label{104}
\end{equation}
Такое $\varepsilon_l$ существует ввиду формулы~\eqref{103}. Заметим также, что ввиду~\eqref{99} выполняется
\[
\sharp (\partial B_{|\bar x u_m|}(\bar x)\cap \Sigma) \geq 2.
\] 
Можно также считать, что для произвольного $\delta \in [|\bar x u_m|,\varepsilon_l[$ выполняется $\sharp (\partial B_{\delta}(\bar x)\cap \Sigma) \geq 2$.

Кроме того, пусть 
\[
k:=\max_{s \in \Sigma \cap \overline{B_{\varepsilon_l}}: \sharp (\Sigma \cap _{|s \bar x|}(\bar x))} \angle ixs,
\]
тогда $|k-\pi/2|=o_\rho(1)$.
Тогда $K := \Lambda((ix),k)$ --- область возможного расположения точек $s_l$. 


%Кроме того, пусть $K \subset \Lambda((\bar x y(\bar x)), o_\rho(1))$ --- область возможного расположения точек $s_l$ (угол с вершиной в $\bar x$, раствором $o_\rho(1)$ и перпендикуляром к $(ix)$ в качестве биссектрисы), а 
Пусть $Q$ --- псевдоконус или объединение двух псевдоконусов с вершиной в $\bar x$, содержащих все энергетические точки $B_{\varepsilon_l}(\bar x)$, тогда
\begin{equation}
d \defeq \dist(u_m, Q \cup K)\geq \frac{\sqrt{2}}{2}|\bar xu_m|-o_\rho(1)\varepsilon> \frac{17}{36}\varepsilon_l,
%\label{105}
\end{equation}
где последнее неравенство верно ввиду~\eqref{104}. 
Ясно, что, ввиду единичного порядка $\bar x$ и определения компоненты связности $q$, выполняется $\H(q) \geq 2d$. В таком случае, ввиду неравенства коплощади для $\Sigma \setminus q$, верно
\[
\H(\Sigma \cap B_{\varepsilon_l}(\bar x)) \geq H(\Sigma \cap B_{\varepsilon_l}(\bar x) \setminus q)+\H(q) \geq \varepsilon_l +2d\geq
\varepsilon_l (1+ \frac{17}{18}).
\]
Полученное противоречие с~\eqref{101} завершает доказательство пункта~\ref{__1} леммы.

\end{itemize}
\item Пусть $\oord_{\bar x} \Sigma =2$ и $\bar x \in X_\Sigma$, и для некоторого $\varepsilon>0$ выполняется $\Sigma \cap \overline{B_{\varepsilon}(\bar x)}=[s\bar x] \sqcup [t\bar x]$. 
\label{Q3}

Утверждение сразу следует из пункта~(C).

\item% Докажем пункт~\ref{__3} Леммы.
%\begin{proof}
Ввиду Леммы~\ref{con} пп~\ref{BB} и~\ref{reb} существует $Q$ --- псевдоконус или объединение двух  псевдоконусов  таких, что $G_\Sigma \cap B_{\varepsilon_0}(\bar x) \subset Q$ для достаточно малого $\varepsilon_0$. 
%Не умаляя общности, ввиду пункта~\ref{ordball_} будем считать $\varepsilon>0$ таким, что $\sharp(\Sigma \cap \partial B_\varepsilon(x^i_k)) \leq 2$. 
При этом  ввиду следствия~\ref{alm_parr} оси псевдоконусов почти параллельны $(ix)$. 
Если хотя бы одно из двух ребер $\bar x$ направлено в две стороны, пункт тривиален ввиду Замечания~\ref{star}. Аналогично пункт тривиален, если ребра направлены в разные стороны, то есть для достаточно малого $\varepsilon_0>0$ точки $M$, соответствующие энергетическим точкам из множества $B_{\varepsilon_0}(\bar x) \setminus \bar{x}$ располагаются в обеих частях плоскости, разделенной энергетическими ребрами $\bar x$. Таким образом, можно считать, что каждое ребро направлено в одну сторону и что один из двух углов между энергетическими ребрами не содержит точек $M$, соответствующих энергетическим точкам из $Q$. Будем называть этот угол внутренним. Нетрудно заметить, что ввиду п.~\ref{orientation} Замечания~\ref{emptyball} величина этого угла не превосходит $\pi$. 

Пусть $(q_1\bar x]$ --- луч, лежащий во внутреннем угле и не совпадающий ни с одним энергетическим ребром $\bar x$. Тогда, ввиду определения псевдоконуса найдется такое $\varepsilon_1>0$, что $(q_1\bar x] \cap Q \cap B_{\varepsilon_1}(\bar x)=\emptyset$. Поскольку ввиду пункта~\ref{QQ} доказываемой леммы, замечания~\ref{rem_ord} и леммы~\ref{ordball_}, выполняется $\oord_{\bar x} \Sigma =\oordball_{\bar x}\Sigma=2$, потребуем, чтобы $\varepsilon_1>0$ удовлетворяло условию $\sharp (\Sigma \cap \partial B_{\varepsilon_1}(\bar x))=2$. Покажем, что тогда найдется такое $\varepsilon_2>0$, что 
\[
B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x], 
\]
либо 
найдется такое $\varepsilon_2>0$, что 
\[
B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = \bar x. 
\]
 Пусть не реализовался ни один из двух случаев. Тогда, в частности, множество $\Sigma \cap B_{\varepsilon_1}(\bar x) \cap (q\bar x]$ содержит бесконечное число точек. Кроме того, любая точка из множества $\Sigma \cap B_{\varepsilon_1}(\bar x) \cap (q\bar x]$ не энергетическая и, значит, является центром отрезка или правильной треноги.
%, а множество $\Sigma \cap B_{\varepsilon}(\bar x) \setminus Q$ является штейнеровским лесом. 
Пусть $L_1$ обозначает ту часть внутреннего угла, которая ограничена $(q_1\bar x]$, $\partial B_{\varepsilon_1}(\bar x)$ и перпендикуляром к $(ix)$, проходящим через $\bar x$ (положим для начала, что луч $(q_1\bar x]$ не перпендикулярен $(ix)$). Будем полагать $L_1$ открытым множеством. Тогда $S := \overline{L_1\cap \Sigma}$ является штейнеровским лесом, причем все концевые вершины $ S$, число которых бесконечно, за исключением не более чем трех точек, принадлежащих $\partial B_{\varepsilon_1} (\bar x) \cup \{ x \}$, лежат на $(q\bar x]$ или на перпендикуляре. Тогда ввиду Леммы~\ref{St_l} число концевых точек леса $\partial S$, принадлежащих перпендикуляру, бесконечно. а значит найдется сходящаяся к $\bar x$ бесконечная последовательность точек $\{u_l\}$ таких, что $\angle((u_l,\bar x)(ix))=\pi/2$ для каждого номера $l$. Однако существование такой последовательности противоречит пункту~(B). Таким образом, существует такое $\varepsilon_1$, что $\Sigma \cap (q_1\bar x] \cap \overline {B_{\varepsilon_1}(\bar x)}$ равно $\{\bar x\}$ или совпадает с $(q_1\bar x] \cap B_{\varepsilon_1}(\bar x) $. Будем также считать, что $\sharp(\partial B_{\varepsilon_1}(\bar x)\cap \Sigma)=2$ и $Q \cap B_{\varepsilon_1}(\bar x) \cap (q_1\bar x] = \emptyset$.

Пусть $(m\bar x]$ --- энергетическое ребро $\bar x$. Выберем такие строго убывающие к нулю последовательности $\{\bar{\varepsilon}_i \}$ и $\{ \gamma_i\}$, что 
\begin{itemize}
\item $Q \cap B_{\bar \varepsilon_i}(\bar x)$ содержится внутри угла с биссектрисой $(m\bar x]$ и раствором $2\gamma_i$;
\item границы угла с биссектрисой $(m\bar x]$ и раствором $2\gamma_i$, при пересечении с множеством $\Sigma \cap \cap B_{\bar\varepsilon_{i+1}}(\bar x)$, совпадают с $\{ \bar x \}$, либо с радиусом $B_{\bar \varepsilon_{i+1}}(\bar x)$. 
\end{itemize}
Положим $\gamma_1 \leq \pi/12$, $\bar \varepsilon_1 \defeq \varepsilon_1$.
Если при каком-то номере (ввиду леммы~\ref{angles2} не более чем при одном) реализовался случай совпадения с радиусом, обозначим этот номер за $j$. В противном случае положим $j=0$.

Определим псевдоконус 
\[
Q_1 \defeq Q^{m,\bar x}_{\overline{\varepsilon}_{j+1}}\defeq \bigcup_{i=j+1}^{\infty} \left(Q(m,\overline x, \gamma_i, \overline{\varepsilon_i}) \setminus B_{\overline{\varepsilon}_{i+1}}(\bar x)\right).
\]
Если $\bar x$ обладает двумя энергетическими ребрами, то аналогично определим псевдоконус $Q_2$ со вторым энергетическим ребром в качестве оси. 
%$(a \bar x$ и $(b \bar x]$, то аналогично определим псевдоконус $Q^{b, \bar x}_{\bar \varepsilon_1}$

Таким образом произвольная компонента связности $\Sigma \cap B_{\varepsilon_1}(\bar x)\setminus \{x\}$ либо находится внутри псевдоконуса $Q_1$ или $Q_2$, либо находится вне псевдоконуса $Q$. Поскольку $\bar x$ имеет энергетическое ребро, хотя бы одна из двух компонент содержится внутри псевдоконуса. Тогда она имеет касательную в точке $\bar x$(причем данная касательная $\rho-$почти параллельна $(ix]$), а значит к ней применима лемма~\ref{angles2}. Если вторая компонента связности не содержится в псевдоконусе, то она является отрезком (поскольку имеет не более двух концевых точек: точку $\{ \bar x\}$ и точку на $\partial B_{\varepsilon_1}(\bar x)$). В обоих случаях вторая компонента связности имеет в точке $\bar x$ касательную. Таким образом ко второй компоненте связности применим пункт $(C)$ доказываемой леммы. Утверждение пункта доказано.


 
% \begin{remark}
 %Заметим также, то угол между ребрами, содержащий соответствующую $x^i_k$ точку $y^i$, не может быть меньше $\pi$ (если покрытые $x^i_k$ точки есть в обеих полуплоскостях, то угол между ребрами составляет ровно $\pi$).
 %\label{rovno}
 %\end{remark}

\end{enumerate}
 \end{proof}

%\begin{proof}
%\begin{enumerate}
  %  \item

Докажем следующее техническое утверждение:
\input{pictures/dvapo}

\begin{proposition}
Для произвольного $x \in E_\Sigma$ и $\bar c>0$ найдется такое $\rho>0$, что если $\Sigma \cap B_\rho(x)$ содержит ломаную $L_1-L_2-L_3-L_4-L_5$, узлы которой являются энергетическими точками ребра $(ix]$, то $\angle((L_iL_{i+1}),(ix)\leq \bar c$ для $i=1, \dots, 4$.  
И ВСЕ ВН ТОЧКИ ЛОМАНОЙ -- СТЕПЕНИ 2 
\label{brrrr}
\end{proposition}
\begin{proof}
Предположим противное, то есть (ввиду Леммы~\ref{alm} п.~\ref{__2} для $c= \bar c/ 10$) что для сколь угодно малого $\rho > 0$ существует такая ломаная $L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\rho}$, что все углы $\angle((L_iL_{i+1}),(ix))> \bar{c}/2$ при $i=1,2,3,4$. 
Будем считать $(ix)$ осью абсцисс, а $\bar{c}$ достаточно малым. Не умаляя общности, точкам $L_1$, $L_3$, $L_5$ соответствуют верхние точки множества $M$, а точкам $L_2, L_4$ --- нижние: ввиду пункта~\ref{1145} доказательства Леммы~\ref{Losiu} и неравенства $\angle L_{i-1}L_{i}L_{i+1} \leq \pi-\bar{c}$, $i=2,3,4$ двум подряд идущим точкам не могут соответствовать одновременно верхние или нижние точки.
 Заметим теперь, что отношения между отрезками ломаной линейные (то есть отношение оценивается сверху и снизу константой, зависящей от $\bar{c}$), и замена ломаной на отрезки $L_1-L_2-L_4-L_5$ уменьшит длину на величину, линейно зависящую от $[L_1L_2]$:
 поскольку $L_3 \notin B_r(y(L_1))$ выполняется 
 \[
 |Pr_{(y(L_1)L_1)}[L_2L_3]|<|Pr_{(y(L_1)L_1)}[L_1L_2]|+o(|L_1L_3|).
 \label{1111}
 \]
  Поскольку 
  \[
  |\angle (y(L_1)L_1), (ix])-\pi/2| =o_\rho(1)
  \]
 выполняется 
 \[
 |L_2L_3|_y<|L_1L_2|_y+o(|L_1L_2|+|L_2L_3|),
 \]
 где $|\cdot |_y$ означает длину проекции на прямую, перпендикулярную $(ix)$. Тогда
 \[
 |L_2L_3|\sin \frac{ \bar{c}}{2}<|L_1L_2|+o(|L_1L_2|+|L_2L_3|),
 \]
 то есть
 \[
 |L_2L_3|< \frac{1}{\sin \frac{ \bar{c}}{2}}|L_1L_2|+o(|L_1L_2|+|L_2L_3|). 
 \]
%Тогда для достаточно малого $\rho$ выполняется

 Аналогично, поскольку  $L_3 \notin B_r(y(L_1))$ и $|\angle (y(L_3)L_3), (ix])-\pi/2| =o_\rho(1)$ выполняется
  \[
 [L_2L_1]<\frac{1}{\sin \frac{ \bar{c}}{2}}|L_3L_2|+o(|L_1L_2|+|L_2L_3|). 
 \]
 В таком случае
 \[
\sin\frac{ \bar{c}}{2}- \frac{o(|L_1L_2|+|L_2L_3|)}{|L_3L_2|}\leq  \frac{|L_2L_3|}{|L_1L_2|}\leq \frac{1}{\sin \frac{ \bar{c}}{2}}+\frac{o(|L_1L_2|+|L_2L_3|)}{|L_1L_2|},
 \]
 а значит, для достаточно малого $\rho$ верно
 \[
\frac{\bar c}{3} < \sin \frac{ \bar{c}}{2}- \frac{o(|L_2L_3|(1+\frac{1}{\sin\frac{ \bar{c}}{2}}|L_1L_2|+o_\rho(1)))}{|L_3L_2|}\leq  \frac{|L_2L_3|}{|L_1L_2|}\leq \frac{1}{\sin \frac{ \bar{c}}{2}}+\frac{o(|L_1L_2|(1+ \frac{1}{\sin \frac{ \bar{c}}{2}}+o_\rho(1)))}{|L_1L_2|}< \frac{3}{\bar{c}}.
 \]
 
  %\[[L_2L_3]_y>|L_1L_2|_y-|L_1L_3| o_{\varepsilon(c)}(1)\]
 %|L_1L_2|-\bar{\varepsilon}^2,\]
  %где нижний индекс $y$ означает проекцию на ось абсцисс. То есть $|L_2L_3|>\sin c |L_1L_2|-o_{\bar{\varepsilon}}(1)|L_1L_3|$.
% И наоборот, $|L_1L_2|>\sin \bar{c} |L_2L_3|-o_{\bar{\varepsilon}}(1)|L_1L_3|$. 
 %Из этого очевидным образом следует существование $c_1, c_2>0$ таких, что $c_2|L_2L_3|\geq |L_1L_2| \geq c_1|L_1L_3|$.   
 Аналогично и для остальных $L_i$. 
 
 Замена ломаной $L_1-L_2-L_3-L_4-L_5$ на $L_1-L_2-L_4-L_5$ уменьшит ее длину не меньше, чем на величину, линейно зависящую от $|L_1L_2|$, поскольку $\angle L_2L_3L_4 \leq \pi-\bar{c}$ (а значит $\cos \angle L_2L_3L_4 \geq  -\cos \bar{c}$):
 \begin{multline*}
 |L_2L_3|+|L_3L_4|-|L_2L_4|=\frac{(|L_2L_3|+|L_3L_4|)^2-|L_2L_4|^2}{|L_2L_3|+|L_3L_4|+|L_2L_4|}>\\
 > \frac{2|L_2L_3||L_3L_4| (1+ \cos \angle L_2L_3L_4)}{2(|L_2L_3|+|L_3L_4|)}\geq
 \frac{|L_3L_4|(1- \cos \bar{c})}{ \left (1+\frac{|L_3L_4|}{|L_2L_3|} \right)}\geq  \frac{(\frac{\bar{c}}{3})^3}{(1+\frac{3}{\bar{c}})}|L_1L_2|.
\end{multline*}
 
 
 
% \[
% |L_2L_3|+|L_3L_4|-|L_2L_4|\geq  |L_2L_3|(1+\frac{c}{3}-\frac{1}{\sin c})>|L_2L_3|(1+\frac 2 c),
 %\]
 %поскольку 
 %\[
 %|L_2L_4|=\sin \angle L_2L_3L_4 \frac{|L_2L_3|}{\sin L_2L_4 L_3}\leq  \frac{|L_2L_3|}{\sin L_2L_4 L_3} \leq  \frac{|L_2L_3|}{\sin (\pi-c)}= \frac{|L_2L_3|}{\sin c}.
 %\]
 %ой ОЙОЙ ТУТ НЕ ТАК
 
% \begin{multline*}
 %|L_2L_3|+|L_3L_4|-\sqrt{ |L_2L_3|^2+|L_3L_4|^2+2 %|L_2L_3||L_3L_4|\cos (2c) }\geq \\
%|L_1L_2| \left(\sin c+\sin^2 c-\sqrt{\frac{1}{\sin^2 c}+\frac{1}{\sin^4 c}+2\frac{\cos (2c)}{\sin^3 c}})+o_{\varepsilon(c)}(1|L_1L_2| \right),
% \end{multline*}
%Таким образом замена уменьшает длину множества на величину, линейно зависящую от $|L_1L_2|$.
%\input{pictures/dvapo}
%Обозначим точки $L_6 \defeq [L_1y(L_3)] \cap \partial B_r(y(L_3))$ и $L_7 \defeq [L_5y(L_3)] %\cap \partial B_r(y(L_3))$ где $y(L_3)$ произвольная соответствующая $L_3$ точка. Тогда %$$B_r([L_1L_6]) \cup B_r([L_5L_7]) \supset B_r([L_1L_3]) \cup B_r([L_3L_5]).$$ и %$\H([L_1L_6]) \cup B_r([L_5L_7]))=o_{[L_1L_2]}(1)$ (это следует из теоремы Пифагора и  %пункта~\ref{1145} доказательства Леммы~\ref{Losiu}). Тогда можно заменить ломаную  %$L_1-L_2-L_3-L_4-L_5$ на $L_6-L_1-L_2-L_4-L_5-L_7$ и получить противоречие с оптимальностью %$\Sigma$ (см. рис~\ref{fig:dvapo}).
%А значит
%\[
%\H([L_1L_2]\cup [L_2L_4]\cup[L_4L_5]\cup S^{[L_1L_5]})\leq \H(L_1-L_2-L_3-L_4-L_5)-|L_2L_3|(1+\frac 2 c)+o(|L_1L_5|)<\H(L_1-L_2-L_3-L_4-L_5).
%\]
Тогда множество $ \Sigma \setminus ([L_2L_3] \cup [L_3L_4]) \cup [L_2L_4]\cup S^{[L_1L_5]}$ лучше $\Sigma$: является связным (поскольку все внутренние точки исходной ломаной --- степени два), обладает меньшей длиной и не большей энергией. Противоречие с оптимальностью $\Sigma$ (см. рис~\ref{fig:dvapo}).
%ПОМЕНЯТЬ РИСУНОК ИЛИ ВЕРНУТЬ ЗАКОМЕНЧЕННОЕ


\end{proof}

\begin{lemma}
Пусть $x \in E_\Sigma$ и  существует $Q^{a,x}_\varepsilon$ такой, что $Q^{a,x}_\varepsilon \cap \Sigma$ является дугой. Тогда для произвольного $c>0$ найдется $\varepsilon(c)>0$ такой, что все односторонние касательные к точкам множества $Q^{a,x}_\varepsilon \cap B_{\varepsilon(c)}(x) \cap \Sigma$ имеют угол с прямой $(ax)$, не больший $2c$.
\label{zapred}
\end{lemma}

\begin{proof}
Предположим противное, то есть что существует последовательность точек, в которых односторонняя касательная имеет угол с $(ix)$, больший $2c$ (не умаляя общности полагаем $2c \leq \pi/2$). Ввиду утверждения пункта~\ref{__3} Леммы~\ref{alm} это могут быть только точки из множества $X_\Sigma \sqcup S_\Sigma$. Поскольку точек ветвления нет, в точках $S_\Sigma$ направление касательной не меняется, то есть найдется сходящаяся к $x$ последовательность точек из $X_\Sigma$ таких, что хотя бы один из двух входящих в точку отрезков имеет угол с $(ix)$, больший $2c$. Пусть $L_1$ --- такая точка, достаточно близкая к $x$ (то есть $L_1 \in B_{\varepsilon(c)}(x)$, где $\varepsilon(c)$ выбирается для $c/5$ как в Лемме~\ref{alm} $\rho$ выбирается для $c$). Ввиду утверждения пункта~\ref{__2} Леммы~\ref{alm} оба входящих в $L_1$ отрезка имеют угол с $(ix)$, больший $9/5c$. Тогда отрезок, лежащий на пути из $L_1$ в $x$ обязательно заканчивается точкой $L_2 \in X_\Sigma$. Но отрезок, выходящий из $L_2$ должен иметь угол с $(ix)$, больший $8/5c$, и заканчиваться точкой $L_3 \in X_\Sigma$. Ясно, что таким образом для любого  сколь угодно малого $\bar \varepsilon$ существует такая ломаная $L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\bar{\varepsilon}}(x)$, что все углы $\angle((L_iL_{i+1}),(ix))>c$ при $i=1,2,3,4$. Противоречие с утверждением~\ref{brrrr}.
\end{proof}

Докажем Лемму~\ref{uggi}.
\begin{proof}
Докажем первый пункт. Не умаляя общности, будем считать $\rho_2$ удовлетворяющим утверждению леммы~\ref{alm} для $c=\frac{\pi}{100}$ и утверждению~\ref{zapred} для $c=\frac{1}{20}$. Кроме того, можно  выбрать $\rho_2>0$ таким, чтобы 
\[
\sharp(\Sigma \cap Q \cap \partial B_{\rho_2}(x))=\oordball_x(\Sigma\cap Q)\leq \oordball_x(\Sigma)\leq 3. 
\]
Несложно понять, что $\oordball_x(\Sigma \cap Q)=1$: в противном случае ввиду неравенства коплощади можно было бы уменьшить длину $\Sigma$, заменив $\Sigma \cap Q$ на множество $T^Q$, определенное в доказательстве Леммы~\ref{angles2} и обладающее длиной $\rho_2 +o(\rho_2)$. При такой замене энергия не увеличится, а связность сохранится. Таким образом, мы будем полагать $\sharp (\partial B_{\rho_2(x)} \cap \Sigma) =1$.
Пусть $Q_1 \defeq Q \cap \overline{B_{\rho_2}(x)}$.
Пусть $z \defeq \partial Q_1 \cap \Sigma$.
%Предположим, что $\Sigma \cap Q_1$ содержит бесконечное %число точек ветвления. Тогда найдется дуга 
%дуга $\breve{[sx]} \subset \Sigma \cap Q_1$ такая что %$|sx|=\rho_1$, содержащая бесконечное число точек %ветвления. 

Разберем два случая:
\begin{itemize}
\item[(А)] Пусть ребро $(ax]$ направлено в одну сторону.
Будем считать $(ax]$ отрицательной половиной оси абсцисс. Тогда будем полагать $\rho_2$ таким, чтобы все точки, соответствующие энергетическим точкам $\Sigma \cap Q_1$ располагались в одной (не умаляя общности, будем называть её верхней) полуплоскости.
% (это корректно, как было показано в доказательстве Леммы~\ref{Losiu}). 
%Поскольку $\Sigma$ не содержит циклов, путь между любыми двумя точками $\Sigma$ однозначно определен.
 Посчитаем изменение направления касательной вдоль дуги $\breve{[zx]}$. Поскольку ввиду конечной длины касательная есть почти во всех точках $\Sigma$, то будем воспринимать $\turn(\breve{[zx]})$ как верхний предел (супремум) по всем последовательностям точек кривой:
 \[
 \turn(\breve{[zx]})=\sup_{n\in \N, z\preceq t_1 \prec \dots \prec t_n \preceq x} \sum_{i=2}^{n} \angle(t^i,t^{i-1}),
 \]
 где  $t^i$ означает луч касательной к кривой $\breve{[zt_i]}\subset \breve{[zx]}$, а ${t_1,\dots, t_n}$ --- разбиение кривой $\breve{[zx]}$ в порядке, соответствующем параметризации, при которой $z$ --- начало кривой, а $x$ --- конец, такое, что в каждой точке $t_i$ кривая $\breve{[zx]}$ имеет касательную. В данном случае угол $\angle(t^i,t^{i-1}) \in [-\pi,\pi[$ между двумя лучами считается от луча $t^i$ к лучу $t^{i-1}$, положительное направление --- против часовой стрелки.
 
Заметим, что ввиду условий на $\rho_1$ верно
 \[
|\turn ([zx])| \leq 2\pi.
 \]
Покажем, что на пути из $z$ в $x$ конечное число точек ветвления. Для этого рассмотрим произвольную точку ветвления $D_2$ на дуге $\breve{[zx]}$. %Рассмотрим такую точку ветвления $D_2$ на дуге $\breve{[sx]}$, что на пути из $D_2$ в $x$ бесконечно точек ветвления, а на пути из $s$ в $D_2$ достаточно много точек ветвления. 
Из точки $D_2$ выходят три отрезка $[D_1D_2]$, $[D_2D_3]$ и $[D_2C]$ с попарными углами $2\pi/3$, где, не умаляя общности, ломаная $D_1-D_2-D_3$ --- подмножество пути из $z$ в $x$.  Заметим, что вклад в поворот $\breve{[zx]}$ точки $D_2$ составляет $-\pi/3$, поскольку угол $\angle D_1D_2D_3$, посчитанный против часовой стрелки, составляет $2\pi/3$. %и определяется %однозначно: в выбранных обозначениях угол, посчитанный %против часовой стрелки, составляет $2\pi/3$, то есть %поворот составляет $\pi/3$. 
 Это так, поскольку путь, начавшийся с отрезка $[D_2C]$ должен закончиться энергетической точкой, а значит должен идти в верхнюю  половину шара $B_{\rho_1}(x)$. 
 Аналогичное верно для произвольной точки ветвления внутри пути из $z$ в $x$.
Из Леммы~\ref{alm} и того, что ребро $(ax]$ направлено вверх (и ввиду выбора $\rho_1$) следует, что угол направления касательной в энергетических точках  на пути из $z$ в $x$ меняется по часовой стрелке (на величину, не превосходящую $\pi/6+1/100$), то есть вклад в $\turn$ неположительный.

(Строго говоря, в п~\ref{__2} леммы~\ref{alm} не сказано, что для энергетической точки $\bar x \in X_\Sigma$ точка $s$ встречается на пути из $z$ в $x$ раньше, чем точка $t$ (в противном случае вклад точки $\bar x$ в поворот мог бы быть отрицательным). Однако в данной ситуации это так, поскольку в противном случае пустой шар $B_r(y(\bar x))$ и путь из $z$ в $\bar x$ делают невозможным существование в $\Sigma \cap Q_1$ пути из $\bar x$ в $x$. Аналогичным способом нужно действовать в ситуации $\bar x \in E_\Sigma$).

В остальных точках $\breve{[zx]}$ направление касательной не меняется. Таким образом на пути из $z$ в $x$ конечное количество (не более $6$) точек ветвления. А значит найдется такое положительное $\rho_2<\rho_1$, что $\breve{[zx]} \cap \overline B_{\rho_2}(x)$ не содержит точек ветвления. Потребуем также, чтобы 
\[
\sharp (\partial B_{\rho_2}(x) \cap \Sigma) = \oordball_x(\Sigma \cap Q)=1.
\]
%и обозначим
%\[
%Q_2 \defeq Q \cap \overline{B_{\rho_2}(x)}.
%\]
В таком случае $\Sigma \cap \overline{B_{\rho_2}(x)}$ является дугой.
\begin{remark}
Таким образом мы доказали, что точка $x\in E_\Sigma$ может быть пределом точек ветвления только если у неё есть направленное в две стороны ребро.  
 \label{remA}
\end{remark}
\item[(Б)] Пусть ребро $(ax]$ направлено в обе стороны.


%Выберем  $\rho$ не превосходит $\rho$ из %Леммы~\ref{alm} для $c=\pi/100$ и $\rho$ из %Утверждения~\ref{zapred} для $c=\frac{1}{20}$. 

Предположим, что $Q \cap \Sigma$ содержит бесконечное число точек ветвления. Тогда оно также содержит бесконечное число концевых точек. 

%Пусть $W$ такая концевая точка. Тогда, ввиду п.~\ref{__1} Леммы~\ref{alm} она принадлежит множеству $X_\Sigma$ и имеет %порядок $1$. Обозначим максимальный выходящий из неё отрезок за $[WD_1]$. Тогда $|\angle((WD_1),(ix))-\pi/2|<\pi/100$. %Точка $D_1$, ввиду пп.~\ref{__2} (см Следствие~\ref{__2c}) и~\ref{__3} Леммы~\ref{alm} может быть только точкой %ветвления. Пусть $[D_1 D_2]$ максимальный отрезок на пути $\Sigma$ из $D_1$ в $x$. Поскольку $|\angle (D_1D_2), (ix) %-\pi/6|<\pi/100$, точка $D_2$ может быть только точкой дискретного энергетического множества порядка $2$ или точкой %ветвления.

%Из Леммы~\ref{alm} следует, что в каждой точке $\bar x \in B_\rho(x) \cap G_\Sigma \setminus \{x\}$ существуют %односторонние касательные. 

Несложно заметить, что поскольку $\sharp (\partial B_{\rho_2}(x) \cap \Sigma)=1$, каждая точка ветвления на пути из $z$ в $x$ соединена ребром с концевой точкой:

%БЛИН ДОЛЖНО ЖЕ БЫТЬ ПРОСТОЕ ОБЪЯСНЕНИЕ

Предположим противное. В таком случае на пути из $z$ в $x$ найдется точка ветвления $A$, соединенная с точкой ветвления $B$, не лежащей на пути из $z$ в $x$.  При этом хотя бы один из двух отрезков $\Sigma \setminus [AB]$, инцидентных $B$, не является перпендикулярным или параллельным $(ax]$ с точностью до $\pi/100$, таким образом он неизбежно заканчивается точкой ветвления, из которой также исходит хотя бы один отрезок, который не является перпендикулярным или параллельным $(ax]$ с точностью до $\pi/100$. И так далее. В таком случае найдется путь, начинающийся с этого отрезка и никогда не заканчивающийся, причем направления отрезков одинаковой четности --- одинаковые. Несложно заметить, что предельная точка $w$ этого пути должна принадлежать непрерывному энергетическому множеству и лежать в шаре  $B_\rho(x)$, а тогда, ввиду изложенного в пункте (А) (см замечание~\ref{remA}), её энергетическое ребро должно быть направлено в две стороны. 
Однако в таком случае, при достаточно малом $\rho_2$ выполняется $\partial B_{xw}(x) \cap \Sigma \cap Q_1=\{w \}$, а это противоречит существованию пути из $z$ в $x$ лежащего в $Q_1$ и не содержащего $w$.


%Но мы считаем ребро $(ax]$ отрицательной полуосью абсцисс, а точку $w$ лежащей выше пути из $z$ в $x$, а в таком случае любая точка, соответствующая точке $w$ должна находиться в верхней полуплоскости. 
% а значит $B_r(y(w))$ содержал бысти (поскольку, как следует из  п.3. доказательства Леммы~\ref{Losiu}, $(w, y(w))$ %перпендикулярна $(ax)$ с точностью до $\pi/100$). 
Получили противоречие с тем, что энергетическое ребро точки $w$ направлено в две стороны).

Таким образом, ввиду п.~\ref{__1} Леммы~\ref{alm} в каждой точке ветвления на пути из $z$ в $x$ угол между входящим в нее отрезком этого пути и прямой $(ax)$ находится в промежутке $[\pi/6-\pi/100, \pi/6+\pi/100]$. Пусть $D_1$ --- точка ветвления на пути  из $z$ в $x$ и пусть $[D_1 D_2]$ --- максимальный отрезок на пути $\Sigma$ из $D_1$ в $x$. Поскольку $|\angle (D_1D_2), (ax) -\pi/6|<\pi/100$, точка $D_2$ может быть только точкой дискретного энергетического множества порядка $2$ или точкой ветвления.
Если точка $D_2$ --- точка ветвления, то, аналогично, конец максимального отрезка $[D_2D_3]$ может быть точкой дискретного энергетического множества порядка $2$ или точкой ветвления, а угол $\angle((D_2D_3),(ax))=\pi/3-\angle((D_1D_2),(ax))$, то есть находится в промежутке $[\pi/6-\pi/100, \pi/6+\pi/100]$. Если же $D_2$ --- точка дискретного энергетического множества порядка $2$, то ввиду п.~\ref{__2} Леммы~\ref{alm}
\[
\angle((D_2D_3),(ix)) \in [\angle((D_1D_2),(ix))-\pi/100, \angle((D_1D_2),(ix))+\pi/100] \subset [\pi/6-\pi/50,\pi/6+\pi/50],
\]
где $[D_2D_3]$ --- максимальный отрезок пути из $D_2$ в $x$. Таким образом путь из $D_1$ в $x$ начинается с ломаной. При этом угол между односторонней касательной и прямой $(ix)$ в узлах ломаной либо принадлежит промежутку $[\pi/6-\pi/100, \pi/6+\pi/100]$ (если узел был точкой ветвления), либо меняется на величину, не превосходящую $\pi/100$. Поскольку, ввиду утверждения~\ref{brrrr}, путь $[sx]$ не может содержать ломаную с пятью подряд узлами в энергетических точках, односторонние касательные в которых имеют угол с $(ax)$, больший $1/10$, среди первых пяти после $D_1$ узлов ломаной должна встретиться точка ветвления $C$. При этом поскольку все односторонние касательные к точкам пути между $D_1$ и $C$ имеют угол c $(ax)$, больший $\pi/6-\pi/20>\pi/10$, там не будет точек из непрерывного энергетического множества.

Повторяя рассуждения для точки $C$ в качестве $D_1$, а затем итерируя, получаем путь $\sigma$, все односторонние касательные вдоль которого имеют угол с $(ax)$, больший $1/10$. Пусть $\bar x$ предельная точка такого пути ($\bar x$ принадлежит пути из $z$ в $x$ и может совпадать с $x$). Ясно, что $\oordball_\sigma \bar x =1$. Выберем $\rho_0>0$ таким, что 
\[
\sharp (\sigma \cap \partial B_{\rho_0}(x_0))=1.
\]
Определим \[z_0=z_0(\rho_0) \defeq \partial B_{\rho_0}(x_0) \cap \sigma.\]
Пусть $(a_0x_0]$ энергетическое ребро $x_0$ ближайшее к энергетическим точкам $\sigma \cap B_{\rho_0}(x_0)$.
Тогда 
\[
\angle z_0x_0a_0=o_1(\rho_0)
\]
и 
\[ 
\H(Pr_{(a_0x_0]}(\sigma \cap B_{\rho_0}(x_0))) \geq \cos (\angle z_0x_0a_0) |z_0 x_0|.
\]
При этом $\angle ((ax], (a_0x_0])=o_{\rho_2}(1)$, а значит, при достаточно малом $\rho_2$, все односторонние касательные к $\sigma \cap B_{\rho_0}(x_0)$ имеют угол с $(a_0x_0]$, больший $1/20$.
Тогда
\[
\H(\sigma \cap B_{\rho_0}(x_0)) \geq \frac{Pr_{(a_0x_0]}(\sigma \cap B_{\rho_0}(x_0))}{\cos \frac{1}{10}}\geq \frac{\cos (\angle  z_0x_0a_0)}{\cos \frac{1}{10}}|z_0 x_0|=\frac{\cos (o_{\rho_0}(1))}{\cos \frac{1}{10}}\rho_0.
\]
С другой стороны, поскольку ребро $(a_0x_0]$ направлено в обе стороны, выполняется $\H(\sigma \cap B_{\rho_0}(x_0))=\rho_0+o_{\rho_0}(1)$. Противоречие для достаточно малого $\rho_0$.


%То есть при достаточно малом $\rho_0$ выполняется $\H(\sigma \cap B_{\rho_0}(x_0)) > |z_0x_0|(1+10^{-4})$.



%Тогда \[\H(\sigma \cap B_{\rho_0}(\bar x))>\frac{\rho_1}{\cos {\frac{1}{10}}}|z_0\bar x|.\]
%Пусть $\beta(\rho_0)$ --- минимальный угол с вершиной в $\bar x$, содержащий все точки $Q_\Sigma \cap \sigma \cap B_{\rho_0}(\bar x)$. Заметим, что $\angle \beta(\rho_0)=o_{\rho_0}(1)$. Обозначим 
%\[
%\breve{u_0v_0} \defeq \beta(\rho) \cap \partial B_{\rho_0}(\bar x).
%\]
%Тогда множество
%\[
%\Sigma \setminus (\sigma \cap B_{\rho_0}(\bar x)) \cup [\bar x z_0] \cup \breve{u_0v_0} \cup S^{[u_0\bar x]} \cup S^{[v_0 \bar x]}
%\]
%имеет длину $|z_0x_0|+o(|z_0x_0|)$, а значит данное множество связно, обладает меньшей длиной и не большей энергией, чем $\Sigma$. Противоречие.

%Пусть $(\bar a \bar x]$ --- %энергетическое ребро $\bar x$, к %которому сходятся энергетические точки %пути (он существует ввиду ). В таком %случае 



%Заметим, что для любого $\rho_1<|D_1x|$ такого, что $\sharp(\partial %B_{\rho_1}(x))=1$, выполняется $\H(\Sigma \cap Q \cap %B_{\rho_1}(x))>\frac{\rho_1}{\cos {\frac{1}{10}}}$. Получили %противоречие с тем, что $\H(\Sigma \cap Q \cap %B_{\rho_1}(x))=\rho_1+o(\rho_1)$.
%Утверждение про наклон касательной непосредственно следует из Утверждения~\ref{zapred}.
\end{itemize}
Осталось доказать пункт~\ref{AB}. 
Не умаляя общности будем считать, что ребро $(ax]$ направлено в одну сторону, поскольку в противном случае применим пункт~\ref{A} (см замечание~\ref{remA}).
Пусть $\varepsilon>0$ такое, что $\sharp (\partial B_\varepsilon(x)\cap \Sigma)=\oordball_x\Sigma \leq 3$. И пусть $s \in \partial B_\varepsilon(x)$ такая, что путь из $s$ в $x$ лежит в $\overline{B_\varepsilon(x)}$.

Рассмотрим величину поворота пути: $|\turn(\breve{sx})|<2\pi$. Аналогично рассуждениям в предыдущем пункте заметим, что конечность величины поворота и наличие в компоненте связности энергетических точек только одного ребра, причем направленного в одну сторону, влечет конечность числа точек ветвления на пути из $s$ в $x$. Таким образом можно выбрать $\varepsilon>0$ таким, что $\breve{sx}$ не содержит точек ветвления.

Тогда ввиду Леммы~\ref{dug_ok}  $\breve{sx}$  содержится внутри некоторого псевдоконуса.

%Пусть инъективная функция $f: [0;1] \rightarrow \R^2$ параметризует $\breve{[sx]}$. Множество $\breve{[sx]} \cap G_\Sigma$ содержится в псевдоконусе $Q_{\rho}^{a,x}$. Будем также считать, что это псевдоконус имеет следующий вид: $Q^{a,x}_{\varepsilon} \defeq \bigcup_{k=1}^{\infty} \left( Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) \right)$ для некоторых сходящихся к нулю монотонных последовательностей неотрицательных чисел $\{s_k\}$ и $\{\rho_k\}$, где $\rho_1=\varepsilon$ (см Лемму~\ref{con}). Будем считать выбранные последовательности минимальными по включению. Пусть точки $c,d \in [0;1]$ такие, что $f([c,d])\cap G_\Sigma=f(c) \cup f(d)$. Тогда, ввиду отсутствия на дуге $\breve{[sx]}$ точек ветвления, выполняется $f([c,d])=[f(c),f(d)]$. В таком случае, если $f(c) \in Q(\rho_{k-1},s_{k-1},x,a) \setminus B_{\rho_{k}}(x) $, $f(d) \in Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) $, то выполняется $[f(c);f(d)] \subset  Q(\rho_{k-1},s_{k-1},x,a) \setminus B_{\rho_{k+1}}(x)$. А значит, 
%\[
%\breve{[sx]}=f([0;1]) \subset \bar{Q}^{a,x}_{\varepsilon} \defeq \bigcup_{k=1}^{\infty} \left(Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+2}}(x) \right).
%\]
%Тогда к $\breve{[sx]}$ применим пункт~\ref{A}.
%МОЖЕТ НАДО ВЕРНУТЬ
%\end{proof}

\end{proof}

%Докажем лемму~\ref{eva}. может вернем сюда
%ВРОДЕ ИЗ ТОГО, ЧТО ДАЛЬШЕ --- НИЧЕГО НЕ НУЖНО. ПЕРЕНЕСЛА ЭТО в trash801 %пока

ОСТАТКИ ПЕРЕВОДА ДЛЯ ФИНЛЯНДИИ:

In fact, in the announced work even stronger result is proven: all these statements hold for a larger class of local minimizers.

 \begin{definition}
    Let $M \subset \mathbb{R}^2$ be a planar compact set. A connected set $\Sigma$ is called \emph{local minimizer} if it covers $M$
    and there is an $\varepsilon > 0$ such that for every connected $\Sigma'$ covering $M$ and satisfying
    $\diam (\Sigma \Delta \Sigma') \leq \varepsilon$ one has $\H (\Sigma) \leq \H (\Sigma')$.
    \label{local}
\end{definition}


\begin{theorem2}
Let $\Sigma$ be a local minimizer. Then all the statements of Theorems~\ref{mainT1} and~\ref{persp} hold.
\label{TTT}
\end{theorem2}

\begin{corollary}
Theorem~\ref{mainT1} (accordingly~\ref{TTT}) implies that the set of branching points of a (local) minimizer is finite.  
\end{corollary}



==> parts/per.tex <==
\section{Остальные локальные свойства минимайзеров}
\label{per}


Использованные в статье методы позволяют получить большое количество утверждений относительно гладкости и локальной структуры $\Sigma$. %В частности,

%\subsection{Еще несколько результатов}

%\begin{remark}
%А обозначениях теоремы~\ref{mainT1} можно считать, что каждая инъективная кривая имеет на конце непрерывную касательную. Иными словами, односторонние касательные ко внутренним точкам кривой сходятся к касательной в концевой точке.
%\end{remark}

\begin{theorem2}
Пусть $\Sigma$ --- минимайзер максимального расстояния для плоского компактного множества $M$.  Тогда
\begin{enumerate}
\item в окрестности произвольной точки $x\in \Sigma$ множество $\Sigma$ совпадает с одной, двумя или тремя дугами с концами в $x$, имеющими в $x$ непрерывную касательную %(соответствующие им функции имеют в $x$ непрерывную первую производную).   
Также в каждой из точек каждой из дуг есть односторонняя касательная, односторонние касательные непрерывно сходятся к касательной к дуге в точке $x$.
Каждая из дуг является графиком функции, имеющей в точке $x$ непрерывную производную (за абсциссу считаем касательную). 
%Для краткости будем называть такие функ
\label{f}
\item в достаточно малой окрестности $B_{\varepsilon}(x)$ произвольной точки $x\in \Sigma$ выполняется
 \[
  \oord_x\Sigma \cdot \varepsilon \leq \H(\Sigma \cap B_\varepsilon(x)) = \oord_x \Sigma \cdot \varepsilon +o(\varepsilon).
 \]
 Заметим, что это уточняет константы регулярности по Альфорсу (см. свойства минимайзеров п.~\ref{j});
 \label{len1}
\item для произвольной точки $x\in \Sigma$ выполняется $\oord_x\Sigma=\oordball_x\Sigma$; 
\label{oo}
\item множество $\Sigma$ в окрестности произвольной $x \in G_\Sigma$ является графиком некоторой функции %(для краткости будем называть такую функцию "соответствующей"). 
Если точка $x \in G_\Sigma$ имеет два различных касательных луча, угол между которыми меньше $\pi$, то $\Sigma$
%(как функция) 
локально нестрого выпукла в окрестности точки $x$ (выпукла внутрь меньшего угла). В таком случае соответствующая функция нестрого выпукла, то есть, в частности,
%$\Sigma$ в окрестности $x$ является графиком нестрого выпуклой функции, то есть, в частности, функции, которая 
%Это, в частности означает, что соответствующая ей функция 
почти всюду имеет вторую производную;
\label{conv_}
\item если (содержащаяся в $\Sigma$) инъективная кривая с концом в точке $x$ не является нестрого выпуклой в её окрестности, то 
\label{nevv}
\begin{enumerate}
\item если она имеет кривизну, то кривизна по модулю не превосходит $1/r$ (если соответствующая данной кривой функция имеет в точке $x$ вторую производную, то она по модулю не превосходит $1/r$);
\item её односторонние касательные сходятся к односторонней касательной в точке $x$ (соответствующая данной кривой функция имеет непрерывную первую производную в точке $x$);
\label{ggg}
\item если существует другая инъективная кривая с концом в $x$, то  ее кривизна, в случае наличия, по модулю не превосходит $1/r$, а её односторонние касательные сходятся к односторонней касательной в точке $x$. При этом односторонние касательные к обеим инъективным кривым образуют прямую (то есть, функция, соответствующая $\Sigma$, имеет непрерывную производную в $x$); 
\item в достаточно малой окрестности $B_{\varepsilon}(x)$  выполняется
 \[
\oord_x\Sigma \cdot \varepsilon  \leq \H(\Sigma \cap B_\varepsilon(x)) \leq \oord_x\Sigma \cdot \varepsilon +O(\varepsilon^2).
 \]
 \label{len2}
\end{enumerate}
\end{enumerate}
\label{persp}
\end{theorem2}
\begin{proof}

Докажем пункт~\ref{f}. Из доказательства Теоремы~\ref{mainT1}  следует, что
каждая такая дуга либо является отрезком, либо содержится в псевдоконусе с вершиной в $x$ и энергетическим ребром в качестве оси. В первом случае утверждение пункта очевидно, а во втором следует из леммы~\ref{zapred}.
%\end{proof}
%леммы~\ref{eva} ы~\ref{uggi}
Покажем верность пункта~\ref{len1}. Множество $\Sigma \setminus \{x\}$ имеет $\oord_x \Sigma \leq 3$ компонент связности. Каждая из компонент связности, ввиду Теоремы~\ref{mainT1} имеет в точке $x$ касательную, а значит ввиду замечания~\ref{len0}, в достаточно малом шаре $B_\varepsilon(x)$ имеет длину $\varepsilon+ o(\varepsilon)$. 

Таким образом
\[
\H(\Sigma \cap B_\varepsilon(x)) =\oord_x \Sigma \varepsilon +o(\varepsilon).
\]
 Неравенство $\H(\Sigma \cap B_\varepsilon(x)) $ напрямую следует из неравенства коплощади

Покажем верность пункта~\ref{oo}. Предположим противное, то есть, ввиду замечания~\ref{rem_ord}, что $\oordball_x\Sigma >\oord_x\Sigma $.
В таком случае для достаточно малого $\varepsilon$
\[
\H(\Sigma \cap B_\varepsilon(x)) \geq \oordball_x \Sigma \varepsilon \geq (\oord_x \Sigma +1) \varepsilon,
\]
что противоречит утверждению пункта~\ref{len1}.

Докажем пункт~\ref{conv_}. Утверждение интересно только для $x\in E_\Sigma$. В таком случае хотя бы одна из двух касательных является энергетическим ребром, при этом ребро направлено в одну сторону. Рассмотрим дугу $\breve{sx}$, являющуюся замыканием компоненты связности $\Sigma \cap B_\varepsilon(x) \setminus \{x\}$ для достаточно малого $\varepsilon$, для которой данное энергетическое ребро является касательной в точке $x$. Не умаляя общности, будем полагать это ребро совпадающим с отрицательной частью оси абсцисс и будем полагать его направленным вверх. Будем также полагать, что для всех энергетических точек, принадлежащих $\breve{sx}$, соответствующие им точки находятся в верхней полуплоскости (это возможно ввиду показанного в лемме~\ref{Losiu}). В таком случае не существует двух точек $z_1, z_2 \in \breve{]sx[} $ таких, что поддуга $\breve{sx}$, их соединяющая, находится ниже соединяющего их отрезка: в противном случае замена дуги на отрезок уменьшило бы длину, без ущерба для связности и энергии. Несложно заметить, что данное свойство влечет нестрогую выпуклость вверх дуги $\breve{sx}$. Также мы показали, что $\breve{sx}$ можно рассматривать как график нестрого выпуклой функции.

Перейдем к пункту~\ref{nevv}: как было показано выше точка $x$ должна принадлежать множеству $E_\Sigma$, причем иметь энергетическое ребро, направленное в две стороны. В таком случае найдутся такие точки $y_1$, $y_2$, что прямая $(y_1y_2)$ перпендикулярна энергетическому ребру, \[|y_1x|=r=|xy_2|\] и \[B_r(y_1) \cap \Sigma =\emptyset = B_r(y_2)\cap \Sigma.\]
Отсюда тривиально следуют все утверждения пункта.
%\begin{remark}
%Доказательство  пунктов~\ref{len1} и~\ref{len2} можно было бы провести и аналитически, сопоставив кривой график функции $f$, точке $x$ начало координат, а касательной к кривой в точке $x$ --- ось абсцисс. Тогда $f(0)=0=f'(0)$. В случае~\ref{len2} кривую также пришлось бы сгладить, после чего заметить ограниченность модуля второй производной гладкой функции, приближающей $f$, числом $1/r$. 
%\end{remark}

\end{proof}
%Доказательства Теоремы~\ref{persp} 
%можно найти в разделе~\ref{prf}, 
%и объяснение, как методами данной статьи получать другие локальные утверждения можно найти в разделе~\ref{per}.
%Доказаны также некоторые еще утверждения про выпуклость %множества $\Sigma$ (см Леммой~\ref{main_ld}).


На самом деле, мы доказали даже более сильный результат, поскольку в доказательствах Теорем~\ref{mainT1} и~\ref{persp}  использовались только локальные аргументы, и поэтому его можно провести и для определенного ниже локального минимайзера.

\begin{definition}
Для заданного компактного множества $M \subset \R^2$ и числа $r>0$ локальным минимайзером функционала максимального расстояния будем называть такое связное замкнутое множество $\Sigma \subset \R^2$, что $F_M(\Sigma)\leq r$ и существует такое $\varepsilon>0$, что для произвольного замкнутого связного $\Sigma'$ такого, что $F_M(\Sigma')\leq r$ и $\diam \Sigma \triangle  \Sigma' < \varepsilon$ выполняется $\H(\Sigma)\leq \H(\Sigma')$.
\end{definition}

\begin{theorem2}
Пусть $\Sigma$ --- локальный минимайзер максимального расстояния.  Тогда выполняются все утверждения Теорем~\ref{mainT1} и~\ref{persp}.
%\begin{itemize}
%\item[(i)] множество $\Sigma$ является объединением конечного числа инъективных кривых;
%\item[(ii)] угол между любыми двумя касательными лучами в произвольной точке $x \in \Sigma$ не меньше $2 \pi/3$.
%\end{itemize}
%\label{mainT2}
\end{theorem2}

%\begin{corollary}
%Из Теоремы~\ref{mainT1} следует конечность числа точек порядка $3$ в (локальном) минимайзере максимального расстояния.
%\end{corollary}






%Покажем  верность Теоремы~\ref{persp}.


Поговорим о том, как получать иные утверждения о локальном поведении $\Sigma$. Оно интересует нас только в окрестностях точек из множества $E_\Sigma$. Ясно, что точки $E_\Sigma$ бывают следующих типов:
%\begin{enumerate}
%\item точки ветвления $x\in S_\Sigma$ степени $3$. Таких точек конечное число, поэтому при исследовании окрестностей точек $x\in %E_\Sigma$ можно считать, что их не существует.
%\item точки $x\in S_\Sigma$ степени $2$. Касательная в этих точках не меняется.
%\item точки $x\in X_\Sigma$ степени два такие, что существуют две окружности с центрами в $y_1,y_2$ такие, что $|y_1y_2|=2r$ и %$B_r(y_1)\cap \Sigma=\emptyset=B_r(y_2)\cap \Sigma$. В этом случае в точке $x$ касательная не меняется.
%\item Более интересные точки:
\begin{itemize}
%\item [(a)] точки $x\in X_\Sigma$ степени два такие, что в них $\Sigma$ имеет два разных отрезка с углом, не равным $\pi$; 
\item [(i)] точки $x\in E_\Sigma$ такие, что не существует двух окружностей с центрами в $y_1,y_2$ таких, что $|y_1y_2|=2r$ и $B_r(y_1)\cap \Sigma=\emptyset=B_r(y_2)\cap \Sigma$. Тогда $\Sigma$ в окрестности точки $x$ (нестрого) выпукла. % (однако хотя бы одна окружность $B_r(y)$, такая что $B_r(y)\cap\Sigma=\emptyset$ существует и ее расположение задает направление выпуклости). 
А значит, имеет субградиент, а также почти всюду выпукла и являются графиком функции, которая почти всюду %(но не обязательно в $x$)
имеет производную, которая монотонна;
\item [(ii)] точки $x\in E_\Sigma$ такие, что существуют две окружности с центрами в $y_1,y_2$, такие что $|y_1y_2|=2r$ и $B_r(y_1)\cap \Sigma=\emptyset=B_r(y_2)\cap \Sigma$. Тогда $\Sigma$ является графиком функции, которая имеет непрерывную производную в точке $x$. А если она имеет вторую производную, то та ограничена по модулю величиной $1/r$. 
\end{itemize}
%\end{enumerate}
%При этом точки типа (ii) являются пределом либо точек степени (ii), либо точек типа (i) или (a), где пустые окружности расположены по разную сторону от кривой. При этом выпуклость может меняться только в точках типа (ii), либо (в некотором смысле) в таких точках типа (i), что одна из кривых --- прямолинейный отрезок.

Если какая-то дуга минимайзера (c концом в $x$) целиком состоит из точек типа (i), то она наследует свойства некоторого подмножества множества $M$: утверждается, что множество $M$ тогда должно иметь кривую (или счетный набор кривых), полученную из данной дуги отступлением по внешней (если считать дугу границей выпуклой фигуры) нормали на $r$ во всех точках, где нормаль единственна (то есть в почти всех точках дуги). В частности, если дуга была непрерывно дифференцируемой, то ей соответствует дуга множества $M$. Причем данная дуга $\Sigma$ тогда должна быть дважды дифференцируемой, соответствующая ей дуга множества $M$ также должна быть дважды дифференцируемой, причем её вторая производная должна не превосходить $1/r$. Если она строго меньше $1/r$, то есть минимальный радиус кривизны дуги $M$ больше $r$, то тогда минимальный радиус кривизны дуги $\Sigma$ в точности равен разности между минимальным радиусом кривизны дуги $M$ и числом $r$. Доказательство данного факта мы приводить не будем, оно является достаточно очевидным следствием основного свойства энергетических точек. 

Если какая-то дуга целиком состоит из точек типа (ii), то она является непрерывно дифференцируемой. Тогда множество $M$ содержит две дуги полученных из данной дуги $\Sigma$ отступами по обеим нормалям на $r$. Несложно заметить, что тогда исходная дуга является дважды дифференцируемой и значит её вторая производная по модулю ограничена величиной $1/r$. При этом радиусы кривизны кривых $M$ отличаются от её радиусов кривизны в каждой точке на $r$.

Таким образом, получается что точки всех видов обладают рядом полезных свойств, комбинируя которые можно получать новые свойства $\Sigma$ или отвечать на вопрос, может ли то или иное множество быть минимайзером (отвечать отрицательно или конструктивно строить множество $M$, для которого данное множество может быть минимайзером). В частности --- графики элементарных функций, поскольку они (кроме графиков константы) обязаны состоять только из точек типа (i) и (ii).

\begin{example}
Может ли кривая, являющаяся графиком функции $f(x)= x^2\sin(\frac{1}{x})$ в окрестности нуля быть минимайзером для некоторого множества $M$?
\end{example}
\begin{proof}
Заметим, что точка $0$ --- точка типа (ii). Но производная функции $f$ не является непрерывной в нуле и значит график данной функции не может быть минимайзером. 
\end{proof}

\begin{example}
Может ли кривая, являющаяся графиком функции $f(x)= x^2 \sin \left (\frac{1}{\sqrt{x}} \right)$ в окрестности нуля быть минимайзером для некоторого множества $M$?
\end{example}
\begin{proof}
Заметим, что точка $0$ --- точка типа (ii). Теперь производная $f$ непрерывна в нуле. Поскольку для каждой точки $x\neq 0$ вторая производная существует, непрерывна и ее значение по модулю стремится к бесконечности при приближении к нулю и, значит, можно считать, что она больше, чем $1/r$. Тогда каждая точка, кроме $0$ может быть только типа (i). Но знак второй производной все время меняется и, значит, существует стремящаяся к нулю последовательность точек, в которых кривая меняет выпуклость. Ввиду отсутствия прямолинейных отрезков получили противоречие.
\end{proof}
%а выпуклость может меняться?



%Покажем верность правых частей в неравенствах пунктов~\ref{len1} и~\ref{len2}. Для этого достаточно показать, что %длина каждой из кривой


%Осталось доказать пункты~\ref{len1} и~\ref{len2}. Левые части следуют из неравенства ко-площади Предположим, это не так и длина какой-то из кривых
%ой еще про орд равно ордболл


%точки первого и второго типа
%пример: рассказ почему x^2\sin(\sqrt{x}) не подходит, хотя казалось бы а ой нет она же гладкая вне нуля и значит вт произв дб ограничены а они нет

==> parts/trash.tex <==


Let $Q_1$ and $Q_5$ be such cusps with vertices at $L_1$ and $L_5$ and axes almost parallel to $o_rho(\bar x)$ that 

Let $S$ be the point of intersection $\partial B_r(y(L_1))$ and $\partial B_r(y(L_3))$. Let $A'$ be an area bounded by $[L_1,L_5]$, $\breve{L_1S}, $\breve{L_5S}$ where the arcs are the arcs of circumferences $\partial B_r(y(L_1))$ and $\partial B_r(y(L_3))$. And let $A$ be the union of $A'$ and its reflection regarding to $L_1L_5$. Thus $A$ is a union of two cusps $Q_1\in \mathbb{Q_{|L_1S|}}^{L_5,L_1}$ and $Q_5\in \mathbb{Q_{|L_5S|}}^{L_1,L_5}$. Then sets $S^{Q_1}$ and $S^{Q_5}$ defined at the proof of lemma~\ref{angles2} are such that $\H(S^{Q_1})=o(|L_1S|)$, $\overline{B_r(Q_1)}\subset \overline{B_r(S^{Q_1})}$
URURU


Let us construct a 


Now look at the set $ \Sigma \setminus ([L_2L_3] \cup [L_3L_4]) \cup [L_2L_4]\cup S^{[L_1L_5]}$, where $S^{[L_1L_5]}$ is defined in the proof of lemma~\ref{angles2}.



  
 Тогда множество $ \Sigma \setminus ([L_2L_3] \cup [L_3L_4]) \cup [L_2L_4]\cup S^{[L_1L_5]}$ лучше $\Sigma$: является связным (поскольку все внутренние точки исходной ломаной --- степени два), обладает меньшей длиной и не большей энергией. Противоречие с оптимальностью $\Sigma$ (см. рис~\ref{fig:dvapo}).



Предположим противное, то есть (ввиду Леммы~\ref{alm} п.~\ref{__2} для $c= \bar c/ 10$) что для сколь угодно малого $\rho > 0$ существует такая ломаная $L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\rho}$, что все углы $\angle((L_iL_{i+1}),(ix))> \bar{c}/2$ при $i=1,2,3,4$. 
Будем считать $(ix)$ осью абсцисс, а $\bar{c}$ достаточно малым. Не умаляя общности, точкам $L_1$, $L_3$, $L_5$ соответствуют верхние точки множества $M$, а точкам $L_2, L_4$ --- нижние: ввиду пункта~\ref{1145} доказательства Леммы~\ref{Losiu} и неравенства $\angle L_{i-1}L_{i}L_{i+1} \leq \pi-\bar{c}$, $i=2,3,4$ двум подряд идущим точкам не могут соответствовать одновременно верхние или нижние точки.
 Заметим теперь, что отношения между отрезками ломаной линейные (то есть отношение оценивается сверху и снизу константой, зависящей от $\bar{c}$), и замена ломаной на отрезки $L_1-L_2-L_4-L_5$ уменьшит длину на величину, линейно зависящую от $[L_1L_2]$:
 поскольку $L_3 \notin B_r(y(L_1))$ выполняется 
 \[
 |Pr_{(y(L_1)L_1)}[L_2L_3]|<|Pr_{(y(L_1)L_1)}[L_1L_2]|+o(|L_1L_3|).
 \label{1111}
 \]
  Поскольку 
  \[
  |\angle (y(L_1)L_1), (ix])-\pi/2| =o_\rho(1)
  \]
 выполняется 
 \[
 |L_2L_3|_y<|L_1L_2|_y+o(|L_1L_2|+|L_2L_3|),
 \]
 где $|\cdot |_y$ означает длину проекции на прямую, перпендикулярную $(ix)$. Тогда
 \[
 |L_2L_3|\sin \frac{ \bar{c}}{2}<|L_1L_2|+o(|L_1L_2|+|L_2L_3|),
 \]
 то есть
 \[
 |L_2L_3|< \frac{1}{\sin \frac{ \bar{c}}{2}}|L_1L_2|+o(|L_1L_2|+|L_2L_3|). 
 \]
%Тогда для достаточно малого $\rho$ выполняется

 Аналогично, поскольку  $L_3 \notin B_r(y(L_1))$ и $|\angle (y(L_3)L_3), (ix])-\pi/2| =o_\rho(1)$ выполняется
  \[
 [L_2L_1]<\frac{1}{\sin \frac{ \bar{c}}{2}}|L_3L_2|+o(|L_1L_2|+|L_2L_3|). 
 \]
 В таком случае
 \[
\sin\frac{ \bar{c}}{2}- \frac{o(|L_1L_2|+|L_2L_3|)}{|L_3L_2|}\leq  \frac{|L_2L_3|}{|L_1L_2|}\leq \frac{1}{\sin \frac{ \bar{c}}{2}}+\frac{o(|L_1L_2|+|L_2L_3|)}{|L_1L_2|},
 \]
 а значит, для достаточно малого $\rho$ верно
 \[
\frac{\bar c}{3} < \sin \frac{ \bar{c}}{2}- \frac{o(|L_2L_3|(1+\frac{1}{\sin\frac{ \bar{c}}{2}}|L_1L_2|+o_\rho(1)))}{|L_3L_2|}\leq  \frac{|L_2L_3|}{|L_1L_2|}\leq \frac{1}{\sin \frac{ \bar{c}}{2}}+\frac{o(|L_1L_2|(1+ \frac{1}{\sin \frac{ \bar{c}}{2}}+o_\rho(1)))}{|L_1L_2|}< \frac{3}{\bar{c}}.
 \]
 
  %\[[L_2L_3]_y>|L_1L_2|_y-|L_1L_3| o_{\varepsilon(c)}(1)\]
 %|L_1L_2|-\bar{\varepsilon}^2,\]
  %где нижний индекс $y$ означает проекцию на ось абсцисс. То есть $|L_2L_3|>\sin c |L_1L_2|-o_{\bar{\varepsilon}}(1)|L_1L_3|$.
% И наоборот, $|L_1L_2|>\sin \bar{c} |L_2L_3|-o_{\bar{\varepsilon}}(1)|L_1L_3|$. 
 %Из этого очевидным образом следует существование $c_1, c_2>0$ таких, что $c_2|L_2L_3|\geq |L_1L_2| \geq c_1|L_1L_3|$.   
 Аналогично и для остальных $L_i$. 
 
 Замена ломаной $L_1-L_2-L_3-L_4-L_5$ на $L_1-L_2-L_4-L_5$ уменьшит ее длину не меньше, чем на величину, линейно зависящую от $|L_1L_2|$, поскольку $\angle L_2L_3L_4 \leq \pi-\bar{c}$ (а значит $\cos \angle L_2L_3L_4 \geq  -\cos \bar{c}$):
 \begin{multline*}
 |L_2L_3|+|L_3L_4|-|L_2L_4|=\frac{(|L_2L_3|+|L_3L_4|)^2-|L_2L_4|^2}{|L_2L_3|+|L_3L_4|+|L_2L_4|}>\\
 > \frac{2|L_2L_3||L_3L_4| (1+ \cos \angle L_2L_3L_4)}{2(|L_2L_3|+|L_3L_4|)}\geq
 \frac{|L_3L_4|(1- \cos \bar{c})}{ \left (1+\frac{|L_3L_4|}{|L_2L_3|} \right)}\geq  \frac{(\frac{\bar{c}}{3})^3}{(1+\frac{3}{\bar{c}})}|L_1L_2|.
\end{multline*}
 
 
 
% \[
% |L_2L_3|+|L_3L_4|-|L_2L_4|\geq  |L_2L_3|(1+\frac{c}{3}-\frac{1}{\sin c})>|L_2L_3|(1+\frac 2 c),
 %\]
 %поскольку 
 %\[
 %|L_2L_4|=\sin \angle L_2L_3L_4 \frac{|L_2L_3|}{\sin L_2L_4 L_3}\leq  \frac{|L_2L_3|}{\sin L_2L_4 L_3} \leq  \frac{|L_2L_3|}{\sin (\pi-c)}= \frac{|L_2L_3|}{\sin c}.
 %\]
 %ой ОЙОЙ ТУТ НЕ ТАК
 
% \begin{multline*}
 %|L_2L_3|+|L_3L_4|-\sqrt{ |L_2L_3|^2+|L_3L_4|^2+2 %|L_2L_3||L_3L_4|\cos (2c) }\geq \\
%|L_1L_2| \left(\sin c+\sin^2 c-\sqrt{\frac{1}{\sin^2 c}+\frac{1}{\sin^4 c}+2\frac{\cos (2c)}{\sin^3 c}})+o_{\varepsilon(c)}(1|L_1L_2| \right),
% \end{multline*}
%Таким образом замена уменьшает длину множества на величину, линейно зависящую от $|L_1L_2|$.
%\input{pictures/dvapo}
%Обозначим точки $L_6 \defeq [L_1y(L_3)] \cap \partial B_r(y(L_3))$ и $L_7 \defeq [L_5y(L_3)] %\cap \partial B_r(y(L_3))$ где $y(L_3)$ произвольная соответствующая $L_3$ точка. Тогда %$$B_r([L_1L_6]) \cup B_r([L_5L_7]) \supset B_r([L_1L_3]) \cup B_r([L_3L_5]).$$ и %$\H([L_1L_6]) \cup B_r([L_5L_7]))=o_{[L_1L_2]}(1)$ (это следует из теоремы Пифагора и  %пункта~\ref{1145} доказательства Леммы~\ref{Losiu}). Тогда можно заменить ломаную  %$L_1-L_2-L_3-L_4-L_5$ на $L_6-L_1-L_2-L_4-L_5-L_7$ и получить противоречие с оптимальностью %$\Sigma$ (см. рис~\ref{fig:dvapo}).
%А значит
%\[
%\H([L_1L_2]\cup [L_2L_4]\cup[L_4L_5]\cup S^{[L_1L_5]})\leq \H(L_1-L_2-L_3-L_4-L_5)-|L_2L_3|(1+\frac 2 c)+o(|L_1L_5|)<\H(L_1-L_2-L_3-L_4-L_5).
%\]
Тогда множество $ \Sigma \setminus ([L_2L_3] \cup [L_3L_4]) \cup [L_2L_4]\cup S^{[L_1L_5]}$ лучше $\Sigma$: является связным (поскольку все внутренние точки исходной ломаной --- степени два), обладает меньшей длиной и не большей энергией. Противоречие с оптимальностью $\Sigma$ (см. рис~\ref{fig:dvapo}).
%ПОМЕНЯТЬ РИСУНОК ИЛИ ВЕРНУТЬ ЗАКОМЕНЧЕННОЕ



\[ 
\H(Pr_{(a_0x_0]}(\sigma \cap B_{\rho_0}(x_0))) \geq \cos (\angle z_0x_0a_0) |z_0 x_0|\geq 
\]
Herewith $\angle ((ax], (a_0x_0])=o_{\rho_2}(1)$, а значит, при достаточно малом $\rho_2$, все односторонние касательные к $\sigma \cap B_{\rho_0}(x_0)$ имеют угол с $(a_0x_0]$, больший $1/20$.
Тогда
\[
\H(\sigma \cap B_{\rho_0}(x_0)) \geq \frac{Pr_{(a_0x_0]}(\sigma \cap B_{\rho_0}(x_0))}{\cos \frac{1}{10}}\geq \frac{\cos (\angle  z_0x_0a_0)}{\cos \frac{1}{10}}|z_0 x_0|=\frac{\cos (o_{\rho_0}(1))}{\cos \frac{1}{10}}\rho_0.
\]
С другой стороны, поскольку ребро $(a_0x_0]$ направлено в обе стороны, выполняется $\H(\sigma \cap B_{\rho_0}(x_0))=\rho_0+o_{\rho_0}(1)$. Противоречие для достаточно малого $\rho_0$.


Не умаляя общности будем считать, что ребро $(ax]$ направлено в одну сторону, поскольку в противном случае применим пункт~\ref{A} (см замечание~\ref{remA}).
Пусть $\varepsilon>0$ такое, что $\sharp (\partial B_\varepsilon(x)\cap \Sigma)=\oordball_x\Sigma \leq 3$. И пусть $s \in \partial B_\varepsilon(x)$ такая, что путь из $s$ в $x$ лежит в $\overline{B_\varepsilon(x)}$.

Рассмотрим величину поворота пути: $|\turn(\breve{sx})|<2\pi$. Аналогично рассуждениям в предыдущем пункте заметим, что конечность величины поворота и наличие в компоненте связности энергетических точек только одного ребра, причем направленного в одну сторону, влечет конечность числа точек ветвления на пути из $s$ в $x$. Таким образом можно выбрать $\varepsilon>0$ таким, что $\breve{sx}$ не содержит точек ветвления.

Тогда ввиду Леммы~\ref{dug_ok}  $\breve{sx}$  содержится внутри некоторого псевдоконуса.

%Пусть инъективная функция $f: [0;1] \rightarrow \R^2$ параметризует $\breve{[sx]}$. Множество $\breve{[sx]} \cap G_\Sigma$ содержится в псевдоконусе $Q_{\rho}^{a,x}$. Будем также считать, что это псевдоконус имеет следующий вид: $Q^{a,x}_{\varepsilon} \defeq \bigcup_{k=1}^{\infty} \left( Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) \right)$ для некоторых сходящихся к нулю монотонных последовательностей неотрицательных чисел $\{s_k\}$ и $\{\rho_k\}$, где $\rho_1=\varepsilon$ (см Лемму~\ref{con}). Будем считать выбранные последовательности минимальными по включению. Пусть точки $c,d \in [0;1]$ такие, что $f([c,d])\cap G_\Sigma=f(c) \cup f(d)$. Тогда, ввиду отсутствия на дуге $\breve{[sx]}$ точек ветвления, выполняется $f([c,d])=[f(c),f(d)]$. В таком случае, если $f(c) \in Q(\rho_{k-1},s_{k-1},x,a) \setminus B_{\rho_{k}}(x) $, $f(d) \in Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) $, то выполняется $[f(c);f(d)] \subset  Q(\rho_{k-1},s_{k-1},x,a) \setminus B_{\rho_{k+1}}(x)$. А значит, 
%\[
%\breve{[sx]}=f([0;1]) \subset \bar{Q}^{a,x}_{\varepsilon} \defeq \bigcup_{k=1}^{\infty} \left(Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+2}}(x) \right).
%\]
%Тогда к $\breve{[sx]}$ применим пункт~\ref{A}.
%МОЖЕТ НАДО ВЕРНУТЬ
%\end{proof}

усть $\Sigma'$ --- замыкание компоненты связности $\Sigma \setminus \{x\}$ и пусть $\Sigma'$ содержит бесконечную последовательность энергетических точек ребра $(ax]$, сходящуюся к $x$. Пусть кроме того $\Sigma' \cap \overline{B_{\rho}(x)}$ не содержит иных энергетических точек для некоторого $\rho>0$. Тогда $\Sigma' \cap \overline{B_{\rho}(x)}$ содержит конечное число точек ветвления.  
%То есть найдется такое $\rho_1>0$, что множество $\overline{B_{\rho_1}(x)} \cap \Sigma'$ является дугой. 
Кроме того найдется такое $\rho_1>0$ и псевдоконус $Q_1 \in Q^{a,x}_{\rho_1}$, что $\Sigma' \cap \overline{B_{\rho_1}(x)}\subset Q_1$. %При этом прямые, содержащие односторонние касательные к $\Sigma $ в энергетической точке $\bar x$ ребра $(ix]$, стремятся к $(ix)$ при $\bar x \rightarrow x$, $i=a,b$.


Для любой точки $\bar{x} \in G_\Sigma \cap  \Sigma' \cap U \setminus \{ x\}$ касательные лучи к $\bar x$ параллельны ближайшему к ней энергетическому ребру $(ix]$ с точностью до $\alpha/100$.

Докажем утверждение шага от противного: пусть, не умаляя общности, точка $x^a_1 \subset Q^{a,x}_\rho \cap U \cap \Sigma' \cap X_\Sigma$ имеет порядок два. 
Пусть $[x^a_1;t]$ --- максимальный по включению  отрезок, содержащийся на пути из $x^a_1$ в $x$. Тогда, по предположению и ввиду следствия~\ref{sm_an},
\[
\alpha/100< \angle((ax),(x^a_1t)) \leq \pi/6+\alpha/100.  
\]
Несложно заметить, что $\angle ((x^a_1t],(ax])= \angle((ax),(x^a_1t))$ (а не $\pi-\angle((ax),(x^a_1x))$) поскольку в противном случае любой путь, начинающийся с $x^a_1-s$, где $[x^a_1s]$ --- второй максимальный отрезок инцидентный $x$, находится внутри области, ограниченной путем из $x^a_1$ в $x$ и двумя пустыми шарами с радиусом $r$ и с центрами в точке, соответствующей $x^a_1$, и в точке сгущения точек, соответствующих энергетическим точкам ребра $(ax]$. В таком случае такой путь не может содержать энергетических точек ребра $(bx]$, а значит концевыми точками для него могут быть только энергетические точки ребра $(ax]$ степени $1$, ввиду леммы~\ref{alm} принадлежащие $X_\Sigma$. Но путь, начинающийся с $x^a_1-s$ и в точках ветвления продолжающийся не тем отрезком, который является почти перпендикулярным $(ax]$, 
%(нетрудно заметить, что всегда найдется два направления, имеющих с ребром угол, не больший $\pi/6+\alpha/100$), 
не будет содержать энергетических точек ребра $(ax]$ степени $1$ (а также точек $\partial U$, точки $x$ и энергетических точек ребра $(bx]$ степени $1$), а значит никогда не закончится.


==> pictures/trash/4proofs.tex <==
\section {Доказательство основной Леммы и Теоремы~\ref{persp}} \label{prf}

\begin{proof}[Доказательство Леммы~\ref{main_l}]
Пусть $\rho_0>0$ достаточно мало. Точка $x\in E_\Sigma$ имеет одно или два энергетических ребра. Пункты доказательства c 1. по 8. содержат утверждения для одного ребра, поэтому относятся ко всем утверждениям Леммы сразу.  %СЕМЬ ИЛИ ВОСЕМЬ
После того, как первые восемь пунктов будут доказаны, мы будем предполагать, что у точки $x$, имеющей два энергетических ребра, порядок $\oord_x \Sigma = 1$. После того, как этот случай будет исключен, будут последовательно разобраны все случаи Леммы, не исключая также и случай энергетического ребра, направленного сразу в две стороны. 

Все дальнейшие рассуждения будут проводиться в множестве $\Sigma \cap B_{\rho_0}(x)$, а все утверждения будут доказаны для $\Sigma \cap B_{\rho}(x)$ для достаточно малого $\rho< \rho_0$, где ограничения сверху на $\rho$ будут появляться в процессе доказательства. 
%, где $\rho<\rho_0$, а $\rho_0>0$ --- достаточно малое число. 
Как было показано в Утверждении~\ref{edgeangle}, все энергетические точки множества $\Sigma \cap B_{\rho_0}(x)$ содержатся в объединении двух псевдоконусов $U^a(\rho_0)$ и $U^b(\rho_0)$ с биссектрисами $(ax]$ и $(bx]$ соответственно и раствором $\alpha(\rho_0)$ (в дальнейшем $\alpha$) (или внутри одного псевдоконуса $U^a(\rho_0)$, если $x$ имела ровно одно энергетическое ребро $(ax]$).
Поскольку $\rho_0$ достаточно мало, выполняется $U^a(\rho_0) \cap U^b(\rho_0) =x$.

Выберем также произвольные (бесконечные) последовательности энергетических точек $\{x^a_k\} \subset U^a(\rho_0) \cap G_\Sigma$ и $\{x^b_k\} \subset U^b(\rho_0) \cap G_\Sigma$ такие, что
$x^i_k \xrightarrow{}x$ и $(x^i_k x]\xrightarrow{}(ix]$, где буква $i$ означает $a$ или $b$ (или одну последовательность, если $x$ имело ровно одно энергетическое ребро $(ax]$). В процессе доказательства мы неоднократно, без перенумерации, будем переходить к подпоследовательностям $\left\{x^i_k \right \}$. При этом выбор последовательности и переход к подпоследовательностям устроены таким образом, что для достаточно малого $\rho_0$ все доказанные для $x^i_k$ точные (не содержащие значка $o$-малое или слова ``почти'') утверждения верны для произвольной энергетической точки из $B_{\rho}(x)\setminus x$. 



Пусть $\rho_0 \geq \rho(k) \xrightarrow{}0$ при $k \xrightarrow{}\infty$. Например, перейдя к подпоследовательности, можно выбрать монотонную функцию, в целых точках совпадающую с $\rho(k) \defeq |x^i_kx|$.
Слово ``почти''\ означает ``с точностью до величины $o_\rho(1)$'', то есть с точностью до величины, стремящейся к нулю при $\rho \xrightarrow{}0$ (а значит и при $k \xrightarrow{}\infty$).

\begin{enumerate}

\item Раствор дуги, покрываемой $x^i_k$, $\rho$-узок, то есть составляет $o_\rho(1)$. 
То есть все такие точки $y^i_k \in M$, что $|x^i_k y^i_k|=r$ и $B_r(y^i_k) \cap \Sigma = \emptyset$, удовлетворяют условию 
\[
\left|\frac{\pi}{2}-\angle ((ix), (y^i_kx^i_k))\right| = o_\rho (1)
\]
или, иначе говоря, для произвольного $c>0$ найдется такой номер $N$, что для каждого номера $k>N$ выполняется  
\[
\left|\frac{\pi}{2}-\angle ((ix), (y^i_kx^i_k))\right|<c.
\]
\label{angles}

\begin{proof}
Предположим противное. То есть можно выбрать подпоследовательность точек $\{ x^i_k\}$, соответствующих им точек $\{y^i_k\}$ и число $c>0$ такие, что 
\begin{equation}
\left|\frac{\pi}{2}-\angle ((ix),(y^i_kx^i_k))\right| > c.
\label{losloh}
\end{equation}
Но тогда для любой предельной точки $y^i$ множества $\{y^i_k\}$ верно, что $B_r(y^i) \cap \Sigma =\emptyset$, $|y^ix|=r$ и $|\frac{\pi}{2}-\angle ixy^i| \geq c$.
Но $\frac{\pi}{2}-\angle i x y^i \geq c$ противоречит определению ребра $(ix]$, поскольку в таком случае $B_\varepsilon(x^i_k) \cap U^i(\rho_0)\setminus B_r(y^i) =\emptyset$ для достаточно малого $\varepsilon>0$. А  $\angle i x y^i-\frac{\pi}{2} \geq c$, как несложно заметить, влечет
$\angle x^i_lxy^i \geq \frac{\pi}{2} + \frac{c}{2}$, для достаточно большого номера $l$.
А значит, не умаляя общности, $\angle x^i_lxy^i_l \geq \frac{\pi}{2} + \frac{c}{4}$ и $\angle x_l x_m y_l \geq \frac{\pi}{2} + \frac{c}{8}$ для достаточно большого номера $m>l$.
Но тогда $|x^i_my^i_l|<|x^i_ly^i_l|=r$, а значит $B_r(y^i_l)\cap \Sigma \neq \emptyset$. Полученное противоречие завершает доказательство пункта.

В частности, формула~\ref{losloh} и п.~\ref{perp_edge} Замечания~\ref{emptyball} влекут
\begin{corollary}
Энергетические ребра точек $x^i_k$ почти параллельны энергетическому ребру $(ix]$. 
\label{edges}
\end{corollary}

\end{proof}
\begin{remark}
В случае энергетического ребра, направленного сразу в две стороны, предлагается по отдельности провести рассуждение для двух подпоследовательностей точек $x^i_k$ таких, что внутри одной подпоследовательности точки $y^i_k$ расположены в одной полуплоскости относительно $(ix)$. Две подпоследовательности могут иметь общие точки.
\end{remark}

\item Зафиксируем произвольную точку $x^i_k$. Тогда существует такое $\varepsilon_k>0$, что для $0<\varepsilon <\varepsilon_k$ и такой точки $w \in \partial B_{\varepsilon}(x^i_k)$, что луч $[wx^i_k)$ почти параллелен $(ix]$ (то есть $\angle((ix)(wx^i_k))=o_\rho(1)$), верно, что существует такое связное множество $S \ni w$, что 
%\[
%M \cap B_r(\Sigma \cap B_\varepsilon(x^i_k)) \subset B_r(S)
%]
\[
F_M(\Sigma \setminus B_\varepsilon(x^i_k) \cup S) \leq F_M(\Sigma)
\]
и $\H(S)=o_\varepsilon(1)+\varepsilon o_\rho(1)$. 
В частности, это верно для $w=x^i_k$.
\label{Losiu}

\begin{proof}
Пусть $\{ \varepsilon_l \}$ --- сходящаяся к нулю последовательность, такая что для произвольных номеров $l$ и $m$ выполняется $B_{\varepsilon_l}(x^i_l)\cap B_{\varepsilon_m}(x^i_m)=\emptyset$ (очевидно, такие $\varepsilon$ можно выбрать для любой сходящейся нестабилизирующейся последовательности $\{ x^i_k \}$). Кроме того, уменьшим, при необходимости числа $\varepsilon_k$ так, чтобы выполнялось
\begin{equation}
\frac{\varepsilon_k}{|x^i_kx|} \xrightarrow[k \xrightarrow{} \infty]{} 0.
\label{y}
\end{equation}
Для произвольного номера $l$ определим множество 
$$U^i_l \defeq \{y\in M | \dist(y, \overline{B_{\varepsilon_l}(x^i_l)})\leq r, \dist(y, \Sigma \setminus \overline{B_{\varepsilon_l}(x^i_l)})> r \}.$$
Заметим, что тогда 
\begin{equation}
F_{M \setminus U^i_l}(\Sigma \setminus B_{\varepsilon_l}(x^i_l)) \leq r. 
\label{0}
\end{equation}

Пусть $\{u_l\}$ --- произвольная последовательность точек $u_l \in U^i_l$, а $\{v_l\}$ --- такая последовательность точек, что $v_l \in B_{\varepsilon_l}(x^i_l)$ и $|u_lv_l| \leq r$. Тогда покажем, что 
\begin{equation}
\left |\angle((u_lv_l),(ix))-\frac{\pi}{2} \right|=o_\rho(1).
\label{1}
\end{equation}

Предположим, что формула~(\ref{1}) неверна, тогда найдется такое $c>0$, что $|\angle((u_lv_l),(ix))-\frac{\pi}{2}|>2c$. 

Пусть существует такая подпоследовательность, что $\angle((u_lv_l],(ix])-\frac{\pi}{2}>2c$. Несложно заметить, ввиду условия~\ref{y}, что $|\angle((ix),(v_lx))|=o_\rho(1)$, а значит, не умаляя общности, и ввиду определения ребра, можно считать что существует такая подпоследовательность, что $\angle u_l v_l x < \frac{\pi}{2} - c$ для каждого $l$. Поскольку последовательность $v_m$ сходится к точке $x$, можно выбрать такое достаточно большое $l$, что $\angle v_l u_l x < \frac{c}{4}$. Для этого $l$ можно выбрать такое, достаточно большое $m>l$, что $\angle v_l u_l v_m < \frac{c}{2}$ и $\angle u_l v_l v_m < \frac{\pi}{2} - \frac{c}{2}$. Тогда $|v_mu_l|<|v_lu_l|\leq r$, что невозможно ввиду определения множества $U^i_l$.

Значит, для достаточно большого $l$ выполняется неравенство 
$$\angle((u_lv_l],(ix]) < \frac{\pi}{2}-2c.$$ 
Тогда $\dist(u_l,(ix))\leq \sin (\frac{\pi}{2} - c)r$ для достаточно большого номера $l$. Но тогда $B_r(u_l)\cap (ix]$ является подмножеством хорды $\partial B_r(u_l)$. Тогда для достаточно большого номера $m>l$ верно $B_{\varepsilon_m}(v_m) \subset B_r(u_l)$. Что противоречит определению множества $U^i_l$. Таким образом, формула~(\ref{1}) доказана.


Отныне будем считать, не умаляя общности, что все множества $U^i_l$ лежат в одной полуплоскости относительно прямой $(ix)$. Это верно, за исключением конечного числа множеств, во всех случаях кроме ребра $(ix]$, направленного в две стороны. Но в таком случае все рассуждения можно провести для двух наборов множеств, каждый из которых лежит по одну сторону $(ix)$.

Покажем теперь, что для произвольного набора точек $w_l \in B_{\varepsilon_l}(x^i_l)$, в том числе для $w_l=x^i_l$, выполняется
\begin{equation}
\left |\angle ((u_l,w_l),(ix]) - \frac{\pi}{2} \right |=o_{\rho}(1).
\label{2}
\end{equation}
Посмотрим на треугольник $\triangle u_l v_l w_l$: сторона $|v_lu_l|\geq r-|u_l u_{l+1}|=r-o_{\rho}(1)$ ввиду фундаментальности $\{u_l\}$, сторона $|v_l w_l|\leq 2\varepsilon_l$, таким образом по теореме синусов $\sin \angle v_lu_lw_l = o_{\rho}(1)$. Тогда и $\angle v_lu_lw_l=o_{\rho}(1)$, а значит $\angle ((u_l,w_l),(ix]) = \angle((u_lv_l),(ix])+o_\rho(1)$, что влечет $|\angle ((u_l,w_l),(ix]) - \frac{\pi}{2}|=o_{\rho}(1)$. Таким образом, формула~(\ref{2}) доказана.

Покажем теперь, что 
\begin{equation}
\angle((v_lx^i_l),(ix])=o_\rho(1)
\label{3}
\end{equation}
(в частности, при $v_l = x^i_l$ данный угол будем считать нулевым).
Посмотрим на $\triangle u_lv_l x^i_l$. 
Пусть $y^i_k$ --- произвольная точка, удовлетворяющая условиям, перечисленным в  пункте~\ref{angles} (то есть $y^i_k \in M$, $|x^i_l y^i_l|=r$ и $B_r(y^i_k) \cap \Sigma = \emptyset$). Тогда, ввиду пункта~\ref{angles} ясно, что для произвольной точки $v^l \in \Sigma \cap B_{\varepsilon_l}(x^i_l) \setminus \{ x^i_l\}$ либо $\angle v^l x^i_l y^i_l=o_\rho(1)$, либо  $\angle v^l x^i_l y^i_l>\frac{\pi}{2}$. Пусть предположение неверно, то есть найдется такое $c>0$, что $\angle((v_lx^i_l),(ix])>c$ для каждого $l$. Тогда, для $v_l \neq x^i_l$ верно  $\angle v_l x^i_l y^i_l>\frac{\pi}{2}$, а значит $\angle v_l x^i_l y^i_l \geq \frac{\pi}{2} +c$. Тогда для достаточно малого $\rho_0$ можно считать $\angle v_l x^i_l u_l \geq \frac{\pi}{2} + \frac{c}{2}$. Тогда $|x^i_lu_l|\leq \cos(\frac{\pi}{2} + \frac{c}{2})|v_lu_l|\leq r(1 - \frac{c^2}{3})$. Тогда для предельной точки $\hat u=\lim\limits_{l \xrightarrow{} \infty} u_l$ верно, что $|x \hat u|\leq r(1 - \frac{c^2}{3})$, что не может быть правдой, поскольку по определению $U^i_l$ верно
$||x^i_lu_l|-r|\leq \varepsilon_l+\varepsilon_{l+1} +|x^i_lx^i_{l+1}|$, а значит $|x \hat u|=r$. Полученное противоречие завершает доказательство формулы~(\ref{3}).


Пусть теперь $w$ из условия доказываемого пункта, а $u$ --- самая дальняя от неё точка множества $U^i_k$. 
Пусть $v \in B_{\varepsilon_k}(x^i_k)$ такая, что $|vu| \leq r$. Покажем, что $|wu|=r+\varepsilon o_\rho(1)+o_\varepsilon(1)$. Для этого нам придется сначала показать, что $|x^i_ku|=r+\varepsilon o_\rho(1)+o_\varepsilon(1)$.

Ввиду формул~(\ref{1}) и (\ref{3}) несложно заметить, что
\begin{equation*}
\left |\angle uvx^i_k - \frac{\pi}{2} \right |=o_\rho(1).
%\label{4}
\end{equation*}
При этом $|x^i_kv|\leq \varepsilon$ и $|vu|\leq r$.
Тогда по теореме косинусов для $\triangle x^i_kvu$
\begin{equation}
|x^i_ku|=\sqrt{|x^i_kv|^2+|uv|^2-2|x^i_ku||uv|\cos \angle uvx^i_k}=  \sqrt{\varepsilon^2 + r^2 + \varepsilon o_\rho(1)}=r+\varepsilon o_\rho(1)+o_\varepsilon(1).
\label{5}
\end{equation}


Ввиду формулы~(\ref{2}) для $l=k$, $w_l=x^i_k$ и условия $\angle((ix)(wx^i_k))=o_\rho(1)$ несложно заметить, что
\begin{equation*}
\left |\angle wx^i_ku - \frac{\pi}{2} \right |=o_\rho(1).
%\label{6}
\end{equation*}
При этом $|x^i_kw|\leq \varepsilon$ и, ввиду~(\ref{5}), $|x^i_ku|\leq r+\varepsilon o_\rho(1)+o_\varepsilon(1)$.
Тогда по теореме косинусов для треугольника $\triangle x^i_kwu$  
\begin{multline*}
|wu|=\sqrt{|x^i_kw|^2+|x^i_ku|^2-2|x^i_kw||x^i_ku|\cos \angle  wx^i_ku}= \\
= \sqrt{\varepsilon^2+(r+\varepsilon o_\rho(1)+o_\varepsilon(1))^2+\varepsilon o_\rho(1)(r+\varepsilon o_\rho(1)+o_\varepsilon(1))}=r+\varepsilon o_\rho(1)+o_\varepsilon(1).
\end{multline*}

А значит $U^i_k \subset \overline{B_{r+\varepsilon o_\rho(1)+o_\varepsilon(1)}(w)}$. С другой стороны, ввиду формулы~(\ref{2}) можно говорить, что множество $U^i_k$ содержится в углу с вершиной $w$ и с раствором $o_\rho(1)$. Не умаляя общности, положим луч $[wu)$ биссектрисой данного угла и назовем этот угол $\Lambda^i_k$.
Тогда 
\[
U^i_k \subset B_{|wu|}(w) \cap \Lambda^i_k.
\]
Обозначим за $G$ один из двух концов дуги $\partial B_{|wu|}(w) \cap \Lambda^i_k$. Пусть $T \in [wu]$ --- такая точка, что $|TG|=r$. Несложно заметить, что 
\[
\overline{B_r([wT])} \supset \overline{B_{|wu|}(w) \cap \Lambda^i_k} \supset U^i_k. 
\]
Таким образом, ввиду формулы~(\ref{0}), осталось показать, что длина множества $|wT|=\varepsilon o_\rho(1)+o_\varepsilon(1)$ и тогда искомое множество $S \defeq [wT]$ будет найдено.

Пусть $\phi \defeq \angle Gwu$ (то есть $\phi=o_\rho(1)$), $\psi \defeq \angle GTu$ и $h\defeq|wu|-r$ (то есть $h=\varepsilon o_\rho(1)+o_\varepsilon(1)$). Тогда
\[
\begin{array}{ccc}
    \sin \psi &=& (1+\frac{h}{r}) \sin \phi;  \\
    \sin \psi -\sin \phi &=& \varepsilon o_\rho(1)+o_\varepsilon(1);\\
    \psi - \phi &=& \varepsilon o_\rho(1)+o_\varepsilon(1);\\
    \cos \phi -\cos \psi = -2\sin \left (\frac{\phi + \psi}{2} \right)\sin \left (\frac{\phi - \psi}{2} \right) &=& \varepsilon o_\rho(1)+o_\varepsilon(1).\\
\end{array}
\]
Тогда 
\[
    |wT| = |wu| - |Tu| = r\left(\left(1 + \frac{h}{r}\right)\cos \phi - \cos \psi\right ) =\varepsilon o_\rho(1)+o_\varepsilon(1).
\]

Таким образом, множество $S \defeq [wT]$ удовлетворяет всем заявленным условиям.
\end{proof}

\item Для произвольной точки $x^i_k$ ее круговой порядок $\oordball_{x^i_k}\Sigma$ не превосходит двух.
Из этого, благодаря Замечанию~\ref{rem_ord}, следует $\oord_{x^i_k}\Sigma \leq 2$.
\label{ordball}

\begin{proof}
Пусть $n \defeq \oordball_{x^i_k}\Sigma$ и пусть $\varepsilon>0$ достаточно малое число такое, что 
\[
\sharp (\partial B_{\varepsilon}(x^i_k) \cap \Sigma) = n. 
\]
%сослаться  на формулу коплощади
Тогда, согласно формуле коплощади $\H(B_\varepsilon(x^i_k)\cap \Sigma) \geq n \varepsilon$. Предположим, что $n > 2$. Поскольку все эти $n$ точек располагаются на дуге окружности $\partial B_{\varepsilon_l}(x^i_k)$ размера $\pi+o(\varepsilon)$, нетрудно заметить, что штейнеровское дерево $St$, соединяющие все эти $n$ точек и точку $x^i_k$, имеет такую длину, что $n \varepsilon - \H(St)=c_n\varepsilon \geq c_3$, где $c_3$ --- положительная константа, которую можно посчитать. 
Применив пункт~\ref{Losiu} для $w=x^i_k$, получим множество $S$, такое что для достаточно малых $\rho_0$ и $\varepsilon$  величина $\H(S)$ строго меньше $n \varepsilon - \H(St)$. Таким образом, замена $\Sigma$ на $\Sigma \setminus B_\varepsilon(x^i_k) \cup St \cup S$ уменьшает длину, не увеличивает энергию и сохраняет связность. Противоречие. 
\end{proof}

\item В случае, если  $\oord_{x^i_k} \Sigma =1$, точка $x^i_k$ принадлежит множеству $X_\Sigma$.
\label{discr}

\begin{proof}
Предположим противное: пусть точка $x^i_k$ принадлежит множеству $E_\Sigma$. Тогда существует последовательность энергетических точек $\{x'_l\}$, сходящихся к $x^i_k$. Энергетическое ребро или ребра, к которым они сходятся, должны лежать на прямой, почти параллельной $(ix]$ ввиду Замечания~\ref{edges}.  

Ввиду пункта~\ref{ordball} достаточно разобрать только следующие случаи:
\begin{itemize}
\item[(a)] Случай $\oordball_{x^i_k}\Sigma=1$.
Пусть $\varepsilon_0(k)>0$ достаточно мало, а $\varepsilon_l>0$ последовательность стремящихся к нулю чисел, меньших $\varepsilon_0(k)$ таких, что $\sharp (\partial B_{\varepsilon_l}(x^i_k) \cap \Sigma )=1$. Обозначим $s^l\defeq \partial B_{\varepsilon_l}(x^i_k) \cap \Sigma$. Тогда $(s^lx^i_k)$ почти перпендикулярно $(ix)$. Предположим, что это не так, то есть существуют константа $c>0$ и последовальность $K \subset \mathbb{N}$ такие, что для любого $k \in K$ существует сколь угодно большой номер $l$, такой что выполняется неравенство $|\angle ((s^lx^i_k), (ix))-\frac{\pi}{2}| > c$.
 
Пусть тогда $w$ --- основание перпендикуляра, опущенного из $s^l$ на прямую, параллельную $(ix)$ и проходящую через $x^i_k$: $(wx^i_k)\ ||\ (ix)$ и $(ws^l) \perp (ix)$. Тогда определим множество $S \ni w$  как в пункте~\ref{Losiu}. При этом длина этого множества $\H(S)=o_{\varepsilon_l}(1)+o_\rho(1)\varepsilon_l$, поскольку $|wx^i_k|= \cos \angle ([s^lx^i_k],(ix]) \cdot |s^lx^i_k|< \varepsilon_l$. В то же время $|ws^l|=\sin \angle([s^lx^i_k],(ix]) \cdot |s^lx^i_k| < (1 - \frac{c^2}{2}) \varepsilon_l$ и $\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq \varepsilon_l$. Таким образом, 
\[
\H(\Sigma \setminus  B_{\varepsilon_l}(x^i_k) \cup [s^lw] \cup S)\leq \H(\Sigma)-\varepsilon_l+\left(1-\frac{c^2}{2}\right)\varepsilon_l+o_{\varepsilon_l}(1)+o_\rho(1)\varepsilon_l<\H(\Sigma).
\]

То есть связное множество $\Sigma \setminus [s^lx^i_k] \cup [s^lw] \cup S$ будет иметь длину  меньше, а энергию не больше, чем $\Sigma$. Получили противоречие с оптимальностью $\Sigma$, то есть предположение о неперпендикулярности было неверным. То есть $(s^lx^i_k)$ почти перпендикулярно $(ix)$:
\begin{equation}
\left|\angle ((s^lx^i_k), (ix))-\frac{\pi}{2}\right| =o_\rho(1).
\label{99}
\end{equation}
Заметим теперь, что для каждого $\varepsilon_l$ верно
\begin{equation}
\H(B_{\varepsilon_l}(x^i_k)\cap \Sigma)=\varepsilon_l+o_{\varepsilon_l}(1)+o_\rho(1)\varepsilon.
\label{100}
\end{equation}

Формула~\eqref{100} верна ввиду пункта~\ref{Losiu}: в противном случае можно было бы заменить $\Sigma$ на связное множество $\Sigma \setminus B_{\varepsilon_l}(x^i_k) \cup [x^i_ks^l]\cup S$, где $S$ определено в пункте~\ref{Losiu} при $w=x^i_k$, и получить противоречие с оптимальностью $\Sigma$. 

Можно считать, что 
\begin{equation}
\H(B_{\varepsilon_l}(x^i_k)\cap \Sigma)<\varepsilon_l \left(1+\frac{1}{18}\right).
\label{101}
\end{equation}
Теперь заметим, что можно считать, что 
\begin{equation}
\frac{\varepsilon_l}{\varepsilon_{l+1}}\leq \frac{18}{17}.
\label{103}
\end{equation}
Пусть не так, тогда найдется $\varepsilon_l$ такой, что $\sharp ( \partial B_{\varepsilon_l}(x^i_k)\cap \Sigma)\geq 2$ для каждого $\varepsilon \in [\frac{17\varepsilon_l}{18},\varepsilon_l[$. Но тогда, ввиду неравенства коплощади
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k))\geq \H(\Sigma \cap B_{\frac{17\varepsilon_l}{18}}(x^i_k)) +\H(\Sigma \cap (B_{\varepsilon_l}(x^i_k) \setminus  B_{\frac{17\varepsilon_l}{18}}(x^i_k))\geq \varepsilon_l \left (1+\frac{1}{18} \right),
\]
что противоречит~\eqref{101}.
Ввиду наличия у $x^i_k$ ребра, существования последовательности $\{ s_l \}$ и единичного порядка $\oord{x^i_k}(\Sigma)=1$ существует также сходящаяся к $x^i_k$ последовательность точек $\{ u_l\}\subset \Sigma$ таких, что $\angle((u_lx^i_k),(ix)) = \frac{\pi}{4}$.

Рассмотрим произвольную такую точку $u_m$. Выберем такой номер $l$, что 
\begin{equation}
0<\varepsilon_l-|x^i_ku_m|\leq \frac{1}{18}\varepsilon_l.
\label{104}
\end{equation}
Такое $\varepsilon_l$ существует ввиду формулы~\eqref{103}. Заметим также, что ввиду~\eqref{99} выполняется
\[
\sharp (\partial B_{|x^i_k u_m|}(x^i_k)\cap \Sigma) \geq 2.
\] 
Кроме того, 
\begin{equation}
d \defeq \dist(u_m, Q_a\cup Q_b \cup Q)\geq \frac{\sqrt{2}}{2}|x^i_ku_m|-o_\rho(1)\varepsilon> \frac{1}{\sqrt{3}}|x^i_ku_m|,
%\label{105}
\end{equation}
где $Q$ --- область возможного расположения точек $s_l$ (угол с вершиной в $x^i_k$, раствором $o_\rho(1)$ и перпендикуляром к $(ix)$ в качестве биссектрисы).
Пусть $q$ ---  компонента связности $\Sigma \cap Q$, содержащая $u_m$. Пусть теперь $c$ --- длина проекции $q$ на ближайшую к $u_m$ сторону угла $Q$ (то есть на луч с вершиной в $x^i_k$, имеющий угол $\frac{\pi}{2}-o_\rho(1)$ с прямой $(ix)$). Тогда
%а $var(c)$ величина проекции на эту координату. Тогда
\[
\H(q)\geq \frac{c+d}{2}.
\]
Тогда 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq \varepsilon_l-c+\frac{c+d}{2}.
\]
С другой стороны, по неравенству коплощади 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq \varepsilon_l+c.
\]
А значит верно и неравенство с полусуммой:
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq \varepsilon_l+\frac{c+d}{4}>\varepsilon_l+\frac{d}{4}>\varepsilon_l+ \frac{|x^i_ku_m|}{4\sqrt{3}}.
\]

Тогда, ввиду~\eqref{104}, 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k))>\varepsilon_l \left(1+\frac{17}{72\sqrt{3}}\right).
\]
Полученное противоречие с~\eqref{101} завершает доказательство случая.
\item [(б)] Случай $\oordball_{x^i_k}\Sigma=2$.
Пусть $\varepsilon_0(k)>0$ достаточно мало, а $\varepsilon_l>0$ последовательность чисел, меньших $\varepsilon_0(k)$ таких, что $\sharp (\partial B_{\varepsilon_l}(x^i_k) \cap \Sigma )=2$. Обозначим  $s^l, t^l \defeq \partial B_{\varepsilon_l}(x^i_k) \cap \Sigma$. Ясно, что угол $\angle s^lx^i_kt^l > \frac{2\pi}{3} - o_\rho(1)$ (в противном случае замена $\Sigma \setminus B_\varepsilon(x^i_k) \cup St(s^l,t^l,x^i_k)$, где $S \ni x^i_k$ --- множество, определенное в пункте~\ref{Losiu} для точки $w=x^i_k$, а $St(s^l,t^l,x^i_k)$ --- дерево Штейнера, соединяющее точки $s^l$,$t^l$ и $x^i_k$, имело бы не большую энергию и строго меньшую длину, чем множество $\Sigma$). 

То есть
\begin{equation}
\angle ((s^lx^i_k), (t^lx^i_k))\geq \frac{2\pi}{3}.
\label{990}
\end{equation}
Заметим теперь, что для каждого $\varepsilon_l$ верно
\begin{equation}
\H(B_{\varepsilon_l}(x^i_k)\cap \Sigma)=2\varepsilon_l+o_{\varepsilon_l}(1)+o_\rho(1)\varepsilon.
\label{1000}
\end{equation}
Формула~\eqref{1000} верна ввиду пункта~\ref{Losiu}: в противном случае, можно было бы заменить $\Sigma$ на связное множество $\Sigma \setminus B_{\varepsilon_l}(x^i_k) \cup [x^i_ks^l]\cup S$, где $S$ определено в пункте~\ref{Losiu} при $w=x^i_k$, и получить противоречие с оптимальностью $\Sigma$. 
Можно считать, что 
\begin{equation}
\H(B_{\varepsilon_l}(x^i_k)\cap \Sigma)<2\varepsilon_l \left (1+\frac{1}{36}\right).
\label{1010}
\end{equation}


Теперь заметим, что можно считать, что 
\begin{equation}
\frac{\varepsilon_l}{\varepsilon_{l+1}}\leq \frac{18}{17}.
\label{1030}
\end{equation}
Пусть не так, тогда найдется $\varepsilon_l$ такое, что $\sharp \left( \partial B_{\varepsilon_l}(x^i_k)\cap \Sigma
\right) \geq 3$ для каждого $\varepsilon \in [\frac{17\varepsilon_l}{18},\varepsilon_l[$. Но тогда, ввиду неравенства коплощади
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k))\geq \H(\Sigma \cap B_{\frac{17\varepsilon_l}{18}}(x^i_k)) +\H(\Sigma \cap (B_{\varepsilon_l}(x^i_k) \setminus  B_{\frac{17\varepsilon_l}{18}}(x^i_k))\geq 2\varepsilon_l\left(1+\frac{1}{36}\right),
\]
что противоречит (\ref{1010}).
Ввиду наличия последовательностей $\left\{s^l\right\}$, $\left \{t^l\right \}$ и единичного порядка $\oord_{x^i_k}(\Sigma)=1$ существует также сходящаяся к $x^i_k$ последовательность точек $\{ u_l\}$ таких, что $\angle((u_lx^i_k),(ix))=\frac{\pi}{2}$.

Рассмотрим произвольную такую точку $u_m$. Выберем такой номер $l$, что 
\begin{equation}
0<\varepsilon_l-|x^i_ku_m|\leq \frac{1}{18}\varepsilon_l.
\label{1040}
\end{equation}
Такое $\varepsilon_l$ существует ввиду формулы~\eqref{1030}. Заметим также, что ввиду~\eqref{990} выполняется
\[
\sharp (\partial B_{|x^i_k u_m|}(x^i_k)\cap \Sigma) \geq 3.
\] 
Кроме того, 
\begin{equation}
d \defeq \dist(u_m, Q)\geq \frac{1}{2}|x^i_ku_m|-o_\rho(1)\varepsilon> \frac{1}{3}|x^i_ku_m|,
\label{1050}
\end{equation}
где $Q$ --- область возможного расположения точек $s^l, t^l$ (множество $Q$ не пересекается с углом с вершиной в $x^i_k$, раствором $\frac{\pi}{3} - o_\rho(1)$ и перпендикуляром к $(ix)$ в качестве биссектрисы).
Пусть $q$ --- компонента связности $\Sigma \setminus Q$, содержащая $u_m$. Пусть теперь $c$ --- длина проекции $q$ на ту сторону $Q$, чье пересечение с $q$ не пусто, тогда
%а $var(c)$ величина проекции на эту координату. Тогда
\[
\H(q)\geq \frac{c+d}{2}.
\]
Тогда 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq 2\varepsilon_l-2c+\frac{c+d}{2}.
\]
С другой стороны, по неравенству коплощади 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq 2\varepsilon_l+c.
\]
А значит верно и такое неравенство:
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq
\frac{2}{5}\left(2\varepsilon_l-2c+\frac{c+d}{2}\right)+\frac{3}{5}\left(2\varepsilon_l+c \right)\geq 2\varepsilon_l+\frac{d}{5}.
\]
Тогда, ввиду~\eqref{1050},
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq 2\varepsilon_l+\frac{|x^i_ku_m|}{15}.
\]
Но тогда, ввиду~\eqref{1040}, 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k))>2\varepsilon_l \left( 1+\frac{17}{540} \right).
\]
Полученное противоречие с~\eqref{1010} завершает доказательство пункта.
\end{itemize}

\end{proof}
\item В случае, если  $\oord_{x^i_k} \Sigma = 1$, отрезок, входящий в  $x^i_k$, будет почти перпендекулярно ребру $(ix]$.
\label{perp_edge2}

\begin{proof}
Сперва поясним корректность формулировки. Ввиду пункта~\ref{discr} точка $x^i_k \in X_\Sigma$.  Ввиду Утверждения~\ref{discr_str} можно выбрать такое $\varepsilon > 0$, что $\Sigma \cap B_{\varepsilon}(x^i_k)$ совпадает с отрезком $[sx^i_k]$, где $s \in \partial B_{\varepsilon}(x^i_k)$. Утверждается, что тогда ребро $[sx^i_k] \subset \Sigma$ будет почти перпендекулярно ребру $(ix]$, то есть $|\frac{\pi}{2} - \angle ([sx^i_k],(ix])|=o_\rho(1)$.

Мы видим, что $\oordball_{x^i_k} \Sigma = 1$, а значит нам нужно лишь повторить доказательство случая (а) из пункта~\ref{discr} (в качестве $s^l$ можно брать произвольную точку $\Sigma \cap B_\varepsilon(x^i)$).
\end{proof}


\item  Пусть $\oord_{x^i_k} \Sigma =2$ и $x^i_k \in X_\Sigma$, тогда, согласно Утверждению~\ref{discr_str}, существует такое $\varepsilon$, что $\Sigma \cap \overline{B_{\varepsilon}(x^i_k)}=[sx^i_k] \sqcup [tx^i_k]$, причем угол 
$\angle sx^i_kt \geq \frac{2\pi}{3}$. Утверждается, что тогда
\[
\angle((sx^i_k], (ix))=\angle( (ix),(tx^i_k] )+ o_\rho(1).
\]

\label{ugli}

\begin{corollary}

В частности, тогда

\[
\angle((sx^i_k], (ix))=\angle( (ix),(tx^i_k] )+ o_\rho(1)\leq \frac{\pi}{6}.
\] 

\end{corollary}

\begin{proof}
Предположим противное: не умаляя общности, найдется число $c_1>0$, такое что 
\[
\eta \defeq \angle((sx^i_k], (ix))-\angle( (ix),(tx^i_k]) \geq c_1.
\]
Пусть $l$ --- прямая, проходящая через точку $x^i_k$ и параллельная $(ix)$. Отразим отрезок $[tx^i_k]$ относительно $l$. Пусть $t'$ --- образ точки $t$ при этом отображении. Тогда $|t'x^i_k|=\varepsilon$ и
\[
|sx^i_k|+|tx^i_k|=|sx^i_k|+|t'x^i_k|=2\varepsilon.
\]
В то же время по теореме косинусов для $\Delta sx^i_kt'$
\[
|st'|^2 = |sx^i_k|^2+|x^i_kt'|^2-2|sx^i_k||x^i_kt'|\cos \angle sx^i_kt'=2\varepsilon^2(1-\cos \eta),
\]
поскольку $\angle sx^i_kt'=\pi+\angle((tx^i_k], (ix))-\angle( (ix),(sx^i_k])=\pi-\eta$.
Таким образом,
\[
|sx^i_k|+|t'x^i_k|-|st'| > c_2\varepsilon,
\]
где $c_2 > 0$ константа, зависящая только от $\eta$.

Пусть теперь точка $d \defeq [st']\cap l$. Тогда $\angle((sd], (ix))=\angle( (ix),(td])$ и 
%\begin{equation*}
\[(|sx^i_k|+|tx^i_k|)-(|sd|+|dt|)= 2\varepsilon - |st'|>c_2\varepsilon.\]
%\end{equation*}

Пусть $S \ni d$ --- множество, определенное в пункте~\ref{Losiu}. Тогда $\H(S)=o_\varepsilon(1)+o_\rho(1)\varepsilon$.
А значит связное множество $\Sigma \setminus ([sx^i_k]\cup[tx^i_k]) \cup S \cup [sd] \cup [td]$ при достаточно малых $\rho$ и $\varepsilon$ будет лучше $\Sigma$, поскольку имеет не большую энергию и длину, не превосходящую $\H(\Sigma)-c_2\varepsilon+ o_\rho(1)\varepsilon+o(\varepsilon)$. Полученное противоречие с оптимальностью $\Sigma$ завершает доказательство пункта.
\end{proof}

%небольшие проблемы с аккуратностью про конусы
%и надо поменять формулировку: что совпадает с дугами (и про концы дуг сказать)
\item Пусть  $\oord_{x^i_k} \Sigma =2$ и $x^i_k \in E_\Sigma$, тогда
%, согласно Лемме~\ref{ord_arcs}, 
существует такое $\varepsilon$, что $\Sigma \cap \overline{B_{\varepsilon}(x^i_k)}$ содержит две дуги $\breve{[sx^i_k]}$ и $\breve{[tx^i_k]}$, пересекающиеся только по точке $x^i_k$. Докажем, что эти дуги содержатся в узких  псевдоконусах с биссектрисами, $o_\rho(1)$-почти образующими развернутый угол и $o_\rho(1)$-почти параллельными $(ix]$ и с раствором $\gamma(\rho) = o_\rho(1)$.


\label{arc_par}
\begin{proof}
Напомним, что $x^i_k$ имеет одно или два энергетических ребра, причем они почти параллельны $(ix)$. Пусть $Q = Q_1 \cup Q_2$ --- объединение двух узких  псевдоконусов  с биссектрисами почти параллельными $(ix]$ и
$G_\Sigma \cap B_{\varepsilon}(x^i_k) \subset Q$. Оно существует ввиду Утверждения~\ref{edgeangle}. Не умаляя общности, ввиду пункта~\ref{ordball} будем считать $\varepsilon>0$ таким, что $\sharp(\Sigma \cap \partial B_\varepsilon(x^i_k)) \leq 2$.
 
Если хотя бы одно из двух ребер $x^i_k$ направлено в две стороны, пункт тривиален ввиду Утверждения~\ref{star}. Таким образом, можно считать, что каждое ребро направлено в одну сторону. Угол между ребрами, не содержащий точек $y^i_k$, соответствующих энергетическим точкам из $Q$, будем называть внутренним. Величина его не превосходит $\pi$.
 
Пусть $(qx^i_k]$ --- луч, не совпадающий ни с одним ребром $x^i_k$. Покажем, что тогда либо число пересечений $\sharp \left(\Sigma \cap B_{\varepsilon}(x^i_k) \cap (qx^i_k] \right)$ конечно, либо $\Sigma$ содержит отрезок этого луча ненулевой длины c концом в $x^i_k$. Во втором случае, не умаляя общности, будем рассматривать $\varepsilon$, не превосходящий длину этого отрезка. 

Пусть не реализовался ни один из двух случаев и множество $\Sigma \cap B_{\varepsilon}(x^i_k) \cap (qx^i_k]$ содержит бесконечное число точек. Заметим, что любая точка из множества $\Sigma \cap B_{\varepsilon}(x^i_k) \cap (qx^i_k]$ не энергетическая и, значит, является центром отрезка или правильной треноги, а множество $\Sigma \cap B_{\varepsilon}(x^i_k) \setminus Q$ является штейнеровским лесом. 

Пусть $L$ обозначает ту часть внутреннего угла, которая ограничена $(qx^i_k]$ и перпендикуляром к $(ix)$, проходящим через $x^i_k$ (если луч $(qx^i_k]$ не перпендикулярен $(ix)$). Тогда $S := L\setminus Q \cap \overline{B_\varepsilon (x^i_k)}\cap \Sigma$ является штейнеровским лесом, причем все точки $\partial S$ (число которых бесконечно), за исключением конечного числа принадлежащих $(\partial B_\varepsilon (x^i_k) \cap L \setminus Q)\cap \Sigma$, лежат на $(qx^i_k]$ или на перпендикуляре. Тогда ввиду Леммы~\ref{St_l} число концевых точек леса $\partial S$, принадлежащих перпендикуляру, бесконечно, а значит найдется сходящаяся к $x^i_k$ бесконечная последовательность точек $\{u_l\}$ таких, что $\angle((u_l,x^i_k)(ix))=\pi/2$ для каждого номера $l$. Однако существование такой последовательности приводит к противоречию, как было показано в случае (б) пункта ~\ref{discr}.


%Поскольку луч $(qx^i_k]$ произвольный, из этого сразу будет следовать конечность 
Покажем, что число пересечений $\Sigma$ и внутренней (то есть лежащей во внутреннем углу) границы произвольного псевдоконуса $q_{inn}$ конечно. 

Предположим противное, то есть что множество $\left(\Sigma \cap B_{\varepsilon}(x^i_k) \cap q_{inn} \right)$ бесконечно. Пусть при этом $\varepsilon>0$ такое, что $\sharp(\partial B_\varepsilon(x^i_k) \cap \Sigma) =2$. Выберем луч $(qx^i_k]$ так, чтобы в шаре $B_\varepsilon(x^i_k)$  он не пересекался с $Q$ %и чтобы $\Lambda$ (фигура, ограниченная  $q_{inn}$, $(qx^i_k]$ и $\partial B_\varepsilon(x^i_k)$), была такова, что $\sharp (\overline{\Lambda} \cap \Sigma \cap \partial B_\varepsilon(x^i_k)) \leq 2$.
и не содержал точек $\Sigma$ (возможно, $\varepsilon$ пришлось заменить на меньший радиус, сохраняя условие $\sharp(\partial B_\varepsilon(x^i_k) \cap \Sigma) =2$).  

Заметим, что $\Lambda \setminus q_{inn}$ не содержит энергетических, а значит и концевых точек $\Sigma$. Пусть теперь $W$ --- гладкая кривая между $q_{inn}$ и $(qx^i_k]$, то есть такая кривая, пересечением которой и произвольной окружности с центром в $x^i_k$ и радиусом $\varepsilon'<\varepsilon$, является точка, принадлежащая внутренности дуги с концами в точках $q_{inn}$ и $(qx^i_k]$. Потребуем кроме того, чтобы ребро $x^i_k$ было односторонней касательной к $W$. Если $\sharp (\Sigma \cap W)$ конечно, переопределим псевдоконус, заменив $q_{inn}$ на $W$. Предположим, что это множество бесконечно. Пусть $\Lambda$ --- фигура, ограниченная  $W$, $(qx^i_k]$ и $\partial B_\varepsilon(x^i_k)$. По нашему предположению $\partial \Lambda \cap \Sigma$ не содержит точек на  $(qx^i_k]$, содержит не более двух точек на $\partial B_\varepsilon(x^i_k)$ и бесконечно много точек на $W$. Заметим, что изменение наклона касательной к $W$ внутри $B_\varepsilon(x)$ зависит от $\varepsilon$ и сколь угодно мало. Обозначим его за $\xi_1$. Пусть $ \varepsilon_1<\varepsilon$ достаточно мало. За $\xi_2$ обозначим максимальный угол, под которым дуга $\Lambda \cap \partial  B_\varepsilon(x^i_k)$ видна из $\Lambda \cap B_{ \varepsilon_1}$
%$\angle ix^i_kq$, соответствующий изменению касательной к $\partial B_\varepsilon(x^i_k) \cap \overline \Lambda$.
 Покажем, что в области $\Lambda \cap B_{ \varepsilon_1}(x^i_k)$ нет точек ветвления $\Sigma$. Предположим противное: пусть точка ветвления существует. Продолжим исходящие из неё ребра лучами и заметим, что один из лучей пересек $\partial \Lambda \cap (qx^i_k]$, поскольку $\xi_1+\xi_2+\pi<4\pi/3$. Но  это означает, что и $\Sigma \cap \Lambda \cap (qx^i_k] \neq \emptyset$, поскольку $\Lambda \cap \Sigma \subset S_\Sigma$. Полученное противоречие показывает, что $\Sigma \cap \Lambda \cap B_{ \varepsilon_1}(x^i_k)$ состоит из отрезков, соединяющих точки, лежащие на $W$. Ясно, что последовательное соединение счетного числа точек $\{z_l\}\subset W$, имеющих единственную точку сгущения $x^i_k$ дает возможную границу псевдоконуса (поскольку $\angle((z_l z_{l+1}), (ix^i_k])$ стремится к нулю, а значит для $z\in[z_l z_{l+1}]$ угол $\angle zx^i_ki \leq z_lx^i_ki \rightarrow 0$, и другие условия на границу псевдоконуса также выполнены). Но тогда можно выбрать такой псевдоконус $Q$ (переопределив $\varepsilon \defeq \varepsilon_1$), что все точки $\{z_l\} \subset \Int(Q)$.

%МОЖЕТ БЫТЬ НАДО НАПИСАТЬ ЭТО ВСЕ КАК ОБЩЕЕ УТВЕРЖДЕНИЕ ПРО ПСЕВДОКОНУС, А ТУТ ПРОСТО СОСЛАТЬСЯ

% Применив Следствие~\ref{1} к штейнеровскому лесу, образованного пересечением $\Sigma$ и областью, ограниченной $%\partial W$, $\partial B_\varepsilon'(x^i_k)$, получим, что  число пересечений $\left(\Sigma \cap U \cap \partial W \right)$ %конечно, и переопределим псевдоконус, заменив границу $Q_{inn}$ кривой $W$.

Таким образом, можно считать $\varepsilon>0$ настолько малым, что пересечение $\Sigma \cap B_\varepsilon(x^i_k) \cap \partial Q =\emptyset$, а значит каждая из двух дуг $\breve{[sx^i_k]}$ и $\breve{[tx^i_k]}$ либо содержится в конусе $Q_1$ или $Q_2$, либо совпадает с отрезком внутри множества $B_{\varepsilon}(x^i_k) \setminus (Q_1 \cup Q_2)$. Если дуга содержится в псевдоконусе $Q_i$ ($i=1,2$), то она имеет одностороннюю касательную, а значит к ней применима Лемма~\ref{angles2}. Поскольку $x^i_k \in E_\Sigma$, она имеет хотя бы одно энергетическое ребро, а значит, ввиду определения ребра и условия на $\varepsilon$, хотя бы одна из дуг должна содержаться в каком-либо псевдоконусе. Не умаляя общности, $\breve{[sx^i_k]} \subset Q_1$. Тогда ввиду Леммы~\ref{angles2} вторая дуга $\breve{[tx^i_k]}$ не может содержаться в том же псевдоконусе. Пусть $\breve{[tx^i_k]}$ не содержится в псевдоконусе $Q_2$. Тогда она является отрезком, причем $\breve{[tx^i_k]}=[tx^i_k]\subset B_\varepsilon(x^i_k)\setminus Q$. Предположим, что этот отрезок не является $o_\rho(1)$-почти параллельным $(ix)$, то есть 
\[
|\angle(s_{\bar{\varepsilon}}x^i_k),(ix))-\angle(t_{\bar{\varepsilon}}x^i_k),(ix))|>c_1,
\]
 где $s_{\bar{\varepsilon}} \defeq \breve{[sx^i_k]} \cap \partial B_{\bar{\varepsilon}}(x^i_k)$, $t_{\bar{\varepsilon}} \defeq [tx^i_k] \cap \partial B_{\bar{\varepsilon}}(x^i_k)$, $0<\bar{\varepsilon}<\varepsilon$, а $c_1>0$ является константой, не зависящей от $\bar{\varepsilon}$ и $\rho$. Тогда, как было показано в пункте~\ref{ugli}
 \[
 |s_{\bar{\varepsilon}}x^i_k|+|t_{\bar{\varepsilon}}x^i_k|-|s_{\bar{\varepsilon}}d|-|t_{\bar{\varepsilon}}d| > c_2 \bar \varepsilon,
 \]
 где $d \in B_{\bar{\varepsilon}}(x^i_k)$ такая точка, что $\angle(s_{\bar{\varepsilon}}x^i_k),(ix))=\angle(t_{\bar{\varepsilon}}x^i_k),(ix))$, а прямая $(dx^i_k)$ параллельна $ix$; а положительная константа $c_2$ зависит только от $c_1$. Тогда замена множества $\Sigma$ на связное множество $\Sigma \setminus B_{\bar{\varepsilon}}(x^i_k) \cup [s_{\bar{\varepsilon}}d] \cup [t_{\bar{\varepsilon}}d] \cup S$, где $S$ определено в пункте~\ref{Losiu} при $w=d$ и для шара $B_{\bar{\varepsilon}}(x^i_k)$, демонстрирует противоречие с оптимальностью $\Sigma$. Таким образом, $\breve{[tx^i_k]}$ содержится в псевдоконусе $Q_2$, либо является отрезком, принадлежащим прямой  $o_\rho(1)$-почти параллельным $(ix)$. В этом случае переопределим $Q_2$ как произвольный псевдоконус с биссектрисой $[x^i_kt)$,  и утверждение пункта будет доказано.
\end{proof} 
 \begin{remark}
 Мы также доказали, что $\Sigma \cap B_\varepsilon(x^i_k) \setminus Q =\emptyset$.
 \end{remark}
 \begin{remark}
 Заметим также, то угол между ребрами, содержащий соответствующую $x^i_k$ точку $y^i$, не может быть меньше $\pi$ (если покрытые $x^i_k$ точки есть в обеих полуплоскостях, то угол между ребрами составляет ровно $\pi$).
 \label{rovno}
 \end{remark}


\begin{remark}
Поскольку $\Sigma$ не содержит циклов и имеет конечную длину, между любыми точками $x_1, x_2 \in \Sigma$ существует единственный несамопересекающийся путь. В дальнейшем мы будем опускать формальности и просто писать ``путь из $x_1$ в $x_2$''.
\end{remark}

\item В окрестности произвольной $x^i_k$ конечное число точек ветвления.
\label{fsinite}
\begin{proof}
Случай $x^i_k \in X_\Sigma \cup S_\Sigma$ тривиален; согласно пункту~\ref{discr} точка $x^i_k \in E_\Sigma$ имеет порядок $2$.
Тогда, ввиду пункта~\ref{arc_par}, найдется такое, сколь угодно малое, $\varepsilon>0$, что:
\begin{itemize}
\item $B_\varepsilon(x^i_k) \cap \Sigma \supset \breve{[sx^i_k]}\cup \breve{[tx^i_k]}$,
\item $\{s, t \}= \partial B_\varepsilon(x^i_k) \cap \Sigma$,
\item $\breve{[sx^i_k]} \subset Q_1$, $\breve{[tx^i_k]} \subset Q_2$ где $Q_1$, $Q_2$ --- псевдоконусы с ребрами $x^i_k$ (которые почти параллельны $(ix)$) в качестве биссектрис.
\item $B_\varepsilon(x^i_k) \cap \Sigma \setminus Q_1 \setminus Q_2$ пусто.  
\end{itemize}
%Пусть предположене пункта неверно, тогда, не умаляя общности, %$\breve{[sxi_k]} \subset Q_1$, где $Q_1$ псевдоконус, %содержащий бесконечное число точек ветвления. 

Предположим, что дуга $\breve{[sx^i_k]}$ содержит бесконечное число точек ветвления. 

Разберем два случая:
\begin{itemize}
\item[(А)] пусть ребро, совпадающее с биссектрисой $Q_1$, направлено в одну сторону.

Заметим, что в этом случае шар $B_\varepsilon(x^i_k)$ разбит дугами на две половины, одна из которых не может содержать энергетических точек (не умаляя общности, назовем её ``верхней'', а дугу $[sx^i_k]$ ``левой'').

Рассмотрим такую точку ветвления $D_2$ на дуге $\breve{[sx^i_k]}$, что на пути из $D_2$ в $x^i_k$ бесконечно точек ветвления, а на пути из $s$ в $D_2$ достаточно много точек ветвления. Из точки $D_2$ выходит три отрезка $[D_1D_2]$, $[D_2D_3]$ и $[D_2C]$ с попарными углами $2\pi/3$. Не умаляя общности, путь $D_1-D_2-D_3$ подмножество пути из $s$ в $x^i_k$. Заметим, что ввиду условий на $[sx^i_k]$ верно
 \[
| \turn (D_1-D_2-D_3-\dots -x^i_k)| \leq |\turn ([sx^i_k])| \leq 2\pi,
 \]
 где $\turn$ обозначает изменение направления касательной вдоль дуги. Поскольку касательная есть в почти всех точках, то будем воспринимать $\turn(\breve{[sx^i_k]})$ верхний предел (супремум) по всем последовательностям точек кривой:
 \[
 \turn(\breve{[sx^i_k]})=\sup_{n\in \N, s\preceq t_1 \prec \dots \prec t_n \preceq x^i_k} \sum_{i=2}^{n} |t^i-t^{i-1}|,
 \]
 где $t^i \in [-\pi,\pi]$ означает наклон касательной к кривой $\breve{[sx^i_k]}$ в точке $t_i$, а ${t_1,\dots, t_n}$ --- разбиение кривой $\breve{[sx^i_k]}$ в порядке, соответствующем параметризации, при которой $s$ --- начало кривой, а $x^i_k$ --- конец, такое, что в каждой точке $t_i$ кривая $\breve{[sx^i_k]}$ имеет касательную. Заметим, что направление угла $\angle D_1D_2D_3=2\pi/3$ определяется однозначно: в выбранных обозначениях угол направлен против часовой стрелки, то есть $\turn=\pi/3$. Это так, поскольку путь, начавшийся с отрезка $[D_2C]$ должен закончиться энергетической точкой, а значит идти в верхнюю  половину шара $B_\varepsilon(x^i_k)$.
Рассмотрим теперь путь  из $D_1$ в $x^i_k$. Начав с отрезка $[D_2D_3]$, путь движется по прямой вплоть до первой точки ветвления или энергетической точки. Из пункта~\ref{arc_par}, Замечания~\ref{rovno} и того, что ребра направлены только в одну сторону следует, что угол направления касательной в энергетических точках меняется в ту же сторону (то есть $\turn$ положительный). При этом в каждой точке ветвления путь поворачивает на $\pi/3$ против часовой стрелки, то есть поворот $\turn$ увеличивается на $\pi/3$. Таким образом, показано, что $\turn ([sx^i_k]) =\infty$. Противоречие.
(Иначе говоря, бесконечно закручивающаяся кривая, принадлежащая псевдоконусу, не может иметь пределом его вершину.)

% из множества $X_\Sigma$ или $E_\Sigma$, в которых  меняется направление односторонней касательной: Однако, как было показано  в пункте~\ref{arc_par}, если и меняется, то в ту же сторону (угол между односторонними касательными изменился не больше, чем на $\pi/3$). В то же время как следует из утверждения пункта~\ref{arc_par} и замечания~\ref{rovno} если в точке из множества $E_\Sigma$ направление односторонней касательной почти не меняется, а если и изменяется, то в ту же сторону. Встретив же точку ветвления, мы обязаны повернуть на $\pi/3$ в ту же сторону.  Таким образом путь из $D_1$ в $x^i_k$ бесконечно ``закручивается''(иначе говоря $turn(\breve{[sx^i_k}=\infty)$). Но, поскольку он при этом содержится в псевдоконусе $Q$, точка $x^i_k$ не может быть его пределом. Противоречие. 
 
\item[(Б)] пусть ребро, совпадающее с биссектрисой $Q_1$, направлено в обе стороны.

Несложно понять, что $\oordball x^i_k=1$ и можно считать достаточно малое $\delta$ таким, что $\sharp (\Sigma \cap \partial B_{\delta}(x^i_k)\cap Q_1) =1$ (в противном случае ввиду неравества коплощади можно было бы уменьшить длину $\Sigma$ (заменив $\Sigma \cap Q_1 \cap B_{\delta}(x^i_k)\cap Q_1$ на множество с длиной $\delta +o(\delta)$)).
В данном пункте ``почти'' будет означать ``с точностью до $o_\delta(1)$''. Биссектрису $Q_1$ будем обозначать $(qx^i_k]$. Все доказанные для $x$ и $\rho$ утверждения верны и для $x^i_k$ и $\delta$.

Поскольку количество точек ветвления в $Q_1$ бесконечно, бесконечно и количество концевых точек. Пусть $W$ --- концевая точка. Ей соответствует точка $y_W \in M$ такая, что $|wy_W|=r$ и $B_r(y_W) \cap \Sigma =\emptyset$. Условно будем говорить, что точки из множества $M$, соответствующие концевым точкам из $Q_1$ могут располагаться ``сверху'' или ``снизу'' (полагаем прямую $(qx^i_k]$ горизонтальной). Точка $y_W$, не умаляя общности, располагается ``сверху''. Также, не умаляя общности, полагаем точку $x^i_k$ находящейся ``справа'' от точки $W$.
%\input{pictures/9netputi}
Из точки $W$ выходит отрезок $[WD_1]\subset \Sigma$, почти перпендикулярный $(qx^i_k]$, где $D_1$ --- точка ветвления: из-за условия почти-перпендикулярности $D_1$ не может быть точкой из $X_\Sigma$ степени $2$ или точкой из $E_\Sigma$ (см. пункты~\ref{discr}, ~\ref{arc_par}  и следствие из пункта~\ref{ugli}). Ясно, что путь $L$ из $D_1$ в $x^i_k$ начинается с отрезка $[D_1D_2]$, направленного в сторону $x^i_k$: в противном случае, если бы путь $L$ начинался с отрезка $[D_1D_{-2}]$, направленного от $x^i_k$, то, ввиду условия  $B_r(y_W) \cap \Sigma =\emptyset$ (и ввиду дугообразной связности, из-за которой путь $L$ должен существовать в достаточно малой окрестности $x^i_k$, а значит не может иметь диаметр, больший $r$), он ``отрезал'' бы путь $P$, начинающийся со второго отрезка $[D_1D_{2}]$ и в каждой точке ветвления поворачивающий ''вниз'', от находящихся ``снизу'' точек множества $M$: то есть либо пути $L$ и $P$ должны пересечься, либо пустая окружность радиуса $r$, касающаяся энергетической точки, которой заканчивается путь $P$, должна пересекать путь $L$, что также невозможно (см. рис.~\ref{fig:netputi}). 

\input{pictures/dvap}
Точка $D_2$ может быть точкой степени $2$ или $3$, в любом случае путь $L$ продолжается отрезком $[D_2D_3]$, направленным ``вправо'' (и ввиду утверждения пункта~\ref{ugli} имеющим относительно $(qx^i_k]$ угол почти $\pi/6$): если бы он продолжался отрезком $[D_2D_{-3}]$, направленным вниз,  то существовал бы путь, выходящий из $D_{-3}$ и поворачивающий на каждом шагу ``налево''. Наличие аналогичного пути из $D_{-2}$  влечет противоречие с выбором $\delta$ (оба пути не могут закончиться энергетической точкой степени $1$, поскольку все составляющие их отрезки имеют угол с $(qx^i_k]$ почти $\pi/6$. То есть каждый из путей должен пересечь $\partial B_{\delta} (x^i_k)$ (см. рис.~\ref{fig:dvap})).

Далее можно повторять те же рассуждения с точностью до симметрии относительно $(qx^i_k]$ и взяв точку $D_{-3}$ (в случае её наличия) в качестве точки $W$. В случае же ее отсутствия, точка $D_2$ будет выступать в роли отрезка $[WD_1]$, поскольку входящие в нее отрезки имеют угол почти $\pi/6$ с $(qx^i_k]$.

То есть путь $L$ содержит отрезок $[D_2D_3]$, где $D_3$ либо точка ветвления, либо точка степени $2$. Несложно заметить, что в первом случае $\Sigma$ содержит отрезок $[D_3G]$, где $G$ концевая точка (иначе существовал бы начавшийся в $G$ и не заканчивающийся энергетической точкой путь, в каждой точке ветвления, поворачивающий от точки $x^i_k$). Во втором случае, как следует из пункта~\ref{ugli}, $L$ продолжается отрезком $[D_3D_4]$, имеющим почти такой же угол с $(qx^i_k]$, что и $(D_2D_3)$ (то есть отличающийся от $\pi/6$ на величину $o_\delta(1)$). То есть точка $D_4$ может быть либо точкой ветвления, либо точкой степени $2$ (причем в таком случае она должна принадлежать $X_\Sigma$) и т.д. 

Заметим, что путь $L$ не может содержать ломаную $L_1-L_2-L_3-L_4-L_5$, где все точки $L_i$ имеют степень $2$, а углы $\angle (L_iL_{i+1}), (ix)), \angle (L_iL_{i-1}), (ix))  \geq  \pi/7$. Поскольку данное утверждение потребуется нам за пределами пункта, сформулируем его в более общем виде:
\begin{proposition}
Пусть $\bar x \in E_\Sigma$ и существуют такие точки $y_1, y_2$, что $|y_1y_2|=2r$, $|y_1\bar x|=r =|y_2 \bar x|$ и $B_r(y_1)\cap \Sigma = B_r(y_2)\cap \Sigma =\emptyset $. Пусть, кроме того $\bar{\varepsilon}>0$ такой, что $B_\varepsilon(\bar{x}) \cap \Sigma$ является дугой. Тогда для произвольного $c>0$ найдется $\varepsilon(c)>0$ такой, что все односторонние касательные к точкам $B_{\bar \varepsilon}(\bar{x}) \cap \Sigma$ имеют угол с прямой $(y_1y_2)$ находящийся в промежутке $[\pi/2-2c, \pi/2]$.
\label{zapred}
\end{proposition}

\begin{proof}
Предположим противное, то есть что существует последовательность точек, в которых односторонняя касательная имеют угол с $(y_1y_2)$ вне указанного промежутка. Ввиду утверждения пункта~\ref{arc_par} (для $\bar{x}$ в качестве $x$ и энергетических точек из этой последовательности в качестве точек $x^i_k$) достаточно рассматривать только точки из множества $X_\Sigma \sqcup S_\Sigma$. Поскольку в точках $S_\Sigma$ направление касательной не меняется ясно, что найдется сходящаяся к $\bar{x}$ последовательность точек из $X_\Sigma$ таких, что хотя бы один из двух входящих в точку отрезков имеет угол с $(y_1y_2)$, меньший $\pi/2-2c$. Пусть $L_1$ такая точка, достаточно близкая к $\bar{x}$. Ввиду утверждения пункта~\ref{ugli}, можно считать, что оба входящих в $L_1$ отрезка имеют угол с $(y_1y_2)$, меньший $\pi/2-9/5c$. Тогда отрезок, лежащий на пути из $L_1$ в $\bar{x}$ обязательно заканчивается точкой $L_2 \in X_\Sigma$. Но отрезок, выходящий из $L_2$ должен иметь угол с $(y_1y_2)$, меньший $\pi/2-8/5c$ и заканчиваться точкой $L_3 \in X_\Sigma$. Ясно, что таким образом для любого, сколь угодно малого $\varepsilon$ существует такая ломаная $L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\bar{\varepsilon}}$, что все углы $\angle((L_iL_{i+1}),(Y_1y_2))<\pi/2-c$ при $i=1,2,3,4$. 
Не умаляя общности будем считать $(y_1y_2)$ осью ординат, а точку $\bar{x}$ началом координат. Не умаляя общности, точкам $L_1$, $L_2$, $L_3$ соответствуют верхние точки множества $M$, а точкам $L_2, L_4$ --- нижние: ввиду утверждения пункта~\ref{angles} и неравенства $\angle L_{i-1}L_{i}L_{i+1} \leq \pi-2c, i=2,3,4$ двум подряд идущим точкам не могут соответствовать одновременно верхние или нижние точки.
 Заметим теперь, что отношения между отрезками ломаной линейные, и замена ломаной на отрезки $L_1-L_2-L_4-L_5$ уменьшит длину на величину, линейно зависящую от $[L_1L_2]$. 

Строго говоря, поскольку $B_r(y_{L_{i+1}})\cap [L_{i-1}L_{i}]=\emptyset = B_r(y_{L_{i-1}})\cap [L_{i}L_{i+1}]$, где $y_{L_j} \in M$ соответствует $L_j$, $j= 1 \dots 5$, $i=2,3,4$ и ввиду пункта~\ref{angles}, выполняется \[[L_2L_3]_y>|L_1L_2|_y-|L_1L_3| o_{\bar{\varepsilon}}(1)\]
 %|L_1L_2|-\bar{\varepsilon}^2,\]
  где нижний индекс $y$ означает проекцию на $(y_1y_2)$. То есть $|L_2L_3|>\sin c |L_1L_2|-o_{\bar{\varepsilon}}(1)|L_1L_3|$.
 И наоборот, $|L_1L_2|>\sin c |L_2L_3|-o_{\bar{\varepsilon}}(1)|L_1L_3|$. 
 %Из этого очевидным образом следует существование $c_1, c_2>0$ таких, что $c_2|L_2L_3|\geq |L_1L_2| \geq c_1|L_1L_3|$.   
 Аналогично и для остальных $L_i$. Замена ломаной на $L_1-L_2-L_4-L_5$ уменьшит ее длину не меньше, чем на
 \begin{multline*}
 |L_2L_3|+|L_3L_4|-\sqrt{ |L_2L_3|^2+|L_3L_4|^2+2 |L_2L_3||L_3L_4|\cos (2c) }\geq \\
|L_1L_2| \left(\sin c+\sin^2 c-\sqrt{\frac{1}{\sin^2 c}+\frac{1}{\sin^4 c}+2\frac{\cos (2c)}{\sin^3 c}})+o_{\bar{\varepsilon}}(1|L_1L_2| \right),
 \end{multline*}
то есть замена, действительно, уменьшает длину на величину, линейно зависящую от $|L_1L_2|$.
\input{pictures/dvapo}
Кроме того, несложно понять (как обычно используя пункт~\ref{angles}), что существуют
% отрезки $[L_1L_{6}]$ и $[L_5L_7]$
точки $L_6$ и $L_7$  такие, что $$B_r([L_1L_6]) \cup B_r([L_5L_7]) \supset B_r([L_1L_3]) \cup B_r([L_3L_5]).$$ Причем эти отрезки имеют длину $o_{[L_1L_2]}(1)$. 

 Тогда можно заменить ломаную  $L_1-L_2-L_3-L_4-L_5$ на $L_6-L_1-L_2-L_4-L_5-L_7$ и получить противоречие с оптимальностью $\Sigma$ (см. рис~\ref{fig:dvapo}).
 \end{proof}

%тут уруру конечно ужасно лень аккуратно писать но в общем выпуклости у нас нет, но зато есть почти выпуклость из-за того что окружности для L_1 и L_5 всё выгрызли и L_3 не могла высоко подпрыгнуть
Вернемся к пути $L$. Теперь ясно, что он является ломаной с узлами в точках ветвления и энергетических точках степени $2$. Причем последние не могут встречаться более четырех раз подряд, если их угол с осью абсцисс достаточно велик. А из узлов в точках ветвления отходят (не принадлежащие $L$) отрезки, почти перпендикулярные $(ix)$. Тогда все отрезки ломаной $L$ имеют угол с $(ix)$, больший, чем $\pi/7$ (поскольку в отрезках, выходящих из точек ветвления угол почти $\pi/6$, а в точках степени два угол падения почти равен углу отражения, причем погрешность не накапливается, поскольку не может быть больше четырех точек ветвления подряд). 

Но тогда длина пути $L$ составляет не меньше, чем
\[
Pr_{(ix)}(L) \left (1+\tg \frac{\pi}{7} \right )=\delta \left (1+\tg \frac{\pi}{7} \right),
\]
где $Pr_{(ix)}(L)$ ---  проекция пути $L$ на прямую $(ix)$.
С другой стороны из условий на $Q$ следует, что длина $\Sigma \cap B_{\delta}(x^i_k)\cap Q$, а значит и длина пути $L$, не превосходит $\delta+o(\delta)$. Полученное противоречие завершает доказательство пункта.
\end{itemize}





\end{proof}

\begin{remark}
Заметим, что в пункте~\ref{fsinite} доказано утверждение о конечности точек ветвления на дуге $\breve{[sx]}$ для произвольной точки $x \in E_\Sigma$ в случае если $\breve{[sx]}$ лежит в каком либо псевдоконусе $Q$ и $\Sigma \cap \partial Q =\emptyset.$
\label{rfinite}
\end{remark}

\item Покажем, что компонента связности $\Sigma \cap B_\rho(x) \setminus \{x\}$ содержит бесконечное число энергетических точек не более чем одного энергетического ребра (иначе говоря, находящихся не более чем в одном псевдоконусе).
\label{rozo4ki}

\begin{remark}
В доказательстве данного пункта в случае $\oord_x \Sigma =1$ компоненту связности множества $\Sigma \cap B_\rho(x) \setminus \{x\}$ можно считать совпадающей с данным множеством.
\end{remark}

В доказательстве данного пункта рассматриваются только точки принадлежащие данной компоненте. Для простоты записи будем считать, что рассматривается ситуация $\oord_x \Sigma =1$.

\begin{proof}
Предположим противное утверждению пункта~\ref{rozo4ki}.
\begin{enumerate}


\item Точка $x^i_k \in X_\Sigma$ не может иметь порядок $2$. 
\label{9}
\begin{proof}
Пусть $x$ имеет два ребра $(ax]$ и $(bx]$, $\alpha \in]0, \pi]$ --- угол между этими лучами, $\rho>0$ достаточно мало и $\sharp(\partial B_\rho(x) \cap \Sigma) \leq 3$ (корректно ввиду Замечания~\ref{ord_en}), $Q^a$, $Q^b$ --- псевдоконусы с ребами в качестве биссектрис, содержащие все энергетические точки этих ребер (в достаточно малой окрестности $B_\rho(x)$). Меньший угол между ребрами называется внутренним (а если оба угла равны $\pi$, то внутренним называется угол, не содержащий точку $y \in M$, соответствующую точке $x$: можно считать, что ребра направлены в одну сторону, иначе утверждение пункта тривиально).


Не умаляя общности, $i=a$. Предположим противное утверждению пункта: пусть точка $x^a_k \in X_\Sigma$ имеет степень два. Воспользуемся пунктом~\ref{ugli} и обозначим, с точностью до $o_\rho(1)$, угол между входящими в $x^a_k$ отрезками и ребром $(ax]$ за $\delta$.
Выполняется неравенство $\delta \leq \frac{\pi}{6} + o_\rho(1)$. 

Обозначим за $[x^a_k t]$ тот отрезок из $x^a_k$, который направлен к $x$. Возможны два варианта:


\begin{itemize}
\item Отрезок $[x^a_k t]$ заканчивается точкой ветвления. Если $t$ соединена со следующей энергетической точкой того же ребра $[ax]$ (то есть лежащего в криволинейном  псевдоконусе этого ребра, определенном в Утверждении~\ref{edgeangle}), то угол между $(tx^a_{k+1})$ и $(ax)$ будет равен $\frac{\pi}{3} - \delta \leq \frac{\pi}{6} + o_\rho(1)$. В таком случае, $\delta = \frac{\pi}{6} + o_\rho(1)$ (как изображено на Рис.~\ref{norm1}). 
Если точка $t$ не соединена с $x^a_{k+1}$, то она соединена с точкой ветвления $C$ такой, что отрезок $[tC]$ направлен от ребра $(bx]$ (как изображено на Рис.~\ref{norm11}). Тогда путь, начинающийся с отрезков $[x^a_k t]$ и $[tC]$ и продолжающийся поворотами в ту же сторону сможет закончиться только если $C$ соединена с $x^a_{k+1}$. 
\begin{remark}
Здесь и в дальнейшем доказательстве пункта~\ref{rozo4ki} можно считать, что ни один рассматриваемый путь не может закончиться на $\partial B_\rho(x)$ (поскольку число пересечений $\partial B_\rho (x) \cap \Sigma$ конечно и значит можно выбрать $\rho>0$ так, чтобы это было верно).
\end{remark}
В этом случае угол между отрезком $[Cx^a_{k+1}]$, и ребром $(ax]$ будет равен $\frac{\pi}{3} +\delta$. Значит, точка $x^a_{k+1}$ имеет порядок один. Но в этом случае указанный угол должен совпадать с $\frac{\pi}{2}+o_\rho(1)$, поэтому все равно $\delta = \frac{\pi}{6} +o_\rho(1)$.
%\input{pictures/norm1}

Оставшийся отрезок точки $t$ (обозначим его за $[tD]$) имеет угол 
$$\frac{2\pi}{3} - \delta - \alpha = \frac{\pi}{2}-\alpha + o_\rho (1)$$
 со вторым ребром $(bx]$. То есть если $J \defeq [tD) \cap (bx]$, то $\angle tJx =\frac{\pi}{2} -\alpha +  o_\rho (1)$. Тогда точка $D$ не может быть энергетической точкой степени один или точкой из $E_\Sigma$ степени два. Энергетической точкой из $X_\Sigma$ степени два или точкой ветвления она также не может быть, потому что тогда найдется бесконечный путь, начинающийся с $[sx^a_k], [x^a_{k}t], [tD], \dots$, где
$[sx^a_k]$ --- отрезок, входящий в $x^a_k$, а поворот на каждом шаге не меньше $\frac{2\pi}{3}$. Противоречие.

%\input{pictures/norm11}

\item Точка $t$ является энергетической точкой ребра $(bx]$, то есть совпадает с точкой $x^b_l$.

Тогда $x^b_l$ должна быть степени два (иначе нет пути из $x^a_k$ в $x$) и принадлежать множеству $X_\Sigma$, т.к. $\angle((x^a_kx^l_b],(bx])=\alpha+\delta+o_\rho(1) \neq o_\rho(1)$. Ситуация $\angle((x^a_kx^l_b],(bx])=\pi+o_\rho(1)$ также невозможна ввиду наличия окружностей $B_r(x^a_k)$, $B_r(y_l^b)$ и $B_r(y)$, не пересекающихся с $\Sigma$.


 %$B_{\min(|xx^b_{l}|, |xx^a_{k}|)}(x) \cap \Sigma$, связности). 
Но тогда есть отрезок $[x^b_l d] \subset \Sigma$, выходящий из  $x^b_l$ с углом $\angle xx^b_ld = \angle bx^b_lx^a_k +  o_\rho (1)$.
%= \pi-\delta -\alpha$.  
Разберем ситуацию, когда он не разветвился, а также воткнулся в энергетическую точку $x^a_{k+1}$ первого ребра. Пусть и новый отрезок не разветвился и $[x^a_{k+1}x^b_{l+1}] \subset \Sigma$, где $x^b_{l+1}$ --- энергетическая точка второго ребра. И так далее. Несложно заметить, что тогда углы падения и отражения будут увеличиваться c каждым шагом на $\alpha + o_\rho (1)$ (как изображено на Рис.~\ref{norm2}).
Но они не должны превосходить $\frac{\pi}{6}$. Ситуация, когда какой-то из отрезков уже разветвился разобрана выше. Противоречие. 

%\input{pictures/norm2}

\end{itemize}
\end{proof}
\item Все точки $x^i_k$ принадлежат множеству $X_\Sigma$.

\begin{proof}
Предположим, что найдется точка $x^a_k$ из $E_\Sigma$. Тогда, согласно пункту~\ref{discr}, $\oord_{x^a_k}\Sigma = 2$, тогда, ввиду пункта~\ref{arc_par},  в $x^a_k$ входят две дуги, локально почти параллельные $(ax]$. Посмотрим на путь в $\Sigma$ от $x^a_k$ к $x$. Покажем, что он не может содержать точки ветвления до выхода из псевдоконуса $Q^a$. Предположим противное и обозначим за $A$ первую точку ветвления на пути (такая точка существует ввиду утверждения пункта~\ref{fsinite}). Тогда $A \in S_\Sigma$. И пусть --- $B$ последняя энергетическая точка на пути из $x^a_k$ в $A$ (может совпадать с $x^a_k$). Тогда путь из $B$ в $A$ является отрезком, причем, ввиду доказанного в пункте~\ref{arc_par}, отрезок $[BA]$ почти параллелен лучу $(ax]$.

Рассмотрим путь, начинающийся с отрезка $[BA]$ и продолжающийся отрезком $[AC]$, направленным от ребра $(bx]$, то есть его угол с ребром $(ax]$ составляет $\frac{\pi}{3}$. 
Ясно, что $C$ не может быть энергетической точкой степени один, поскольку это противоречит пункту~\ref{perp_edge2} и не может быть энергетической точкой степени два, поскольку это противоречит пункту~\ref{arc_par}, а значит $C$ --- точка ветвления. Повернем в точке $C$ в ту же сторону, что и в точке $A$. Угол нового отрезка с ребром $(ax]$ также составляет почти $\frac{\pi}{3}$. Рассматриваемый нами путь, в котором мы в каждом узле поворачиваем  от ребра $(bx]$, никогда не закончится (поскольку число пересечений $\partial B_\rho (x) \cap \Sigma$ конечно и значит можно выбрать $\rho>0$ таким, чтобы считать, что ни один путь не мог закончиться на $\partial B_\rho(x)$). Полученное противоречие влечет отсутствие точки ветвления на пути $x^i_k$ в $x$ до выхода из псевдоконуса $Q^a$. Пусть такой выход произошел (в противном случае несложно получить противоречие с условием $\oord_x \Sigma = 1$) и $G$ --- первая точка на пути из $x^a_k$ в $x$ такая, что $G\in \partial Q^a$ и 
\[
\forall \delta>0 \qquad (\Sigma \cap B_\delta(G)\cap Q^a \neq \emptyset)   \wedge (\Sigma \cap B_\delta(G)\setminus Q^a \neq \emptyset ). 
\]
Тогда путь продолжается отрезком $[GH]$, где $H\in Q^b$ и $\angle ((GH], (bx])=\alpha+o(\rho)$. Ясно, что точку $H$ можно считать точкой ветвления. Тогда от нее в сторону ребра $(ax]$ выходит отрезок $[HS]$ с углом $\angle ((HS], (ax])=\pi/3$. Но путь, начавшийся с отрезка $[HS]$ и содержащий только отрезки, имеющие угол с $(ax]$ почти $\pi/3$, никогда не закончится. Противоречие.
\end{proof}

%Заметим, что из доказанного следует, что все энергетические точки множества $G_\Sigma \cap B_{\rho}(x) \setminus x$ %изолированные, а значит можно выбрать последовательности $\{ x^i_k\}$ так, чтобы они содержали все точки %энергетические точки множества $G_\Sigma \cap B_{\rho}(x) \setminus x$, а также чтобы для последовательных точек %выполнялось неравенство $\dist (x, x^i_k) > \dist (x, x^i_{k+1})$.



%\end{proof}

\item Таким образом, $\Sigma$ --- локально минимальное штейнеровское дерево, без вершин степени $2$. Это означает, что отрезки $\Sigma$ могут быть только шести направлений. Но поскольку $\Sigma$ содержит отрезки, $o_\rho(1)$-почти перпендикулярные обоим ребрам $(ax]$ и $(bx]$, угол $\alpha = \angle axb$ может составлять только $\frac{\pi}{3}$ или $\frac{2\pi}{3}$.
%\end{enumerate}
\begin{itemize}


\item Пусть $\alpha := \frac{\pi}{3}$. Нарисуем розу ветров (см. определение~\ref{roza_v}), среди лучей которой есть перпендикуляры к обоим ребрам $x$. При этом, если расположить центр розы ветров во внутреннем угле $x$, то на лучах, перпендикулярных $(ax]$ ($(bx]$) и направленных к $(ax]$ ($(bx]$) стоит число $1$ (данная роза ветров изображена на Рисунке~\ref{fig:roza1}). 
 Выберем также достаточно малое $\rho_1<\rho$ так, чтобы $\sharp(\Sigma \cap \partial(B_{\rho_1}(x)))\leq 3$.

Тогда с одной стороны, ввиду Замечания~\ref{main_rose_property2}, сумма всех чисел во всех вершинах штейнеровского леса $\Sigma \cap (\overline{B_\rho(x)}\setminus B_{\rho_1}(x))$, равна $0$.

А с другой стороны, поскольку $\sharp(\Sigma \cap (\partial(B_\rho(x))\cup \partial(B_{\rho_1}(x)))\leq 6$, сумма сколь угодно велика, поскольку содержит бесконечно много положительных слагаемых и не больше шести отрицательных.
% присвоим каждой концевой вершине дерева число, соответствующее одному из шести направлений, и замет%им, что у любого локально минимального штейнеровского дерева сумма направлений будет нулевой. 
%Выберем такую малую окрестность $U(x)$, что $\sharp (\partial U(x) \cap \Sigma) = 1$, сопоставим обоим направлениям, %перпендикулярным $(ax]$ и $(bx]$ число $1$, и заметим, что можно выбрать такую окрестность $V(x)\subset U(x)$, что $%\sharp (\partial V(x) \cap \Sigma) = 1$ и что сумма направлений поддерева $\Sigma \cap (U(x)\setminus V(x))$ будет сколь %угодно велика, поскольку содержит много вершин положительных направлений и не больше двух отрицательных.  

%\input{pictures/roza1}

\item Пусть $\alpha := \frac{2\pi}{3}$. Повторим рассуждение из предыдущего пункта, взяв другую розу ветров (которая изображена на Рисунке~\ref{fig:roza2}: на луче, перпендикулярном $(ax]$ и направленном к нему, поставим $1$, а на луче, перпендикулярном $(bx]$ и направленном к нему, поставим $2$).

\input{pictures/roza2}
\end{itemize}
\end{enumerate}

Полученное противоречие завершает доказательство пункта.

\end{proof}

\item Завершение доказательства Леммы.
\label{finfin}
\begin{proof}
Поскольку $x\in E_\Sigma$ и ввиду Замечания~\ref{emptyball} пункта~\ref{netri} возможно два варианта:
\begin{enumerate}
    \item $x$ имеет одно энергетическое ребро
    Пусть $\rho$ такое, что $\sharp( \partial B_\rho(x) \cap \Sigma) \leq 3$, что возможно ввиду Замечания~\ref{ord_en}. Тогда посмотрим на замыкание множества $\Sigma \setminus Q$, где $Q$ --- псевдоконус энергетического ребра. Все концевые точки этого множества, кроме не более, чем $\oord_x \Sigma$, располагаются на $\partial Q$. Несложно заметить, что в таком случае можно считать, что $\sharp(\Sigma \cap \partial Q \cap  B_\rho(x)) <\infty$. Но тогда, не умаляя общности, можно считать $\Sigma \cap \partial Q \cap B_\rho(x)=\emptyset$. Тогда ввиду пункта~\ref{fsinite} и Замечания~\ref{rfinite} число точек ветвления в множестве $\Sigma \cap Q \cap  B_\rho(x)$ конечно. Конечно и число точек ветвления в множестве $\Sigma \cap  B_\rho(x) \setminus Q$, ввиду конечности числа концевых точек. Тогда, не умаляя общности, в множестве $\Sigma \cap B_\rho(x)$ нет точек ветвления и оно является объединением дуги $\breve{[qx]}$, лежащей в $Q$ и отрезков с одним концом в $x$ и другим на $\partial B_\rho (x)$. Поскольку биссектриса псевдоконуса $Q$ является односторонней касательной для $\breve{[qx]}\subset Q$, применима Лемма~\ref{angles2} и, значит, отрезок может быть только один, причем его угол с односторонней касательной $\breve{[qx]}$ составляет хотя бы $2\pi/3$. 
    Таким образом, в данном случае $\overline{B_\rho(x)} \cap \Sigma =\breve {qx} \cup [wx]$ или $\overline{B_\rho(x)} \cap \Sigma =\breve {qx}$, причем дуга $\breve{[qx]}$ имеет одностороннюю касательную и, в первом случае, ее угол с $[wx]$ составляет хотя бы $2\pi/3$.
    \item $x$ имеет два энергетических ребра.
        \begin{enumerate}
            \item[i] Хотя бы одно ребро направлено в обе стороны.
            В этом случае $\Sigma \cap B_\rho(x)$ является объединением двух множеств, каждое из которых содержится в каком-либо псевдоконусе с вершиной в $x$. Тогда к каждому из множеств можно применить пункт~\ref{fsinite} и Замечание~\ref{rfinite}. Таким образом, можно, считать, что множество $\Sigma \cap B_\rho(x)$ является объединением двух дуг, имеющих односторонние касательные с углом $\pi$ между этими касательными.
            \item[ii] Каждое ребро направлено в одну сторону. 
            Обозначим ребра $(ax]$ и $(bx]$, а соответствующие псевдоконусы за $Q^a$ и $Q^b$ (в процессе доказательства мы будем корректировать выбор псевдоконусов, не изменяя обозначений). Ввиду $\oord_x \Sigma < \infty$ и ввиду определения энергетического ребра, существует компонента связности $\Sigma \cap B_\rho(x)\setminus \{x\}$, содержащая бесконечное число энергетических точек ребра $(ax[$ (энергетических точек, принадлежащих псевдоконусу $Q^a$). Ввиду пункта~\ref{rozo4ki} можно так же считать, что эта компонента связности не содержит энергетических точек ребра $(bx]$ (энергетических точек, принадлежащих псевдоконусу $Q^b$). Повторяя рассуждения случая[А] доказательства пункта~\ref{fsinite} несложно убедиться, что тогда указанная компонента связности содержит не более, чем конечное число точек ветвления. А значит, можно считать, что не содержит точек ветвления вообще. Аналогичное верно для компоненты связности $\Sigma \cap B_\rho(x)\setminus \{x\}$, содержащей бесконечное число энергетических точек ребра $(bx[$ (энергетических точек, принадлежащих псевдоконусу $Q^b$). Таким образом, каждая из этих компонент связности является дугой, содержащей либо энергетические точки (принадлежащие соответствующему псевдоконусу), либо точки из $S_\Sigma$, являющиеся серединой отрезка. Несложно заметить, что тогда, ввиду определения энергетических ребер, каждая из указанных дуг содержится в некотором псевдоконусе энергетического ребра.
            
            Тогда энергетические ребра являются односторонними касательными указанных дуг, а значит к указанным дугам применима Лемма~\ref{angles2}. Тогда ясно, что угол между энергетическими ребрами $(ax]$ и $(bx]$ составляет хотя бы $2\pi/3$. Также несложно заметить, что $\Sigma \cap B_\rho(x)$ является объединением этих дуг (обозначим их $\breve{[qx]}$, $\breve{[sx]}$). В противном случае рассмотрим $\Sigma' \defeq \Sigma \setminus (\breve{[qx]} \cup \breve{[sx]})$. Тогда 
            \[
            \oord_x \Sigma'=\oord_x\Sigma -2 \leq 1
            \]
            (последнее неравенство верно ввиду Леммы~\ref{ord_en} и Замечания~\ref{rem_ord}).
            Если $\oord_x\Sigma'=1$, то существует дуга $\breve{[fx]} \subset B_\rho(x)$. Она, очевидно, не содержит точек ветвления и энергетических точек, кроме $x$, а значит является отрезком. Но тогда к ней применима Лемма~\ref{angles2} и, значит, дуга $\breve{[fx]}$ не может принадлежать $\Sigma$ одновременно с $\breve{[qx]}$ и $\breve{[sx]}$. То есть $\oord_x\Sigma'=0$, а значит найдется такая окрестность $U \ni x$, что $\Sigma' \cap \partial U=\emptyset$. Ввиду связности $\Sigma'$ найдется такой $\bar{\rho}>0$, что $\Sigma' \cap B_{\bar{\rho}}(x)=\emptyset$, то есть 
            \[
            \Sigma \cap B_{\bar{\rho}}(x)=\breve{[sx]}\cup \breve{[qx]}.
            \]
  
      \end{enumerate}
    
\end{enumerate}
\end{proof}
 
\end{enumerate}

\end{proof}

Таким образом, основная Лемма~\ref{main_l} доказана. 

%\begin{proof}
%\end{proof}



%завершает доказательство Теоремы~\ref{mainT1}.


==> ⥪�騩 ���᪨� ⥪�� (in english)/2_5examples.tex <==
\section{Полная классификация локального поведения $\Sigma$. Примеры} \label{ex}

Напомним, что $\Sigma$ является минимайзером функционала максимального расстояния для плоского компакта $M$.
Нас интересует вопрос о поведении множества $\Sigma$ в окрестности точки $x \in \Sigma$.
Из доказательства Теоремы~\ref{mainT1} следует полная классификация вариантов локального поведения $\Sigma$. Мы приведем примеры для каждого из возможных вариантов.% На рисунках заданные множества $M$ обозначаются зеленым цветом, энергетические точки минимайзера $\Sigma$ --- красным, остальные точки множества %$\Sigma$ --- фиолетовым. 

Обычно достаточно сложно доказать, что конкретное множество $\Sigma$ является минимайзером для конкретного $M$. На иллюстрации~\ref{horseFig} множество $M$ --- окружность радиуса $R > r$, а множество $\Sigma$ --- объединение дуги окружности радиуса $R-r$ и двух отрезков касательных к этой окружности. Миранда, Степанов и Паолини~\cite{mir} предположили, что $\Sigma$ --- минимайзер для $M$. 
Доказательство того, что множество $\Sigma$ является минимайзером при условии $R > 4.98r$, можно найти в работе~\cite{cherkashin2015horseshoe}.

Стоит отметить, что если $M$ является конечным множеством точек, то существует простой критерий: связное множество $\Sigma$ является минимайзером для $M$ и числа $r>0$, если выполняется неравенство $\H(\Sigma) \leq \H(St(M))-r \sharp{M}$, где $\sharp{M}$ --- количество элементов множества $M$, а $St(M)$ --- связное множество с наименьшей длиной, содержащее все точки $M$ (иначе говоря,  произвольное дерево Штейнера для множества $M$). Несложно также заметить, что строгое неравенство в этом выражении невозможно. Этот критерий показывает, что в примерах на Рис.~\ref{X2},~\ref{X1ill},~\ref{X2non120} множество $\Sigma$ действительно минимайзер. 

Из Теорем~\ref{mainT1} и~\ref{persp} следует Теорема о классификации локального поведения минимайзера в произвольной точке.

\begin{theorem2}

Пусть $\Sigma$ --- минимайзер максимального расстояния, содержащий хотя бы две точки. Тогда
\begin{enumerate}
\item  Если $x \in S_\Sigma$, то найдется такое $\varepsilon > 0$, что $\Sigma \cap B_{\varepsilon}(x)$ является одним из двух множеств:
%(см свойства минимайзеров~\ref{g})
\begin{enumerate}
\item отрезком %, и в этом случае точка $x$ имеет порядок $2$ 
 (точка $S$ на Рис.~\ref{horseFig},~\ref{X2},~\ref{ElimX},~\ref{X1ill},~\ref{X2non120});
\item правильной треногой %, и в этом случае точка $x$ имеет порядок $3$ 
 (точка $F$ на Рис.~\ref{X1ill}).
\end{enumerate} 

\item Если $x \in X_\Sigma$, то найдется такое $\varepsilon > 0$, что $\Sigma \cap B_{\varepsilon}(x)$ является одним из двух множеств:
%(cм Утверждение~\ref{discr_str}) 
\begin{enumerate}
\item отрезком с концом в $x$ %, то есть точка $x$ имеет порядок $1$
 (точка $D$ на Рис.~\ref{horseFig},~\ref{X2},~\ref{ElimX},~\ref{X1ill},~\ref{X2non120});
\item объединением двух отрезков с концами в $x$ и углом большим (точка $E$ на Рис.~\ref{X2non120} и Рис.~\ref{ElimX}) или равным (точка $E$ на Рис.~\ref{X2}) $2\pi/3$, между ними.%, и в этом случае точка $x$ имеет порядок $2$.
\end{enumerate}


\item  Если $x \in E_\Sigma$, то найдется такое $\varepsilon > 0$, что $\Sigma \cap B_{\varepsilon}(x)$ является одним из двух множеств:
\begin{enumerate}
\item дугой с концом в $x$, имеющей в этой точке одностороннюю касательную. % (в этом случае точка $x$ имеет порядок $1$).
При этом точка $x$ может
\begin{enumerate}
\item являться предельной точкой множества $X_\Sigma$ (точка $G$ на Рис.~\ref{ElimX});
\item не являться предельной точкой множества $X_\Sigma$ (точка $G$ на Рис.~\ref{E1}).
\end{enumerate}

\item объединением двух отрезков дуг с концами в $x$, имеющих в этой точке односторонние касательные с углом, не меньшим $2\pi/3$, между ними %; в этом случае %точка $x$ имеет порядок $2$ 
 (точки $H_1$ и $H_2$ на Рис.~\ref{horseFig} и точка $H_2$ на Рис.~\ref{E1}).
\end{enumerate}
\end{enumerate}

\end{theorem2}


\input{pictures/horseshoe}
\input{pictures/X2}
\input{pictures/ElimX}
\input{pictures/X1ill}
\input{pictures/X2non120}
\input{pictures/E1}

%\begin{figure}[H]
%\begin{subfigure}[width=0.25\linewidth]
%\input{pictures/horseshoe}
%\end{subfigure}
%\begin{subfigure}[width=0.25\linewidth]
%\input{pictures/horseshoe}
%\end{subfigure}
%\end{figure}

%https://ru.wikipedia.org/wiki/%D0%92%D0%BF%D0%BE%D0%BB%D0%BD%D0%B5_%D0%BD%D0%B5%D1%81%D0%B2%D1%8F%D0%B7%D0%BD%D0%BE%D0%B5_%D0%BF%D1%80%D0%BE%D1%81%D1%82%D1%80%D0%B0%D0%BD%D1%81%D1%82%D0%B2%D0%BE
%https://ru.wikipedia.org/wiki/%D0%92%D0%BF%D0%BE%D0%BB%D0%BD%D0%B5_%D0%BD%D0%B5%D1%81%D0%B2%D1%8F%D0%B7%D0%BD%D0%BE%D0%B5_%D0%BF%D1%80%D0%BE%D1%81%D1%82%D1%80%D0%B0%D0%BD%D1%81%D1%82%D0%B2%D0%BE

Приведем пример ``плохого'' множества $M$:
\begin{example}
Пусть $M$ --- компактное вполне несвязное множество, дерево Штейнера для которого обладает бесконечным числом точек степени 3. 
Явный пример такого множества $M$ был построен в работе~\cite{paolini2015example}.
В то же время из результатов анонсируемой статьи следует, что для любого числа $r < \diam M$ минимайзер будет содержать конечное число точек ветвления. 
\end{example}



%Интересно может ли быть не прямолинейный отрезок
%\input{pictures/X2}

==> ⥪�騩 ���᪨� ⥪�� (in english)/e_2_5examples.tex <==
\section{Classification of minimizer's local behavior. Examples.} \label{ex}

Recall, that $\Sigma$ is a maximal distance minimizer for a flat compact $M$. We are interested in the behavior of the set $\Sigma$ near $x \in \Sigma$.
 
Usually it is not easy to prove that a certain set is a minimizer. At the figure~\ref{horseFig} the set $M$ is a circle of radius $R > r$. The set $\Sigma$, depicted at the figure is a union of an arc of the circumference of radius $R-r$ and two segments tangent to this circumference. One can find the proof of the fact that $\Sigma$ is a minimizer in the case $R>5r$ in the work~\cite{cherkashin2015horseshoe}.

Note that if $M$ is a finite set of points there is an easy criterion: a connected set $\Sigma$ is a minimizer for a set $M$ and a number $r>0$, if the inequality $\H(\Sigma) \leq \H(St(M))-r \sharp{M}$ holds, where $\sharp{M}$ is a quantity of elements of set $M$, and $St(M)$ is an arbitrary Steiner set for $M$. It is easy to show that strong inequality can not be true. This criterion shows that at Fig.~\ref{X2},~\ref{X1ill},~\ref{X2non120} the set $\Sigma$ is a minimizer. 

Theorems~\ref{mainT1} and~\ref{persp} imply the classification of all possibilities for the local behavior of $\Sigma$. We will give an example for each possible case.

%Из Теорем~\ref{mainT1} и~\ref{persp} следует Теорема о классификации %локального поведения минимайзера в произвольной точке.

\begin{theorem2}

Let $\Sigma$ be a maximal distance minimizer contaning at least two point. Then 
\begin{enumerate}
\item  If $x \in S_\Sigma$, there exists such $\varepsilon > 0$, that $\Sigma \cap B_{\varepsilon}(x)$ coincides with one of two sets: 
\begin{enumerate}
\item a segment %, и в этом случае точка $x$ имеет порядок $2$ 
 (point $S$ at Fig.~\ref{horseFig},~\ref{X2},~\ref{ElimX},~\ref{X1ill},~\ref{X2non120});
\item a regular tripod  %, и в этом случае точка $x$ имеет порядок $3$ 
 (point $F$ at Fig.~\ref{X1ill}).
\end{enumerate} 

 If $x \in X_\Sigma$, there exists such $\varepsilon > 0$ that $\Sigma \cap B_{\varepsilon}(x)$  coincides with one of two sets:
\begin{enumerate}
\item a segment with an end at $x$ (point $D$ at Fig.~\ref{horseFig},~\ref{X2},~\ref{ElimX},~\ref{X1ill},~\ref{X2non120});
\item a union of two segments with common end at $x$ and an angle greater (point $E$ at Fig.~\ref{X2non120}) or equal (point $E$ at Fig.~\ref{X2}) to $2\pi/3$ between them.  
\end{enumerate}
\item  For $x \in E_\Sigma$  there exists such $\varepsilon > 0$ that $\Sigma \cap B_{\varepsilon}(x)$ coincides with one of two sets:
\begin{enumerate}
\item an arc with an end at $x$ having in this point a one-sided tangent line. Herewith $x$ can 
\begin{enumerate}
\item be a limit of points from  $X_\Sigma$ (point $G$ at Fig.~\ref{ElimX});
\item not be a limit of points from $X_\Sigma$ (point $G$ at Fig.~\ref{E1}).
\end{enumerate}

\item a union of two arcs with a common end at the point $x$, having in this point the one-sided tangent lines with angle greater or equal to $2\pi/3$ between them (points $H_1$ and $H_2$ at Fig.~\ref{horseFig} and point $H_2$ at Fig.~\ref{E1}).
\end{enumerate}
\end{enumerate}

\end{theorem2}


\input{e_shortparts/horseshoe}
\input{e_shortparts/X2}
\input{e_shortparts/ElimX}
\input{e_shortparts/X1ill}
\input{e_shortparts/X2non120}
\input{e_shortparts/E1}

Let us give an example of a ``bad'' set $M$:
%Приведем пример ``плохого'' множества $M$:
\begin{example}
Let $M$ be a totally disconnected compact set such that the unique Steiner tree connecting it has an infinite number branching points. An explicit example of such a set was constructed in the work~\cite{paolini2015example}. The results of the announced work imply that for each number $r < \diam M$ the minimizers will contain only a finite number of branching points. 
\end{example}



%Интересно может ли быть не прямолинейный отрезок
%\input{pictures/X2}

==> ⥪�騩 ���᪨� ⥪�� (in english)/parts/1intro.tex <==
\section{Introduction}

For a given compact set $M \subset \mathbb{R}^2$ consider the functional
\[
	F_{M}(\Sigma)\defeq \sup _{y\in M}\dist (y, \Sigma),
\]
where $\Sigma$ is a closed subset of $\R^2$ and $\dist(y, \Sigma)$ stands for the Euclidean distance between $y$ and $\Sigma$ (naturally, $F_{M} (\emptyset) \defeq +\infty$). The quantity $F_M (\Sigma)$ will be called the \emph{energy} of $\Sigma$.
Consider the class of closed connected sets $\Sigma \subset \R^2$ satisfying $F_M(\Sigma) \leq r$ for some $r > 0$. We are interested in the properties of
sets of the minimal length (one-dimensional Hausdorff measure) $\H(\Sigma)$ over the mentioned class. Such sets will be further called \emph{minimizers}. %They can be viewed as the shortest possible
%pipelines arriving at a distance at most $r$ to every point of $M$ which in %this case is considered as the
%set of customers of the pipeline.


%(более общую постановку и детали см. в статье~\cite{mir})
%Доказано (более строгие утверждения и детали стоит смотреть в работе~\cite{mir}), ч
It is known that for all $r>0$ the set  of minimizers is nonempty. It is proven also that for each minimizer of positive length the equality $F_M(\Sigma)=r$ holds. Furthermore the set of minimizers coincides with the set of solutions of the dual problem: minimize $F_M$ over all closed connected sets  $\Sigma \subset \mathbb{R}^2$ with prescribed bound on the total length $\H(\Sigma) \leq l$. Thus the required sets are called maximal distance minimizers.
For the rigorous statements and proofs of these claims, including the general $n$-dimensional case, see~\cite{mir}.

Let $B_\rho (x)$ be the open ball of radius $\rho$ centered at a point $x$, and let $B_\rho(M)$ be the open $\rho$-neighborhood of $M$ i.e.\
	\[
        		B_\rho(M) \defeq \bigcup_{x\in M} B_\rho(x).
	\]
	
It is easy to see that the set $\Sigma$ is bounded (and, thus, compact), since $\Sigma \subset \overline{B_r(\conv M)}$, where $\conv M$ stands for the convex hull of the set $M$. 
 
 \begin{definition}
A point $x \in \Sigma$ is called \emph{energetic}, if for all $\rho>0$ one has
 	\[
		F_{M}(\Sigma \setminus B_{\rho}(x)) > F_{M}(\Sigma).
	\]
\end{definition}
Denote the set of all energetic points of $\Sigma$ by $G_\Sigma$.

Each minimizer $\Sigma$ can be split into three disjoint subsets:
        \[
        \Sigma=E_{\Sigma}\sqcup\X_{\Sigma}\sqcup\S_{\Sigma},
        \]
        where $X_{\Sigma}\subset G_\Sigma$ 
is the set of isolated energetic points 
(i.e.\ every $x\in X_\Sigma$ is energetic and there is a $\rho>0$ possibly depending on $x$ such that $B_{\rho}(x)\cap G_{\Sigma}=\{x\}$), $E_{\Sigma} := G_{\Sigma}\setminus X_{\Sigma}$ is the set of non isolated energetic points and $S_\Sigma \defeq \Sigma \setminus G_\Sigma$ is the set of non energetic points also called the \textit{Steiner part}.
Clearly, the limit points of $G_\Sigma$ belong to $E_\Sigma$.


 In~\cite{mir} (for the plane) and in~\cite{PaoSte04max} (for the general case) the following properties of minimizers have been proven:
        \begin{itemize}
        \item[(a)] A minimizer cannot contain loops (homeomorphic images of circles).
        \label{aaaa}
        \item[(b)] For every point $x \in G_\Sigma$ there exists a point $y \in M$ (may be not unique) such that $\dist (x, y) = r$ and $B_{r}(y)\cap \Sigma=\emptyset$.
         \label{bbbb}
        \item[(c)] For all $x \in S_\Sigma$ there exists an $\varepsilon>0$ such that $S_\Sigma \cap B_{\varepsilon}(x)$ is either a segment or a regular tripod, i.e.\ the union of three segments with an endpoint in $x$ and relative angles of $2\pi/3$. %If a point $x \in S_\Sigma$ is %a center of a regular tripod, then it called a \textit{Steiner %point} (or a \textit{branching point}) of $\Sigma$.
       
        \end{itemize}


Also, since $\Sigma$ is connected closed set of finite length, the following statements hold. 
 	\begin{itemize}
	\item[(d)]
	$\Sigma$ has a tangent line at almost every point of $\Sigma$ % (for the definition see~\ref{diff}).
    \label{e}
    \item[(f)] Set $\Sigma$ is Ahlfors regular, id est there exists such constants $c>0$ and $C>0$ that for every point $x \in \Sigma$ or sufficiently small $\rho>0$  the inequality
    \[
    c\rho \leq \H(\Sigma \cap B_\rho(x))\leq C\rho.
    \]
    \label{j}
   In this work we find exact constants $c$ and $C$ for each point $x$: we will show that \[
   \H(\Sigma \cap B_\rho(x))=\oord_x\Sigma \rho+o(\rho)
   \]
   where $\oord_x\Sigma$ is equal to $1$, $2$ or $3$.
\end{itemize}
%возможно, стоит дать определение.    



The main result of this article is formulated in Theorem~\ref{mainT1}: let $\Sigma$ be a maximal distance minimizer for a compact set $M \subset \mathbb{R}^2$. Then \begin{itemize}
\item[(i)] $\Sigma$ is a union of a finite number of injective images of the segment.
\item[(ii)] The angle between each pair of tangent rays at every point of $\Sigma$ is greater or equal to $2\pi/3$.
\item[(iii)] By (ii) the number of tangent rays at every point of $\Sigma$ is not greater than $3$. If it is equal to $3$, then there exists such a neighbourhood of $x$ that the arcs $\Sigma$ coincide with three line segments and by (ii) the pairwise angles between them are equal to $2\pi/3$. 
\end{itemize}

Theorem~\ref{mainT1} implies that the number of branching points is always finite for each maximal distance minimizer. Note that this is not true for the Steiner problem: an example of Steiner tree with infinite number of branching points can be found in~\cite{paolini2015example}.

We should also mention the problem of minimizing the average distance functional (for more details about this problem, see the survey~\cite {L} and~\cite{lemenant2011regularity}). Maximum and average distance minimizers have a number of similar geometric and topological properties (see~\cite{PaoSte04max}). The finiteness of the number of branching points for the minimizers of the average distance was proved in~\cite{BS1}.

The article actually proved a number of geometric properties of minimizers, but in order not to clutter up the narrative, we will not dwell on them in this work. The article is organized as follows. Section~\ref{stp} contains the statement of the Steiner problem and some technical statements about Steiner trees (the advanced reader can skip this chapter); Chapter~\ref{not} introduces used designations, basic definitions and elementary statements; Chapter~\ref{res} contains the statement and proof of the main result.

%Enjoy reading!

%Оставшаяся часть статьи устроена следующим образом: Раздел~\ref{res} содержит формулировки анонсированных результатов,
%в Разделе~\ref{ex} приводятся все возможные варианты окрестностей $x \in \Sigma$.


==> ⥪�騩 ���᪨� ⥪�� (in english)/parts/1steiner.tex <==
\subsection{Steiner problem} \label{stp}
Let the finite set of points $C \defeq \{ A_1, \dots, A_n \} \subset \R^2$ is given. Then the shortest (having a minimal one-dimensional Hausdorff measure) connected (contained) it set $S\subset \R$ is called a \textit{Steiner tree}. It is known that Steiner tree exists (but may be not unique) and coincides with a finite union of straight segments. So we can identify $S$ with a plane graph whose vertex set contains $ C $ and whose edges are rectilinear. This graph is connected and does not contain cycles, so it is a tree. It is known that the vertices of this graph cannot have degree greater than $ 3 $. Wherein only the vertices $ A_i $ can have degrees $ 1 $ and $ 2 $, the remaining vertices have degrees $ 3 $ and are called \textit{Steiner points} (or \textit{branching points}). Then the number of Steiner vertices does not exceed $ n-2 $. The pairwise angles between edges incident to an arbitrary vertex are at least $ 2 \pi / 3 $.

Thus, a Steiner point has exactly three edges with pairwise angles $ 2 \pi / 3 $. If all vertices $ A_i $ have degree $ 1 $, then the number of Steiner points is equal to $ n-2 $ (the converse is also true) and $ S $ is called a \textit{full} Steiner tree. A set, each connected component of which is a (full) Steiner tree, is called a \textit{(full) Steiner forest}.
For a given three-point set $C=\{A_1, A_2, A_3\}$ Steiner tree is unique and is a
\begin{itemize}
    \item union of two segments $[A_kA_l] \cup [A_lA_m]$, if $\angle A_k A_l A_m \geq 2\pi/3$, where $\angle A_kA_lA_m$ is a maximal angle of the triangle $\triangle A_1A_2A_3$, for $\{k,l,m\}=\{ 1,2,3\}$.  
    \item union of three segments $[A_1F] \cup [A_2F] \cup [A_3F]$ otherwise, where  $F$ is (unique) such point that \[\angle A_1FA_2= \angle A_2FA_3=\angle A_3FA_1=2\pi/3.\]
    %$\angle A_sFA_t = 2\pi/3$ for $\{s,t\} \subset \{1,2,3\}$.
\end{itemize}

The proof of the listed properties of Steiner trees and other interesting information about them one can find in the book~\cite{hwang1992steiner} and in~\cite{gilbert1968steiner}. The problem can also be posed in a more general form: let $ C $ be a compact subset of the metric space, and required set $ S $ has the minimum one-dimensional Hausdorff measure among all sets $ S'$ such that $ S' \cup C $ is connected. In this case, the set $ \bar{S} $ will be called a solution to the Steiner problem and will have some properties. In particular, it is known that $ \bar S $ exists, $ \bar{S} $ does not contain cycles, and $ S \setminus C $ is at most countable union of geodesic curves of a metric space. See~\cite{PaoSte13Steiner} for more details.

%Таким образом для произвольного компакта $C \subset \R^2$ каждая компонента связности решения задачи Штейнера будет являться объединением не более чем счетного числа отрезков, и будет %обладать всеми перечисленными свойствами %дерева Штейнера, кроме конечности числа %отрезков.  
 
Finally, by a \textit{local Steiner forest (tree)} we mean a (connected) compact set $ S $ such that for an arbitrary point $ x \in \Relint (S \setminus C) $ (where $ \Relint $ stands for the relative interior of the set) there exists an open neighborhood $ U \ni x $ such that $ S \cap \overline U $ coincides with the Steiner tree connecting the points $ S \cap \partial U $. A local Steiner tree has the following properties of a Steiner tree: it consists of a countable set of geodesic segments, i.e. in the case of the Euclidean plane, it consists of segments, and the angles between the segments incident to the same point of $ S $ are at least $ 2 \pi / 3 $.

\begin{proposition}
Let $ A $, $ B $ and $ C $ be three different points of the plane such that all angles of the triangle $ \triangle ABC $ are strictly less than $ 2 \pi / 3 $, and the lengths of the sides $ AB $ and $ BC $ are equal $ \varepsilon $. Then 
\[
2 \varepsilon - \H (St (A, B, C)) = d \varepsilon,
\]
where $ St(A, B, C) $ is a Steiner tree for the set $ \{A, B, C \} $ and $ d > 0 $ is a constant depending only on the angles of the triangle $ \triangle ABC $.
\label{angles4}
\end{proposition}

\begin{definition}
We define the ``wind rose'' as six rays from the origin, with an angle $ \pi / 3 $ between any two adjacent ones, equipped with weights (real numbers) that have the following property: the weight on each ray is the sum of the weights of the rays adjacent to it. (From this, in particular, it follows that the weights on opposite (forming a straight line) rays add up to zero.)
\label{roza_v}
\end{definition}
An example is shown in Figure~\ref{fig:roza1}. A similar construction, but for physical reasons, appears in~\cite{gilbert1968steiner}.
%jiocb: мне не очень нравятся слова про физические соображения


\begin{remark}
A full Steiner tree consists of segments belonging to three straight lines with pairwise angles $ \pi / 3 $. Let $ T $ be an arbitrary full Steiner tree. Take an arbitrary wind rose, consisting of rays, parallel to the segments of $ T $, and assign to each end vertex of $ T $ the weight of the ray of this wind rose, co-directed with the segment entering this vertex. Then the sum of numbers over all vertices of $ T $ will be zero.
\label{main_rose_property}
\end{remark}

\begin{remark}
Remark~\ref{main_rose_property} is also true for a local Steiner tree as well as for a full Steiner forest and a local Steiner forest (in the case of forests, multiple wind roses may be required to assign weights to).
\end{remark}


\begin{lemma}
Let $ S $ be a full Steiner forest and  let $ l $ be an arbitrary line such that no connected component of $ S $ is contained in $ l $. Then
\[
\sharp(\partial S \cap l) \leq 2\sharp(\partial S \setminus l),
\]
where $\partial S$ is a vertex set of $S$ 
%В частности, бесконечность левой части неравенства влечет неограниченность правой.
\label{St_l_c}
\end{lemma}

\begin{proof}%[Доказательство Леммы~\ref{St_l_c}:]
Let $ S $ have a finite number of vertices. Let $ l^{+} $, $ l^{-} $ be open half-planes bounded by $ l $. It is easy to see that it is sufficient to separately prove the inequalities for $ \overline {S \cap l^{+}} $, $ \overline {S \cap l^{-}} $. Moreover, it suffices to prove the assertion for one connected component of these sets. Thus, we will prove the assertion for the closure of an arbitrary Steiner tree lying in an open half-plane bounded by $ l $.
We place the center of the wind rose in the same open half-plane, choose a wind rose such that all those and only those rays that intersect $ l $ have a positive weight: obviously, such a wind rose exists, since $ l $ intersect $ 2 $ or $ 3 $ in a row going ray. In the first case, we will equip them with weights $ 1, 2, 1 $, in the second $ 1, 1 $. Then the rest of the rays will have weights $ -1, -2, -1 $ or $ 0, -1, -1, 0 $. Let's assign weights to the leaf vertices in the same way as it was done in Remark~\ref{main_rose_property}. Then the sum over the endpoints of $ l $ is at least $ \sharp (S \cap l) $. Due to Remark~\ref{main_rose_property} the sum over all endpoints must be zero, so endpoints not belonging to $ l $ must be at least $ \frac{\sharp (S \cap l)}{2} $.
Let $ S $ have an infinite number of vertices (but still, by the general statement of Steiner problem, is contained in a compact and has a finite length). Assume the statement opposite to the lemma, that is, that $ \sharp (S \cap l) = \infty $, and $ \sharp (\partial S \setminus l) $, on the contrary, is finite. It suffices to prove the statement for each of the half-planes $ l^{+} $ and $ l^{-} $. Without loss of generality, there is a connected component $ S \cap l^{+} $ such that its closure $ T $ has an infinite number of vertices on $ l $. Let $ l'$ be parallel to $ l $ and contained in $ l^{+} $. We will move the straight line $ l'$ inside this half-plane, parallel to $ l $, and denote by $ S (l') $ the Steiner forest, which is the intersection of $ T $ and the half-plane bounded by $ l'$ and not containing $ l $. %As $\H(T)<\infty$ for almost every such lines $\sharp(T\cap l')<\infty$. But if every 
For an arbitrarily large $ N $, there is $ l_0 $ such that $ N <\sharp (l_0 \cap T) <\infty $. Let's choose this $ l_0 $ for $ N = 3 \sharp (\partial T \setminus l) $. This contradicts the already proven statement for $ S (l_0) $.

\end{proof}

\begin{corollary}
Let $ T $ be a full (that is, having no vertices of degree $ 2 $) Steiner tree, $ l $ an arbitrary line such that $ T \not \subset l $. Then
\[  
\sharp(\partial T \cap l)\leq 2\sharp(\partial T \setminus l).
\]
%
\label{St_l}
\end{corollary}

==> ⥪�騩 ���᪨� ⥪�� (in english)/parts/2notation.tex <==
\section{Notations and definitions}\label {not}
For a given set $X$ the sets $\overline{X}$, $\Int (X)$ and $\partial X$ represent accordingly its closure, interior and boundary.

Let $B$ and $C$ be points. Then $[BC]$, $]BC]$ and $]BC[$ denote closed, semi-closed and open interval accordingly, $[BC)$ and $(BC)$ represent the ray and the line containing these points.

%The angle between the rays, unless otherwise stated, will be assumed to be positive and not exceeding $ \pi $, which uniquely determines its value.  %The angle between three points, unless otherwise stated, belongs to $(-\pi,\pi]$. 
%следить по тексту
The symbol $\angle$, unless otherwise  stated, denotes angle belonging to $[0,\pi]$  for ray and points (or to $[0,-\pi/2]$ for lines). The symbol $\widehat{}$  unless otherwise  stated, denotes order sensitive angle belonging to $(-\pi;\pi]$ for ray and points (or to $[-\pi/2,-\pi/2]$ for lines), where the counterclockwise direction is positive. Both symbols are applicable to two lines, two rays or three points.
%order insensitive
For a (usually finite) set $ M $, the number of elements of the set will be denoted by $ \sharp M $.
\begin{definition}
We say that the order of a point $ x $ in the set $ \Sigma $ is $ n $ (and write $\oord_x \Sigma = n $) if there exists such $ \varepsilon_0 = \varepsilon_0 (x)> 0  $, that for of any open set $ U $ such that $ x \in U $ and $ \diam U < \varepsilon_0 $ the cardinality of the intersection $ \sharp (\partial U \cap \Sigma) $ is at least $ n $, and for any $ \varepsilon <\varepsilon_0 $ there is an open set $ V \ni x $ with $ \diam V <\varepsilon $ and $ \sharp (\partial V \cap \Sigma) = n $.
\end{definition}
%что-то человечество другой объект называет порядком точки(( что делать? 


Note that, since $ \Sigma $ is connected, for any point $ x \in \Sigma $, the order $ \oord_x \Sigma> 0 $ (if $ \Sigma $ contains more than one point).
%, а ввиду конечности длины $\Sigma$ --- ограниченный, то есть $0 <\oord_x \Sigma < \infty$ для любой точки $x \in \Sigma$. (это неверно, так как априори может быть \infty).

\begin{definition}
We say that $ \oordball_x \Sigma = n $ (the circular order $\oordball_x \Sigma $ of the point $ x $ in the set $ \Sigma $ is $ n $) if there exists $ \varepsilon_0> 0 $ such that for any $ \delta <\varepsilon_0 $ the inequality $ \sharp (\partial B_\delta (x) \cap \Sigma) \geq n $ holds, and for any $ \varepsilon <\varepsilon_0 $ there is such $ \eta <\varepsilon $ that $ \sharp (\partial B_{\eta} (x) \cap \Sigma) = n $.
\end{definition}

\begin{remark}
The inequality $\oordball_x \Sigma \geq \oord_x \Sigma$ holds.
\label{rem_ord}
\end{remark}

\begin{proof}
Suppose the opposite:
\[
k \defeq \oordball_x \Sigma  < n \defeq \oord_x \Sigma. 
\]
Then in view of the definition of $\oord$,
\[
\exists \varepsilon_0: \forall U\ni x: \diam U <\varepsilon_0 \quad \sharp (\partial U \cap \Sigma) \geq n
\]
Thus for each $\delta<\frac {\varepsilon_0} 2$ holds
\[
 \sharp (\partial B_{\delta}(x) \cap \Sigma) \geq n.
\]
But on the other hand, in view of the definition of $\oordball$, there exists such $\delta_0<\varepsilon_0/2$, that 
\[
 \sharp (\partial B_{\delta_0}(x) \cap \Sigma) =k<n.
\]
We got a contradiction.
\end{proof}

\begin{remark}
For every $x\in \Sigma$ the inequality $\oord_x\Sigma \leq \oordball_x\Sigma\leq 2\pi<7$ holds due to coarea inequality. Otherwise the set $\Sigma \setminus B_\varepsilon(x) \cup \partial B_\varepsilon(x)$ for sufficiently small $\varepsilon >0$ is better than $\Sigma$: it has not greater energy and strictly less length than $\Sigma$, and is still connected, so we have a contradiction with optimality of $\Sigma$.
\end{remark}

\begin{definition}
The \textit{arc} $ \breve {[ax]} \subset \Sigma $ ($\breve {]ax]}$ or $\breve {]ax[}$) 
 is the continuous injective image of the closed (semi-closed or open, respectively) interval. If inclusion and exclusion of the ends of the arc don't matter we will write $\breve{ax}$.

\end{definition}

\begin{definition}
We say that the ray $ (ax] $ is the \textit{tangent ray} of the set $ \Sigma $ with a vertex at the point $ x\in \Sigma $ (or shortly \textit{of $\Sigma$ at $x$}) if there exists non  stabilized sequence of points $ x_k \in \Sigma $ such that $ x_k \rightarrow x $ and $ \angle x_kxa \rightarrow 0 $.
Sometimes, instead of converging angles, it will be more convenient for us to write convergence of rays: $ (x_k x] \rightarrow (a x] $.
\end{definition}


%\color{red}
Let's repeat the key definitions already introduced in the previous section.
 \begin{definition}
A point $x \in \Sigma$ is called \emph{energetic}, if for all $\rho>0$ one has
 	\[
		F_{M}(\Sigma \setminus B_{\rho}(x)) > F_{M}(\Sigma)
	\]
	where 
	\[
		F_{M}(\Sigma)\defeq \sup _{y\in M}\dist (y, \Sigma).
	\]
\end{definition}
The set of all energetic points of $\Sigma$ is denoted by $G_\Sigma$.

Each minimizer $\Sigma$ can be split into three disjoint subsets:
        \[
        \Sigma=E_{\Sigma}\sqcup\X_{\Sigma}\sqcup\S_{\Sigma},
        \]
        where $X_{\Sigma}\subset G_\Sigma$ 
is the set of isolated energetic points 
(i.e. every $x\in X_\Sigma$ is energetic and there is a $\rho>0$ possibly depending on $x$ such that $B_{\rho}(x)\cap G_{\Sigma}=\{x\}$), $E_{\Sigma} := G_{\Sigma}\setminus X_{\Sigma}$ is the set of non isolated energetic points and $S_\Sigma \defeq \Sigma \setminus G_\Sigma$ is the set of non energetic points also called the \textit{Steiner part}.


 For every point $x \in G_\Sigma$ there exists a point $y \in M$ (may be not unique) such that $\dist (x, y) = r$ and $B_{r}(y)\cap \Sigma=\emptyset$. 
 %если оставить тут эту фразу то внизу надо убрать as we said in the introduction
 %и может быть как-то описать что это важное свойство чтобы потом к нему обращаться
 %We will call this property of energetic points -- basic.
 We will refer to this property as \textit{basic property of energetic points}.
 
\begin{remark}
Due to the definition of energetic points for each non energetic point $x$ there exists such $\rho>0$ that $\overline{B_\rho(x) \cap \Sigma}$ is a Steiner forest %with all terminal points (id est points of order $1$) belonging to 
with $C \subset \partial B_\rho(x)$. Thus there exists such $\varepsilon>0$ that $\overline{B_\varepsilon(x) \cap \Sigma}$ is a segment or a regular tripod centered at $x$, in the case of a tripod we will call $x$ a  \textit{branching} (or Steiner) point. So  for each non energetic point $x$ there exists such $\rho_1>0$ that $\overline{B_\rho(x) \cap \Sigma}$ is a Steiner tree.
%Each non energetic point $x$ has such a neighborhood that its intersection with $\Sigma$ is a Steiner tree for points at the border of the neighborhood: the such neighborhood is suitable that separates the connected component containing $x$ in the ball $B_\rho(x)$ not change the energy (such ball exists by the definition of an energetic point): $F_M(\Sigma)=F_{M\setminus B_{\rho}x)}$. Thus, in view of Steiner trees' properties, for each non energetic point $x$ there exists such open neighborhood $U_x\ni x$ that $\Sigma \cap U_x$ is a segment or a regular tripod with $x$ at the center of it in the both cases, in the case of a tripod we will call $x$ a  \textit{branching} (or Steiner) point. Thereby $S_\Sigma$ is a local Steiner forest (for some set of points $C\subset \Sigma$) and satisfies all its properties listed at the section\ref{stp}. All ends points of $C \cup S_\Sigma$ belong to $G_\Sigma$
\label{stpt}
\end{remark}
%\color{black}

\begin{definition}
We say that a ray $ (ax] $ is the \textit{energetic ray} of the set $ \Sigma $ with a vertex at the point $ x\in \Sigma $ if there exists non  stabilized sequence of energetic points $ x_k \in G_\Sigma $ such that $ x_k \rightarrow x $ and $ \angle x_kxa \rightarrow 0 $.
%\color{red}
%energetic edge?
%\color{black}

\end{definition}


\begin{remark}
A point $x \in \Sigma$ belongs to the set of non isolated energetic points $E_\Sigma$ iff there exists an energetic ray with vertex at $x$.
\end{remark}

\begin{remark}
Each energetic ray is also a tangent ray.
\end{remark}

\begin{remark}
Let $\{x_k\} \subset G_\Sigma$ and let $x\in E_\Sigma$ be the limit point of $\{x_k\}$:  $x_k \rightarrow x$.
By basic property of energetic points for every point $x_k \in G_\Sigma$ there exists a point $y_k \in M$ (may be not unique) such that $\dist (x_k, y_k) = r$ and $B_{r}(y_k)\cap \Sigma=\emptyset$. In this case we will say that $y_k$ \textit{corresponds} to $x_k$.

Let $y$ be an arbitrary limit point of the set $\{y_k\}$. Then the following statements are true:

\begin{enumerate}
\item Set $\Sigma$ doesn't intersect $r$-neighbourhood of $y$: $B_r(y) \cap \Sigma =\emptyset$. The point $y$ belongs to $M$ and corresponds to $x$.   
\item Let $(zx)$ be orthogonal to $(xy)$. Then it contains the energetic ray of $\Sigma$ with a vertex at $x$. 

Without loss of generality let $(zx]$ be energetic ray.
\item Let us define an \textit{orientation} (clockwise or counterclockwise) of $(zx]$ such way that the orientated angle in this direction from $(zx]$ to $(yx]$ is equal to $\pi/2$.
 \label{orientation}

%вместо orientation использовать излучение? emit, radiate или свечение?
It is easy to notice that then the orientated angle in this direction from $(zx]$ to another energetic ray (if it exists) with a vertex at $x$, is not less than $\pi$.

\item Let $x \in E_\Sigma$. Then there exists one or two energetic ray with vertex at $x$.
\label{netri}
\item
One energetic ray $(zx]$ can have two orientations (we say that it is orientated in the both directions or two-orientated) if there exist two different limit points of $y_k$, where $y_k$ corresponds to $x_k$. Otherwise it is one-orientated.

%лишнее же?
\item In the case of two-orientated $(zx]$ each energetic ray is perpendicular to the line, connecting the limit points of $y_k$. 
The angle between $(zx]$ and another energetic ray (if it exists) is equal to $\pi$. 

\end{enumerate}
\label{emptyball}
\end{remark}


\begin{definition}
We say that the line $ (ax) $ is the \textit{tangent line} of the set $ \Sigma $  at the point $ x\in \Sigma $ if for each non  stabilized sequence of points $ x_k \in \Sigma $ such that $ x_k \rightarrow x $ holds $\angle ((x_kx),(ax)) \rightarrow 0$. 
\end{definition}

\begin{definition}
We say that the ray $ (ax] $ is a \textit{one-sided tangent} of the set $ \Sigma $ at the point $ x\in \Sigma $ if there exists such a connected component of $\Sigma \setminus \{x\}$, let us call it $\Sigma'$, that  for each non  stabilized sequence of points $ x_k \in \Sigma' $ such that $ x_k \rightarrow x $ holds $ \angle x_kxa \rightarrow 0 $. 
%if there exists an arc $\breve{wx} \subset \Sigma$ such that $(ax)$ is a tangent line to $\breve{wx}$ with a vertex at the point $x$. Может надо чет такое дописать, что иногда интересует односторонние касательные дуг
\end{definition}

\begin{remark}
If there exists a tangent line of the set $\Sigma$ at the point $x$ then there also exists a one-sided tangent of $\Sigma$ at $x$, but not vice versa. If there exists a one-sided tangent of the set $\Sigma$ at the point $x$ then there exists also a tangent ray of $\Sigma$ at $x$, but not vice versa.
\end{remark}

%------------лось дочитал до сюдыма-----------------

\color{black}

\begin{definition}
We will write $f(\rho)=o_\rho(1)$ if and only if $f(\rho)\rightarrow 0$ as $\rho \rightarrow 0$.
\end{definition}

\begin{definition}
For a given ray $(ax]$ and a number $\rho>0$ we will denote by a set of \textit{cusps}  $\mathbb{Q}_{\rho}^{a,x}$ the set consisting of such 
closed simply connected sets that $\forall Q \in \mathbb{Q}_{\rho}^{a,x}$ the following statements hold: %ТОЧНО ЛИ ЛИШНИЕ НЕ ПОДХОДЯТ?
\begin{itemize}
    \item $Q \subset \overline{B_{\rho}(x)}$;
    \item $Q \cap \partial B_{\rho'}(x)$ for each $0<\rho'\leq \rho$ is an arc (actually it is sufficient to state it only for $\rho'=\rho$)
    \item $(ax] \cap \overline{B_{\rho}(x)} \subset Q$;
    \item for an arbitrary sequence of points $z_k \in Q$ converging to $x$ holds $\angle z_k x a \rightarrow 0$.
The ray $(ax]$ will be called the \textit{axis of cusp $Q$}.
%    \item for each point $z \in \partial Q \setminus \partial B_{\rho}(x)$ holds $[zx]\cap \Int(Q)=\emptyset$ (actually  this item is overabundant and follows from the previous).

%надо бы использовать слово ващет 
%биссектриса псевдоконуса тоже такое себе. я бы скорее ось предлагал
\end{itemize}
\end{definition}

\begin{remark}
Let $x\in E_\Sigma$ has a two-orientated energetic ray (id est there exists an energetic ray $(ix]$ orientated in the both directions). Then
\begin{enumerate}
    \item There exist two points $y_1, y_2 \in M$ such that  $\Sigma \cap B_r(y_1)=\Sigma \cap B_r(y_2) =\emptyset$, $|y_1x|=|y_2x|=r$, $x \in [y_1y_2]$ and $(ix) \perp (y_1y_2)$.
    \item For a sufficiently small $\rho>0$ there exist two cusps which union contains $\Sigma \cap B_\rho(x)$. One cusp is from set $Q^{i,x}_\rho$ and another one --- from set of cusps with axis, complementing ray $(ix]$ to line (ix). For example it can be the closures of the connected components of the set \[ \overline{B_\rho(x)}\setminus B_r(y_1) \setminus B_r(y_2) \setminus \{x\}.\]
    \item There is exactly one or two tangent rays of $\Sigma$ at $x$. If two then both of them should be contained in $(ix)$ (note that in this case there still can be only one energetic ray of $\Sigma$ at $x$). Anyway $\Sigma$ has a tangent line at the point $x$. 
    %\color{green} 
    %\item Если $\Sigma$ (или компонента связности $\Sigma \setminus x$)  имеет в точке $x$ кривизну, то она по модулю не превосходит $1/r$. %в этой статье не нужно, нужно в другой
\color{black}
\end{enumerate}

\label{star}
\end{remark}

\begin{lemma}
\begin{enumerate}
\item Let a set $W\ni x$ has tangent line $(ax)$ and moreover for each non  stabilized sequence of points $ x_k \in W$ such that $ x_k \rightarrow x $ holds $ \angle x_kxa \rightarrow 0 $. . Then for sufficiently small $\varepsilon>0$ there exists such cusp  $Q \in \mathbb{Q}_\varepsilon^{a,x}$ that $(W \cap \overline{B_\varepsilon(x)})\subset Q$ and $(W \cap \partial Q) \subset (\partial B_\varepsilon(x) \cup \{x\})$.
\label{kas} %$\breve{[Wx]}$
\item Let $\Sigma$ at point $x$ has exactly one energetic ray $(ax]$. Then for sufficiently small $\varepsilon>0$ there exists such cusp $Q \in \mathbb{Q}_\varepsilon^{a,x}$ that $G_\Sigma \cap  \overline{B_\varepsilon(x)} \subset Q$.
\label{en}
\item Let $\Sigma$ at point $x$ has two energetic rays $(ax]$ and $(bx]$.  
Then for sufficiently small $\varepsilon>0$ there exist such cusps $Q^a \in \mathbb{Q}_\varepsilon^{a,x}$ and $Q^b \in \mathbb{Q}_\varepsilon^{b,x}$, that  $(G_\Sigma \cap  \overline{B_\varepsilon(x)}) \subset Q^{a} \cup Q^{b}$.
\label{reb}
\item For each  $x\in E_\Sigma$ $\rho>0$ there exist such $\beta(\rho)>0$ that all energetic points from the ball $B_{\rho}(x)$ belong to the corner with opening $\beta(\rho)$ and with some energetic ray $(ax]$ as a bisector, where $\beta=o_\rho(1)$. Also it is easy to note that in view of compactness $E_\Sigma$ the value $\beta(\rho)$ doesn't depend on $x$.

 \label{BB}
%\item Для любого $\beta>0$ и для любой $x \in E_\Sigma$, найдется %такое $\rho(\beta)>0$, что все энергетические точки из шара %$B_{\rho(\beta)}(x)$ лежат в углу с раствором $\beta$ и с %каким-то энергетическим ребром с концом в $x$ в качестве %биссектрисы. Причем $\rho(\beta)=o_\beta(1)$.
% \label{BB}
\end{enumerate}
\label{con}
\end{lemma}
\begin{proof}
%монотонно = строго?
The proof of item~\ref{kas}. The existence of a one-sided tangent implies that there exists strictly decreasing sequence $r_k\rightarrow 0$ and non strictly decreasing sequence $s_k \rightarrow 0$ such that
\[
\forall z \in B_{\rho_k}(x) \cap W \text{ holds } \angle zxa <s_k.
\]
%В противном случае нашлось бы такое $s>0$
Denote 
\[
Q(\rho,s,x,a) \defeq \{z \big| |zx|\leq \rho, \angle zxa \leq s\}.
\]
Then the set \[
\bigcup_{k=1}^{\infty} \left(Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) \right)
\]
belongs to $\mathbb{Q}_{\rho_1}^{a,x}$.
%будет удовлетворять всем требованиям к псевдоконусу.
The proof of item~\ref{en}. As there exits only one energetic ray at point $x$ for sufficiently small  $\varepsilon>0$ the line $(ax]$ is a tangent line for the set $G_\Sigma \cap B_\varepsilon(x)$ and the condition on item~\ref{kas} holds and condition of the statement~\ref{kas} holds. Then the previous item implies the statement.

The proof of item~\ref{reb} is similar and also follow from the definition of an energetic ray and item~\ref{kas}. 
The last item~\ref{BB} follows from remark~\ref{emptyball} item~\ref{netri},  items~\ref{en} and~\ref{reb} of this lemma and from the definition of cusps. 
\end{proof}

\begin{definition}
In the notations of the item~\ref{reb} of Lemma~\ref{con} an energetic point $\bar x$ from the set $G_\Sigma \cap Q^i$ will be called \textit{the energetic point of the energetic ray (ix]}, where $i=\{a,b\}$. In this case the ray $(ix]$ will be called \textit{the energetic ray, closest to $\bar x$}.
This definition doesn't depend of chosen cusps and have sense only in the neighbourhood of $x$. 
\end{definition}
\begin{lemma}
Let the intersection of a connected component of $\Sigma\setminus \{ x\}$ with the sufficiently small closed neighbourhood of $x$ be an arc and contain infinitely many energetic points of the energetic ray $(ix]$ and do not contain another energetic points. Then there exists a cusp with $(ix]$ as an axis, which contains this arc.
%или все же лучше шарик оставить и обозначения
%видимо шарик потому что важна инфа про границы(( кажется
\label{dug_ok}
\end{lemma}
\begin{proof}
For sufficiently small $\rho>0$ the intersection of the connected  component of $\Sigma\setminus \{ x\}$ with a ball $\overline{B_\rho(x)}$ is an arc. Denote this arc by $\breve{[sx]}$. Let an injective function $f: [0;1] \rightarrow \R^2$ parameterizes the arc $\breve{[sx]}$. By the definition of an energetic ray the ray $(ix]$ is a one-sided tangent for the set $\breve{[sx]} \cap G_\Sigma$. I.e. for each sequence of energetic points  $\{g_j\}_{j=1}^\infty \subset \breve{[sx]} \cap G_\Sigma$ converging to $x$ the sequence of angles with the energetic ray $\angle g_jxi$ converges to $0$. But as energetic points forms a closed set, for each nonenergetic point $z \in \breve{[sx]}\setminus G_\Sigma$ there exists  such $c,d \in [0,1]$ that  $f(c),f(d) \in \breve{[sx]}  \cap G_\Sigma$, $f((c,d))\ni z$ and $f((c,d)) \subset \breve{[sx]}\setminus G_\Sigma$. Then the arc $f([c,d])$ should be a line segment. Thus $\angle zxi \leq \max (\angle f(c)xi, \angle f(d)xi)$.
So for each sequence of points $\breve{[sx]}$ converging to $x$ there exists the sequence of energetic points  $\breve{[sx]}$ converging to $x$  with larger angles with $(ix]$, still converging to $0$. Thus $(ix]$ is one-sided tangent for the whole $\breve{[sx]}$. Applying of the item~\ref{kas} Lemma~\ref{con} completes the proof.
%тут изменилось доказательство. Стало оно лучше или хуже? Понятное ли оно? Может надо расписать это или вернуть старое?




%Пусть инъективная функция $f: [0;1] \rightarrow \R^2$ параметризует $\breve{[sx]}$. Несложно заметить, что множество $\breve{[sx]} \cap G_\Sigma$ содержится в псевдоконусе $Q \in \mathbb{Q}_{\rho}^{i,x}$ следующего вида \[Q \defeq \bigcup_{k=1}^{\infty} \left( Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) \right)\] для некоторых сходящихся к нулю монотонных последовательностей неотрицательных чисел $\{s_k\}$ и $\{\rho_k\}$, где $\rho_1=\rho$. Будем считать выбранные последовательности минимальными по включению. Пусть точки $c,d \in [0;1]$ такие, что $f([c,d])\cap G_\Sigma=f(c) \cup f(d)$. Тогда, ввиду отсутствия на дуге $\breve{[sx]}$ точек ветвления, выполняется $f([c,d])=[f(c),f(d)]$. В таком случае, если $f(c) \in Q(\rho_{k-1},s_{k-1},x,i) \setminus B_{\rho_{k}}(x) $, $f(d) \in Q(\rho_k,s_k,x,i) \setminus B_{\rho_{k+1}}(x) $, то выполняется $[f(c);f(d)] \subset  Q(\rho_{k-1},s_{k-1},x,a) \setminus B_{\rho_{k+1}}(x)$. А значит, 
%\[
%\breve{[sx]}=f([0;1]) \subset Q' \defeq \bigcup_{k=1}^{\infty} \left(Q(\rho_k,s_k,x,i) \setminus B_{\rho_{k+2}}(x) \right).
%\]
\end{proof}

% Нужно ли написать что такое угол между прямыми?
\begin{definition}
Let $M$ be a planar compact set. A connected set $\Sigma$ is called \textit{local minimizer} if $M \subset \overline{B_r(\Sigma)}$ and there exists an $\varepsilon >0$ such that for every connected $\Sigma_0$ such that $M \subset \overline{B_r(\Sigma_0)}$ and $\diam (\Sigma \triangle \Sigma_0) \leq \varepsilon$ one has $\H(\Sigma) \leq \H(\Sigma_0)$.
\end{definition}
\begin{remark}
As far as all arguments are local all statements of this work are true not only for maximal distance minimizers but also for local minimizers. 
\label{lcl}
\end{remark}


==> ⥪�騩 ���᪨� ⥪�� (in english)/parts/3results.tex <==
\section{Results} \label{res}

It is known (see~\cite{kuratowski2014topology}) that as $\Sigma$ has a finite length then the following lemma holds:
%потеряля теорему(  вот книжка вроде https://b-ok.cc/book/2367794/ca7b47
%поменяла формулировку леммы, надо проверить, осталась ли она верной
%\color{black}

%Поскольку множество $\Sigma$ имеет конечную длину, оно обладает свойством локальной (дугообразной) связности (см.~\cite{kuratowski2014topology}). 
%А значит, выполняется следующая лемма:

\begin{lemma}
Let the order of a point $ x $ in the set $ \Sigma $ is $ n $. Then for a sufficiently small $\varepsilon=\varepsilon(x) > 0$ the set $\Sigma \cap B_\varepsilon (x)$ contains $n$ arcs with one end at $\partial B_\varepsilon(x)$ and another at the $x$ intersecting only at the point $x$.
\label{ord_arcs}
\end{lemma}

In this work it is proved that $\Sigma \cap B_\varepsilon (x)$ coincides with these arcs. %Now then the main result of this work.

\subsection{The main theorem}

\begin{theorem2}
Let $\Sigma$ be a maximal distance minimizer for a compact set $M \subset \mathbb{R}^2$. Then \begin{itemize}
\item[(i)] $\Sigma$ is a union of a finite number of arcs (injective images of the segment $[0;1]$).
\item[(ii)] The angle between each pair of tangent rays at every point of $\Sigma$ is greater or equal to $2\pi/3$.
\item[(iii)] By (ii) the number of tangent rays at every point of $\Sigma$ is not greater than $3$. If it is equal to $3$, then there exists such a neighbourhood of $x$ that the arcs in it coincide with line segments and by (ii) the pairwise angles between them are equal to $2\pi/3$. 
\end{itemize}
\label{mainT1}
\end{theorem2}

%Such point is called a \textit{Steiner point} (or a \textit{branching point}) of $\Sigma$.
%надо бы не забыть их определить!

\begin{proof}
Let $U\ni x$ be such a sufficiently small domain that
\[
\sharp (\partial U \cap \Sigma)=\oord_x\Sigma.  
\]
During the proof we will impose new restrictions on $U$ and it may be changed to the smaller one. Let $\Sigma'$ be a closure of a connected component of  $\Sigma \cap U \setminus \{x\}$. In view of the Corollary~\ref{oord_en} the number of such components is no more than three. Each component contains a point $x$ and certainly one point at the border $\partial U$. Without loss of generality the neighbourhood $U$ could be considered such small that every connected component of  $\Sigma \cap U \setminus \{x\}$ either doesn't contain any energetic points or contains infinitely many of them.  

If $\Sigma'$ doesn't contain any energetic points except $x$ then, in view of the Remark~\ref{stpt}, it is a line segment connecting $x$ with a point at the $\partial U$.

Let $\Sigma'$ contains infinitely many energetic points. Then for sufficiently small $U$ in view of the key Lemma~\ref{eva} all these energetic points are of the same energetic ray, denote it by $(ix]$. Thus in view of Lemma~\ref{uggi} it should be an arc and by Lemma~\ref{dug_ok} should be contained in some cusp with $(ix]$ as an axis. 

Then each connected component $\Sigma \cap U \setminus \{ x\}$ has one-sided tangent at the point $x$. Wherein, by the Lemma~\ref{angles2}, angles between these one-sided tangent is larger or equal $2\pi/3$. Then, if $x$ is an energetic point, there exist only one or two connected components   $\Sigma \cap U \setminus \{x\}$ (see~\ref{star} item~\ref{orientation}). In total, the set $\Sigma \cap U $ is one of three sets:
\begin{itemize}
    \item  A union of three line segments with one end at $x$ and another at $\partial U$, with pairwise angle $2\pi/3$ at the point $x$ (a regular tripod with center at $x$). 
    \item An arc with both ends at $\partial U$, which has two one-sided tangents at $x$, with angle greater or equal to $2\pi/3$ between them.
    % union of two arcs with one end at $x$ and another at $\partial U$, both having one-sided tangent at $x$, with angle greater or equal to $2\pi/3$ between it.
    \item  An arc, connecting $x$ and $\partial U$, having one-sided tangent at $x$
\end{itemize}
The theorem is proved as $\Sigma$ is a compact set. 
\end{proof}
\begin{corollary}
Let $\Sigma$ be a local minimizer for a compact set $M \subset \mathbb{R}^2$. Then, in view of remark~\ref{lcl}, if  \begin{itemize}
\item[(i)] $\Sigma$ is a union of a finite number of arcs (injective images of the segment $[0;1]$).
\item[(ii)] The angle between each pair of tangent rays at every point of $\Sigma$ is greater or equal to $2\pi/3$.
\item[(iii)] By (ii) the number of tangent rays at every point of $\Sigma$ is not greater than $3$. If it is equal to $3$, then there exists such a neighbourhood of $x$ that the arcs in it coincide with line segments and by (ii) the pairwise angles between them are equal to $2\pi/3$. 
\end{itemize}
\end{corollary}

We now turn to statements used in the proof of the theorem.

\subsection{Lemmas}
\begin{lemma}
Let $\Sigma$ have two one-sided tangents at $x$. Then the angle between these rays are at least $2\pi/3$. In particular they can not coincide.
\label{angles2}
\end{lemma} 

\begin{proof}
At first we need the following statements:
\begin{enumerate}
\item For a given $r>0$ and an arbitrary segment $[uv]$ of sufficiently small length $\varepsilon>0$ there exists such set $S^{uv}$ that  $|\H(S^{uv})|=o(\varepsilon)$ and $\overline {B_r([uv])} \subset \overline{B_r(S^{uv})}$. Moreover, $S^{uv}=S^u \cup S^v$, where $w\in S^w$ and $S^w$ is connected, with $w\in \{u,v\}$.   
\begin{proof}
Let $C$ be a point equidistant from $u$ and $v$, located at a distance of $r$ from the straight line $(uv)$. And let $C_w$ be such points that $C_w \in [wC]$ and $|C_wC|=r$ with $w\in \{u,v\}$. In addition let the points $C_u^-$ and $C_v^-$ be symmetric reflections of the points $C_u$ and $C_v$ with respect to the line $(uv)$ (see Fig.~\ref{Suv}).
 \input{pictures/Suv}
Then we can define $S^u \defeq [uC_u] \cup [uC_u^-]$ and $S^v \defeq [vC_v] \cup [vC_v^-]$. It is easy to see that these sets meet all conditions.
\end{proof}
\item For an arbitrary cusp $Q\in Q_\varepsilon^{a,x}$ there exists such a set $S^Q$ that $|\H(S^Q)|=o(\varepsilon)$ and $\overline{B_r(Q)} \subset \overline{B_r(S^Q)}$. Moreover, $S^Q=S_1 \cup S_2$, where $S_1 \supset (\partial Q \cap \partial B_\varepsilon(x))$, $x \in S_2$ and both $S^1$ and $S^2$ are connected (see Fig.~\ref{TQ}).%потом скажу
\begin{proof}
Let points $T_1, T_2 \in \partial B_\varepsilon(x)$ be such that $\angle T_1xa = \max_{z\in Q} \angle zxa$ and $T_2$ be a reflection of $T_1$ with respect to $(ax)$. And let $\breve{T_1T_2}$ be the smallest arc of the $\partial B_\varepsilon(x)$. Then, since $ Q $ lies in the figure bounded by $ \breve {T_1T_2} \cup [T_1x] \cup [T_2x] $ the following statement is true:  
\[
\overline{B_r(Q)} \subset \overline{B_r(\breve{T_1T_2}\cup [T_1x] \cup [T_2x])}.
\]
It is easy to see that the set
\[
S^Q \defeq \breve{T_1T_2} \cup S^{T_1x} \cup S^{T_2x}
\]
meets all requirements.
\end{proof}
 \item For a cusp $Q\in Q_\varepsilon^{a,x}$ there exists such connected set $T^Q$ that $|\H(T^Q)|=\varepsilon+o(\varepsilon)$, $\overline{B_r(Q)} \subset \overline{B_r(T^Q)}$ and $T \supset ((\partial Q \cap \partial B_\varepsilon(x)) \cup \{x\})$ (see Fig.~\ref{TQ}).
 \begin{proof}
 In the notations of the previous item let us define $Z \defeq (ax] \cap \partial B_\varepsilon(x)$. Then the set 
 \[
 T^Q \defeq S^Q \cup [Zx].
 \]
 \end{proof}
meets all requirements.
\end{enumerate}

\begin{figure}
\center{\includegraphics[width=0.4\linewidth]{pictures/Suv-1}}
\caption{Construction of the sets $S^Q$, $T^Q$.}
\label{TQ}
\end{figure}

In view of Lemma~\ref{con} i.~\ref{kas} there exists such $\varepsilon_0>0$, %что компонента связности $W_i$ содержится в псевдоконусе
%(не умаляя общности $\varepsilon_0 \leq \varepsilon_1$),
that for an arbitrary $\varepsilon<\varepsilon_0$ inside the ball $B_\varepsilon(x)$ each of these two components lie inside a cusp with its one-sided tangent as an axis.  
Define the closures of intersections of connected components with $B_\varepsilon(x)$ by $W_1$ and $W_2$. Clearly 
\[
\H(W_i)\geq \varepsilon
\]
for $i=\{1,2\}$.

Assume that these two connected components have the same one-sided tangent $(ax]$. Then in view of i.~\ref{kas} Lemma~\ref{con} for $W=W_1 \cup W_2$ there exists such containing them cusp $Q \in  Q_\varepsilon^{a,x}$ such that $\partial Q \cap (W_1 \cup W_2) \subset \partial B_\varepsilon(x)$.

Then the set 
\[
\Sigma \setminus (W_1 \cup W_2) \cup T^Q
\]
is better than $\Sigma$: it is connected, has a shorter length and not larger energy than $\Sigma$. This contradicts the assumption that two connected components can have the same one-sided tangent line.

Let us now show that the angle between one-sided tangents is at least $ 2 \pi / 3 $. Assume the opposite, that is, that the angle between the one-sided tangents $ (ax] $ and $ (bx] $ (of respectively $W_1$ and $W_2$) is strictly less than $ 2 \pi / 3 $. Denote $A \defeq (ax] \cap \partial B_\varepsilon(x)$ and $B \defeq (bx] \cap  \partial B_\varepsilon(x)$. Then, by Proposition~\ref{angles4}, the set
\[
\Sigma \setminus (W_1 \cup W_2) \cup S^{Q_a}\cup S^{Q_b} \cup St(A,B,x)
\]
is connected, has a shorter length and not larger energy than $\Sigma$. Contradiction.


\end{proof}
\begin{corollary}
Let $\Sigma \setminus x$ have one-sided tangent $(ax]$. Then for sufficiently small $\varepsilon>0$ the statement $\H(W \cap B_\varepsilon(x))=\varepsilon+o(\varepsilon)$ holds, where $W$ is a closure of connected component of $\Sigma \setminus \{ x\}$. As in other case the set $\Sigma \setminus (B_\varepsilon(x) \cap W) \cup T^Q$ for some containing $B_\varepsilon(x)\cap W$ cusp $Q\in Q^{a,x}_\varepsilon$ is better than $\Sigma$: it is connected, has a shorter length and not larger energy than $\Sigma$. A contradiction.
\label{len0}
\end{corollary}

%\begin{corollary}
%В условиях замечания~\ref{star} найдется $\varepsilon>0$ такое, что $B_\varepsilon(x) \cap \Sigma$ является дугой (либо лежащей в одном псевдоконусе, либо в объединении двух псевдоконусов с осями, образующими прямую).
%\end{corollary}
%Следующее утверждение показывает регулярность $\Sigma$ в окрестности любой точки из $x$ из $\Sigma \setminus E_\Sigma$.

\begin{proposition}
For an arbitrary point $x\in S_\Sigma \sqcup X_\Sigma$ there exists such $\varepsilon=\varepsilon(x)>0$ that the set $ \Sigma \cap B_\varepsilon (x) $ consists of $ \oord_x \Sigma $ line segments with one end at $ x $ and another one at $\partial B_\varepsilon(x)$, with pairwise angles between them at least $ 2 \pi / 3 $. Moreover, in the case of $ x \in S_ \Sigma $, the set $ \overline{B_\varepsilon (x)} \cap \Sigma $ is a segment or a regular tripod centered at $ x $, and in the case of $ x \in X_\Sigma $ --- a segment with an end at $ x $ and another one at $\partial B_\varepsilon(x)$, or the union of two segments with one end at $ x $ and another one at $\partial B_\varepsilon(x)$, with angle at least $ 2 \pi / 3 $ between them.


\label{discr_str}
\end{proposition}

\begin{proof}
It is easy to see that for each $x \in \Sigma$ the inequality $\oordball_x \Sigma \leq 6$ holds. Assume the contrary, then for sufficiently small $\varepsilon>0$ the co-area inequality entails $\H(\Sigma \cap \overline{B_\varepsilon (x)}) \geq 7 \varepsilon$. But then the set $\Sigma' \defeq \Sigma \setminus B_\varepsilon(x) \cup \partial B_\varepsilon(x)$ is better than $\Sigma$: it is connected, its energy is not greater and its length is strictly less than of $\Sigma$. This gives a contradiction with the optimality of $\Sigma$.

Now let $x \in S_\Sigma \sqcup X_\Sigma$ and let $\varepsilon>0$ be such that $\Sigma \cap \overline{B_\varepsilon(x)} \setminus \{x\} \subset S_\Sigma$. Thus, there exists an infinite monotonically decreasing sequence $\varepsilon_i \rightarrow 0$ such that $\sharp (\partial B_{\varepsilon_i}(x) \cap \Sigma) = \oordball_x \Sigma \leq 6$ for every $i$. Without loss of generality let $\varepsilon_1<\varepsilon$. For numbers $l>k$ let us define the set
\[
\Sigma_{k,l} \defeq \Sigma \cap \overline{{B}_{\varepsilon_k}(x)} \setminus B_{\varepsilon_l}(x).
\]
Note that $\Sigma_{k,l} \subset S_\Sigma$ is a Steiner forest and all its vertices belong to $\partial B_{\varepsilon_k}(x) \cup \partial B_{\varepsilon_l}(x)$. Since $\Sigma_{k,l}$ has not more vertices than $13$, the number of its branching points is at most $11$ for each $l>k$ and $\Sigma_{k,l}$ consists of a finite number of line segments, less than $25$. Then there exists such a number $m>k$ that the set $\Sigma \cap \overline{B_{\varepsilon_m}(x)}$ does not contain a branching points or a maximal segment not containing the point $x$. So the number of segments in $\Sigma \cap \overline{B_{\varepsilon_m}(x)}$ is at most the number of segments of every set $\Sigma_{m,n}$, $n>m$ (which is not greater than $24$); in particular it is finite.    

In view of Lemma~\ref{angles2} the set $\Sigma \cap B_{\varepsilon_m}(x)$ should be either a segment with one end at the point $x$ and another at $\partial B_{\varepsilon_m}(x)$, or the onion of two such segments with the angle at least $2\pi/3$ between them, or the union of three such segments with angles $2\pi/3$ between them (i.e. regular tripod with the center at $x$). 
\end{proof}

Thus, it remains for us to deal with the behavior of $\Sigma$ in the neighborhoods of points of the set $ E_\Sigma $.

\begin{lemma}
The inequality $\oordball_x \Sigma\leq 3$ holds for every point $x \in \Sigma$.

\label{ord_en}
\end{lemma}

\begin{proof}
%ТУТ МНОГО НАДО ДОПИСАТЬ
For a point $ x \in X_\Sigma \cup S_\Sigma $ the statement follows trivially from Proposition~\ref{discr_str}. Now let $ x \in G_\Sigma $ and $ \oordball_x \Sigma \geq 4 $. Then, in view of the co-area inequality for sufficiently small $\varepsilon>0$ one has $ \H (B_\varepsilon (x) \cap \Sigma) \geq 4 \varepsilon $. On the other hand, for a sufficiently small $ \varepsilon> 0 $, the length $ \H (\partial B_ \varepsilon (x) \setminus B_r (y)) <3.5 \varepsilon $, where $ y \in M $ is an arbitrary point corresponding to the point $ x $. But then the set 
\[
(\Sigma \setminus B_\varepsilon(x) \cup \partial B_\varepsilon(x) \setminus B_r(y)) \cup S^{T_1T_2},
\]
where $T_1, T_2 = \partial B_\varepsilon(x) \cap \partial B_r(y(x))$, and the set $ S ^ {T_1T_2} $ is defined in the proof of Lemma~\ref{angles2},
is better than the set $\Sigma $. This contradiction completes the proof of the lemma.
\end{proof}
Then in view of the Remark~\ref{rem_ord} the following corollary is true: 
\begin{corollary}
For every point $x\in \Sigma$ the inequality $\oord_x \Sigma \leq 3$ holds.
\label{oord_en}
\end{corollary}
\begin{lemma} 
Let $x\in E_\Sigma$, $\rho>0$, 
%и $\varepsilon \defeq \varepsilon(\bar{x})$ принимают положительные значения
 $\bar{x}\in B_{\rho}(x)\cap G_\Sigma \setminus \{x\}$  --- an energetic point of a ray $(ix]$,
$\varepsilon<\min(|\bar x x|, \rho-|\bar x x|)$ and let point  
%$w \in Q^{s,\bar{x}}_{\varepsilon}$, где $\angle((s\bar{x}),(ix))=o_\rho(1)$. 
$w\in B_\varepsilon(\bar{x})$ be such that %$\angle((ix)(w\bar x))=o_\rho(1)$. 
$(w\bar{x}) \parallel (ix)$, or $w=\bar{x}$. Then there exists such connected set $S=S(\bar{x},w,x,\varepsilon) \ni w$, that 
%\[
%M \cap B_r(\Sigma \cap B_\varepsilon(\bar x)) \subset B_r(S)
%]
\[
F_M(\Sigma \setminus B_\varepsilon(\bar{x}) \cup S) \leq F_M(\Sigma)
\]
and $\H(S)=\varepsilon o_\rho(1)$.
\label{Losiu}
\end{lemma}

%необходима картинка!
Note that the set $\Sigma \setminus B_\varepsilon(\bar{x}) \cup S$  does not have to be connected.


Usually we will use the following formulation of this lemma:
\begin{multline*}
 \forall c>0 \ \forall x \in E_\Sigma \  \exists \rho_0>0 \ \forall \rho<\rho_0 \ \forall \bar{x}\in B_\rho(x)\cap G_\Sigma \setminus \{x\} \  \exists \varepsilon_0>0:\\ \forall \varepsilon<\varepsilon_0 \  \forall w \in B_\varepsilon(\bar{x}): (w\bar{x}) \parallel (ix) \vee (w=\bar x) \  \exists \mbox{ connected set } S\ni w:\\ F_M(\Sigma \setminus B_\varepsilon(\bar{x}) \cup S) \leq F_M(\Sigma) \mbox{ and } \H(S)<c\varepsilon.
\end{multline*}
Also, in view of compactness of $E_\Sigma$ the second and third predicates can be swapped: \[\forall c>0 \ \exists \rho_0>0 \  \forall x \in E_\Sigma \ \dots.\] 

\begin{proof}

%Since the proof of this lemma is not the easy to understand, we first present the main outline without technical details, and then we present the omitted technical proofs. Some of the concepts and statements introduced in this proof will be used in what follows.

In the further proof, the point $ x \in E_\Sigma $ will be assumed to be fixed; all points and quantities will be assumed to correspond to the conditions of the lemma. For a positive number $ \varepsilon $ and a point $ \bar x $, define the set

\[
U(\bar{x},\varepsilon) \defeq \left \{ y\in M | \dist(y, \overline{B_{\varepsilon}(\bar{x})})\leq r, \dist(y, \Sigma \setminus \overline{B_{\varepsilon}(\bar{x})})> r \right \}.
\]

\begin{enumerate}
    \item If an energetic ray $(ix]$ is one-orientated, then for a sufficiently small $\rho>0$ and $\varepsilon>0$ the set $U(\bar{x},\varepsilon)$ is located in one half-plane bounded by $ (ix) $(the one into which the ray is orientated). %понятно ли учитывая определки?
    
    If an energetic ray $(ix]$ is two-orientated for each $\bar x$ either exist such 
     $\varepsilon>0$, that the set $U(\bar{x},\varepsilon)$ is located in one half-plane bounded by $ (ix) $
     or in both half-planes there exist different points $y (\bar {x}) \in M$ corresponding to $ \bar{x} $. In what follows, we will assume that $\rho> 0 $ and $ \varepsilon> 0 $ satisfy these conditions.% We will give the proof of this item later.  
    \label{1115} 
    \begin{proof}
    The case of two-orientated $(ix]$ is clear.
    Let $(ix]$ be one-orientated. Without loss of generality we can consider $(ix]$ as a negative part of the abscissa, oriented to upper half-plane, i.e. points corresponding to energetic points of ray $(ix]$ lie upper abscissa. 
    Assume the contrary to the statement being proved, i.e. for each $\rho>0$ and $\varepsilon_0>0$ there exists such positive $\varepsilon<\varepsilon_0$ and such energetic point $\bar x \in E_\Sigma \cap B_\rho(x) \setminus \{ x\}$ that the intersection of $U(\bar{x}, \varepsilon)$ with lower half-plane is not empty. So for a point $\bar x$ there exists a sequence $\{\varepsilon_k\}$ monotonically decreasing to $0$ such that each set $U(\bar{x}, \varepsilon_k)$ contains some points of the lower half-plane, denote an arbitrary such point in each set by $u_k$. Note that $U(\bar{x}, \varepsilon_k)\supset U(\bar{x}, \varepsilon_{k+1})$ as $\varepsilon_k>\varepsilon_{k+1}$. Let $u = \lim_{k \rightarrow \infty} u_k$. As $M$ is a closed set $u\in M$. Moreover as $|u_k\bar x|\leq r+\varepsilon_k$, the inequality $|u\bar x| \leq r$ holds. 
    Assume $B_r(u)\cap \Sigma$ is not empty, thus, in view of connectivity of $\Sigma$, the intersection contains a point $x_1 \neq \bar{x}$. Consider such number $L$ that for every $l\geq L$ the inequalities $\varepsilon_l< |x_1\bar x|$ and $|u_lu|<r-|ux_1|$ hold. But then $x_1 \notin B_{\varepsilon_l}(\bar x)$ and $|\dist(x_1,U(\bar{x},\varepsilon_l))|<r$, which contradicts to the definition of the set $U(.,.)$. Thus $B_r(u)\cap \Sigma$ is empty, which means that $u$ corresponds to $\bar x$. Then there exists a sequence of energetic points of the ray $(ix]$ converging to $x$ with a points of $M$, lying in a lower half-plane, corresponding to them. The contradiction to the definition of one-orientated energetic ray.
    
    
    \end{proof}
        \begin{remark}
Obviously, $y(\bar{x}) \in \overline{U(\bar{x},\varepsilon)}$, where $y(\bar{x})\in M$ is an arbitrary point, corresponding to $\bar{x}$.
    \label{rem_c}
    \end{remark}
 %   Assume the contrary, then $\dist(y(\bar x), \Sigma \setminus \overline{B_{\varepsilon}(\bar{x})})<r$ which contradicts to $\Sigma \cap B_r(y(\bar x))=\emptyset$.
%    Осталось доказать что произвольная точка $y(\bar{x})$ принадлежит множеству $\overline{U(\bar{x},\varepsilon)}$.
%Пусть $\varepsilon>0$ произвольно и пусть существует такое $\delta>0$, что $B_\delta(y(\bar{x})) \cap U( \bar{x}, \varepsilon)=\emptyset $. 
%Поскольку $|y(\bar{x})\bar{x}|=r$ выполняется $B_r(B_\delta(\bar{x})) \supset B_\delta(\bar{x})$. При этом
%В таком случае $B_r(\Sigma \setminus B_\varepsilon(\bar{x}))\supset B_\delta(y(\bar{x}))$. Но тогда $\dist (\Sigma \setminus B_\varepsilon(\bar{x}), y(\bar{x})) \leq r-\delta$. Противоречие с тем, что $\dist (y(\bar{x}), \Sigma)=r$.
    
    \item Clearly, as $\Sigma \cap B_\varepsilon(\bar{x}) \subset B_\varepsilon(\bar{x}) \setminus B_r(y(\bar{x}))$, the inequality 
    %\label{112}
    %\item Ввиду~\ref{112}, 
    $\angle y(\bar{x})\bar{x}s>\pi/2-o(\varepsilon)$ holds for every $s \in B_\varepsilon(\bar{x}) \cap \Sigma$ and $y(\bar{x})$, corresponding to $\bar{x}$. In other words
    \[
    \forall c>0 \  \exists \rho>0 \ \exists \varepsilon>0: \forall \bar x \in B_\rho(x) \ \forall s \in B_\varepsilon(\bar x) \quad \angle y(\bar x) \bar x s >\frac{\pi}{2}-c\varepsilon.
    \]
    
    %Утверждение пункта очевидно.
    \label{113}
    %\item  Ввиду пункта~\ref{112} $|\angle((y(\bar{x})\bar{x}),(ix))-\frac{\pi}{2}|=o_\rho(1)$
    %\label{114}
    % Может, это не нужно 
    %убрала из п.3 |\angle u\bar x w - \frac{\pi}{2}|=
    \item For each $u\in U(\bar{x},\varepsilon)$ the following statement is true: $|\angle((u\bar{x}),(ix))-\frac{\pi}{2}|=o_\rho(1)$. %We will give the proof of this item later.  


    %Ввиду условия $(w\bar{x}) \parallel (ix)$, верно $|\angle w\bar{x}u-\frac{\pi}{2}|=o_\rho(1)$.
    \label{1145}
    \begin{proof}
Assume the contrary. Then there exists such number $c>0$, sequence  $\{x_k\}$ of energetic points of the energetic ray $(ix]$ converging to $x$, sequence $\varepsilon_k>0$ decreasing to $0$ and sequence of points $u_k \in U(x_k, \varepsilon_k)$ such that $|\angle((u_k x_k),(ix))-\frac{\pi}{2}|>c$ and, moreover,  $B_{\varepsilon_l}(x_l)\cap B_{\varepsilon_m}(x_m)=\emptyset$ for different numbers $l$, $m$ and $\varepsilon_k < \frac{|x_k x|}{2}$. Note that $x \notin B_{\varepsilon_k}(x_k)$, and thus by the definition of $U$ for each number $k$ the inequality $\dist(x, U(x_k,\varepsilon_k))>r$ holds. %Clearly for every limit point $u$ of the set $\{u_k\}$  the equality $\dist(x,u) = r$ is true .

In this case, at least one of two options is realized:\begin{itemize}
\item [I:] There exists a subsequence $\{I_{j=1}^\infty\}$ of numbers
such that $\angle([u_{I_k} x_{I_k}),(ix])<\frac{\pi}{2}-c$ for each number $k$. As $\{x_{I_k}\}$ are energetic points of an energetic ray $(ix]$ converging to $x$ there exists such number $N$ that for every number $\forall k >N$ the inequalities $\angle ixx_{I_k}<c/4$ and $\angle x_{I_k}u_{I_k}x<c/4$  hold. Thus $\angle u_{I_k} x_{I_k} x\leq \angle([u_k x_{I_k}),(ix])+\angle ixx_{I_k}<\frac{\pi}{2}-\frac{3c}{4}$. Then
\[
|u_{I_k}x|=\frac{|u_{I_k}x_{I_k}| \sin \angle u_{I_k}x_{I_k}x}{\sin \angle x_{I_k}xu_{I_k}}<\frac{(r+\varepsilon_k) \sin(\frac{\pi}{2}-\frac{3c}{4})}{\sin(\frac{\pi}{2}+\frac{c}{2})}=\frac{(r+\varepsilon_k) \cos \frac{3c}{4}}{\cos \frac{c}{2}}<r,
\]
where the last inequality is true for a sufficiently large  $ k $ (depending on $ c $), since $ c> 0 $ can be considered less than $ \pi / 2 $. This contradicts to $\dist(x, U(x_{I_k},\varepsilon_{I_k}))>r$.

\item [II:] There exists a subsequence $\{J_{j=1}^\infty\}$ of numbers such that $\angle ([u_{J_k} x_{J_k}),(ix])>\frac{\pi}{2}+c$. Let us consider a limit of the subsequence: $u \defeq \lim_{k \rightarrow \infty} u_{J_k}$. Then $|ux|\leq r$ (and hence $|ux|=r$) and $\angle uxi \leq\pi/2-c$. 

 As $\{x_{J_k}\}$ are energetic points of an energetic ray $(ix]$ converging to $x$ there exists such number $N_1$ that for every number $\forall k >N_1$ the inequalities $\angle ixx_{J_k}<c/4$ (and, therefore $\angle uxx_k<\pi/2 - 3c/4$) and $\angle x_{J_k}ux\leq c/4$ (for $u=\lim_{l \rightarrow \infty} u_{J_l}$)  hold. Then
 \[
|x_{J_k}u|=\frac{\sin \angle x_{J_k}xu}{\sin \angle ux_{J_k}x}|ux|<\frac{\cos \frac{3c}{4}}{\cos{\frac{c}{2}}}r.
\]
There also exists such $N_2$ that for every $m\geq N_2$ the inequality  $|u_{m}u|<r \left (1-\frac{\cos \frac{3c}{4}}{2\cos{\frac{c}{2}}}\right)$ holds. Then for different $J_k\neq m$ with $k>N_1$ the following is true: \[|u_{m}x_{J_k}|< |x_{J_k}u|+|u_{m}u|\leq \frac{\cos \frac{3c}{4}}{\cos{\frac{c}{2}}}r + \left (1-\frac{\cos \frac{3c}{4}}{2\cos{\frac{c}{2}}}\right) < r.\]
We have a contradiction with $x_{J_k} \notin B_{\varepsilon_m}({x_m})$.
 
% энергетические ребра $(ix]$
\end{itemize}
    \end{proof}
    
\begin{remark}
       In view of Remark~\ref{rem_c} also $|\angle((y(\bar{x})\bar{x}), (ix))-\frac{\pi}{2}|=o_\rho(1)$ holds. 
       \label{rem_cc}
\end{remark}
 
    \item  Clearly that for every $x_1 \in B_\varepsilon(\bar{x})$ the inequality $\dist(x_1, U(\bar{x},\varepsilon)) \geq r-\rho$ holds: otherwise $\dist(x, U(\bar{x},\varepsilon)) \leq r$, which is impossible as $\varepsilon<|\bar{x}x|$ which entails $x \in \Sigma \setminus \overline{B_\varepsilon(\bar x)}$. %Утверждение пункта очевидно.
    \label{777}
    \item Let  $\Lambda((nl), \gamma) \defeq \{z \ | \ \angle((zl),(ln)) \leq \gamma \}$. Then $U(\bar{x},\varepsilon) \subset \Lambda({(y(\bar{x}),w),o_\rho(1)})$ where $w$ is defined in the statement of the proven lemma.
    
    
    \begin{remark}
    Hereinafter, in case of $U(\bar{x},\varepsilon)$ located in one half-plane relative to $(ix)$, we could use instead of a set $\{z \ | \ \angle((zl),(ln)) \leq \gamma \}$ --- a set $ \{z \ | \ \angle zln \leq \gamma \}$.
    \end{remark}
    
    
  %  Если $U(\bar{x},\varepsilon)$ располагается в одной полуплоскости относительно $(ix)$ (в частности, если ребро $(ix]$ направлено в одну сторону), то $U(\bar{x},\varepsilon) \subset \Lambda((y(\bar{x})w],o_\rho(1))$, а если в обеих полуплоскостях, то $U(\bar{x},\varepsilon) \subset \Lambda({(y(\bar{x}),w),o_\rho(1)})$, где  \[\Lambda((nl], \gamma) \defeq \{z \ | \ \angle zln \leq \gamma \}\] и \[\Lambda((nl), \gamma) \defeq \{z \ | \ \angle((zl),(ln)) \leq \gamma \}.\]
   \begin{proof}%[~\ref{115}]
It is sufficiently to prove that for every $u\in U(\bar x, \varepsilon)$ the equality $\widehat{(y(\bar x)w),(uw)}=o_\rho(1)+\pi k$ holds for some $k\in \mathbf{Z}$.
In this item the angle between lines is supposed to be counterclockwise orientated and belongs to $[-\pi/2,pi/2]$. Then for every three lines $l_1$, $l_2$ and $l_3$ the equality $\widehat{l_1,l_2}+\widehat{l_2,l_3} = \widehat{l_1,l_3}+\pi k $ for some $k\in \mathbf{Z}$.

%where $l, k\in \mathbf{Z}$.
Applying item~\ref{777} to $x_1 \defeq \bar{x}$ 
   we get $\dist(\bar{x}, U(\bar{x},\varepsilon)) \geq r-\rho$. Then consider the triangle $\triangle u\bar x w$: 
\[
\sin (\angle \bar x u w) =  \frac{|\bar x w|}{|\bar x u|}\sin (\angle \bar x w u)\leq \frac{\varepsilon}{r-\rho}=O(\varepsilon)=o_\rho(1). 
\]
Thus $\angle((uw),(u\bar x))=|\angle \bar x u w| =o_\rho(1)$ and particularly $\angle ((y(\bar x)w),(y(\bar x) \bar x))=\angle \bar x y(\bar x) w =o_\rho(1)$. 

So in view of item~\ref{1145} and Remark~\ref{rem_cc} the equality
\begin{equation*}
\widehat{(y(\bar x) w),(uw)}=\widehat{(y(\bar x)w),(y(\bar x) \bar x)}+\widehat{(y(\bar x) \bar x),(ix)}+ \widehat{(ix),(u \bar x)}+ \widehat{(u\bar x),(uw)}+ \pi l=o_\rho(1)+\pi k
\label{ang} 
\end{equation*} holds for some $l, k\in \mathbf{Z}$.

%And then 
%\begin{equation*}
%\angle((y(\bar x)w),(uw))=\angle((y(\bar x)\bar x),(uw)) \pm \angle ((y(\bar x) \bar x),(y(\bar x)w)+ \pi l=o_\rho(1)+\pi k
%\end{equation*}

%Then %in view of~\eqref{ang}
%\[
%\angle((y(\bar x)w),(uw))=\angle((y(\bar x)\bar x),(uw))-\angle \bar x y(\bar x)w= o_\rho(1)+\pi k
%\]
%\[
%\angle((y(\bar x)w),(uw))=\angle((y(\bar x)\bar x),(uw)) \pm \angle ((y(\bar x)w),(y(\bar x) \bar x))+\pi l= o_\rho(1)+\pi k
%\]
%for $l, k\in \mathbf{Z}$.


   %Applying item~\ref{777} to $x_1 \defeq \bar{x}$ and to $x_1 \defeq w$
  % we get $\dist(\bar{x}, U(\bar{x},\varepsilon)) \geq r-\rho$ and $\dist(w, U(\bar{x},\varepsilon)) \geq r-\rho$.
   
    %Ввиду пункта~\ref{777} для $x_1 \defeq \bar{x}$ и $x_1 \defeq w$ выполняется $\dist(\bar{x}, U(\bar{x},\varepsilon)) \geq r-\rho$ и $\dist(w, U(\bar{x},\varepsilon)) \geq r-\rho$, а поскольку $|w\bar{x}|<\varepsilon$, для произвольной $u\in U(\bar{x},\varepsilon)$, ввиду рассмотрения треугольника $\triangle u\bar x w$ выполняется  $|\angle((uw),(ix)) -\frac{\pi}{2}|=o_\rho(1)$. Тогда ввиду $y (\bar x) \in \overline {U(\bar{x},\varepsilon)}$ выполнено $|\angle((y(\bar{x})w), (ix))-\frac{\pi}{2}|=o_\rho(1)$. Ввиду произвольности $u \in U(\bar{x}, \varepsilon)$ утверждение пункта доказано.
   \end{proof}
   
  
   %А значит, поскольку $u$ произвольна, выполняется $U(\bar{x},\varepsilon) \subset \Lambda_{(y(\bar{x}),w),o_\rho(1)}$
    %, где $\Lambda((nl), \gamma) \defeq \{z \big|\angle((zl),(ln)) \leq \gamma \}$; 
    \label{115}
    \color{black}
    \item For every  $u\in U(\bar{x}, \varepsilon)$ there exists such $v_1$ (does not have to belong to $\Sigma$) that $v_1 \in B_\varepsilon(\bar{x})$, $|v_1u|\leq r$, $\angle ((v_1\bar{x}),(ix))=o_\rho(1)$.
    
    
 %   Для произвольной $u\in U(\bar{x}, \varepsilon)$, существует $v \in \Sigma \cap B_\varepsilon(\bar{x})$ такая, что $|vu| \leq r$. Тогда найдется $v_1$ (не обязательно элемент $\Sigma$) такая, что $v_1 \in B_\varepsilon(\bar{x})$, $|v_1u|\leq r$, $\angle ((v_1\bar{x}),(ix))=o_\rho(1)$.
    \begin{proof}
    For every $u\in U(\bar{x}, \varepsilon)$ there exists such $v \in \Sigma \cap B_\varepsilon(\bar{x})$ that $|vu| \leq r$. Let $y(\bar x)$ be a point of $U(\bar x, \varepsilon)$ corresponding to $\bar x$ and located at the same half-plane as $u$ with respect to $(ix)$.
    Define $v_1 \defeq v$ in case that $\pi/2> \angle y(\bar{x})\bar{x}v$. Note that $\angle y(\bar{x})\bar{x}v>\pi/2-o_\varepsilon(1)$ by item~\ref{113}. And in the case $\angle y(\bar{x}) \bar{x} v \geq \pi/2$ one can define $v_1 \in [vu]$ such way that $(v_1\bar x) \perp ( x y(\bar x))$.

    \end{proof}

    \label{117}
    \item The inequality $|wu|\leq r+o(\varepsilon)+\varepsilon o_\rho(1)$ holds. Thus $U(\bar{x},\varepsilon) \subset B_{r+\varepsilon o_\rho(1)}(w)$.
    \label{118}
    \begin{proof}
Note that by items~\ref{1145} and~\ref{117} lines $(u\bar x)$, $(uw)$, $(uv_1)$ are almost perpendicular to $(ix)$ and lines $(\bar xw)$, $(\bar xv_1)$ are almost parallel to $(ix)$.  Id est $|\angle((ux),(ix))-\pi/2|, |\angle((uw),(ix))-\pi/2|, |\angle((uv_1),(ix))-\pi/2|=o_\rho(1)$
and $\angle((\bar x w),(ix)), \angle((\bar x v_1),(ix))=o_\rho(1)$.
Thus $|\angle uv_1\bar x-\pi/2|=o_\rho(1)$ and $|\angle u\bar xw-\pi/2|=o_\rho(1)$. 

Then applying law of cosines to the triangle $\triangle uv_1 \bar x$ we get $|u\bar x|^2=|uv_1|^2+|v_1\bar x|^2-2|uv_1||v_1\bar x| \cos \angle uv_1\bar x$. Which entails $|u\bar x|^2\leq r^2+\varepsilon^2+o_\rho(1)\varepsilon$,
so $|u\bar x|\leq r+o_\rho(1)\varepsilon$.

Now by law of cosines for the triangle $\triangle uw\bar x$: $|uw|^2=|u\bar x|^2+|w\bar x|^2-2|u\bar x||w\bar x|\cos(\angle u\bar xw)$.
Then $|uw|^2\leq ( r+o_\rho(1)\varepsilon)^2+\varepsilon^2+\varepsilon o_\rho(1)$, which implies $|uw|\leq r+o_\rho(1)\varepsilon$.

    \end{proof}
    \item
 Clearly, $U(\bar{x},\varepsilon) \subset \Lambda({(y(\bar{x}),w),o_\rho(1)})\cap B_{r+o_\rho(1)\varepsilon}(w)$.
   % В таком случае, если $U(\bar{x},\varepsilon)$ располагается в одной полуплоскости относительно $(ix)$ (т.е. в частности, если ребро $(ix]$ направлено в одну сторону), то, ввиду пунктов~\ref{1115},~\ref{115},~\ref{118}, \[U(\bar{x},\varepsilon) \subset \Lambda((y(\bar{x}),w],o_\rho(1)) \cap B_{r+\varepsilon o_\rho(1)}(w),\]
    %, где $\Lambda((nl], \gamma) \defeq \{z \big|\angle zln \leq \gamma \}$; 
    %а если в  обеих полуплоскостях, то \[U(\bar{x},\varepsilon) \subset \Lambda(w,(y(\bar{x})w),o_\rho(1)) \cap B_{r+\varepsilon o_\rho(1)}(w).\]%, где $\Lambda(w,l, \gamma) \defeq \{z \big| \angle((zw),l) \leq \gamma \}$.
    \label{119}
    \color{black}
    %Утверждение пункта очевидно.
    \item There exists a connected set $S\ni w$ such that $\H(S)=\varepsilon o_\rho(1)$ and 
    \[
    (\Lambda ((y(\bar{x})w), \gamma) \cap B_{a}(w))\subset \overline{B_r(S)},
    \]
where $\gamma=o_\rho(1)$, $a=r+\varepsilon o_\rho(1)$.

%При этом в случае, если $U(\bar{x},\varepsilon)$ располагается в одной полуплоскости относительно $(ix)$ (т.е. в %частности, если ребро $(ix]$ направлено в одну сторону), $S$ можно выбрать отрезком, а если нет, то объединением %двух отрезков.
    \label{120}
\begin{proof}
Let us construct $S$ in the following way: 
\[ 
S \defeq \left(( (wy(\bar x)) \cap B_{a-r}(w)) \cup \partial  B_{a-r}(w))\right)\cap \Lambda ((y(\bar{x})w), \gamma).
\] 
$S$ obviously satisfies both conditions.


%Известно, что $U(\varepsilon, \bar{x}) \subset (B_a(w) \cap \Lambda)$, где $\Lambda=\Lambda((y(\bar x)w], \gamma)$, если $U(\varepsilon, \bar{x})$ находится в одной полуплоскости относительно $(ix)$ или $\Lambda=\Lambda((y(\bar x)w), \gamma)$ иначе; $a=r+o_\rho(1)\varepsilon$, $\gamma=o_\rho(1)$ для произвольной $y(\bar x)$ соответствующей $\bar x$. Построим $S$ следующим образом:
%\[ 
%S \defeq \left(( (wy(\bar x)) \cap B_{a-r}(w)) \cup \partial  B_{a-r}(w))\right)\cap \Lambda.
%\] 
%Очевидно, что условие на энергию выполнено, поскольку \[\overline{B_r(S)}\supset
%\overline{B_r(\partial  B_{a-r}(w)\cap \Lambda)} \supset  (\overline{B_a(w)} \cap \Lambda) \supset U(\varepsilon, \bar{x}).\] 
%При этом 
%\[
%H(S)=|a-r|+o_\rho(1)(a-r)=o_\rho(1)\varepsilon+(o_\rho(1)\varepsilon o_\rho(1)=o_\rho(1)\varepsilon.
%\]
%Таким образом, все требования на $S$ выполнены.
\end{proof}    
\begin{remark}
It is easy to see that in case $U(\bar{x},\varepsilon)$ is located in one half-plane with respect to $(ix)$ (and hence with respect to a line $l_w$ containing $w$ and parallel to $(ix)$) the set $S$ can be chosen half as long: only one part of two symmetrical about $l_w$ is sufficient.
\end{remark}
\end{enumerate}
Items~\ref{119}, \ref{120} and the definition of the set $U(\bar{x},\varepsilon)$  imply the statement of the lemma. 
\end{proof}
%мМожно замечание про половинку S

Hereinafter we will write $o_\rho(1)$-almost, if something is true to within $o_\rho(1)$. 

\begin{corollary}
Item~\ref{1145} of Lemma~\ref{Losiu}, in view of the Remark~\ref{emptyball}, entails that the energetic rays of an arbitrary point $\bar{x} \in E_\Sigma \cap B_\rho(x) $ are $o_\rho(1)$-almost parallel to $(ix)$, id est $|\angle((ix),l_{\bar x})=o_\rho(1)|$ where $l_{\bar x}$ is a line containing an energetic ray of the set $\Sigma$ with a vertex at the point $ \bar x$.%ВИДИМО ТУТ ИЛИ ПЕРЕД ЭТИМ НАДО ОПРЕДЕЛИТЬ СЛОВО ПОЧТИ
\label{alm_parr}
\end{corollary}

\begin{lemma} For an arbitrary $x\in E_\Sigma$ there exists such $\rho>0$, that for every $\bar{x}\in B_{\rho}(x)\cap G_\Sigma \setminus \{x\}$ the inequality $\oordball_{\bar{x}}\Sigma \leq 2$ holds. 
\label{ordball_}
\end{lemma}

\begin{proof}
Let $n \defeq \oordball_{\bar x}\Sigma$ and let $\varepsilon>0$ be such a sufficiently small number that 
\[
\sharp (\partial B_{\varepsilon}(\bar x) \cap \Sigma) = n. 
\]
%сослаться  на формулу коплощади
Then, in view of the definition of the circular order and of co-area inequality the following is true: $\H(B_\varepsilon(\bar x)\cap \Sigma) \geq n \varepsilon$. %Предположим, что $n > 2$.
As $\bar{x}$ is an energetic point, these intersection is empty $B_r(y(\bar x)) \cap \Sigma =\emptyset$. So all $n$ points of  $\Sigma \cap \partial B_\varepsilon(\bar x)$ are located at the arc with size $\pi+o(\varepsilon)$.

Let $n \geq 4$. There exists such $\varepsilon_0$ that for every positive number $\varepsilon<\varepsilon_0$ the inequality $\H(\partial B_\varepsilon(\bar x) \setminus B_r(y(\bar x)))<3.5 \varepsilon$ holds. Clearly, for every $\varepsilon$ and $y(\bar x)$ there exists such point $w \in \partial B_\varepsilon(\bar x) \setminus B_r(y(\bar x))$, that $(w\bar x) \parallel (ix)$. Then in view of Lemma~\ref{Losiu} there exists such a connected set $S \ni w$, that $\H(S)<\varepsilon/4$ and $F_M(\Sigma \setminus B_\varepsilon(\bar x)\cup S) \leq F_M(\Sigma)$. Thus the set 
\[
\Sigma \setminus B_\varepsilon(\bar x) \cup (\partial B_\varepsilon(\bar x) \setminus B_r(y(\bar x))) \cup S,
\]
is strictly shorter than $\Sigma$ and has not larger energy. So we have a contradiction with an optimality of $\Sigma$.  

Let now $n=3$. Let us denote points $\Sigma \cap \partial B_\varepsilon(\bar x)$ by $A_1$, $A_2$ and $A_3$.  For each location of these points there exists two of them (without loss of generality let it be $A_1$ and $A_2$) form with $\bar x$ an isosceles triangle with an angle at the apex less than $\angle A_1 \bar x A_2 \leq \pi/2+o(\varepsilon)$. Then, in view of Proposition~\ref{angles4} the set $St(A_1, \bar x, A_2) \cup [A_3 \bar x]$ has the length not greater than $(3-c)\varepsilon$ where $c>0$ is a constant and $St(A_1, \bar x, A_2)$ is a Steiner tree for these three points. Thus the set
\[
\Sigma \setminus B_\varepsilon(\bar x) \cup (St(A_1, \bar x, A_2) \cup [A_3 \bar x] \cup S),
\]
where $S$ is constructed in Lemma~\ref{Losiu} for $w=\bar x$, is strictly shorter than $\Sigma$ and has not greater energy. The contradiction with the optimality of $\Sigma$ implies $n\leq 2$.
\end{proof}

\begin{corollary}% [следствие Леммы~\ref{ordball_}]
In view of~\ref{rem_ord} for arbitrary $x\in E_\Sigma$ there exists such $\rho >0$, that for every $\bar x \in G_\Sigma \cap B_\rho(x)\setminus \{x\}$the inequality $\oord_{\bar{x}}\Sigma \leq 2$ holds.
\end{corollary}
%дальше тут еще вставить леммочку 
\begin{proposition}%\label{QuQuQu}

For an arbitrary point $x\in E_\Sigma$ we will prove some facts concerning energetic points in its sufficiently small neighbourhood.
%Для произвольных $c>0$ и $x\in E_\Sigma$ найдется такое $\rho>0$, что для каждого $\bar x \in G_\Sigma \cap B_\rho(x)  \setminus \{x\}$ и для $(ix]$, ближайшего к $\bar x$ ребра $x$, выполняется
\begin{enumerate}
\item\label{W}
The following holds: $|\angle ((s^\varepsilon \bar x), (ix))-\pi/2|=o_\rho(1)$ if $s^\varepsilon \defeq \partial B_{\varepsilon}(\bar x) \cap \Sigma$ and $B_\varepsilon(\bar x) \subset (B_\rho(x)\setminus \{x\})$.

In other words, for each $c>0$ there exists such $\rho>0$ that for every $\bar{x} \in B_\rho(x) \setminus \{ x\}$ such that $\oordball_{\bar x}\Sigma=1$, for every $\varepsilon<\min(|\bar x x|, \rho-|\bar x x|)$ such that $\sharp(\partial B_{\varepsilon}(\bar x) \cap \Sigma)=1$ the inequality $|\angle ((s^\varepsilon \bar x), (ix))-\pi/2|<c$ holds, where $s^\varepsilon = \partial B_{\varepsilon}(\bar x) \cap \Sigma$.
\begin{proof}
%[вспомогательного утверждения А]
Assume the contrary, id est there exists such $c>0$ that for every $\rho>0$ there exists such $\varepsilon_0>0$ that $\bar x \in \Sigma \cap B_{\rho-\varepsilon_0}(x) \setminus \overline{B_{\varepsilon_0} (x)} $ and the inequality $|\angle ((s_0\bar x), (ix))-\frac{\pi}{2}| > c$ holds for $s_0 \defeq \partial B_{\varepsilon_0}(\bar x) \cap \Sigma $. 

Let the point $w^0$ be the foot of the perpendicular from $s_0$ to the line, parallel $(ix)$ and containing $\bar x$:  $(w^0\bar x)\ ||\ (ix)$ and $(w^0s_0) \perp (ix)$. Then we denote the set $S \ni w^0$ as in Lemma~\ref{Losiu} for $w=w^0$. Then the length of this set is small: $\H(S)=o_\rho(1)\varepsilon_0$.

At the same time the inequality
\[
|w^0s_0|=\sin \angle((s_0\bar x],(ix]) \cdot |s_0\bar x|< \cos c |s_0\bar x| < (1 - \frac{c^2}{2}) \varepsilon_0
\]
holds for sufficiently small $c$. Herewith $\H(\Sigma \cap B_{\varepsilon_0}(\bar x)) \geq \varepsilon_0$. Thus \[
\H(\Sigma \setminus  B_{\varepsilon_0}(\bar x) \cup [s_0w^0] \cup S)\leq \H(\Sigma)-\varepsilon_0+\left(1-\frac{c^2}{2}\right)\varepsilon_0+o_\rho(1)\varepsilon_0<\H(\Sigma).
\]
Hence $\Sigma \setminus  B_{\varepsilon_0}(\bar x) \cup [s_lw^l] \cup S$ is a connected set with the length less than and energy not greater than $\Sigma$. The contradiction with optimality of $\Sigma$ completes the proof.
\end{proof}
\item\label{WW}
Let $x \in E_\Sigma$. Then for sufficiently small $\rho>0$ for each $\bar x \in G_\Sigma \cap B_\rho(\Sigma)\setminus \{ x\}$ with a circular order  $\oordball_{\bar x}\Sigma = 2$, there exists such a  small $\varepsilon>0$ that for every $s^l, t^l \defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$ where $\varepsilon_l \leq \varepsilon$ the inequalities $\angle s^l\bar xt^l > \frac{2\pi}{3} - \varepsilon_lo_\rho(1)$, $\angle ((s^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ and $\angle ((t^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ hold. 
%\label{D}
\begin{proof}
The second and third inequalities follow from the first one and the fact that there exists such a point $y(\bar x)$ that $B_r(y(\bar x)) \cap \Sigma = \emptyset$ and $|\angle ((y(x)x),(ix)) - \pi/2| =o_\rho(1)$. The first inequality is true otherwise the connected set $\Sigma \setminus B_{\varepsilon_l}(\bar x) \cup St(s^l,t^l,\bar x) \cup S$, where $S \ni \bar x$ with length $\varepsilon_l o_\rho(1)$ is defined in Lemma~\ref{Losiu} for a point $w=\bar x$, and $St(s^l,t^l,\bar x)$ is a Steiner tree connecting points $s^l$, $t^l$ and $\bar x$ has not larger energy and strictly less length than $\Sigma$, which is impossible.
\end{proof}


\item\label{WWW}
Let $x \in E_\Sigma$. Then for sufficiently small $\rho>0$ for each $\bar x \in G_\Sigma \cap B_\rho(\Sigma)\setminus \{ x\}$ with a circular order  $\oordball_{\bar x}\Sigma = 2$, there exists such a  small $\varepsilon>0$, that for every $u \in \Sigma \cap B_\varepsilon(\bar x)$ the inequality $\angle((u \bar x),(ix)) \neq \pi/2$ holds.

In other words if the point $\bar x \in G_\Sigma \cap B_\rho(\Sigma)\setminus \{ x\}$ has a circular order $\oordball_{\bar x}\Sigma = 2$, there doesn't exist any consequence $\{u_m\}\subset \Sigma$ converging to $\bar x$ such that $\angle((u_m\bar x),(ix))=\pi/2$. %ДЛЯ ПРОСТО ОРД=2 НЕ НАДО?
%Note that remark and lemma imply $\ordball_{\bar x}\Sigma=2$
%Пусть $x \in E_\Sigma$. Найд ется такое $c>0$, что для достаточно малого $\rho>0$ для каждого $\bar x \in G_\Sigma \cap B_\rho(\Sigma)\setminus \{ x\}$, имеющего порядок $\oordball_{\bar x}\Sigma = 2$, найдется такое $\varepsilon>0$, что для каждой  $u \in \Sigma \cap B_\varepsilon(\bar x)$ выполняется $|\angle((u \bar x),(ix))-\pi/2|>c$.  Иными словами касательный луч к энергетической точке $\bar x  \in G_\Sigma \cap B_\rho(\Sigma)\setminus \{ x\}$, имеющей порядок $\oordball_{\bar x}\Sigma = 2$, не является $o_\rho(1)$ почти перпендикулярным $(ix]$,

%не существует такой последовательности энергетических точек $\bar x_k$ степени 2 сходящихся к x , что найдутся касательные лучи к Sigma в $\bar x_k$, сходящиеся к перпендикуляру к $(ix]$ в точке $x$.

%Иными словами никакой касательный луч к $\Sigma$ в точке $\bar x$ не является почти перпендикулярным к $(ix]$
%\color{black}

\begin{proof} %%Note that remark and lemma imply $\ordball_{\bar x}\Sigma=2$

%Clearly, that $\angle s^l\bar xt^l > \frac{2\pi}{3} - \varepsilon_lo_\rho(1)$: otherwise the connected set $\Sigma \setminus B_{\varepsilon_l}(\bar x) \cup St(s^l,t^l,\bar x) \cup S$, where $S \ni \bar x$ with length $\varepsilon_l o_\rho(1)$ is defined in lemma~\ref{Losiu} for a point $w=\bar x$, and $St(s^l,t^l,\bar x)$ --- is a Steiner tree connecting points $s^l$, $t^l$ and $\bar x$ has not larger energy and strictly less length than $\Sigma$, which is impossible.
%On the other hand $B_r(y(\bar x)) \cap \Sigma = \emptyset$ and $|\angle ((y(x)x),(ix)) - \pi/2| =o_\rho(1)$ in view of item~3 of the proof of the lemma~\ref{Losiu}. Note then that $\angle ((s^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ and $\angle ((t^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$.

Assume the contrary to the statement of the item: that there exists such sequence $\{u_m\}$, converging to $\bar x$ that $\angle((u_m\bar x),(ix))=\pi/2$ for each $m$. 
Let $\{\varepsilon_l\}$ be such a decreasing to $0$ consequence that $\sharp (\partial B_{\varepsilon_l}(\bar x) \cap \Sigma )=2$ and $\varepsilon_1 < \min (|\bar x x|, \rho-|\bar x x|)$. Denote  $s^l, t^l \defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$. Then, from item~\ref{WW} the inequalities $\angle s^l\bar xt^l > \frac{2\pi}{3} - \varepsilon_lo_\rho(1)$, $\angle ((s^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ and $\angle ((t^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ hold.
Then 
\[
\sharp (\Sigma \cap \partial B_{|\bar x u_l|}(\bar x))\geq 3.
\]
for sufficiently small $\varepsilon_1>|u_1\bar x|$.

Note that for every $\varepsilon_l$ the following is true:
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)=2\varepsilon_l+o_\rho(1)\varepsilon_l.
\label{1000}
\end{equation}
Really $\H(B_{\varepsilon_l}(\bar x)\cap \Sigma) \geq 2\varepsilon_l$ in view of co-area inequality. And in other hand $\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)\leq 2\varepsilon_l+o_\rho(1)\varepsilon_l$ because otherwise changing in the set $\Sigma$ the subset $\Sigma \cap B_{\varepsilon_l}(x)$ by the set $ [\bar xs^l]\cup [\bar x t^l]\cup S$, where $s_l,t_l=\partial B_{\varepsilon_l}(\bar{x})\cap \Sigma$, the $S$ is defined at the Lemma~\ref{Losiu} for $w=\bar x$ and has a length $\varepsilon_l o_\rho(1)$, saves the connectivity, reduces the length and not increases the energy, which is impossible.
So one can choose such small $\varepsilon_1$ that
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)<2\varepsilon_l \left (1+\frac{1}{36}\right).
\label{1010}
\end{equation}
Note then that there exists such sequence (add elements to the sequence if necessary) $\{\varepsilon_l\}$ that
\begin{equation}
\frac{\varepsilon_l}{\varepsilon_{l+1}}\leq \frac{18}{17}.
\label{1030}
\end{equation}
Really, assume the contrary, then there exists such $\varepsilon_l$ that $\sharp \left( \partial B_{\varepsilon_l}(\bar x)\cap \Sigma
\right) \geq 3$ for every $\varepsilon \in [\frac{17\varepsilon_l}{18},\varepsilon_l[$. But then, in view of the co-area inequality,
\[
\H(\Sigma \cap B_{\varepsilon_l}(\bar x))\geq \H(\Sigma \cap B_{\frac{17\varepsilon_l}{18}}(\bar x)) +\H(\Sigma \cap (B_{\varepsilon_l}(\bar x) \setminus  B_{\frac{17\varepsilon_l}{18}}(\bar x))\geq \varepsilon_l\left(1+\frac{1}{18}\right),
\]
which contradicts to \eqref{1010}.
Consider an arbitrary $u_m$ and choose such a number $l$ that 
\begin{equation}
0<\varepsilon_l-|\bar xu_m|\leq \frac{1}{18}\varepsilon_l.
\label{1040}
\end{equation}
Such $\varepsilon_l$ exists in view of the inequality~\eqref{1030}. Also we for every $\delta \in ]|\bar x u_m|, \varepsilon_l[$ the inequality $\sharp \left( \partial B_{\delta}(\bar x)\cap \Sigma
\right) \geq 3$ holds (one can add new element to the sequence if necessary).
Let \[\gamma \defeq \max_{s \in \Sigma \cap \overline B_{\varepsilon_l}(\bar x): \sharp (B_{|\bar x s|}(\bar x) \cap \Sigma) <3)} \angle{((ix),(\bar x s)}.\] Then $\gamma\leq \frac{\pi}{3}+ o_\rho(1)$.
Note that~\eqref{1010} implies that
\[
\H(\Sigma \cap \Lambda((i \bar{x}),\gamma) \geq 2\varepsilon_l(1-\frac{1}{36})
\]
Let $q$ be a connected component of $\Sigma \setminus \Lambda((i \bar{x}),\gamma)$ containing $u_m$ (by point $i$ we mean sufficiently far point from $(ix]$).
Then 
\[
\H(q) \geq \dist (u_m, \Lambda((i\bar x),\gamma)) 
=\cos \gamma |u_m \bar x|> \frac{|u_m \bar x|}{3}.
\]
Thus
\[
\H(\Sigma \cap B_{\varepsilon_l}(\bar x))\geq \H(\Sigma \cap B_{\varepsilon_l}(\bar x)\cap \Lambda((i\bar x),\gamma))+\H(q)\geq 2\varepsilon_l(1-\frac{1}{36})+\frac{|u_m \bar x|}{3}>2\varepsilon_l(1+\frac{1}{36}),
\]
which contradicts to~\eqref{1010}. The last inequality follows from~\eqref{1040}.
\end{proof}
\item\label{WWWW}
For every $x\in E_\Sigma$  for each $c>0$ there exists such $\rho>0$, that for every $\bar{x} \in B_\rho(x) \setminus \{ x\}$ for every $\varepsilon$ such that $B_\varepsilon(\bar x)\subset B_\rho(x) \setminus \{x\}$ for $S,T \defeq \partial B_\varepsilon(\bar x)$ the inequality $|\angle ((S \bar x), (ix)) - \angle ((T \bar x), (ix))|<c$ holds.
In other words, $|\angle ((S \bar x), (ix)) - \angle ((T \bar x), (ix))| = o_\rho(1)$

%For every $x\in E_\Sigma$  for each $c>0$ there exists such $\rho>0$, that for every $\bar{x} \in B_\rho(x) \setminus \{ x\}$ such that $\oordball_{\bar x}\Sigma=2$ выполняется $|(\angle (s \bar x], (ix] - (\angle (t \bar x], (ix]| <c$, где $(s \bar x]$ и $(t \bar x]$ --- касательные для компонент связности $\Sigma \setminus \bar x$ в точке $\bar x$.
%Иными словами, $|(\angle (s \bar x], (ix] - (\angle (t \bar x], (ix]| = o_\rho(1)$.
%НАДО НЕ ЗАБЫТЬ ЧТО ЭН РЕБРА ПОЧТИ ПАРАЛЛЕЛЬНЫ ЭНРЕБРУ
\begin{proof}
Assume the contrary: let there exist such $c>0$, that
\[
\eta \defeq \angle((S\bar x), (ix))-\angle( (ix),(T\bar x)) \geq c
\]
for infinitesimal $\rho$.
%Пусть $\varepsilon< \min (\rho-|\bar x x|, |\bar x x|)$ такой, что $\sharp( \partial B_\varepsilon(\bar x) \cap \Sigma) =2$. Обозначим $T, S \defeq \partial B_\varepsilon(\bar x)  \cap \Sigma$. Тогда 
%\begin{equation}
%\angle ((T \bar x],(t\bar x))=o_\rho(1) \mbox{ и } \angle ((S \bar x],(s\bar x))  =o_\rho(1).
%\label{ZAQ}
%\end{equation}
Let $l$ be the line containing $\bar x$ and parallel to $(ix)$. Let point $T'$ be a reflection of $T$ relative to $l$. Then $|T'\bar x|=\varepsilon$ and
\[
|S \bar x|+|T \bar x|=|S\bar x|+|T' \bar x|=2\varepsilon.
\]
At the same time in view of law of cosines for triangle $\Delta S\bar xT'$
\[
|ST'|^2 = |S\bar x|^2+|\bar xT'|^2-2|S\bar x||\bar x T'|\cos \angle S\bar xT'=2\varepsilon^2(1-\cos \eta),
\]
as
\[
\angle S\bar xT'=\pi+\angle((T\bar x), (ix))-\angle( (ix),(S\bar x)).\]
%d est~\eqref{ZAQ}   
%\[
%\angle S\bar xT'=\pi+\angle((t\bar x], (ix))-\angle( %(ix),(s\bar x])+o_\rho(1)=\pi+\angle((t\bar x], %(ix))-\angle( (ix),(s\bar %x])+o_\rho(1)=\pi=\eta+o_\rho(1).
%\] 
%а $\angle S\bar xT'=\angle s \bar x t+o_\rho(1)=\pi-\eta+o_\rho(1)$.
%So, for sufficiently small $\rho$,
%\[
%|S\bar x|+|T'\bar x|-|ST'|> 2(1-\sqrt{2 -2\cos \eta}) \varepsilon.
%\]
%where $c_2 > 0$ --- константа, зависящая только от $\eta$.
Let $d \defeq [ST']\cap l$. Then $\angle((Sd], (ix))=\angle( (ix),(T'd])$ and 
%\begin{equation*}
\[(|S\bar x|+|T\bar x|)-(|Sd|+|dT|)= 2\varepsilon - |ST'|=\varepsilon(2-\sqrt 2+\sqrt 2 \cos \eta).\]
%\end{equation*}

In view of Lemma~\ref{Losiu} for $w=d$ there exists a connected set $S \ni d$ such that  $\H(S)<(2-\sqrt 2+\sqrt 2 \cos \eta)\varepsilon$ and $F_M(\Sigma \setminus B_\varepsilon(\bar x) \cup S)\leq F_M(\Sigma)$. Then the connected set $\Sigma \setminus ([S\bar x]\cup[T\bar x]) \cup S \cup [sd] \cup [td]$ is better than $\Sigma$, as is energy is not greater and its length is strictly less. 
%не превосходящую $\H(\Sigma)-c_2\varepsilon+ \H(S)<\H(\Sigma)$. 
So we have a contradiction with optimality of $\Sigma$.
\end{proof}

%\begin{corollary}
%В ввиду леммы~\ref{angles2} верно $\angle s\bar xt \geq \frac{2\pi}{3}$ и 
%\[
%\angle((s\bar x], (ix))=\angle( (ix),(t\bar x] )+ o_\rho(1)\leq \frac{\pi}{6}+ o_\rho(1).
%\] 
%\label{__2c}
%\end{corollary}
\end{enumerate}
\label{items}
\end{proposition}

%The Proposition~\ref{items} implies the following lemma.
Now we can prove the following lemma.
\begin{lemma}
For every $x\in E_\Sigma$ and  $c>0$ there exists such $\rho>0$, that for every $\bar x \in G_\Sigma \cap B_\rho(x)  \setminus \{x\}$ and for the $(ix]$, closest to $\bar x$ energetic ray of $x$, the following statements are true: 
\begin{enumerate}
\item if $\oord_{\bar x}\Sigma=1$, then $\bar x \in X_\Sigma$ and for the segment $[s\bar{x}] \subset \Sigma$ the following inequality is true:  \[\angle((s\bar{x})(ix))>\pi/2-c.\] 
In other words the segment $[s\bar x]$ is $o_\rho(1)-$almost perpendicular to $(ix)$.
If $(ix]$ is one-oriented energetic ray, then for the point $y\defeq y(x)$, which is the limit of the points corresponding to the energetic points of the energetic ray $(ix]$ the following inequality is true:
 \[
 \angle ([s\bar{x}), [xy))<c;
 \]
\label{__1}
\item if $\bar x \in X_\Sigma$ and  $\oord_{\bar x} \Sigma=2$, then the angle of incidence is almost equal to the angle of reflection:
\[|\angle((s\bar{x}], (ix))-\angle( (ix),(t\bar{x}])|<c\mbox{, where } [s\bar{x}] \cup [t\bar{x}] \subset \Sigma;\]
\label{__2}
\item if $\bar {x} \in E_\Sigma$, then there exists such $\varepsilon>0$ that $B_\varepsilon(\bar x) \cap \Sigma$ is contained in the union of two cusps (and each cusp is not empty) with axes, almost parallel to $(ix)$, id est $|\angle((m\bar{x}],(ix))|<c$ and $|\angle((n\bar{x}],(ix))|<c$, where $\Sigma \cap B_\varepsilon(\bar x) \subset Q_\varepsilon^{m,\bar x}\cup Q^{n, \bar{x}}_\varepsilon$, for $ Q_\varepsilon^{m,\bar x} \in  \mathbb{Q}_\varepsilon^{m,\bar x}$, $ Q_\varepsilon^{n,\bar x} \in \mathbb{Q}_\varepsilon^{n,\bar x}$. 
\label{__3}
\end{enumerate}
\label{alm}
\end{lemma}
\begin{proof}
%окажем пункт~\ref{__1}. The points from the set $S_\Sigma$ can not be of order $1$, otherwise their small neighbourhood can be deleted. 
%НАДО ВЫВЕСТИ ИЗ ПРЕДЫДУЩЕЙ
\begin{enumerate}
  

\item Lets prove that  
%для произвольного $x \in E_\Sigma$ найдется такое $\rho>0$, что для каждого $\bar x \in B_\rho(\Sigma)\setminus \{ %x\}$, 
 $\oord_{\bar x}\Sigma = 1$ implies $\bar x\in X_\Sigma$. 
\label{QQ}
Assume the contrary: let $\bar x \in E_\Sigma \cap B_\rho(x) \setminus x$. 
% Энергетическое ребро или ребра, к которым они сходятся, должны лежать на прямой, почти параллельной $(ix]$ ввиду %Следствия~\ref{alm_parr}.  
%\end{itemize}

In view of Lemma~\ref{ordball_} it is suffices to analyze the following cases:
\begin{itemize}
\item [(a)] Case $\oordball_{\bar x}\Sigma=2$.
Let $\{\varepsilon_l\}$ be a decreasing to $0$ sequence of such numbers that $\sharp (\partial B_{\varepsilon_l}(\bar x) \cap \Sigma )=2$ and $\varepsilon_1 < \min (\rho, \rho-|\bar x x|)$. Denote  $s^l, t^l \defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$. 
We know from the item~\ref{WW} of Proposition~\ref{items} the inequalities $\angle ((s^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ and $\angle ((t^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ hold.%, то есть
%\begin{equation}
%s^l, t^l \in \Lambda((ix), \pi/3+o_\rho(1)).
%\label{LLL}
%\end{equation}
Then, due to the unit order of $\bar x$ there exists a converging to $\bar x$ sequence of such points $\{u_m\}\subset \Sigma$ that \[\angle\left((u_l\bar x),(ix)\right)=\frac{\pi}{2}.\] So we have a contradiction to the item~\ref{WWW} of Proposition~\ref{items}.


\item [(b)] Case $\oordball_{\bar x}\Sigma=1$. 

Let $\varepsilon_l>0$ be a decreasing to $0$ sequence of such numbers that $\sharp (\partial B_{\varepsilon_l}(\bar x) \cap \Sigma )=1$ and $s_l\defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$. Then in view of item~\ref{W} of Proposition~\ref{items} each line $(s_l\bar x)$ is almost perpendicular to $(ix)$:
\begin{equation}
\left|\angle \left((s_l\bar x), (ix)\right)-\frac{\pi}{2}\right| =o_\rho(1).
\label{99}
\end{equation}
Note that for every $\varepsilon_l$ holds
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)=\varepsilon_l+o_\rho(1)\varepsilon.
\label{100}
\end{equation}
The inequality $\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)\geq \varepsilon_l$ is true because of connectivity $\Sigma$ and the inequality in the other side is true in view of Lemma~\ref{Losiu}: otherwise one could replace $\Sigma$ by $\Sigma \setminus B_{\varepsilon_l}(\bar x) \cup [\bar{x}s_l]\cup S$, where $S$ is defined at Lemma~\ref{Losiu} for $w=\bar x$, and get a contradiction with optimality of $\Sigma$. 

So, for sufficiently small $\rho$  \begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)<\varepsilon_l \left(1+\frac{1}{18}\right).
\label{101}
\end{equation}
Then we can say (add elements to $\{\varepsilon_l\}$ if it is necessarily) that
\begin{equation}
\frac{\varepsilon_l}{\varepsilon_{l+1}}\leq \frac{18}{17}.
\label{103}
\end{equation}
Otherwise there exists such $\varepsilon_l$ that $\sharp ( \partial B_{\bar{\varepsilon}}(\bar x)\cap \Sigma)\geq 2$ for every $\bar{\varepsilon} \in [\frac{17\varepsilon_l}{18},\varepsilon[$. Thus, by co-area inequality, 
\[
\H \left(\Sigma \cap B_{\varepsilon_l}(\bar x)\right)\geq \H \left(\Sigma \cap B_{\frac{17\varepsilon_l}{18}}(\bar x)\right) +\H \left(\Sigma \cap B_{\varepsilon_l}(\bar x) \setminus  B_{\frac{17\varepsilon_l}{18}}(\bar x)\right)\geq \varepsilon_l \left (1+\frac{1}{18} \right),
\]
which contradicts to~\eqref{101}.
Note, as $\bar x$ has an energetic ray which is, in view of Corollary~\ref{alm_parr} $o_\rho(1)$-almost parallel to $(ix)$, there exists a sequence of energetic points $\{x_l\}$, converging to $\bar x$ such that $\angle ((x_l\bar x], (ix]) =o_\rho(1)+o_{|x_l\bar x|}(1)$.  The sequences $\{x_l\}$ and $\{ s_l \}$ with unit order $\oord_{\bar x}(\Sigma)=1$ imply the presence of also converging to $\bar x$ sequence of points $\{ u_l\}\subset \Sigma$ such that $\angle \left((u_l\bar x),(ix)\right) = \frac{\pi}{4}$. Consider an arbitrary element $u_m$ of this sequence. In view of the inequality~\eqref{103} there exists such number $l$ that
\begin{equation}
0<\varepsilon_l-|\bar xu_m|\leq \frac{1}{18}\varepsilon_l.
\label{104}
\end{equation}
Note also, that by~\eqref{99} the inequality
\[
\sharp (\partial B_{|\bar x u_m|}(\bar x)\cap \Sigma) \geq 2
\] 
holds.


%Можно также считать, что для произвольного $\delta \in [|\bar x u_m|,\varepsilon_l[$ выполняется $\sharp (\partial B_{\delta}(\bar x)\cap \Sigma) \geq 2$.

Let 
\[
k:=\max_{s \in \Sigma \cap \overline{B_{\varepsilon_l}}: \sharp (\Sigma \cap _{|s \bar x|}(\bar x))=1} \angle((ix),(\bar xs)),
\]
then $|k-\pi/2|=o_\rho(1)$.
Define also $K := \Lambda((p \bar x),k-\pi/2)$, where $(p\bar x) \perp (ix)$. $K$ contains an area of possible location of points $s_l$. 


%Кроме того, пусть $K \subset \Lambda((\bar x y(\bar x)), o_\rho(1))$ --- область возможного расположения точек $s_l$ (угол с вершиной в $\bar x$, раствором $o_\rho(1)$ и перпендикуляром к $(ix)$ в качестве биссектрисы), а 
Let $Q$ be a cusp or a union of two cusps with vertex at $\bar x$, containing all energetic points of  $B_{\varepsilon_l}(\bar x)$, then
\begin{equation}
d \defeq \dist(u_m, Q \cup K)\geq \frac{\sqrt{2}}{2}|\bar xu_m|-o_\rho(1)\varepsilon_l \geq (\frac{17}{18\sqrt 2}+o_\rho(1))\varepsilon_l,
%\label{105}
\end{equation}
where the last inequality follows from~\eqref{104}. 
%Ясно, что, ввиду единичного порядка $\bar x$ и определения компоненты связности $q$, выполняется $\H(q) \geq 2d$. В таком случае, ввиду неравенства коплощади для $\Sigma \setminus q$, верно
Then the length of the connected component of $\Sigma \setminus (Q \cup K)$, containing $u_m$, is greater or equal to $d$.
In view of co-area inequality, item~\ref{W} of Proposition~\ref{items} and inequality ~\eqref{101} the inequality $\H(\Sigma \cap K \cap B_\varepsilon(\bar x)) \geq \frac{17}{18}\varepsilon$ holds.
On the other hand \[
\H(\Sigma \cap B_{\varepsilon_l}(\bar x)) \geq H(\Sigma \cap B_{\varepsilon_l}(\bar x)\cap K)+\H(\Sigma \cap B_{\varepsilon_l}(\bar x) \setminus (K \cup Q)) \geq \frac{17}{18}\varepsilon_l +d\geq
\varepsilon_l (\frac{17}{18}+\frac{17}{18\sqrt 2}-o_\rho(1))>\frac{19}{18}\varepsilon_l.
\]
So we get a contradiction to the inequality~\eqref{101}.
\end{itemize}
\item% Let $\oord_{\bar x} \Sigma =2$ and $\bar x \in X_\Sigma$, и для некоторого $\varepsilon>0$ выполняется $\Sigma \cap \overline{B_{\varepsilon}(\bar x)}=[s\bar x] \sqcup [t\bar x]$. 
%\label{Q3}
The statement immediately follows from item~\ref{WWWW} of Proposition~\ref{items}.

\item% Докажем пункт~\ref{__3} Леммы.
%\begin{proof}
Because of items~\ref{BB} and~\ref{reb} Lemma~\ref{con} there exists $Q$ --- a cusp or a union of two cusps with vertex at $\bar x$ such that $G_\Sigma \cap B_{\varepsilon_0}(\bar x) \subset Q$ for sufficiently small $\varepsilon_0>0$. In view of Corollary~\ref{alm_parr} axes of these cusps are almost parallel to $(ix)$. If at least one energetic ray of $\bar x$ is two-orientated, the statement of the item is trivial because of Remark~\ref{star}. Similarly, the item is trivial if the rays are orientated to the different sides, id est for sufficiently small $\varepsilon_0>0$ points of $M$, corresponding to the energetic points from the set $B_{\varepsilon_0}(\bar x) \setminus \bar{x}$ are locates at both parts of the plane divided by energetic rays of $\bar x$. %Thus we can assume that every energetic rays are one-sided
Let $(q_l\bar x]$ be a ray, not coinciding with any of cusps' axes. Then, because of the definition of cusps, there exists such $\varepsilon_1>0$, that $(q_1\bar x] \cap Q \cap B_{\varepsilon_1}(\bar x)=\{\bar x\}$. We can also assume $\sharp (\Sigma \cap \partial B_{\varepsilon_1}(\bar x))=2$, as  $\oord_{\bar x} \Sigma =\oordball_{\bar x}\Sigma=2$ because of the item~\ref{QQ} of the proven Lemma, Remark~\ref{rem_ord} and Lemma~\ref{ordball_}. We will show that there exists such $\varepsilon_2>0$, that 
\[
B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x], 
\]
or 
\[
B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = \bar x. 
\]

%Пусть $(q_1\bar x]$ --- луч, лежащий во внутреннем угле и не совпадающий ни с одним энергетическим ребром $\bar x$. Тогда, ввиду определения псевдоконуса найдется такое $\varepsilon_1>0$, что $(q_1\bar x] \cap Q \cap B_{\varepsilon_1}(\bar x)=\emptyset$. Поскольку ввиду пункта~\ref{QQ} доказываемой леммы, замечания~\ref{rem_ord} и леммы~\ref{ordball_}, выполняется $\oord_{\bar x} \Sigma =\oordball_{\bar x}\Sigma=2$, потребуем, чтобы $\varepsilon_1>0$ удовлетворяло условию $\sharp (\Sigma \cap \partial B_{\varepsilon_1}(\bar x))=2$. Покажем, что тогда найдется такое $\varepsilon_2>0$, что 
%\[
%B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x], 
%\]
%либо 
%найдется такое $\varepsilon_2>0$, что 
%\[
%B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = \bar x. 
%\]
 Assume neither of the two cases come true. Then the set $\Sigma \cap B_{\varepsilon_1}(\bar x) \cap (q\bar x]$ contains infinitely many points close to $\bar x$. Herewith each point of the set $\Sigma \cap B_{\varepsilon_1}(\bar x) \cap (q\bar x]$ is not energetic and should be a center of a segment or a regular tripod.  
%, а множество $\Sigma \cap B_{\varepsilon}(\bar x) \setminus Q$ является штейнеровским лесом. 
By item~\ref{WWW} Proposition~\ref{items} ray $(qx]$ can not be perpendicular to $(ix]$. Let $L_1$ be an open area bounded by perpendicular to $(ix]$, passing through the point $\bar x$, $(q_1\bar x]$ and $\partial B_{\varepsilon_1}(\bar x)$, not containing any energetic points. Then $S := \overline{L_1\cap \Sigma}$ is a Steiner forest, with all infinitely many terminal points, except at most three from the set $\partial B_{\varepsilon_1} (\bar x) \cup \{ \bar x \}$, located at the perpendicular or at $(q\bar x]$. By Lemma~\ref{St_l} the perpendicular contains infinite number of terminal points of $ S$, thus there exists an infinite sequence of points $\{u_l\}$ such that $\angle((u_l,\bar x)(ix))=\pi/2$ for each $l$ which contradicts to item~\ref{WWW} of Proposition~\ref{items}. Ergo there exists such $\varepsilon_1>0$, that $\Sigma \cap (q_1\bar x] \cap \overline {B_{\varepsilon_1}(\bar x)}$ coincides with $\{\bar x\}$ or $(q_1\bar x] \cap B_{\varepsilon_1}(\bar x) $. We pick such $\varepsilon_1$ that also $\sharp(\partial B_{\varepsilon_1}(\bar x)\cap \Sigma)=2$ and $Q \cap B_{\varepsilon_1}(\bar x) \cap (q_1\bar x] = \emptyset$.

Let $(m\bar x]$ be an energetic ray of $\bar x$. Pick such decreasing to zero sequences $\{\bar{\varepsilon}_i \}$ and $\{ \gamma_i\}$, that 
\begin{itemize}
\item $Q \cap B_{\bar \varepsilon_i}(\bar x)$ is contained in the angle with bisector $(m\bar x]$ and size $2\gamma_i$;
\item the intersection of the borders of this angle (with bisector $(m\bar x]$ and size $2\gamma_i$) with the set $\Sigma \cap \cap B_{\bar\varepsilon_{i+1}}(\bar x)$ coincides with the point $\{ \bar x \}$ or with a boundary of a sector of $B_{\bar \varepsilon_{i+1}}(\bar x)$. 
\end{itemize}
Let $\gamma_1 \leq \pi/12$, $\bar \varepsilon_1 \defeq \varepsilon_1$.
If at some number (at most at one by Lemma~\ref{angles2}) the intersection is the segment, let $j$ be equal to this number. Otherwise let $j=0$.

Define the following cusp: \[
Q_1 \defeq Q^{m,\bar x}_{\overline{\varepsilon}_{j+1}}\defeq \bigcup_{i=j+1}^{\infty} \left(Q(m,\overline x, \gamma_i, \overline{\varepsilon_i}) \setminus B_{\overline{\varepsilon}_{i+1}}(\bar x)\right).
\]
If $\bar x$ has two energetic rays, similarly define the second cusp $Q_2$ with second energetic ray as the axis.

%$(a \bar x$ и $(b \bar x]$, то аналогично определим псевдоконус $Q^{b, \bar x}_{\bar \varepsilon_1}$
Thus an arbitrary connected component of $\Sigma \cap B_{\bar{\overline{\varepsilon_1}}}(\bar x)\setminus \{\bar x\}$ located inside the cusp $Q_1$ and $Q_2$ if it exists, or located outside of it. As $\bar x$ has an energetic ray, at least on of the components should lay inside, then it has a tangent line at the point $\bar x$, which coincides to energetic ray and so $o_\rho(1)-$almost parallel to $(ix]$. Then by Lemma~\ref{angles2} another component can not lay in the same cusp. 
If there is only one cusp there could be one ray $(q \bar x]$, which doesn't intersect the cusp and $\varepsilon_1>0$ such that a connected component in $B_{\varepsilon_1}(\bar x)$ coincides with the segment $(qx]\cap B_{\varepsilon_1}(\bar x)$. 
Then we can choose an arbitrary cusp with $(qx]$ as an axis. Otherwise similarly construct the second cusp for the second energetic ray with decreasing sequence of radii $\{\varepsilon_k\}$.
Note that as $\bar x$ (due to item~1 of this lemma) can not have a unit order due to the item~3 from the proof of the Lemma~\ref{angles2}) the set $\Sigma \cap B_{\bar \varepsilon}(\bar x)$ can not be located in the one cusp for any $\bar \varepsilon>0$. So by Lemma~\ref{angles2} there is certainly two cusps. Applying an item~\ref{WWWW} Proposition~\ref{items} we get that there is an infinite strictly decreasing to $0$ sequence $\varepsilon_k$ such that for $S_k,T_k\defeq \partial B_{\varepsilon_k}(\bar x)$ the inequality $|(\angle S \bar x], (ix] - \angle (T \bar x], (ix]| = o_\rho(1)$ holds, so the axes of both cusps should be $o_\rho(1)$-almost parallel to $(ix]$, which is required for $\varepsilon$ equal to minimum of $\varepsilon_1$ and $\overline{\varepsilon_1}$.  
\end{enumerate}
 
% \begin{remark}
 %Заметим также, то угол между ребрами, содержащий соответствующую $x^i_k$ точку $y^i$, не может быть меньше $\pi$ (если покрытые $x^i_k$ точки есть в обеих полуплоскостях, то угол между ребрами составляет ровно $\pi$).
 %\label{rovno}
 %\end{remark}
 \end{proof}



%Доказательство данной Леммы технически сложное и приведено полностью в разделе~\ref{new_proofs}.
\begin{corollary}
For every $x\in E_\Sigma$ and $c>0$ there exists such $\rho>0$ that for each point $\bar x \in B_\rho(x)\cap \Sigma \setminus \{ x\}$ there exists a one-sided tangent of $\Sigma$ at it. 
Moreover if $\bar x \in E_\Sigma$ then there are exactly two one-sided tangent at the $\bar x$ with angle, greater than $\pi-c$ between it.
Existence of one-sided tangents (one, two or three of them) and the size of angles between them in case $\bar x \in X_\Sigma \cup E_\Sigma$ immediately follows from Proposition~\ref{discr_str}. 
\label{1sdd}
%$\bar x$ \in $S_\Sigma$ there are two or three  one-sided tangents with angles of size $\pi$ or $2\pi/3$ between them correspondingly;
\end{corollary}
\begin{remark}
By the compactness of $E_\Sigma$ one can swap the predicates in Lemma~\ref{alm}: $ \forall c>0 \ \exists \rho>0 \ \forall x \in E_\Sigma \ldots$
\end{remark}


\begin{corollary}

In the notations of item~\ref{__2} Lemma~\ref{alm} 
\begin{enumerate}
    \item the inequality $|\angle t \bar x y - \angle y \bar x s| <c$ holds, where $y$ is the limit point of the points corresponding to energetic points of the energetic ray $(ix]$ converging to $x$; 
    \item also the inequality  $|\angle s\bar xt| \geq 2\pi/3$ holds, and hence $\angle((s\bar{x}), (ix)) \leq \pi/6+c$ and $\angle((t\bar{x}), (ix)) \leq \pi/6+c$;
    \item %let $\Sigma' \supset \{s,\bar x, t \}$ is a connected component of $\Sigma \setminus \{x\}$, and let us define some open area $U\in x$ such that $\sharp(\partial U \cap \Sigma')=1$. Assume, without loss of generality, that points $s,\bar x, t,x$ located at $\Sigma'$ in the same order. Then
%    let there exists a path in $\Sigma$ from $s$ to $x$ containing $t$ (and thus $\bar x$). Then $-\pi/6-c \leq \angle((s\bar{x}], (ix]) \leq \pi/6+c$ and $\angle((t\bar{x}], (ix]) \geq 5\pi/6+c$ or $\angle((t\bar{x}], (ix]) \leq -5\pi/6-c$. Moreover, if $\angle ((ix],(yx]) \geq 0$ (and hence almost equal to $\pi/2$) then $-c \leq \angle((s\bar{x}], (ix]) \leq \pi/6+c$ and $\angle((t\bar{x}], (ix]) \geq 5\pi/6-c$.
let there exists a path in $\Sigma$ from $\bar x$ to $x$ containing $t$. Then $\angle((s\bar{x}], (ix]) \leq \pi/6+c$ and $\angle((t\bar{x}], (ix]) \geq 5\pi/6-c$. Moreover, if $\angle ixy >0$ (i.e. equal to $\pi/2$ up to $c$), then $\angle s\bar x y>0$ (and belongs to $[\pi/2-c; \frac{2}{3}\pi+c]$) and $\angle t\bar x y<0$.
\end{enumerate}
\label{sm_an}
\end{corollary}
\begin{proof}
The first item is trivial and the second one follows from the first by Lemma~\ref{angles2}. So we only have to prove the third one. Let $\Sigma'$ be a connected component of $\Sigma \setminus \{ x\}$. Then there exists such open area $U \subset B_\rho(x)$ that $\sharp (\partial U \cap \Sigma')=1$. We can also assume that $\bar x, s, t \in U$. 
Note that there exists such $\bar y=y(\bar x) \in M$ that 
\[
B_r(\bar y) \cap \Sigma =\emptyset = B_r(y) \cap \Sigma  
\]
and 
\[
B_r(\bar y) \cap B_r(y) \neq \emptyset.
\]
Thus, if the proving statement is not true and $\angle((s\bar{x}], (ix]) \geq 5\pi/6-c$ then the point $s$ is inside the area, bounded by $\partial B_r(y)$, $\partial B_r(\bar y)$ and by the path from $\bar x$ to $x$, located in $B_\rho(x)$. But if there are any energetic points in this area, the points of $M$, corresponding to it, are located in the same half-plane with respect to $(ix)$ as $y$. But the path, that began from $\bar x-t$ should contain an energetic point with corresponding point from the another half-plane. 
\end{proof}

%В следующей лемме показано, что если компонента связности минимайзера $\Sigma \setminus \{x\}$ содержит сходящуюся к $x$ бесконечную последовательность энергетических точек ребра, то она является дугой.


Let us prove the following technical lemma:
\input{pictures/dvapo}

\begin{proposition}
For an arbitrary $x \in E_\Sigma$ and $\bar c>0$ there exists such $\rho>0$, that if $\Sigma \cap B_\rho(x)$ contains a polyline $L_1-L_2-L_3-L_4-L_5$, the nodes of which are energetic points of the same energetic ray $(ix]$ and all its internal points are of order $2$, then $\angle((L_jL_{j+1}),(ix)) \leq \bar c$ for every $j=1, \dots, 4$ (see Fig.~\ref{fig:dvapo}).  
\label{brrrr}
\end{proposition}
\begin{proof}
Let $\rho>0$ be such small that conditions of Lemma~\ref{alm} for $c=\bar c/10$ holds. Assume the contrary to the desired statement: id est $\angle((L_jL_{j+1}),(ix) > \bar c$ for some $j\in\{1,\dots,4\}$. Due to  Lemma~\ref{alm} points $L_1$,\ldots, $L_5$ belong to $X_\Sigma$ and the inequality $\angle((L_jL_{j+1}),(ix))> \bar{c}/2$ holds for every $j=1,2,3,4$. By Remark~\ref{rem_cc}, for sufficiently small $\rho>0$ $\angle ((L_{j-1}L_{j}],(L_{j+1},L_j]) \leq \pi-\bar c/2$ for $j \in \{2,3,4\}$, so points of $M$ corresponding to $L_j$ with odd and even indices located at the different semi-plane with respect to $(ix)$. %Really, from Remark~\ref{rem_cc} we have $|\angle((ix), (L_jy(L_j))-\pi/2|<\bar c/10$ for every $j\in 1, \ldots, 5$, 
Note that the ratio between the lengths of the sides of the polyline is linear. Really, by law of sines and the inequality $\angle L_{j-1}L_jL_{j+1}\geq 2\pi/3$ we get
\[
\frac{|L_{j-1}L_j|}{|L_jL_{j+1}|}=\frac{\sin \angle L_{j-1}L_{j+1}L_j}{\sin \angle L_jL_{j-1}L_{j+1}}\geq \frac{\sin (c/2+o_\rho(1))}{\sin (\pi/3)}\geq \frac{\bar c}{3}.
\]
On the other hand
\[
\frac{|L_{j-1}L_j|}{|L_jL_{j+1}|}=\frac{\sin \angle L_{j-1}L_{j+1}L_j}{\sin \angle L_jL_{j-1}L_{j+1}}\leq \frac{\sin \frac{\pi}{3}}{\sin (\bar c/2+o_\rho(1))}\leq \frac{3}{\bar c}.
\]
Thus we get \[\frac{\bar c}{3} \leq \frac{|L_{j-1}L_j|}{|L_jL_{j+1}|}\leq \frac{3}{\bar c}\]
for every $j\in \{2,3,4\}$.
 Then the replacement the polyline $L_1-L_2-L_3-L_4-L_5$ by the polyline $L_1-L_2-L_4-L_5$ reduces the length by amount, linearly dependent on  $|L_1L_2|$:
 \begin{multline*}
 |L_2L_3|+|L_3L_4|-|L_2L_4|=\frac{(|L_2L_3|+|L_3L_4|)^2-|L_2L_4|^2}{|L_2L_3|+|L_3L_4|+|L_2L_4|}>\\
 > \frac{2|L_2L_3||L_3L_4| (1+ \cos \angle L_2L_3L_4)}{2(|L_2L_3|+|L_3L_4|)}\geq
 \frac{|L_3L_4|(1- \cos \frac{\bar{c}}{2})}{ \left (1+\frac{|L_3L_4|}{|L_2L_3|} \right)}\geq  \frac{\bar{c}^4}{24(1+\frac{3}{\bar{c}})}|L_1L_2|.
\end{multline*}
Let $A'$ be a figure bounded by $[L_1,L_5]$, $\partial B_r(y(L_1))$ and $\partial B_r(y(L_3))$. The boundary of $A'$ is the union $[L_1L_5] \cup \breve{L_1C} \cup \breve{L_5C}$ where $C$ is a point of intersection $\partial B_r(y(L_1))$ and $\partial B_r(y(L_3))$. Note that $\dist(C,(L_1L_5))=o(|L_1L_5|)=o(|L_1L_2|)=o(\rho)$. Thus there exists a set $S=S_1\cup S_5$ such that $\H(S) = o(|L_1L_2|)$, $L_j\in S_j$ and $S_j$ is connected for $j\in \{1;5\}$. And we also will impose some condition on the energy of $S$. Let $L_j'$ be such point that $L_1'$,$C$ and $L_5'$ lie on the same line parallel to $(L_1L_5)$ and $(L_jL_j')\perp (L_1L_5)$ for $j\in \{1;5\}$. And let $C'$ be such point that $|CC'|=r$,$(CC')\perp (L_1L_5)$ and $[CC')\cap (L_1L_5)=\emptyset$. Now let $L_j''\defeq \partial B_r(C')\cap [L_i'C']$ for $i\in \{1;5\}$. Then $S\defeq [L_1L_1']\cup [L_1'L_1'']\cup [L_5L_5']\cup [L_5'L_5'']$. Thus $\H(S)=o(|L_1L_2|)=o(\rho)$. 
It is easy to see that the connected set  
\[
S \cup [L_1L_2] \cup [L_2L_4]\cup [L_4L_5]
\]
for sufficiently small $\rho>0$ has strictly smaller length and not greater energy than $\Sigma$, so we get a contradiction with optimality of $\Sigma$.
  \end{proof}

\begin{lemma}
Let $x \in E_\Sigma$ and let there exist such a  cusp $Q\in \mathbb{Q}^{a,x}_\varepsilon$ that $Q^{a,x}_\varepsilon \cap \Sigma$ is an arc. Then for each $c>0$ there exists such $\varepsilon=\varepsilon(c)>0$ that every one-sided tangent at the points of the set $Q^{a,x}_\varepsilon \cap B_{\varepsilon(c)}(x) \cap \Sigma$ has an angle not greater than $2c$ with a line $(ax)$.
\label{zapred}
\end{lemma}

\begin{proof}
Assume the contrary, id est there exists a sequence of points with one-sided tangents having an angle with $(ax)$ greater than $2c$, converging to $x$. Without loss of generality assume $c<\pi/2$. By item~\ref{__3} of Lemma~\ref{alm} for sufficiently small $\varepsilon$ this sequence consists only on the points of $X_\Sigma \sqcup S_\Sigma$. As there is no branching points, the direction of tangents doesn't change at points of $S_\Sigma$, that is there is a sequence of points from $ X_\Sigma $ converging to $ x $ such that at least one of the two segments incident to the point has an angle with $ (ax) $ greater than $ 2c $. Let $L_1$ be such a point and let $\varepsilon$ be chosen not greater than $\rho$ for $c/5$ in Lemma~\ref{alm}. By item~\ref{__2} of Lemma~\ref{alm} both segments incident to $L_1$ has an angle with $(ax)$ greater than $9/5c$. Then the segment lying on the path from $L_1$ to $x$ should end with point $L_2\in X_\Sigma $. But the segment leaving $ L_2 $ must have an angle with $ (ax) $ greater than $ 8/5c $ and end with point $ L_3 \in X_\Sigma $. Thus for any arbitrarily small $ \bar \varepsilon$ there exists a broken line $ L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\bar \varepsilon} (x) $ such that all angles $ \angle ((L_jL_{j + 1}), (ax))> c $ for $j = 1,2,3,4 $. This is a contradiction with Proposition~\ref{brrrr}.
\end{proof}


\begin{lemma}
Let $x\in E_\Sigma$. 
\begin{enumerate}
\item Let $\Sigma'$ be a closure of a connected component of $\Sigma \setminus \{x\}$, let $(ax]$ be one-orientated energetic ray, let $\Sigma'$ contain an infinite sequence of energetic points of $(ax]$ converging to $x$, and doesn't contain (in the neighbourhood of $x$) any energetic points of other energetic rays.
%other converging to $x$ sequences of energetic points. 
Then there exists such 
$\rho_1>0$ that $\Sigma'\cap B_{\rho_1}(x)$ is an arc and contained in a cusp $Q \in \mathbb{Q}_{\rho_1}^{a,x}$.
\label{0}
\item If there exists such a cusp $Q\in \mathbb{Q}_\rho^{a,x}$ that $\Sigma \cap \partial Q \subset \{x\} \cup \partial B_\rho(x)$, then 
%$\Sigma \cap Q$ содержит конечное число точек ветвления.% Более того, 
there exists such $\rho_2>0$, that $Q \cap B_{\rho_2}(x) \cap \Sigma$ is an arc or coincides with the point $\{x\}$.
%(we consider a point as a special case of an arc).
%При ��том прямые содержащие односторонние касательные к $\Sigma $ в точке $\bar x$  стремятся к $(ax)$ при $\bar x \rightarrow x$.
\label{A}
\item  Let $\Sigma'$ be a closure of a connected component of $\Sigma \setminus \{x\}$, let $(ax]$ be an energetic ray, let $\Sigma'$ contain an infinite sequence of energetic points of $(ax]$ converging to $x$, and doesn't contain (in the neighbourhood of $x$) any energetic points of other energetic rays. Then there exists such 
$\rho_1>0$ that $\Sigma'\cap B_{\rho_1}(x)$ is an arc and is contained in a cusp $Q \in \mathbb{Q}_{\rho_1}^{a,x}$.
\label{AB}
\end{enumerate}
\label{uggi}
\end{lemma}
%Доказательство данной леммы технически сложное и приведено полностью в разделе~\ref{new_proofs}.
\begin{proof}
Let us prove item~\ref{0}. \begin{proof}
Without loss of generality we assume that $(ax] $ is the negative half of the abscissa axis, $ \rho $ is such that all points corresponding to the energetic points of $ \Sigma' \cap B_\rho(x) $ are located in the upper half-plane (we work in a neighbourhood of $x$, so it is possible due to item~\ref{1115} of Lemma~\ref{Losiu}) and $\sharp (\partial B_\rho(x) \cap \Sigma')=\oordball_x\Sigma'$ and $z\in \partial B_\rho(x) \cap \Sigma'$ is such that the path between $z$ and $x$ is contained in $\overline B_\rho(x)$. 


We will monitor changes in the slope of the one-sided tangent to the arc $\breve{[zx[}$, where as a connected component we will choose a one containing $z$. By Corollary~\ref{1sdd} for sufficiently small $\varepsilon>0$ such one-sided tangent exists at each point of $\breve{[zx[}$ (and, due to the finite length of $\Sigma$, almost everywhere is contained in the tangent line at the same point).

Thus we can define 
$ \turn (\breve {[zx]}) $ as the upper limit (supremum) over all sequences of points of the curve:
  \[
 \turn(\breve{[zx]})=\sup_{n\in \N, z\preceq t_1 \prec \dots \prec t_n \prec x} \sum_{i=2}^{n} \widehat{t^i,t^{i-1}},
 \]
 where $ t ^ i $ denotes the ray of the one-sided tangent to the curve $ \breve {[zt_i]} \subset \breve {[zx[} $ at the point $t_i$, and $ {t_1, \dots, t_n}$ is the partition of the curve $ \breve{[zx[} $ in the order corresponding to the parameterization, for which $ z $ is the beginning of the curve and $ x $ is the end. In this case, the angle $ \widehat (t^i, t^{i+1}) \in [-\pi, \pi [$ between two rays is counted from ray $ t^i $ to ray $ t^{i+1} $; positive direction is counterclockwise.
 
Note that in view of $B_r(y(x))\cap \breve{[zx]} = \emptyset$, it is true that
 \[
|\turn ([zx])|  < 2 \pi.
 \]
Let us show that there are finitely many branching points on the path from $ z $ to $ x $. To do this, consider an arbitrary branching point $ D_2 $ on the arc $ \breve {[zx]} $.
Three segments $ [D_1D_2] $, $ [D_2D_3] $ and $ [D_2C] $ with pairwise angles $ 2 \pi / 3 $ emerge from the point $ D_2 $, where, without loss of generality, the broken line $ D_1-D_2-D_3 $ is a subset of the path from $ z $ to $ x $. Note that the contribution to the turn $ \breve {[zx]} $ of the point $ D_2 $ is $ - \pi / 3 $, since the counterclockwise angle $ \widehat{ D_1D_2D_3} $ is $ 2 \pi / 3 $. This is so, since the path that started from the segment $ [D_2C] $ must end with an energy point, and therefore must go to the upper half of the ball $ B_\rho (x) $.
 The same is true for an arbitrary branching point inside the path from $ z $ to $ x $.
 
For sufficiently small $\rho$ from Lemma~\ref{alm} and Corollary~\ref{sm_an} %, the fact that the edge $ (ax] $ is orientated upwards and thus for each energetic point $\bar x \in B_\rho(x)\setminus \{x\}$ there exists the ball $B_r(y(\bar x))$ such that $y(x)$ lays in the upper half-plane and $B_r(y(\bar x))\cap \Sigma =\emptyset$, and there also $B_r(y)\cap \Sigma =\emptyset$, where $y$ (also from the upper half-plane) is a limit point for points corresponding to energy points of energetic ray $(ax]$ and thus $B_r(y)\cap B_r(y(\bar x)) \neq \emptyset$, the fact that the path $\breve{]zx]}$ lay in $B_\rho(x)$ --- all these facts implies that 
we get that the angle of the tangent direction at the arbitrary energetic point $\bar x$ on the path from $ z $ to $ x $ changes clockwise (the change at $\bar x$ does not exceed $ \pi / 6 + o_\rho(1)$), that is, the contribution to $ \turn $ is non-positive.

So there is a positive $ \rho_4 <\rho $ such that $ \breve {[zx]} \cap \overline B_{\rho_2} (x) $ does not contain branching points and thus is an arc.
Moreover, due to Lemma~\ref{dug_ok} there exists such positive $\rho_1<\rho_4$ and such a cusp $Q\in \mathbb{Q}^{a,x}_{\rho_1}$ that $\breve{[zx]}\cap B_{\rho_1}(x) \subset Q$ and $\sharp(\partial B_{\rho_1}(x) \cap \breve{[zx]})=\oordball_z\breve{[zx]}=1$.
\end{proof}
\begin{remark}
In this way, we have proved that a point $x \in E_\Sigma$ can be the limit of branching points only if it has a two-orientated energetic ray.
\label{remA}
\end{remark}

Let us prove item~\ref{A}.
\begin{proof}
Let $ \rho_2>0 $ satisfy the assertion of the Lemma~\ref{alm} for $ c = \frac{\pi}{100} $ and the assertion of the Lemma~\ref{zapred} for $ c = \frac{1}{20} $.In addition, we choose $ \rho_2> 0 $ such that
\[
\sharp(\Sigma \cap Q \cap \partial B_{\rho_2}(x))=\oordball_x(\Sigma\cap Q)\leq \oordball_x(\Sigma)\leq 3. 
\]
Clearly, $\oordball_x(\Sigma \cap Q)=1$: otherwise by co-area inequality one could decrease length of $\Sigma$ by replacing $\Sigma \cap Q$ with $T^Q$, which is defined in the proof of Lemma~\ref{angles2} and has a length $\rho_2 +o(\rho_2)$. Then energy will not increase and connectivity will remain, so we have a contradiction with an optimality of $\Sigma$. 

 Thus we assume $\sharp (\partial B_{\rho_2}(x) \cap \Sigma) =1$.
Let $Q_1 \defeq Q \cap \overline{B_{\rho_2}(x)}$ and $z \defeq \partial Q_1 \cap \Sigma$. 
We have to check only the case when the energetic ray $(ax]$ is two-orientated (if $(ax]$ is not an energetic ray at all everything is clear).

Assume $Q \cap \Sigma$ contains infinite number of branching points, then it also contains infinitely many terminal points. 

As $\sharp (\partial B_{\rho_2}(x) \cap \Sigma)=1$, each branching point in the path from $z$ to $x$ is connected with a terminal point by a segment. Suppose the contrary. In this case, on the path from $ z $ to $ x $, there is a branching point $ A $ connected to a branching point $ B $ that does not lie on the path from $ z $ to $ x $. Moreover, at least one of the two segments $ \Sigma \setminus [AB] $ incident to $ B $ is not perpendicular or parallel to $ (ax] $ up to $ \pi / 100 $, so it inevitably ends with a branching point, from which at least one segment also originates that is not perpendicular or parallel to $ (ax] $ up to $ \pi / 100 $, and so on. Thus there is a path that starts with this segment and never ends, and the segments of the same parity are parallel. It is easy to see that the limit point $ w $ of this path must belong to $E_\Sigma$ and lie in the ball $ B_\rho (x) $, due to Remark~\ref{remA}, its energetic ray should be two-orientated. But then (for sufficiently small $\rho_2>0$) $\partial B_{|xw|}(x) \cap \Sigma \cap Q_1=\{w \}$ which contradicts to the existence of the path from $z$ to $x$ lying in $Q_1 \cap \overline{B_{\rho_2}(x)}$ and is not containing $w$. So we have a contradiction to the assumption of the existence on the path such a branching point, which is not connected to a terminal point.

Thus, by item~\ref{__1} of Lemma~\ref{alm} in every branching point at the path from $z$ to $x$ the angle between a one-sided tangent to a path and a line $(ax)$ is modulo belongs to the interval $[\pi/6-\pi/100, \pi/6+\pi/100]$. Let $D_1$ be a branching point at the path of $\Sigma$ from $z$ to $x$, and let $[D_1;D_2]$ be a maximal segment of the path of $\Sigma$ from $D_1$ to $x$. As $|\angle (D_1D_2), (ax) -\pi/6|<\pi/100$, the point $D_2$ can be an isolated energetic point with order $2$ or a branching point only. If $D_2$ is a branching point then, similarly, the end of the maximal segment $[D_2;D_3]$ on the path, can be an isolated energetic point with order $2$ or a branching point only, and the angle $\angle((D_2D_3),(ax))=\pi/3-\angle((D_1D_2),(ax))$, and so belongs to the interval $[\pi/6-\pi/100, \pi/6+\pi/100]$. If $D_2$ is an isolated energetic point with order $2$ then, by item~\ref{__2} of Lemma~\ref{alm}
\[
\angle((D_2D_3),(ax)) \in [\angle((D_1D_2),(ax))-\pi/100, \angle((D_1D_2),(ax))+\pi/100] \subset [\pi/6-\pi/50,\pi/6+\pi/50],
\]
where $[D_2;D_3]$ is the maximal segment on the path from $D_2$ to $x$.
Thus, the path from $ D_1 $ to $ x $ starts with a polyline. In this case, the angle between the one-sided tangent and the straight line $ (ax) $ at the nodes of the polyline either belongs to the interval $ [\pi / 6- \pi / 100, \pi / 6 + \pi / 100] $ (if the node was a branching point), or changes by an amount not exceeding $ \pi / 100 $. Thus, in view of the Proposition~\ref {brrrr}, among the first four nodes of the polyline after $D_1$, there must be a branching point $ C $. Moreover, since all one-sided tangents to the path points between $ D_1 $ and $ C $ have an angle with $ (ax) $ greater than $ \pi / 6- \pi / 20> \pi / 10 $, there will be no points from the set $E_\Sigma$.
%, the path $ \breve{[zx]} $ cannot contain a polyline with five nodes in a row at energy points, one-sided tangents in which have an angle with $ (ax) $ greater than $ 1/10 $,
Repeating the reasoning for the point $ C $ as $ D_1 $, and then iterating, we get the path $ \sigma $, all one-sided tangents along which have an angle with $ (ax) $ greater than $ 1/10 $. Let $ \bar x $ be the limit point of such a path ($ \bar x $ belongs to the path from $ z $ to $ x $ and may coincide with $ x $). It is clear that $ \oordball_{\bar x}\sigma= 1 $. Let $ \rho_0> 0 $ be sufficiently small and such that
\[
\sharp (\sigma \cap \partial B_{\rho_0}(\bar x))=1.
\]
Define \[z_0=z_0(\rho_0) \defeq \partial B_{\rho_0}(\bar x) \cap \sigma.\]
Let $(a_0\bar x]$ be an energetic ray  of $\bar x$ closest to an infinite sequence of energetic points of $\sigma \cap B_{\rho_0}(\bar x)$.
Then, as $(a_0\bar x]$ due to item~\ref{0} and Remark~\ref{star} is two-orientated energetic ray, then
\[
\angle z_0\bar xa_0=o_{\rho_0}(1)
\]
and 
\begin{equation}
   \H(\sigma \cap B_{\rho_0}(\bar x))=\rho_0+o_{\rho_0}(1).
    \label{smll}
\end{equation}
On the other hand $\angle ((ax], (a_0\bar x])=o_{\rho_2}(1)$  and thus, for sufficiently small $\rho_0$ and $\rho_2$, all one-sided tangents to $\sigma \cap B_{\rho_0}(\bar x)$ have angles with $(a_0\bar x]$, greater than $\pi/10$. But it means that 
\[
\H(\sigma \cap B_{\rho_0}(\bar x)) \geq \frac{Pr_{(a_0\bar x]}(\sigma \cap B_{\rho_0}(\bar x))}{\cos \frac{\pi}{10}}\geq \frac{Pr_{(a_0\bar x]}([z_0\bar x])}{\cos \frac{\pi}{10}} \geq \frac{\cos \angle  z_0\bar x a_0}{\cos \frac{\pi}{10}}|z_0 \bar x|=\frac{\cos (o_{\rho_0}(1))}{\cos \frac{\pi}{10}}\rho_0.
\]
So we get a contradiction with~\eqref{smll}. 
\end{proof}
And now we have to prove item~\ref{AB}. 
\begin{proof}
If $(ax]$ is one-orientated energetic ray, then item~\ref{0} implies the statement. If $(ax]$ is two-orientated then, by Remark~\ref{star}, $\Sigma' \cap B_\rho(x)$ is contained in a cusp for sufficiently small $\rho>0$ and then item~\ref{A} of Lemma~\ref{uggi} implies the result.  

\end{proof}

\end{proof}
\begin{corollary}
Item~\ref{__3} of Lemma~\ref{alm} can be formulated as follows: if $\bar {x} \in E_\Sigma \setminus x $, then $ \exists \varepsilon : B_\varepsilon (\bar x) \cap \Sigma $ is an arc contained in the union of two cusps with axes almost parallel to $(ix)$ where these axes are one-sided tangents to $\Sigma$ at the point $\bar x$.
\label{notv}
\end{corollary}
\begin{remark}
As in Corollary~\ref{sm_an} in the notations of Corollary~\ref{notv} a path in $\Sigma$ from $\bar x$ to $x$ has a one-sided tangents almost parallel (not almost complementary) to $(ix]$.
\label{retv}
\end{remark}

And now we are finally ready to prove the following lemma, in which it is stated that no connected component of the $ \ Sigma \setminus \{ x \}$ can contain infinite sequences of energy points of two different energetic rays converging to $ x $.
\begin{lemma}
Let $\Sigma$ be the a minimizer, $(ax]$ and $(bx]$ be two different energetic rays with vertex at $x$ and cusps $Q^{a,x}_\rho \in \mathbb{Q}^{a,x}_\rho$ and $Q^{b,x}_\rho \in \mathbb{Q} ^{b,x}_\rho$ be such that $G_\Sigma \cap \overline{B_\rho(x)} \subset  Q^{a,x}_\rho \cup Q^{b,x}_\rho$ for some $\rho>0$. Let $\Sigma'$ be the connected component of $\Sigma \setminus \{x\}$ containing an infinite sequence of points from the set $G_\Sigma \cap  Q^{a,x}_\rho$, converging to $x$. Then there exists such $\rho_3>0$, that 
\[
\Sigma' \cap G_\Sigma \cap  Q^{b,x}_\rho \cap \overline {B_{\rho_3}(x)} = \{x\}.
\]
\label{eva}
\end{lemma}
%возможно вернем потом:
%Доказательство данной Леммы технически сложное и приведено полностью в разделе~\ref{new_proofs}. 
The sketch of the proof is as follows: suppose the opposite, let $ \Sigma '$ contain an infinite sequence of points from the set $G_\Sigma \cap  Q^{b,x}_\rho$, converging to $x$. Then
\begin{enumerate}
\item[Step 1.] There exists such $\rho_1>0$, that $\Sigma' \cap \overline {B_{\rho_1}(x)} \setminus \{ x\}$ doesn't contain the points from $X_\Sigma$ with order $2$ except the ones with incident segments $o_\rho(1)$-almost parallel to the closest energetic ray $(ix]$.
\item[Step 2.] There exists such $\rho_2>0$, that $\Sigma' \cap \overline {B_{\rho_2}(x)}\setminus \{ x\}$ doesn't contain any energetic points with order $2$
\item[Step 3.] The angle $\angle ((ax],(bx])$ can be only $\pi/3$, $2 \pi/3$ or $\pi$.
\item[Step 4.] Obtaining a contradiction in each of the three possible cases.
\end{enumerate}
\begin{proof}
In view of the assumption that the assertion of the lemma is incorrect, we can assume that each of the energetic rays is one-orientated. Let's denote the value of the internal angle between the rays by $ \alpha$ (id est the angle doesn't contain any points corresponding to $x$): $ \alpha \defeq \angle ((ax],(bx]) \leq \pi $. It is possible, without loss of generality, to consider $ \rho_1 \leq \rho $ such that the statements of Lemma~\ref{alm} for $ c \defeq \alpha / 100 $ hold and that for every point $z \in Q^{i,x}_{\rho} \cap \overline{B_{\rho_1}(x)}$ the inequality $|\angle zxi |\leq \alpha/100$ holds, where $i=a,b$. We also get such a small $\rho_1$ that all points corresponding to the same energetic ray (excluding $x$) are located at the same semi-plane with respect to the line containing this energetic ray (It is possible due to item~\ref{1115} of Lemma~\ref{Losiu}). % And we also ask $\sharp \partial B_{\rho_1}(x) \cap \Sigma =\oordbal_x \Sigma$.
In the proof we still use the formulation ``the values \ldots are equal to within $ \bar c $ '', which mean that the absolute value of the difference between the values does not exceed $ \bar c $. %И ПРО ALMOST 
Let area $U \ni x$ be such that $U \subset B_{\rho_1}(x)$ and $\sharp (\partial U \cap \Sigma)=\oord_x\Sigma$. Then $\sharp (\partial U \cap \Sigma')=1$, and hence for each point $\bar x \in \Sigma' \cap U \setminus{x}$ there exists only one path to $\partial U$, and the path from $\bar x$ to $x$ is contained in $U \subset B_\rho(x)$. %Choose such $\rho_4>0$, that $B_{\rho_4}(x) \subset U$ and that for every point $z \in Q^{i,x}_{\rho_4}$ the inequality $\angle zxi \leq \alpha/100$ holds.

\begin{itemize}

\item{Step 1.} For any point $ \bar {x} \in G_\Sigma \cap \Sigma'\cap U \setminus \{x \} $ with $\oord_x\Sigma =2$, the tangent rays to $ \bar x $ are $\alpha/10$-almost parallel to the nearest energetic ray $(ix]$.
%In other words, for every $c>0$ there exists such $\rho>0$ that for every open area $U\subset B_\rho(x)$ such that $\sharp(\partial U \cap \Sigma)=\oord_x\Sigma$ and $x\in U$, for each energetic points $\bar x \in G_\Sigma \cap U$ w  ith $\oord_$

%РАЗОБРАТЬСЯ С РОШКАМИ

Assume the contrary: let there exists such an energetic point 
$\bar x \in B_{\rho_1}(x) \setminus \{x\}$ with order $2$ that it has a tangent ray with angle with the closest to $\bar x$ energetic ray greater then $\alpha/10$. Thus by item~\ref{AB} Lemma~\ref{alm} the point $\bar x$ belongs to $X_\Sigma$ and hence there exists nontrivial segments $[s\bar x], [t\bar x] \subset \Sigma$. Without loss of generality let $[\bar x t]$ be the maximal segment in the path from $\bar x$ to $x$. Thus, by Corollary~\ref{sm_an}, as $\bar x \in Q^{i,x}_{\rho_1}$, $\angle ((t\bar x],(i x]) \leq \pi/6 +\alpha/100$. So
\begin{equation}
\alpha/10 <\angle ((t\bar x],( x \bar x])\leq \pi/6 +\alpha/50.
\label{hu}
\end{equation}
Without loss of generality let $i \defeq a$. The point $t$ can not be an energetic point of the energetic ray $(ax]$ due to Lemma~\ref{alm} and Corollaries~\ref{sm_an} and~\ref{notv}. It also can not coincide with $x$ due to definition of $Q^{a,x}_{\rho_1}\ni x$. Thus point $t$ can be a branching point or an energetic point (of order $2$) of the energetic ray $(bx]$.
% \textcolor{red}{
%The point $t$ also can not be an energetic point of the energetic ray $(bx]$ if $\alpha +\angle t\bar x x \geq \pi/6+\alpha/50$ as $\angle \bar x t x = \pi-\alpha - \angle t\bar x x$ and hence  $\angle \bar x t x  \leq 5\pi/6 -\alpha/50$. It means that, by Corollary~\ref{sm_an} point $t$ can not be an energetic point (of order $2$) at the path from $\bar x$ to $x$.}

%если в каждой точке ветвления 
%$\angle x x^a_1 t=\angle((ax),(x^a_1x))$ (а не $\pi-\angle((ax),(x^a_1x))$). 
 
 \input{pictures/trash/norm1}
\input{pictures/trash/norm2}
\input{pictures/trash/norm11}

\begin{enumerate}
\item Let $t$ be a branching point and let $C$ be such a point that $[tC]$ is a maximal segment in $\Sigma$ 
%and $C$ lays inside the triangle bounded by $(ax]$, $(bx]$ and $(\bar x t)$. Then, by~\eqref{hu},
%if $\pi/3<\angle t\bar x x$ the ray $[tC)$ doesn't intersect $(ax]$ and hence $C$ can not be an energetic point of the energetic ray $(ax]$, otherwise
and the angle $\angle ((tC], (ax])=\pi/3-\angle ([t\bar x),(x \bar x])$. Thus $C$ can not be an energetic point of the energetic ray $(ax]$ of order $1$. Then the following cases are possible:
\begin{enumerate}
    \item $C$ is an energetic point of the energetic ray $(ax]$ of order $2$. By Corollary~\ref{sm_an} $ \angle ((tC], (ax]) \leq \pi/6+\alpha/100$. %and hence
    %\[
    %\angle ((tC], (ax])=\pi/3-\angle t\bar x x \leq \pi/6+\alpha/100,
    %\]
    %id est 
    %\[
    %\angle t\bar x x \geq \pi/6-\alpha/100.
    %\]
    %On the other hand $t\bar x x \leq \pi/6+\alpha/100$ by Corollary~\ref{sm_an} as $\bar x$ is an energetic point of the energetic ray $(ax]$ of order $2$. Thus $\angle t\bar x x$ is equal to $\pi/6$ within $\alpha/100$.
    Hence $\angle ((tC], (ax])$ is equal to $\pi/6$ within $\alpha/50$.
        %Note that it is a case when $\pi/3>\angle t\bar x x$.
    \item $C$ is an energetic point of the energetic ray $(bx]$
    \begin{enumerate}
        \item $C$ is an energetic point of the energetic ray $(bx]$ of order $1$.
        
        If $ C $ were an energetic point of the ray $ (bx] $ of degree $ 1 $, then there would be a contradiction with the fact that $ [\bar x t] $ lies on the path from $ \bar x $ to $ x $: polyline $ [ \bar x t] \cup [tC] $ and four empty balls of radius $ r $ (empty balls touching the points $ \bar x $ and $ C $ with centers at the corresponding points, as well as two empty balls, tangent to the energetic rays $ (ax] $ and $ (bx] $ centered at the limit points of the points corresponding to the energetic points of the rays) entail the absence of a path from $ \bar x $ to $ x $ in $ \Sigma'$. So we get a contradiction.
        
        \item $C$ is an energetic point of the energetic ray $(bx]$ of order $2$.
        
        Let the point $ C $ be an energetic point of the ray $ b $ of degree $ 2 $, then $ \angle ((tC], (bx]) \leq \pi / 6 + \alpha / 100 $. Let $ [tD] $ be the third maximal segment incident to the branching point $ t $. Note that 
         $ \angle ([Dt), (bx])>2\pi/3$. Consider two paths inside $ U $: the path starting from $ t-\bar x $ and the path starting from $ t-D $: we will show that both of them have to contain the single point from $\partial U \cap \Sigma'$, which is impossible: 
        Let the first path does not contain any energetic points of the ray $ (bx] $, so the direction of the tangent along the path changes only at the branching points and energetic points of the ray $ (ax] $ of degree $ 2 $. We require that at the branching points the path continues not by the segment that is $\alpha/50$-almost perpendicular to $ (ax] $.  Then this path does not contain any energetic points of degree $ 1 $ of the ray $ (ax]$ and all the angles between $ (ax) $ and the one-sided tangent to $ \Sigma $ along the path do not exceed $ \pi / 6 + \alpha / 100 $. Clearly this path can not end by a limit point, because by Remark otherwise $\bar x$ has two-orientated energetic ray, which is impossible for sufficiently small $\rho_1>0$ as $(ax]$ and $(bx]$ are one-orientated (in what follows we will omit this reasoning). Thus, this path cannot end with an energetic point of degree $ 1 $ and  point $ x $, but then the path inevitably passes through a single point $ \Sigma'\cap \partial U $. Similar reasoning is true for some path starting with $ t-D $ under the assumption that it does not contain energetic points $ (ax] $.
        
 Thus, it is impossible that at the same time the path starting from $ t-\bar x$ does not contain energetic points of the energetic ray $ (bx] $, and the path starting from $ t-D $ does not contain energetic points of the ray $ (ax] $. But if the path, starting with $ t - \bar x $, contains an energetic point $ (bx] $, then the second path is bounded by the first path and empty balls of radius $ r $, that is, it does not contain the energetic points of the ray $ (ax] $ and of the boundary $\partial U$, which is impossible. Similarly, the situation is impossible when the path starting with $ t-D $ contains an energetic point of the ray $ (ax] $.       

        
        \end{enumerate}
    \item  $C$   is a branching point %Thus, the point $ C $ can only be a branching point. 

 In this case, the path starting from the segments $ [\bar x t] $ and $ [tC] $ and continuing with turns in the same direction can end only if $ C $ is connected by a segment with the energetic point of the energetic ray $ (ax] $ of order $ 1 $ , we denote it by $ x^a_2 $ (this point can not be of order $2$ as $\angle ((Cx^a_2],(ax]) \geq 2\pi/3 - \angle([t\bar x)(ax]) \geq \pi/2-\alpha/50>\pi/6+\alpha/100$. Then the angle $ \angle ((Cx^a_2), (ax)) $ is equal to $ \pi / 2 $ up to $ \alpha / 100 $. In this case, considering the quadrilateral bounded by the lines $ (ax) $, $ (\bar x t), (tC), (Cx^a_2) $, we get 
$\angle  ([t\bar x)(ax])=2\pi/3-\angle ((Cx^a_2),(ax))$,
which, up to $ \alpha / 100 $, is equal to $ \pi / 6 $ (see Fig.~\ref{norm11}).
            \end{enumerate}
Thus, in any case $ \angle ((\bar xt], (ax]) $ is equal to $ \pi / 6 $ up to $ \alpha / 50 $. Let $ [tD] $ be the remaining maximum segment with the end at the point $ t $. Then $ \angle ((tD), (ax)) $ is equal to $ \pi / 2 $ within $ \alpha / 50 $, then either $ [tD) $ and $ (bx ] $ do not intersect (if $ \alpha + \angle ((tD), (ax))> \pi $), or $ \angle ((tD], (bx]) $ equals $ \pi / 2- \alpha $ up to $ \alpha / 50 $. In this case, the point $ D $ cannot be an energetic point of the ray $ (bx] $ of order $1$. The point $D$ also can not be a energetic point of order $2$ or a branching point as in these cases there are two paths in $ \Sigma'$ (a path starting with $ t-\bar x $ and a path starting with $ t-D $) that cannot coexist (the proof is similar to that discussed above).
%: a point of degree $ 1 $ due to Lemma~\ref{alm}, and a point of degree $ 2 $ due to the fact that in this case there are two paths in $ \Sigma'$ (a path starting with $ t\bar x $ and a path starting with $ t-D $) that cannot coexist (the proof is similar to that discussed above).
%Thus, the point $ D $ can only be a branching point. However, in this case too, there is a path starting with $ t-D $ that cannot coexist with some path starting with $ t-\bar x $.

This contradicts the assumption that $ t $ is a branching point.
\item Let $t$ be an energetic point of the energetic ray $(bx]$.
Note that
\[
\angle((\bar x t],(bx])= \angle (( \bar x t],(b x]) + \alpha \leq \pi/6+\alpha/100,
\]
in view of Lemma~\ref{alm} and Corollary~\ref{sm_an}, since $t$ can only be an energetic point of the ray $ (bx] $ of degree $ 2 $ belonging to the set $ X_\Sigma $. The previous item entails that the maximum segment on the path to $\Sigma $ from $t$ to $ x $ ends with an energetic point of the energetic ray $ (ax] $, we denote it by $ x^a_2 $. This point is of order $2$ and $\angle((tx^a_2),(ax))>\alpha/50$ thus the previous item entails the existence in $\Sigma'$ a poly-line $\bar x -t-x^a_2-x^b_2$, where $x^b_2$ is an energetic point of order $2$ of the energetic ray $(bx]$ such that the segment $[x^a_2x^b_2]$ is a maximal segment in a path from $x^a_2$ to $x$ in $\Sigma$. But then the previous item entails the existence in $\Sigma'$ a poly-line $\bar x -t-x^a_2-x^b_2-x^a_3$, where $x^a_3$ is an energetic point of order $2$ of the energetic ray $(ax]$ such that the segment $[x^b_2x^a_3]$ is a maximal segment in a path from $x^a_2$ to $x$ and so on, so there exists an infinite poly-line with alternating energetic points of two energetic rays as the vertices. Wherein at every step the angle between a segment of poly-line and the energetic ray increases by  $\alpha$ within $\alpha/100$ (see Fig.~\ref{norm2}):
$\angle((x^a_kx_k^b],(bx])= \angle ((x_k^bx_k^a], (xx_k^a]) + \alpha $ within $\alpha/100$ and $\angle((x^b_kx^a_{k+1}],(ax])= \angle ((xx^b_k],(x_{k+1}^ax^b_k])+\alpha \geq \angle ((x^a_kx^b_k],(bx])+ \alpha -\alpha/100= \angle ((x_k^bx_k^a], (xx_k^a]) + 2\alpha-\alpha/100$ within $\alpha/100$
for every $k\in \N$ if $x^a_1 \defeq x$ and $x^b_1 \defeq t$.
Thus, there exists a number $ k $ such that $ \angle ((x ^ i_kx ^ j_k), (jx))> \pi / 6 + \alpha / 50 $, where $ \{i, j \} = \{a, b \} $, but then the point $ x^k_j $ cannot be an energetic point of degree $ 2 $ of the ray $ (jx] $. The resulting contradiction completes the proof of the step.
\end{enumerate}


%Из утверждения автоматически следует утверждение для любого шара с центром в $x$, содержащегося в $U$, а значит найдется такое $\rho_1>0$ (например, $\rho_1 \defeq \rho_4$), что для любой точки $\bar{x} \in G_\Sigma \cap  \Sigma' \cap \overline {B_{\rho_1}(x)} \setminus \{ x\}$ касательные лучи к $\bar x$ параллельны ближайшему к ней энергетическому ребру $(ix]$ с точностью до $\alpha/100$.

\item[Step 2.] Every energetic point of $\Sigma' \cap U \setminus \{x\}$ belongs to the set $X_\Sigma$ and has the order $1$.
\begin{proof}
Assume the contrary: due to item~\ref{__1} of Lemma~\ref{alm} and step 1 it means that there exists such $\bar x \in \Sigma' \cap U \setminus \{x\}$ of order $2$ that it belongs to $E_\Sigma$ (and hence by Lemma~\ref{alm} and Corollary~\ref{notv} there exist one-sided tangents at $\bar x$ $\alpha/100$-almost parallel to $(ix]$, the closest energetic ray to $\bar x$) or to $X_\Sigma$ with both incident segments $\alpha/10$-almost parallel to $(ix]$. 

Consider the path from $\bar x$ to $x$. This path is contained in $U$ by definition of $U$ and its points by Remark~\ref{remA} can not be a limit point of the branching points. Thus if this path contains some branching points one can pick the first branching point $C_0$. Then, in view of compactness of $E_\Sigma$, we can take the last energetic point $B$ from the path from $\bar x$ to $C_0$  (it may coincide with $\bar x$). Thus the path from $B$ to $C_0$ has to be a segment and, due to Lemma~\ref{alm}, Corollary~\ref{notv} and step 1, this segment is contained in a line, $\alpha/100$-almost parallel to $(jx]$, energetic ray closest to $B$ for $j\in \{a,b\}$. Without loss of generality let $j=a$. Consider the maximal segment $[C_0C_1]\subset \Sigma'$, such that $\angle((ax](C_0C_1])$ is equal to $\frac{\pi}{3}$ within $\alpha/100$. Hence, by Lemma~\ref{alm} and Corollary~\ref{sm_an} $C_1$ can not be an energetic point and thus it has to be a branching point. Then let $[C_1C_2] \subset \Sigma'$ be such a maximal segment that it is not contained in a almost parallel to $(ax)$ line and hence $\angle((ax](C_1C_2])$ is equal to $\frac{2\pi}{3}$ within $\alpha/100$. Thus $C_2$ has to be a branching point. But then the path, beginning by $C_0-C_1-C_2-\ldots$ and continuing by the alternating turns (id est the injective poly-line $\bigcup_{j=0} [C_j C_{j+1}]$, with $\angle((ax](C_{j}C_{j+1}])=\pi-\angle((ax](C_{j-1}C_{j}])$) can not ends.

If the path from $ \overline{x} $ to $ x $ does not contain any branching points, then the arc $ \breve{]\overline{x} x[} $ will also have no energetic points of the energetic ray $ (bx] $: otherwise, let $ x_b $ be the first such point; and let $ x_a $ be the last energetic point of the ray $ (ax] $ from this arc before $x_b$ ($x_a \in Q^{a,x}_{\rho_1}$ and $x_b \in Q^{b,x}_{\rho_1}$ are the different points because $Q^{a,x}_{\rho_1}\cap Q^{b,x}_{\rho_1} =\{x\}$). In this case, the arc $ \breve{x_a x_b} $ is a segment, contained in a line almost parallel to both energetic-rays, which is impossible:
\[
\angle ((x_a x_b), (ax)) \leq \alpha/10
\]
and
\[
\angle ((x_a x_b), (bx)) \leq \alpha/10
\]
entails
\[
\alpha=\angle((ax],(bx]) =\angle((ax),(bx))\leq \alpha/5,
\]
which is impossible for $\alpha>0$. 

Thus the path from $\bar x$ to $x$ doesn't contain any energetic points of the energetic ray $(bx]$ or any branching points, id est in each point of the path the tangent ray of $\Sigma'$ is $\alpha/10$ almost parallel to $(ax]$. Then there exists such open area $U_0 \subset B_{|\bar x x|}(x)$, that $x \in U_0$, $\sharp (\partial U \cap \Sigma ) = \oord_x \Sigma$. Then $U_0 \cap \Sigma' \subset \breve{\overline{x}x}$ doesn't contain any energetic points of the ray $(bx]$. So we get a contradiction with a definition of $\Sigma'$ for $\rho_2 \defeq \rho_1$.

%для $\rho_2 \defeq \rho_4$.
%Из утверждения автоматически следует утверждение для любого шара с центром в $x$, содержащегося в $U$, то есть найдется такое $\rho_2>0$ (например, $\rho_2 \defeq \rho_4$), что любая точка $\bar{x} \in G_\Sigma \cap  \Sigma' \cap \overline{B_{\rho_2}(x)} \setminus \{ x\}$ принадлежит множеству $X_\Sigma$ и имеет порядок $1$.
\end{proof}

\item [Step 3]
Let $ U_1 \ni x $ be an open area of sufficiently small diameter (so that $ \Sigma'\cap (U \setminus U_1) $ contains sufficiently many energetic points of both energetic rays: for example at least three energetic points of each energetic ray) such that $ U_1 \subset U $, $ \sharp (\partial U_1 \cap \Sigma) = \oord_x \Sigma $.
In view of the previous steps, $\overline{\Sigma'\cap (U \setminus U_1)} $ is a locally minimal tree (with a finite number of vertices) without vertices of degree $ 2 $. Then there exist three lines with pairwise angles $ \pi / 3 $ such that each segment of $ \overline{\Sigma'\cap (U \setminus U_1)} $ is parallel to one of them.
Each endpoint of the Steiner tree $ \overline{\Sigma'\cap (U \setminus U_1)} $, except two points of $ (\partial U \cup \partial U_1) \cap \Sigma' $, lies on a segment belonging to the line $\alpha/100$-almost perpendicular to one of the rays. Therefore, since the set $ \Sigma'\cap (U \setminus U_1) $ contains the energetic points of both rays, the angle $ \alpha = \angle axb \leq \pi$ can only be $\frac{\pi}{3}$, $\frac{2\pi}{3}$ or $\pi$ within $\alpha/100$.
%\end{enumerate}

\item[ Step 4]
\input{pictures/trash/roza1}
\input{pictures/trash/roza2}
\input{pictures/trash/roza3}
Let us construct the wind rose with the center inside the internal angle $\angle axb$ and the lines, containing perpendiculars to both energetic rays $(ax]$ and $(bx]$. We place the weights depending on the angle $\angle axb$:
\begin{itemize}
\item If $\alpha = \frac{\pi}{3}$ then place $1$ at both rays directed towards to $(ax]$ and $(bx]$ and perpendicular to it (see Fig.~\ref{fig:roza1}). Thus there are weights $-1$ at the complementary rays, and weights $2$ and $-2$ at the last line.
 \item If $\alpha = \frac{2\pi}{3}$ then place $1$ at the ray, perpendicular to $(ax]$ and directed towards to it, and place $2$ at the ray, perpendicular to $(bx]$ and directed towards to it (see Fig.~\ref{fig:roza2}). Thus there are weights $-1$ and $-2$ at the complementary rays, and weights $1$ and $-1$ at the last line.
 \item If $\alpha = \pi$ we place $1$ at the ray directed towards to $(ab)$  and perpendicular to it, and weights $-1$ and $0$ at the remaining ones (see Fig.~\ref{fig:roza3}). Thus there are weights $-1$, $1$ and $0$ at the complementary rays.
 \end{itemize}
 
 Now, as in Remark~\ref{main_rose_property}, we assign to each terminal vertex of the tree  $\overline{\Sigma \cap U}$ the weight of the ray of the corresponding wind rose, co-directed with the segment entering this vertex.
 
 
 
% We now associate a tree $\overline{\Sigma \cap U}$ with a directed graph (one segment can be associate to two edges if there are only two vertices at the graph) with weights, where the weight of each edge is equal to the weight of the edge of wind rose, $\alpha/100$-almost co-directional to it.
 
 %Выберем также $\rho_1<\rho_4$ так, чтобы $\sharp(\Sigma \cap \partial(B_{\rho_1}(x)))\leq 3$, а количество энергетических точек $\Sigma' \cap B_{\rho_4}(x)\setminus B_{\rho_1}(x)$ было достаточно велико.
 
By Remark~\ref{main_rose_property}, sum of all weights of $\Sigma' \cap (U \setminus U_1)$ is equal to $0$. On the other hand, sum is positive, as there are arbitrarily many positive terms, and at most two negative. So we get a contradiction.

\end{itemize}

\end{proof}


 
%Заметим, что в частности Лемма~\ref{main_l} утверждает %отсутствие в окрестности точки $x\in E_\Sigma$ точек %ветвления. 
%Лемма~\ref{main_l}, вместе с Утверждением~\ref{discr_str} и %ввиду компактности $\Sigma$ влекут основной результат статьи, %Теорему~\ref{mainT1}.



%\begin{remark}
%A full Steiner tree consists of segments belonging to three straight lines with pairwise angles $ \pi / 3 $. Let $ T $ be an arbitrary complete Steiner tree. Take an arbitrary wind rose, consisting of rays in the same directions as the segments $ T $, and assign to each end vertex of $ T $ the weight of the ray of the fixed wind rose, co-directed with the segment entering this vertex. Then the sum of numbers over all vertices of $ T $ will be zero.
%\label{main_rose_property}
%\end{remark}








==> ⥪�騩 ���᪨� ⥪�� (in english)/parts/new_proofs.tex <==
%\section{Доказательства и технические утверждения}
\subsection{Technical statements and proofs of some lemmas}
\label{new_proofs}
%%\color{blue}
%\begin{definition}
%Let $\bar x\in E_\Sigma$ and $\varepsilon>0$. Then let us define a set 
%\[
%U(\bar{x},\varepsilon) \defeq \left \{ y\in M | \dist(y, \overline{B_{\varepsilon}(\bar{x})})\leq r, \dist(y, \Sigma \setminus \overline{B_{\varepsilon}(\bar{x})})> r \right \}.
%\]
%\end{definition}
%\begin{remark}

%Let $x\in E_\Sigma$ and let $(ix]$ be an energetic ray. If $(ix]$ is one-orientated energetic ray then there exists such $\rho>0$ that for every $\bar x \in E_\Sigma \cap B_\rho(x)$ for sufficiently small $\varepsilon>0$ the set $U(\bar{x},\varepsilon)$ is located in the same half-plane bounded by $ (ix) $ \color{red}(the one into which the edge is orientated).\color{black} %понятно ли учитывая определки?

 % If an energetic ray $(ix]$ is two-orientated for each $\bar x$ either exist such   $\varepsilon>0$, that the set $U(\bar{x},\varepsilon)$ is located in one half-plane bounded by $ (ix) $
  %   or in both half-planes there exist different points $ y (\bar {x}) \in M$ corresponding to $ \bar{x} $. 

%\end{remark}
%\color{black}


Теперь приступим к доказательству Леммы~\ref{alm}. %НАДО СДЕЛАТЬ ОТДЕЛЬНОЙ ЛЕММОЙ

\begin{proof}
%Предположим противное утверждению Леммы: то есть найдется такое $c>0$, что для каждого $\rho>0$ найдется $\bar x \in %B_\rho(x) \setminus \{x\}$ такой, что $|g(\bar x)|>c$. То есть выполняется неравенство:  
%\begin{itemize}
%\item [(i)] $|\pi/2-\angle((s\bar x),(ix))|>c$, если $\bar x \in X_\Sigma$, $\oord_x\Sigma=1$ и $[s\bar x] \subset %\Sigma$;
%\item [(ii)]$|\angle((s\bar{x}], (ix))-\angle( (ix),(t\bar{x}])|>c$,  если $\bar x \in X_\Sigma$, $\oord_x\Sigma=2$ и %$([s\bar x] \cup [t \bar x]) \subset \Sigma$;
%\item [(iii)]$\max \left( \big| \pi- \angle(m(\bar{x}),n(\bar{x})) \big| , \angle(m(\bar{x}),(ix)) \right)>c$, если %$\bar x \in E_\Sigma$, где лучи $m(\bar x)$ и $n(\bar x)$ определены в формулировке Леммы.
%\end{itemize}
Сначала мы докажем вспомогательные утверждения (A), (B) и (C), а после последовательно каждый из пунктов Леммы.

%Мы сначала докажем вспомогательное утверждение, из которого будет следовать пункт~\ref{__1}. После этого докажем %вспомогательное утверждение, которое будет использовано в доказательстве невозможности пункта (ii) и разборе случая %$\oord_x\Sigma =2$. Невозможность пункта (iii) получается автоматически, а вот доказательство того, что $\Sigma \cap %B_\varepsilon(\bar x)$  случае $\oord_x\Sigma =2$ является объединением двух дуг, лежащих в некоторых псевдоконусах, %потребует усилий.
\begin{enumerate}
\item [(А)] \label{W}
Для произвольного $x\in E_\Sigma$  для каждого $c>0$ существует такое $\rho>0$, что для $\bar{x} \in B_\rho(x) \setminus \{ x\}$ такого, что $\oordball_{\bar x}\Sigma=1$ для каждого такого $\varepsilon<\min(|\bar x x|, \rho-|\bar x x|)$, что $\sharp(\partial B_{\varepsilon}(\bar x) \cap \Sigma)=1$, для $s^\varepsilon \defeq \partial B_{\varepsilon}(\bar x) \cap \Sigma$ выполняется $|\angle ((s^\varepsilon \bar x), (ix))-\pi/2|<c$. Иными словами, покажем, что $|\angle ((s^\varepsilon \bar x), (ix))-\pi/2|=o_\rho(1)$. %Заметим, что из этого будет следовать одно из двух утверждений пункта~\ref{__1} Леммы, а именно что в случае $\bar{x}\in X_\Sigma$ и $\oord_{\bar x}\Sigma=\oordball_{\bar x}\Sigma=1$ отрезок $[s\bar x] \subset \Sigma$ почти перпендикулярен $(ix)$
\begin{proof}
%[вспомогательного утверждения А]
Предположим противное, то есть что существует %не зависящая от $\rho>0$
константа $c>0$, такая что для каждого $\rho>0$ найдется $\bar{x} \in B_\rho(x) \setminus \{ x\}$ и такое $\varepsilon>0$, что $B_{\varepsilon_0}(\bar x) \subset B_\rho(x)$ и  $|\angle ((s_0\bar x), (ix))-\frac{\pi}{2}| > c$ для $s_0 \defeq \partial B_{\varepsilon_0}(\bar x) \cap \Sigma $.  Пусть тогда $w^0$ --- основание перпендикуляра, опущенного из $s_0$ на прямую, параллельную $(ix)$ и проходящую через $\bar x$: $(w^0\bar x)\ ||\ (ix)$ и $(w^0s_0) \perp (ix)$. Тогда определим множество $S \ni w^0$  как в Лемме~\ref{Losiu} для $w=w^0$. Тогда длина этого множества $\H(S)=o_\rho(1)\varepsilon_0$, . В то же время 
\[
|w^0s_0|=\sin \angle([s_0\bar x],(ix]) \cdot |s_0\bar x|= \cos c |s_0\bar x| < (1 - \frac{c^2}{2}) \varepsilon_0
\]
для достаточно малого $c$.
При этом $\H(\Sigma \cap B_{\varepsilon_0}(\bar x)) \geq \varepsilon_0$. Таким образом, \[
\H(\Sigma \setminus  B_{\varepsilon_0}(\bar x) \cup [s_0w^0] \cup S)\leq \H(\Sigma)-\varepsilon_0+\left(1-\frac{c^2}{2}\right)\varepsilon_0+o_\rho(1)\varepsilon_0<\H(\Sigma).
\]
Таким образом, $\Sigma \setminus  B_{\varepsilon_0}(\bar x) \cup [s_lw^l] \cup S$ является связным множеством с длиной меньшей и энергией, не большей, чем у $\Sigma$. Противоречие с оптимальностью $\Sigma$ завершает доказательство.
\end{proof}
\item [(B)]
Пусть $x \in E_\Sigma$. Тогда для достаточно малого $\rho>0$ для каждого $\bar x \in G_\Sigma \cap B_\rho(\Sigma)\setminus \{ x\}$, имеющего порядок $\oordball_{\bar x}\Sigma = 2$, найдется такое $\varepsilon>0$, что для каждой  $u \in \Sigma \cap B_\varepsilon(\bar x)$ выполняется $\angle((u \bar x),(ix)) \neq \pi/2$. Иными словами, если $\bar x \in G_\Sigma \cap B_\rho(\Sigma)\setminus \{ x\}$ имеет порядок $\oord_{\bar x}\Sigma = 2$, то не существует бесконечной последовательности точек $u_m\in \Sigma$, сходящейся к $\bar x$, таких что $\angle((u_m\bar x),(ix))=\pi/2$.
\label{QuQuQu}

\begin{proof}
Пусть $\{\varepsilon_l\}$ -- убывающая к нулю последовательность таких чисел, что $\sharp (\partial B_{\varepsilon_l}(\bar x) \cap \Sigma )=2$, а $\varepsilon_1 < \min (\rho, \rho-|\bar x x|)$. Обозначим  $s^l, t^l \defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$. 

Ясно, что угол $\angle s^l\bar xt^l > \frac{2\pi}{3} - o_\rho(1)$: в противном случае замена $\Sigma \setminus B_\varepsilon(\bar x) \cup St(s^l,t^l,\bar x) \cup S$, где $S \ni \bar x$ --- множество, определенное в Лемме~\ref{Losiu} для точки $w=\bar x$, а $St(s^l,t^l,\bar x)$ --- дерево Штейнера, соединяющее точки $s^l$, $t^l$ и $\bar x$, имело бы не большую энергию и строго меньшую длину, чем множество $\Sigma$.

С другой стороны $B_r(y(\bar x)) \cap \Sigma = \emptyset$ и $|\angle ((y(x)x),(ix)) - \pi/2| =o_\rho(1)$ ввиду пункта~3 доказательства леммы~\ref{Losiu}.
Тогда $\angle ((s^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ и $\angle ((t^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$.


Предположим противное утверждению пункта: что существует такая последовательность $u_l$. Тогда при достаточно малом $\rho$ для любого $l$ выполняется 
\[
\sharp (\Sigma \cap \partial B_{|\bar x u_l|}(\bar x))\geq 3.
\]

Заметим теперь, что для каждого $\varepsilon_l$ верно
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)=2\varepsilon_l+o_\rho(1)\varepsilon.
\label{1000}
\end{equation}
Формула~\eqref{1000} верна ввиду Леммы~\ref{Losiu}: в противном случае, можно было бы заменить $\Sigma$ на связное множество $\Sigma \setminus B_{\varepsilon_l}(\bar x) \cup [\bar xs^l]\cup [\bar x t^l]\cup S$, где $S$ определено в Лемме~\ref{Losiu} при $w=\bar x$, и получить противоречие с оптимальностью $\Sigma$. 
Можно считать, что 
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)<2\varepsilon_l \left (1+\frac{1}{36}\right).
\label{1010}
\end{equation}

Теперь заметим, что можно считать, что 
\begin{equation}
\frac{\varepsilon_l}{\varepsilon_{l+1}}\leq \frac{18}{17}.
\label{1030}
\end{equation}
Пусть не так, тогда найдется $\varepsilon_l$ такое, что $\sharp \left( \partial B_{\varepsilon_l}(\bar x)\cap \Sigma
\right) \geq 3$ для каждого $\varepsilon \in [\frac{17\varepsilon_l}{18},\varepsilon_l[$. Но тогда, ввиду неравенства коплощади,
\[
\H(\Sigma \cap B_{\varepsilon_l}(\bar x))\geq \H(\Sigma \cap B_{\frac{17\varepsilon_l}{18}}(\bar x)) +\H(\Sigma \cap (B_{\varepsilon_l}(\bar x) \setminus  B_{\frac{17\varepsilon_l}{18}}(\bar x))\geq 2\varepsilon_l\left(1+\frac{1}{36}\right),
\]
что противоречит (\ref{1010}).

Рассмотрим произвольную точку $u_m$ из последовательности $\{u_l\}$. Выберем такой номер $l$, что 
\begin{equation}
0<\varepsilon_l-|\bar xu_m|\leq \frac{1}{18}\varepsilon_l.
\label{1040}
\end{equation}
Такое $\varepsilon_l$ существует ввиду формулы~\eqref{1030}. Также можно полагать, что для каждого $\delta \in ]|\bar x u_m|, \varepsilon_l[$ выполняется $\sharp \left( \partial B_{\delta}(\bar x)\cap \Sigma
\right) \geq 3$.
Пусть \[\gamma \defeq \max_{s \in \Sigma \cap \overline B_{\varepsilon_l}: \sharp (B_{|\bar x s|}(\bar x) \cap \Sigma) <3)} \angle{ixs}.\] Тогда $\gamma\leq \frac{\pi}{3}+ o_\rho(1)$.
Пусть $q$ --- компонента связности $\Sigma \setminus \Lambda ((ix),\gamma)$, содержащая $u_m$.
Тогда 
\[
\H(q) \geq \dist (u_m, \Lambda((ix),\gamma))=\cos \gamma |u_m \bar x|\geq \frac{|u_m \bar x|}{3}.
\]
Заметим, что, ввиду неравенства коплощади для $\Sigma \setminus q$, верно
\begin{multline}
\H(\Sigma \cap \overline B_{\varepsilon_l}) = \H(q)+\H(\Sigma \cap \overline B_{\varepsilon_l}\setminus q ) \geq \H(q)+2\varepsilon_l\geq  \frac{|u_m \bar x|}{3} +2\varepsilon_l \geq \varepsilon_l (\frac{17}{18*3}+2),
 \end{multline}
где последнее неравенство верно ввиду~\eqref{1040}. Получили противоречие с~\eqref{1010}.
\end{proof}
\item [(C)] Пусть обозначениях леммы $\oordball_x \Sigma =2$ и пусть $(s \bar x]$ и $(t \bar x]$ --- касательные для компонент связности $\Sigma \setminus \bar x$ в точке $\bar x$. Тогда найдется такое $\rho$, что $|(\angle (s \bar x], (ix] - (\angle (t \bar x], (ix]| <c$.
Иными словами $|(\angle (s \bar x], (ix] - (\angle (t \bar x], (ix]| = o_\rho(1)$.
\begin{proof}
Предположим противное: что найдется число $c>0$, такое что 
\[
\eta \defeq \angle((s\bar x], (ix))-\angle( (ix),(t\bar x]) \geq c
\]
для сколь угодно малого $\rho$.
Пусть $\varepsilon< \min (\rho-|\bar x x|, |\bar x x|)$ такой, что $\sharp( \partial B_\varepsilon(\bar x) \cap \Sigma) =2$. Обозначим $T, S \defeq \partial B_\varepsilon(\bar x)  \cap \Sigma$. Тогда 
\begin{equation}
\angle ((T \bar x],(t\bar x))=o_\rho(1) \mbox{ и } \angle ((S \bar x],(s\bar x))  =o_\rho(1).
\label{ZAQ}
\end{equation}
Пусть $l$ --- прямая, проходящая через точку $\bar x$ и параллельная $(ix)$. Отразим отрезок $[T \bar x]$ относительно $l$. Пусть $T'$ --- образ точки $T$ при этом отображении. 
Тогда $|T'\bar x|=\varepsilon$ и
\[
|S \bar x|+|T \bar x|=|S\bar x|+|T' \bar x|=2\varepsilon.
\]
В то же время по теореме косинусов для $\Delta S\bar xT'$
\[
|ST'|^2 = |S\bar x|^2+|\bar xT'|^2-2|S\bar x||\bar x T'|\cos \angle S\bar xT'=2\varepsilon^2(1-\cos (\eta+o_\rho(1))),
\]
поскольку
\[
\angle S\bar xT'=\pi+\angle((T\bar x], (ix))-\angle( (ix),(S\bar x]),\]
то есть ввиду~\eqref{ZAQ}   
\[
\angle S\bar xT'=\pi+\angle((t\bar x], (ix))-\angle( (ix),(s\bar x])+o_\rho(1)=\pi+\angle((t\bar x], (ix))-\angle( (ix),(s\bar x])+o_\rho(1)=\pi=\eta+o_\rho(1).
\] 
%а $\angle S\bar xT'=\angle s \bar x t+o_\rho(1)=\pi-\eta+o_\rho(1)$.


Таким образом, при достаточно малом $\rho$,
\[
|S\bar x|+|T'\bar x|-|ST'|> c_2\varepsilon,
\]
где $c_2 > 0$ --- константа, зависящая только от $\eta$.

Пусть теперь точка $d \defeq [ST']\cap l$. Тогда $\angle((Sd], (ix))=\angle( (ix),(T'd])$ и 
%\begin{equation*}
\[(|S\bar x|+|T\bar x|)-(|Sd|+|dT|)= 2\varepsilon - |ST'|>c_2\varepsilon.\]
%\end{equation*}

Ввиду Леммы~\ref{Losiu} для $w=d$ найдется связное множество $S \ni d$ такое, что $\H(S)<c_2/2\varepsilon$, а $F_M(\Sigma \setminus B_\varepsilon(\bar x) \cup S)\leq F_M(\Sigma)$. Тогда связное множество $\Sigma \setminus ([S\bar x]\cup[T\bar x]) \cup S \cup [sd] \cup [td]$ при достаточно малом $\rho$ будет лучше $\Sigma$, поскольку имеет не большую энергию и строго меньшую длину.
%не превосходящую $\H(\Sigma)-c_2\varepsilon+ \H(S)<\H(\Sigma)$. 
Полученное противоречие с оптимальностью $\Sigma$ завершает доказательство пункта.
\end{proof}

\begin{corollary}
В ввиду леммы~\ref{angles2} верно $\angle s\bar xt \geq \frac{2\pi}{3}$ и 
\[
\angle((s\bar x], (ix))=\angle( (ix),(t\bar x] )+ o_\rho(1)\leq \frac{\pi}{6}+ o_\rho(1).
\] 
\label{__2c}
\end{corollary}

\item Теперь докажем, что 
%для произвольного $x \in E_\Sigma$ найдется такое $\rho>0$, что для каждого $\bar x \in B_\rho(\Sigma)\setminus \{ %x\}$, 
порядок $\oord_{\bar x}\Sigma = 1$ влечет  $\bar x\in X_\Sigma$. 
\label{QQ}
Предположим противное: пусть $\bar x \in E_\Sigma \cap B_\rho(x) \setminus x$. 
% Энергетическое ребро или ребра, к которым они сходятся, должны лежать на прямой, почти параллельной $(ix]$ ввиду %Следствия~\ref{alm_parr}.  
%\end{itemize}


Ввиду Леммы~\ref{ordball_} достаточно разобрать только следующие случаи:
\begin{itemize}
\item [(а)] Случай $\oordball_{\bar x}\Sigma=2$.
Пусть $\{\varepsilon_l\}$ -- убывающая к нулю последовательность таких чисел, что $\sharp (\partial B_{\varepsilon_l}(\bar x) \cap \Sigma )=2$, а $\varepsilon_1 < \min (\rho, \rho-|\bar x x|)$. Обозначим  $s^l, t^l \defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$. 

Как было показано в п. (B), верно $\angle ((s^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ и $\angle ((t^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$.%, то есть
%\begin{equation}
%s^l, t^l \in \Lambda((ix), \pi/3+o_\rho(1)).
%\label{LLL}
%\end{equation}


Тогда ввиду единичного порядка $\oord_{\bar x}(\Sigma)=1$, существует также сходящаяся к $\bar x$ последовательность точек $\{ u_l\}$ таких, что \[\angle\left((u_l\bar x),(ix)\right)=\frac{\pi}{2}.\] 
Противоречие с п.~(B).


\item [(б)] Случай $\oordball_{\bar x}\Sigma=1$. 

Пусть $\varepsilon_l>0$ --- последовательность стремящихся к нулю чисел таких, что $\sharp (\partial B_{\varepsilon_l}(\bar x) \cap \Sigma )=1$, а $s_l\defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$. Тогда ввиду~(A) $(s_l\bar x)$ почти перпендикулярно $(ix)$:
\begin{equation}
\left|\angle \left((s_l\bar x), (ix)\right)-\frac{\pi}{2}\right| =o_\rho(1).
\label{99}
\end{equation}
Заметим теперь, что для каждого $\varepsilon_l$ верно
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)=\varepsilon_l+o_\rho(1)\varepsilon.
\label{100}
\end{equation}

Формула~\eqref{100} верна ввиду Леммы~\ref{Losiu}: в противном случае можно было бы заменить $\Sigma$ на связное множество $\Sigma \setminus B_{\varepsilon_l}(\bar x) \cup [\bar xs_l]\cup S$, где $S$ определено в Лемме~\ref{Losiu} при $w=\bar x$, и получить противоречие с оптимальностью $\Sigma$. 

Можно считать, что 
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)<\varepsilon_l \left(1+\frac{1}{18}\right).
\label{101}
\end{equation}
Теперь заметим, что тогда
\begin{equation}
\frac{\varepsilon_l}{\varepsilon_{l+1}}\leq \frac{18}{17}.
\label{103}
\end{equation}
Пусть не так, тогда найдется $\varepsilon_l$ такое, что $\sharp ( \partial B_{\varepsilon_l}(\bar x)\cap \Sigma)\geq 2$ для каждого $\varepsilon \in [\frac{17\varepsilon_l}{18},\varepsilon_l[$. Но тогда, ввиду неравенства коплощади
\[
\H \left(\Sigma \cap B_{\varepsilon_l}(\bar x)\right)\geq \H \left(\Sigma \cap B_{\frac{17\varepsilon_l}{18}}(\bar x)\right) +\H \left(\Sigma \cap B_{\varepsilon_l}(\bar x) \setminus  B_{\frac{17\varepsilon_l}{18}}(\bar x)\right)\geq \varepsilon_l \left (1+\frac{1}{18} \right),
\]
что противоречит~\eqref{101}.
Заметим, что поскольку $\bar x$ имеет ребро, которое, ввиду Следствия~\ref{alm_parr} $o_\rho(1)$-почти параллельно $(ix)$, существует последовательность энергетических точек $\{x_l\}$, сходящихся к $\bar x$ таких, что $\angle ((x_l\bar x], (ix]) =o_\rho(1)+o_{|x_l\bar x|}(1)$. Ввиду наличия у $\bar x$ ребра, существования последовательности $\{ s_l \}$ и единичного порядка $\oord{\bar x}(\Sigma)=1$ существует также сходящаяся к $\bar x$ последовательность точек $\{ u_l\}\subset \Sigma$ таких, что $\angle \left((u_l\bar x),(ix)\right) = \frac{\pi}{4}$.

Рассмотрим произвольную точку $u_m$ из этой последовательности. Выберем такой номер $l$, что 
\begin{equation}
0<\varepsilon_l-|\bar xu_m|\leq \frac{1}{18}\varepsilon_l.
\label{104}
\end{equation}
Такое $\varepsilon_l$ существует ввиду формулы~\eqref{103}. Заметим также, что ввиду~\eqref{99} выполняется
\[
\sharp (\partial B_{|\bar x u_m|}(\bar x)\cap \Sigma) \geq 2.
\] 
Можно также считать, что для произвольного $\delta \in [|\bar x u_m|,\varepsilon_l[$ выполняется $\sharp (\partial B_{\delta}(\bar x)\cap \Sigma) \geq 2$.

Кроме того, пусть 
\[
k:=\max_{s \in \Sigma \cap \overline{B_{\varepsilon_l}}: \sharp (\Sigma \cap _{|s \bar x|}(\bar x))} \angle ixs,
\]
тогда $|k-\pi/2|=o_\rho(1)$.
Тогда $K := \Lambda((ix),k)$ --- область возможного расположения точек $s_l$. 


%Кроме того, пусть $K \subset \Lambda((\bar x y(\bar x)), o_\rho(1))$ --- область возможного расположения точек $s_l$ (угол с вершиной в $\bar x$, раствором $o_\rho(1)$ и перпендикуляром к $(ix)$ в качестве биссектрисы), а 
Пусть $Q$ --- псевдоконус или объединение двух псевдоконусов с вершиной в $\bar x$, содержащих все энергетические точки $B_{\varepsilon_l}(\bar x)$, тогда
\begin{equation}
d \defeq \dist(u_m, Q \cup K)\geq \frac{\sqrt{2}}{2}|\bar xu_m|-o_\rho(1)\varepsilon> \frac{17}{36}\varepsilon_l,
%\label{105}
\end{equation}
где последнее неравенство верно ввиду~\eqref{104}. 
Ясно, что, ввиду единичного порядка $\bar x$ и определения компоненты связности $q$, выполняется $\H(q) \geq 2d$. В таком случае, ввиду неравенства коплощади для $\Sigma \setminus q$, верно
\[
\H(\Sigma \cap B_{\varepsilon_l}(\bar x)) \geq H(\Sigma \cap B_{\varepsilon_l}(\bar x) \setminus q)+\H(q) \geq \varepsilon_l +2d\geq
\varepsilon_l (1+ \frac{17}{18}).
\]
Полученное противоречие с~\eqref{101} завершает доказательство пункта~\ref{__1} леммы.

\end{itemize}
\item Пусть $\oord_{\bar x} \Sigma =2$ и $\bar x \in X_\Sigma$, и для некоторого $\varepsilon>0$ выполняется $\Sigma \cap \overline{B_{\varepsilon}(\bar x)}=[s\bar x] \sqcup [t\bar x]$. 
\label{Q3}

Утверждение сразу следует из пункта~(C).

\item% Докажем пункт~\ref{__3} Леммы.
%\begin{proof}
Ввиду Леммы~\ref{con} пп~\ref{BB} и~\ref{reb} существует $Q$ --- псевдоконус или объединение двух  псевдоконусов  таких, что $G_\Sigma \cap B_{\varepsilon_0}(\bar x) \subset Q$ для достаточно малого $\varepsilon_0$. 
%Не умаляя общности, ввиду пункта~\ref{ordball_} будем считать $\varepsilon>0$ таким, что $\sharp(\Sigma \cap \partial B_\varepsilon(x^i_k)) \leq 2$. 
При этом  ввиду следствия~\ref{alm_parr} оси псевдоконусов почти параллельны $(ix)$. 
Если хотя бы одно из двух ребер $\bar x$ направлено в две стороны, пункт тривиален ввиду Замечания~\ref{star}. Аналогично пункт тривиален, если ребра направлены в разные стороны, то есть для достаточно малого $\varepsilon_0>0$ точки $M$, соответствующие энергетическим точкам из множества $B_{\varepsilon_0}(\bar x) \setminus \bar{x}$ располагаются в обеих частях плоскости, разделенной энергетическими ребрами $\bar x$. Таким образом, можно считать, что каждое ребро направлено в одну сторону и что один из двух углов между энергетическими ребрами не содержит точек $M$, соответствующих энергетическим точкам из $Q$. Будем называть этот угол внутренним. Нетрудно заметить, что ввиду п.~\ref{orientation} Замечания~\ref{emptyball} величина этого угла не превосходит $\pi$. 

Пусть $(q_1\bar x]$ --- луч, лежащий во внутреннем угле и не совпадающий ни с одним энергетическим ребром $\bar x$. Тогда, ввиду определения псевдоконуса найдется такое $\varepsilon_1>0$, что $(q_1\bar x] \cap Q \cap B_{\varepsilon_1}(\bar x)=\emptyset$. Поскольку ввиду пункта~\ref{QQ} доказываемой леммы, замечания~\ref{rem_ord} и леммы~\ref{ordball_}, выполняется $\oord_{\bar x} \Sigma =\oordball_{\bar x}\Sigma=2$, потребуем, чтобы $\varepsilon_1>0$ удовлетворяло условию $\sharp (\Sigma \cap \partial B_{\varepsilon_1}(\bar x))=2$. Покажем, что тогда найдется такое $\varepsilon_2>0$, что 
\[
B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x], 
\]
либо 
найдется такое $\varepsilon_2>0$, что 
\[
B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = \bar x. 
\]
 Пусть не реализовался ни один из двух случаев. Тогда, в частности, множество $\Sigma \cap B_{\varepsilon_1}(\bar x) \cap (q\bar x]$ содержит бесконечное число точек. Кроме того, любая точка из множества $\Sigma \cap B_{\varepsilon_1}(\bar x) \cap (q\bar x]$ не энергетическая и, значит, является центром отрезка или правильной треноги.
%, а множество $\Sigma \cap B_{\varepsilon}(\bar x) \setminus Q$ является штейнеровским лесом. 
Пусть $L_1$ обозначает ту часть внутреннего угла, которая ограничена $(q_1\bar x]$, $\partial B_{\varepsilon_1}(\bar x)$ и перпендикуляром к $(ix)$, проходящим через $\bar x$ (положим для начала, что луч $(q_1\bar x]$ не перпендикулярен $(ix)$). Будем полагать $L_1$ открытым множеством. Тогда $S := \overline{L_1\cap \Sigma}$ является штейнеровским лесом, причем все концевые вершины $ S$, число которых бесконечно, за исключением не более чем трех точек, принадлежащих $\partial B_{\varepsilon_1} (\bar x) \cup \{ x \}$, лежат на $(q\bar x]$ или на перпендикуляре. Тогда ввиду Леммы~\ref{St_l} число концевых точек леса $\partial S$, принадлежащих перпендикуляру, бесконечно. а значит найдется сходящаяся к $\bar x$ бесконечная последовательность точек $\{u_l\}$ таких, что $\angle((u_l,\bar x)(ix))=\pi/2$ для каждого номера $l$. Однако существование такой последовательности противоречит пункту~(B). Таким образом, существует такое $\varepsilon_1$, что $\Sigma \cap (q_1\bar x] \cap \overline {B_{\varepsilon_1}(\bar x)}$ равно $\{\bar x\}$ или совпадает с $(q_1\bar x] \cap B_{\varepsilon_1}(\bar x) $. Будем также считать, что $\sharp(\partial B_{\varepsilon_1}(\bar x)\cap \Sigma)=2$ и $Q \cap B_{\varepsilon_1}(\bar x) \cap (q_1\bar x] = \emptyset$.

Пусть $(m\bar x]$ --- энергетическое ребро $\bar x$. Выберем такие строго убывающие к нулю последовательности $\{\bar{\varepsilon}_i \}$ и $\{ \gamma_i\}$, что 
\begin{itemize}
\item $Q \cap B_{\bar \varepsilon_i}(\bar x)$ содержится внутри угла с биссектрисой $(m\bar x]$ и раствором $2\gamma_i$;
\item границы угла с биссектрисой $(m\bar x]$ и раствором $2\gamma_i$, при пересечении с множеством $\Sigma \cap \cap B_{\bar\varepsilon_{i+1}}(\bar x)$, совпадают с $\{ \bar x \}$, либо с радиусом $B_{\bar \varepsilon_{i+1}}(\bar x)$. 
\end{itemize}
Положим $\gamma_1 \leq \pi/12$, $\bar \varepsilon_1 \defeq \varepsilon_1$.
Если при каком-то номере (ввиду леммы~\ref{angles2} не более чем при одном) реализовался случай совпадения с радиусом, обозначим этот номер за $j$. В противном случае положим $j=0$.

Определим псевдоконус 
\[
Q_1 \defeq Q^{m,\bar x}_{\overline{\varepsilon}_{j+1}}\defeq \bigcup_{i=j+1}^{\infty} \left(Q(m,\overline x, \gamma_i, \overline{\varepsilon_i}) \setminus B_{\overline{\varepsilon}_{i+1}}(\bar x)\right).
\]
Если $\bar x$ обладает двумя энергетическими ребрами, то аналогично определим псевдоконус $Q_2$ со вторым энергетическим ребром в качестве оси. 
%$(a \bar x$ и $(b \bar x]$, то аналогично определим псевдоконус $Q^{b, \bar x}_{\bar \varepsilon_1}$

Таким образом произвольная компонента связности $\Sigma \cap B_{\varepsilon_1}(\bar x)\setminus \{x\}$ либо находится внутри псевдоконуса $Q_1$ или $Q_2$, либо находится вне псевдоконуса $Q$. Поскольку $\bar x$ имеет энергетическое ребро, хотя бы одна из двух компонент содержится внутри псевдоконуса. Тогда она имеет касательную в точке $\bar x$(причем данная касательная $\rho-$почти параллельна $(ix]$), а значит к ней применима лемма~\ref{angles2}. Если вторая компонента связности не содержится в псевдоконусе, то она является отрезком (поскольку имеет не более двух концевых точек: точку $\{ \bar x\}$ и точку на $\partial B_{\varepsilon_1}(\bar x)$). В обоих случаях вторая компонента связности имеет в точке $\bar x$ касательную. Таким образом ко второй компоненте связности применим пункт $(C)$ доказываемой леммы. Утверждение пункта доказано.


 
% \begin{remark}
 %Заметим также, то угол между ребрами, содержащий соответствующую $x^i_k$ точку $y^i$, не может быть меньше $\pi$ (если покрытые $x^i_k$ точки есть в обеих полуплоскостях, то угол между ребрами составляет ровно $\pi$).
 %\label{rovno}
 %\end{remark}

\end{enumerate}
 \end{proof}

%\begin{proof}
%\begin{enumerate}
  %  \item

Докажем следующее техническое утверждение:
\input{pictures/dvapo}

\begin{proposition}
Для произвольного $x \in E_\Sigma$ и $\bar c>0$ найдется такое $\rho>0$, что если $\Sigma \cap B_\rho(x)$ содержит ломаную $L_1-L_2-L_3-L_4-L_5$, узлы которой являются энергетическими точками ребра $(ix]$, то $\angle((L_iL_{i+1}),(ix)\leq \bar c$ для $i=1, \dots, 4$.  
И ВСЕ ВН ТОЧКИ ЛОМАНОЙ -- СТЕПЕНИ 2 
\label{brrrr}
\end{proposition}
\begin{proof}
Предположим противное, то есть (ввиду Леммы~\ref{alm} п.~\ref{__2} для $c= \bar c/ 10$) что для сколь угодно малого $\rho > 0$ существует такая ломаная $L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\rho}$, что все углы $\angle((L_iL_{i+1}),(ix))> \bar{c}/2$ при $i=1,2,3,4$. 
Будем считать $(ix)$ осью абсцисс, а $\bar{c}$ достаточно малым. Не умаляя общности, точкам $L_1$, $L_3$, $L_5$ соответствуют верхние точки множества $M$, а точкам $L_2, L_4$ --- нижние: ввиду пункта~\ref{1145} доказательства Леммы~\ref{Losiu} и неравенства $\angle L_{i-1}L_{i}L_{i+1} \leq \pi-\bar{c}$, $i=2,3,4$ двум подряд идущим точкам не могут соответствовать одновременно верхние или нижние точки.
 Заметим теперь, что отношения между отрезками ломаной линейные (то есть отношение оценивается сверху и снизу константой, зависящей от $\bar{c}$), и замена ломаной на отрезки $L_1-L_2-L_4-L_5$ уменьшит длину на величину, линейно зависящую от $[L_1L_2]$:
 поскольку $L_3 \notin B_r(y(L_1))$ выполняется 
 \[
 |Pr_{(y(L_1)L_1)}[L_2L_3]|<|Pr_{(y(L_1)L_1)}[L_1L_2]|+o(|L_1L_3|).
 \label{1111}
 \]
  Поскольку 
  \[
  |\angle (y(L_1)L_1), (ix])-\pi/2| =o_\rho(1)
  \]
 выполняется 
 \[
 |L_2L_3|_y<|L_1L_2|_y+o(|L_1L_2|+|L_2L_3|),
 \]
 где $|\cdot |_y$ означает длину проекции на прямую, перпендикулярную $(ix)$. Тогда
 \[
 |L_2L_3|\sin \frac{ \bar{c}}{2}<|L_1L_2|+o(|L_1L_2|+|L_2L_3|),
 \]
 то есть
 \[
 |L_2L_3|< \frac{1}{\sin \frac{ \bar{c}}{2}}|L_1L_2|+o(|L_1L_2|+|L_2L_3|). 
 \]
%Тогда для достаточно малого $\rho$ выполняется

 Аналогично, поскольку  $L_3 \notin B_r(y(L_1))$ и $|\angle (y(L_3)L_3), (ix])-\pi/2| =o_\rho(1)$ выполняется
  \[
 [L_2L_1]<\frac{1}{\sin \frac{ \bar{c}}{2}}|L_3L_2|+o(|L_1L_2|+|L_2L_3|). 
 \]
 В таком случае
 \[
\sin\frac{ \bar{c}}{2}- \frac{o(|L_1L_2|+|L_2L_3|)}{|L_3L_2|}\leq  \frac{|L_2L_3|}{|L_1L_2|}\leq \frac{1}{\sin \frac{ \bar{c}}{2}}+\frac{o(|L_1L_2|+|L_2L_3|)}{|L_1L_2|},
 \]
 а значит, для достаточно малого $\rho$ верно
 \[
\frac{\bar c}{3} < \sin \frac{ \bar{c}}{2}- \frac{o(|L_2L_3|(1+\frac{1}{\sin\frac{ \bar{c}}{2}}|L_1L_2|+o_\rho(1)))}{|L_3L_2|}\leq  \frac{|L_2L_3|}{|L_1L_2|}\leq \frac{1}{\sin \frac{ \bar{c}}{2}}+\frac{o(|L_1L_2|(1+ \frac{1}{\sin \frac{ \bar{c}}{2}}+o_\rho(1)))}{|L_1L_2|}< \frac{3}{\bar{c}}.
 \]
 
  %\[[L_2L_3]_y>|L_1L_2|_y-|L_1L_3| o_{\varepsilon(c)}(1)\]
 %|L_1L_2|-\bar{\varepsilon}^2,\]
  %где нижний индекс $y$ означает проекцию на ось абсцисс. То есть $|L_2L_3|>\sin c |L_1L_2|-o_{\bar{\varepsilon}}(1)|L_1L_3|$.
% И наоборот, $|L_1L_2|>\sin \bar{c} |L_2L_3|-o_{\bar{\varepsilon}}(1)|L_1L_3|$. 
 %Из этого очевидным образом следует существование $c_1, c_2>0$ таких, что $c_2|L_2L_3|\geq |L_1L_2| \geq c_1|L_1L_3|$.   
 Аналогично и для остальных $L_i$. 
 
 Замена ломаной $L_1-L_2-L_3-L_4-L_5$ на $L_1-L_2-L_4-L_5$ уменьшит ее длину не меньше, чем на величину, линейно зависящую от $|L_1L_2|$, поскольку $\angle L_2L_3L_4 \leq \pi-\bar{c}$ (а значит $\cos \angle L_2L_3L_4 \geq  -\cos \bar{c}$):
 \begin{multline*}
 |L_2L_3|+|L_3L_4|-|L_2L_4|=\frac{(|L_2L_3|+|L_3L_4|)^2-|L_2L_4|^2}{|L_2L_3|+|L_3L_4|+|L_2L_4|}>\\
 > \frac{2|L_2L_3||L_3L_4| (1+ \cos \angle L_2L_3L_4)}{2(|L_2L_3|+|L_3L_4|)}\geq
 \frac{|L_3L_4|(1- \cos \bar{c})}{ \left (1+\frac{|L_3L_4|}{|L_2L_3|} \right)}\geq  \frac{(\frac{\bar{c}}{3})^3}{(1+\frac{3}{\bar{c}})}|L_1L_2|.
\end{multline*}
 
 
 
% \[
% |L_2L_3|+|L_3L_4|-|L_2L_4|\geq  |L_2L_3|(1+\frac{c}{3}-\frac{1}{\sin c})>|L_2L_3|(1+\frac 2 c),
 %\]
 %поскольку 
 %\[
 %|L_2L_4|=\sin \angle L_2L_3L_4 \frac{|L_2L_3|}{\sin L_2L_4 L_3}\leq  \frac{|L_2L_3|}{\sin L_2L_4 L_3} \leq  \frac{|L_2L_3|}{\sin (\pi-c)}= \frac{|L_2L_3|}{\sin c}.
 %\]
 %ой ОЙОЙ ТУТ НЕ ТАК
 
% \begin{multline*}
 %|L_2L_3|+|L_3L_4|-\sqrt{ |L_2L_3|^2+|L_3L_4|^2+2 %|L_2L_3||L_3L_4|\cos (2c) }\geq \\
%|L_1L_2| \left(\sin c+\sin^2 c-\sqrt{\frac{1}{\sin^2 c}+\frac{1}{\sin^4 c}+2\frac{\cos (2c)}{\sin^3 c}})+o_{\varepsilon(c)}(1|L_1L_2| \right),
% \end{multline*}
%Таким образом замена уменьшает длину множества на величину, линейно зависящую от $|L_1L_2|$.
%\input{pictures/dvapo}
%Обозначим точки $L_6 \defeq [L_1y(L_3)] \cap \partial B_r(y(L_3))$ и $L_7 \defeq [L_5y(L_3)] %\cap \partial B_r(y(L_3))$ где $y(L_3)$ произвольная соответствующая $L_3$ точка. Тогда %$$B_r([L_1L_6]) \cup B_r([L_5L_7]) \supset B_r([L_1L_3]) \cup B_r([L_3L_5]).$$ и %$\H([L_1L_6]) \cup B_r([L_5L_7]))=o_{[L_1L_2]}(1)$ (это следует из теоремы Пифагора и  %пункта~\ref{1145} доказательства Леммы~\ref{Losiu}). Тогда можно заменить ломаную  %$L_1-L_2-L_3-L_4-L_5$ на $L_6-L_1-L_2-L_4-L_5-L_7$ и получить противоречие с оптимальностью %$\Sigma$ (см. рис~\ref{fig:dvapo}).
%А значит
%\[
%\H([L_1L_2]\cup [L_2L_4]\cup[L_4L_5]\cup S^{[L_1L_5]})\leq \H(L_1-L_2-L_3-L_4-L_5)-|L_2L_3|(1+\frac 2 c)+o(|L_1L_5|)<\H(L_1-L_2-L_3-L_4-L_5).
%\]
Тогда множество $ \Sigma \setminus ([L_2L_3] \cup [L_3L_4]) \cup [L_2L_4]\cup S^{[L_1L_5]}$ лучше $\Sigma$: является связным (поскольку все внутренние точки исходной ломаной --- степени два), обладает меньшей длиной и не большей энергией. Противоречие с оптимальностью $\Sigma$ (см. рис~\ref{fig:dvapo}).
%ПОМЕНЯТЬ РИСУНОК ИЛИ ВЕРНУТЬ ЗАКОМЕНЧЕННОЕ


\end{proof}

\begin{lemma}
Пусть $x \in E_\Sigma$ и  существует $Q^{a,x}_\varepsilon$ такой, что $Q^{a,x}_\varepsilon \cap \Sigma$ является дугой. Тогда для произвольного $c>0$ найдется $\varepsilon(c)>0$ такой, что все односторонние касательные к точкам множества $Q^{a,x}_\varepsilon \cap B_{\varepsilon(c)}(x) \cap \Sigma$ имеют угол с прямой $(ax)$, не больший $2c$.
\label{zapred}
\end{lemma}

\begin{proof}
Предположим противное, то есть что существует последовательность точек, в которых односторонняя касательная имеет угол с $(ix)$, больший $2c$ (не умаляя общности полагаем $2c \leq \pi/2$). Ввиду утверждения пункта~\ref{__3} Леммы~\ref{alm} это могут быть только точки из множества $X_\Sigma \sqcup S_\Sigma$. Поскольку точек ветвления нет, в точках $S_\Sigma$ направление касательной не меняется, то есть найдется сходящаяся к $x$ последовательность точек из $X_\Sigma$ таких, что хотя бы один из двух входящих в точку отрезков имеет угол с $(ix)$, больший $2c$. Пусть $L_1$ --- такая точка, достаточно близкая к $x$ (то есть $L_1 \in B_{\varepsilon(c)}(x)$, где $\varepsilon(c)$ выбирается для $c/5$ как в Лемме~\ref{alm} $\rho$ выбирается для $c$). Ввиду утверждения пункта~\ref{__2} Леммы~\ref{alm} оба входящих в $L_1$ отрезка имеют угол с $(ix)$, больший $9/5c$. Тогда отрезок, лежащий на пути из $L_1$ в $x$ обязательно заканчивается точкой $L_2 \in X_\Sigma$. Но отрезок, выходящий из $L_2$ должен иметь угол с $(ix)$, больший $8/5c$, и заканчиваться точкой $L_3 \in X_\Sigma$. Ясно, что таким образом для любого  сколь угодно малого $\bar \varepsilon$ существует такая ломаная $L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\bar{\varepsilon}}(x)$, что все углы $\angle((L_iL_{i+1}),(ix))>c$ при $i=1,2,3,4$. Противоречие с утверждением~\ref{brrrr}.
\end{proof}

Докажем Лемму~\ref{uggi}.
\begin{proof}
Докажем первый пункт. Не умаляя общности, будем считать $\rho_2$ удовлетворяющим утверждению леммы~\ref{alm} для $c=\frac{\pi}{100}$ и утверждению~\ref{zapred} для $c=\frac{1}{20}$. Кроме того, можно  выбрать $\rho_2>0$ таким, чтобы 
\[
\sharp(\Sigma \cap Q \cap \partial B_{\rho_2}(x))=\oordball_x(\Sigma\cap Q)\leq \oordball_x(\Sigma)\leq 3. 
\]
Несложно понять, что $\oordball_x(\Sigma \cap Q)=1$: в противном случае ввиду неравенства коплощади можно было бы уменьшить длину $\Sigma$, заменив $\Sigma \cap Q$ на множество $T^Q$, определенное в доказательстве Леммы~\ref{angles2} и обладающее длиной $\rho_2 +o(\rho_2)$. При такой замене энергия не увеличится, а связность сохранится. Таким образом, мы будем полагать $\sharp (\partial B_{\rho_2(x)} \cap \Sigma) =1$.
Пусть $Q_1 \defeq Q \cap \overline{B_{\rho_2}(x)}$.
Пусть $z \defeq \partial Q_1 \cap \Sigma$.
%Предположим, что $\Sigma \cap Q_1$ содержит бесконечное %число точек ветвления. Тогда найдется дуга 
%дуга $\breve{[sx]} \subset \Sigma \cap Q_1$ такая что %$|sx|=\rho_1$, содержащая бесконечное число точек %ветвления. 

Разберем два случая:
\begin{itemize}
\item[(А)] Пусть ребро $(ax]$ направлено в одну сторону.
Будем считать $(ax]$ отрицательной половиной оси абсцисс. Тогда будем полагать $\rho_2$ таким, чтобы все точки, соответствующие энергетическим точкам $\Sigma \cap Q_1$ располагались в одной (не умаляя общности, будем называть её верхней) полуплоскости.
% (это корректно, как было показано в доказательстве Леммы~\ref{Losiu}). 
%Поскольку $\Sigma$ не содержит циклов, путь между любыми двумя точками $\Sigma$ однозначно определен.
 Посчитаем изменение направления касательной вдоль дуги $\breve{[zx]}$. Поскольку ввиду конечной длины касательная есть почти во всех точках $\Sigma$, то будем воспринимать $\turn(\breve{[zx]})$ как верхний предел (супремум) по всем последовательностям точек кривой:
 \[
 \turn(\breve{[zx]})=\sup_{n\in \N, z\preceq t_1 \prec \dots \prec t_n \preceq x} \sum_{i=2}^{n} \angle(t^i,t^{i-1}),
 \]
 где  $t^i$ означает луч касательной к кривой $\breve{[zt_i]}\subset \breve{[zx]}$, а ${t_1,\dots, t_n}$ --- разбиение кривой $\breve{[zx]}$ в порядке, соответствующем параметризации, при которой $z$ --- начало кривой, а $x$ --- конец, такое, что в каждой точке $t_i$ кривая $\breve{[zx]}$ имеет касательную. В данном случае угол $\angle(t^i,t^{i-1}) \in [-\pi,\pi[$ между двумя лучами считается от луча $t^i$ к лучу $t^{i-1}$, положительное направление --- против часовой стрелки.
 
Заметим, что ввиду условий на $\rho_1$ верно
 \[
|\turn ([zx])| \leq 2\pi.
 \]
Покажем, что на пути из $z$ в $x$ конечное число точек ветвления. Для этого рассмотрим произвольную точку ветвления $D_2$ на дуге $\breve{[zx]}$. %Рассмотрим такую точку ветвления $D_2$ на дуге $\breve{[sx]}$, что на пути из $D_2$ в $x$ бесконечно точек ветвления, а на пути из $s$ в $D_2$ достаточно много точек ветвления. 
Из точки $D_2$ выходят три отрезка $[D_1D_2]$, $[D_2D_3]$ и $[D_2C]$ с попарными углами $2\pi/3$, где, не умаляя общности, ломаная $D_1-D_2-D_3$ --- подмножество пути из $z$ в $x$.  Заметим, что вклад в поворот $\breve{[zx]}$ точки $D_2$ составляет $-\pi/3$, поскольку угол $\angle D_1D_2D_3$, посчитанный против часовой стрелки, составляет $2\pi/3$. %и определяется %однозначно: в выбранных обозначениях угол, посчитанный %против часовой стрелки, составляет $2\pi/3$, то есть %поворот составляет $\pi/3$. 
 Это так, поскольку путь, начавшийся с отрезка $[D_2C]$ должен закончиться энергетической точкой, а значит должен идти в верхнюю  половину шара $B_{\rho_1}(x)$. 
 Аналогичное верно для произвольной точки ветвления внутри пути из $z$ в $x$.
Из Леммы~\ref{alm} и того, что ребро $(ax]$ направлено вверх (и ввиду выбора $\rho_1$) следует, что угол направления касательной в энергетических точках  на пути из $z$ в $x$ меняется по часовой стрелке (на величину, не превосходящую $\pi/6+1/100$), то есть вклад в $\turn$ неположительный.

(Строго говоря, в п~\ref{__2} леммы~\ref{alm} не сказано, что для энергетической точки $\bar x \in X_\Sigma$ точка $s$ встречается на пути из $z$ в $x$ раньше, чем точка $t$ (в противном случае вклад точки $\bar x$ в поворот мог бы быть отрицательным). Однако в данной ситуации это так, поскольку в противном случае пустой шар $B_r(y(\bar x))$ и путь из $z$ в $\bar x$ делают невозможным существование в $\Sigma \cap Q_1$ пути из $\bar x$ в $x$. Аналогичным способом нужно действовать в ситуации $\bar x \in E_\Sigma$).

В остальных точках $\breve{[zx]}$ направление касательной не меняется. Таким образом на пути из $z$ в $x$ конечное количество (не более $6$) точек ветвления. А значит найдется такое положительное $\rho_2<\rho_1$, что $\breve{[zx]} \cap \overline B_{\rho_2}(x)$ не содержит точек ветвления. Потребуем также, чтобы 
\[
\sharp (\partial B_{\rho_2}(x) \cap \Sigma) = \oordball_x(\Sigma \cap Q)=1.
\]
%и обозначим
%\[
%Q_2 \defeq Q \cap \overline{B_{\rho_2}(x)}.
%\]
В таком случае $\Sigma \cap \overline{B_{\rho_2}(x)}$ является дугой.
\begin{remark}
Таким образом мы доказали, что точка $x\in E_\Sigma$ может быть пределом точек ветвления только если у неё есть направленное в две стороны ребро.  
 \label{remA}
\end{remark}
\item[(Б)] Пусть ребро $(ax]$ направлено в обе стороны.


%Выберем  $\rho$ не превосходит $\rho$ из %Леммы~\ref{alm} для $c=\pi/100$ и $\rho$ из %Утверждения~\ref{zapred} для $c=\frac{1}{20}$. 

Предположим, что $Q \cap \Sigma$ содержит бесконечное число точек ветвления. Тогда оно также содержит бесконечное число концевых точек. 

%Пусть $W$ такая концевая точка. Тогда, ввиду п.~\ref{__1} Леммы~\ref{alm} она принадлежит множеству $X_\Sigma$ и имеет %порядок $1$. Обозначим максимальный выходящий из неё отрезок за $[WD_1]$. Тогда $|\angle((WD_1),(ix))-\pi/2|<\pi/100$. %Точка $D_1$, ввиду пп.~\ref{__2} (см Следствие~\ref{__2c}) и~\ref{__3} Леммы~\ref{alm} может быть только точкой %ветвления. Пусть $[D_1 D_2]$ максимальный отрезок на пути $\Sigma$ из $D_1$ в $x$. Поскольку $|\angle (D_1D_2), (ix) %-\pi/6|<\pi/100$, точка $D_2$ может быть только точкой дискретного энергетического множества порядка $2$ или точкой %ветвления.

%Из Леммы~\ref{alm} следует, что в каждой точке $\bar x \in B_\rho(x) \cap G_\Sigma \setminus \{x\}$ существуют %односторонние касательные. 

Несложно заметить, что поскольку $\sharp (\partial B_{\rho_2}(x) \cap \Sigma)=1$, каждая точка ветвления на пути из $z$ в $x$ соединена ребром с концевой точкой:

%БЛИН ДОЛЖНО ЖЕ БЫТЬ ПРОСТОЕ ОБЪЯСНЕНИЕ

Предположим противное. В таком случае на пути из $z$ в $x$ найдется точка ветвления $A$, соединенная с точкой ветвления $B$, не лежащей на пути из $z$ в $x$.  При этом хотя бы один из двух отрезков $\Sigma \setminus [AB]$, инцидентных $B$, не является перпендикулярным или параллельным $(ax]$ с точностью до $\pi/100$, таким образом он неизбежно заканчивается точкой ветвления, из которой также исходит хотя бы один отрезок, который не является перпендикулярным или параллельным $(ax]$ с точностью до $\pi/100$. И так далее. В таком случае найдется путь, начинающийся с этого отрезка и никогда не заканчивающийся, причем направления отрезков одинаковой четности --- одинаковые. Несложно заметить, что предельная точка $w$ этого пути должна принадлежать непрерывному энергетическому множеству и лежать в шаре  $B_\rho(x)$, а тогда, ввиду изложенного в пункте (А) (см замечание~\ref{remA}), её энергетическое ребро должно быть направлено в две стороны. 
Однако в таком случае, при достаточно малом $\rho_2$ выполняется $\partial B_{xw}(x) \cap \Sigma \cap Q_1=\{w \}$, а это противоречит существованию пути из $z$ в $x$ лежащего в $Q_1$ и не содержащего $w$.


%Но мы считаем ребро $(ax]$ отрицательной полуосью абсцисс, а точку $w$ лежащей выше пути из $z$ в $x$, а в таком случае любая точка, соответствующая точке $w$ должна находиться в верхней полуплоскости. 
% а значит $B_r(y(w))$ содержал бысти (поскольку, как следует из  п.3. доказательства Леммы~\ref{Losiu}, $(w, y(w))$ %перпендикулярна $(ax)$ с точностью до $\pi/100$). 
Получили противоречие с тем, что энергетическое ребро точки $w$ направлено в две стороны).

Таким образом, ввиду п.~\ref{__1} Леммы~\ref{alm} в каждой точке ветвления на пути из $z$ в $x$ угол между входящим в нее отрезком этого пути и прямой $(ax)$ находится в промежутке $[\pi/6-\pi/100, \pi/6+\pi/100]$. Пусть $D_1$ --- точка ветвления на пути  из $z$ в $x$ и пусть $[D_1 D_2]$ --- максимальный отрезок на пути $\Sigma$ из $D_1$ в $x$. Поскольку $|\angle (D_1D_2), (ax) -\pi/6|<\pi/100$, точка $D_2$ может быть только точкой дискретного энергетического множества порядка $2$ или точкой ветвления.
Если точка $D_2$ --- точка ветвления, то, аналогично, конец максимального отрезка $[D_2D_3]$ может быть точкой дискретного энергетического множества порядка $2$ или точкой ветвления, а угол $\angle((D_2D_3),(ax))=\pi/3-\angle((D_1D_2),(ax))$, то есть находится в промежутке $[\pi/6-\pi/100, \pi/6+\pi/100]$. Если же $D_2$ --- точка дискретного энергетического множества порядка $2$, то ввиду п.~\ref{__2} Леммы~\ref{alm}
\[
\angle((D_2D_3),(ix)) \in [\angle((D_1D_2),(ix))-\pi/100, \angle((D_1D_2),(ix))+\pi/100] \subset [\pi/6-\pi/50,\pi/6+\pi/50],
\]
где $[D_2D_3]$ --- максимальный отрезок пути из $D_2$ в $x$. Таким образом путь из $D_1$ в $x$ начинается с ломаной. При этом угол между односторонней касательной и прямой $(ix)$ в узлах ломаной либо принадлежит промежутку $[\pi/6-\pi/100, \pi/6+\pi/100]$ (если узел был точкой ветвления), либо меняется на величину, не превосходящую $\pi/100$. Поскольку, ввиду утверждения~\ref{brrrr}, путь $[sx]$ не может содержать ломаную с пятью подряд узлами в энергетических точках, односторонние касательные в которых имеют угол с $(ax)$, больший $1/10$, среди первых пяти после $D_1$ узлов ломаной должна встретиться точка ветвления $C$. При этом поскольку все односторонние касательные к точкам пути между $D_1$ и $C$ имеют угол c $(ax)$, больший $\pi/6-\pi/20>\pi/10$, там не будет точек из непрерывного энергетического множества.

Повторяя рассуждения для точки $C$ в качестве $D_1$, а затем итерируя, получаем путь $\sigma$, все односторонние касательные вдоль которого имеют угол с $(ax)$, больший $1/10$. Пусть $\bar x$ предельная точка такого пути ($\bar x$ принадлежит пути из $z$ в $x$ и может совпадать с $x$). Ясно, что $\oordball_\sigma \bar x =1$. Выберем $\rho_0>0$ таким, что 
\[
\sharp (\sigma \cap \partial B_{\rho_0}(x_0))=1.
\]
Определим \[z_0=z_0(\rho_0) \defeq \partial B_{\rho_0}(x_0) \cap \sigma.\]
Пусть $(a_0x_0]$ энергетическое ребро $x_0$ ближайшее к энергетическим точкам $\sigma \cap B_{\rho_0}(x_0)$.
Тогда 
\[
\angle z_0x_0a_0=o_1(\rho_0)
\]
и 
\[ 
\H(Pr_{(a_0x_0]}(\sigma \cap B_{\rho_0}(x_0))) \geq \cos (\angle z_0x_0a_0) |z_0 x_0|.
\]
При этом $\angle ((ax], (a_0x_0])=o_{\rho_2}(1)$, а значит, при достаточно малом $\rho_2$, все односторонние касательные к $\sigma \cap B_{\rho_0}(x_0)$ имеют угол с $(a_0x_0]$, больший $1/20$.
Тогда
\[
\H(\sigma \cap B_{\rho_0}(x_0)) \geq \frac{Pr_{(a_0x_0]}(\sigma \cap B_{\rho_0}(x_0))}{\cos \frac{1}{10}}\geq \frac{\cos (\angle  z_0x_0a_0)}{\cos \frac{1}{10}}|z_0 x_0|=\frac{\cos (o_{\rho_0}(1))}{\cos \frac{1}{10}}\rho_0.
\]
С другой стороны, поскольку ребро $(a_0x_0]$ направлено в обе стороны, выполняется $\H(\sigma \cap B_{\rho_0}(x_0))=\rho_0+o_{\rho_0}(1)$. Противоречие для достаточно малого $\rho_0$.


%То есть при достаточно малом $\rho_0$ выполняется $\H(\sigma \cap B_{\rho_0}(x_0)) > |z_0x_0|(1+10^{-4})$.



%Тогда \[\H(\sigma \cap B_{\rho_0}(\bar x))>\frac{\rho_1}{\cos {\frac{1}{10}}}|z_0\bar x|.\]
%Пусть $\beta(\rho_0)$ --- минимальный угол с вершиной в $\bar x$, содержащий все точки $Q_\Sigma \cap \sigma \cap B_{\rho_0}(\bar x)$. Заметим, что $\angle \beta(\rho_0)=o_{\rho_0}(1)$. Обозначим 
%\[
%\breve{u_0v_0} \defeq \beta(\rho) \cap \partial B_{\rho_0}(\bar x).
%\]
%Тогда множество
%\[
%\Sigma \setminus (\sigma \cap B_{\rho_0}(\bar x)) \cup [\bar x z_0] \cup \breve{u_0v_0} \cup S^{[u_0\bar x]} \cup S^{[v_0 \bar x]}
%\]
%имеет длину $|z_0x_0|+o(|z_0x_0|)$, а значит данное множество связно, обладает меньшей длиной и не большей энергией, чем $\Sigma$. Противоречие.

%Пусть $(\bar a \bar x]$ --- %энергетическое ребро $\bar x$, к %которому сходятся энергетические точки %пути (он существует ввиду ). В таком %случае 



%Заметим, что для любого $\rho_1<|D_1x|$ такого, что $\sharp(\partial %B_{\rho_1}(x))=1$, выполняется $\H(\Sigma \cap Q \cap %B_{\rho_1}(x))>\frac{\rho_1}{\cos {\frac{1}{10}}}$. Получили %противоречие с тем, что $\H(\Sigma \cap Q \cap %B_{\rho_1}(x))=\rho_1+o(\rho_1)$.
%Утверждение про наклон касательной непосредственно следует из Утверждения~\ref{zapred}.
\end{itemize}
Осталось доказать пункт~\ref{AB}. 
Не умаляя общности будем считать, что ребро $(ax]$ направлено в одну сторону, поскольку в противном случае применим пункт~\ref{A} (см замечание~\ref{remA}).
Пусть $\varepsilon>0$ такое, что $\sharp (\partial B_\varepsilon(x)\cap \Sigma)=\oordball_x\Sigma \leq 3$. И пусть $s \in \partial B_\varepsilon(x)$ такая, что путь из $s$ в $x$ лежит в $\overline{B_\varepsilon(x)}$.

Рассмотрим величину поворота пути: $|\turn(\breve{sx})|<2\pi$. Аналогично рассуждениям в предыдущем пункте заметим, что конечность величины поворота и наличие в компоненте связности энергетических точек только одного ребра, причем направленного в одну сторону, влечет конечность числа точек ветвления на пути из $s$ в $x$. Таким образом можно выбрать $\varepsilon>0$ таким, что $\breve{sx}$ не содержит точек ветвления.

Тогда ввиду Леммы~\ref{dug_ok}  $\breve{sx}$  содержится внутри некоторого псевдоконуса.

%Пусть инъективная функция $f: [0;1] \rightarrow \R^2$ параметризует $\breve{[sx]}$. Множество $\breve{[sx]} \cap G_\Sigma$ содержится в псевдоконусе $Q_{\rho}^{a,x}$. Будем также считать, что это псевдоконус имеет следующий вид: $Q^{a,x}_{\varepsilon} \defeq \bigcup_{k=1}^{\infty} \left( Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) \right)$ для некоторых сходящихся к нулю монотонных последовательностей неотрицательных чисел $\{s_k\}$ и $\{\rho_k\}$, где $\rho_1=\varepsilon$ (см Лемму~\ref{con}). Будем считать выбранные последовательности минимальными по включению. Пусть точки $c,d \in [0;1]$ такие, что $f([c,d])\cap G_\Sigma=f(c) \cup f(d)$. Тогда, ввиду отсутствия на дуге $\breve{[sx]}$ точек ветвления, выполняется $f([c,d])=[f(c),f(d)]$. В таком случае, если $f(c) \in Q(\rho_{k-1},s_{k-1},x,a) \setminus B_{\rho_{k}}(x) $, $f(d) \in Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) $, то выполняется $[f(c);f(d)] \subset  Q(\rho_{k-1},s_{k-1},x,a) \setminus B_{\rho_{k+1}}(x)$. А значит, 
%\[
%\breve{[sx]}=f([0;1]) \subset \bar{Q}^{a,x}_{\varepsilon} \defeq \bigcup_{k=1}^{\infty} \left(Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+2}}(x) \right).
%\]
%Тогда к $\breve{[sx]}$ применим пункт~\ref{A}.
%МОЖЕТ НАДО ВЕРНУТЬ
%\end{proof}

\end{proof}

%Докажем лемму~\ref{eva}. может вернем сюда
%ВРОДЕ ИЗ ТОГО, ЧТО ДАЛЬШЕ --- НИЧЕГО НЕ НУЖНО. ПЕРЕНЕСЛА ЭТО в trash801 %пока

ОСТАТКИ ПЕРЕВОДА ДЛЯ ФИНЛЯНДИИ:

In fact, in the announced work even stronger result is proven: all these statements hold for a larger class of local minimizers.

 \begin{definition}
    Let $M \subset \mathbb{R}^2$ be a planar compact set. A connected set $\Sigma$ is called \emph{local minimizer} if it covers $M$
    and there is an $\varepsilon > 0$ such that for every connected $\Sigma'$ covering $M$ and satisfying
    $\diam (\Sigma \Delta \Sigma') \leq \varepsilon$ one has $\H (\Sigma) \leq \H (\Sigma')$.
    \label{local}
\end{definition}


\begin{theorem2}
Let $\Sigma$ be a local minimizer. Then all the statements of Theorems~\ref{mainT1} and~\ref{persp} hold.
\label{TTT}
\end{theorem2}

\begin{corollary}
Theorem~\ref{mainT1} (accordingly~\ref{TTT}) implies that the set of branching points of a (local) minimizer is finite.  
\end{corollary}



==> ⥪�騩 ���᪨� ⥪�� (in english)/parts/per.tex <==
\section{Остальные локальные свойства минимайзеров}
\label{per}


Использованные в статье методы позволяют получить большое количество утверждений относительно гладкости и локальной структуры $\Sigma$. %В частности,

%\subsection{Еще несколько результатов}

%\begin{remark}
%А обозначениях теоремы~\ref{mainT1} можно считать, что каждая инъективная кривая имеет на конце непрерывную касательную. Иными словами, односторонние касательные ко внутренним точкам кривой сходятся к касательной в концевой точке.
%\end{remark}

\begin{theorem2}
Пусть $\Sigma$ --- минимайзер максимального расстояния для плоского компактного множества $M$.  Тогда
\begin{enumerate}
\item в окрестности произвольной точки $x\in \Sigma$ множество $\Sigma$ совпадает с одной, двумя или тремя дугами с концами в $x$, имеющими в $x$ непрерывную касательную %(соответствующие им функции имеют в $x$ непрерывную первую производную).   
Также в каждой из точек каждой из дуг есть односторонняя касательная, односторонние касательные непрерывно сходятся к касательной к дуге в точке $x$.
Каждая из дуг является графиком функции, имеющей в точке $x$ непрерывную производную (за абсциссу считаем касательную). 
%Для краткости будем называть такие функ
\label{f}
\item в достаточно малой окрестности $B_{\varepsilon}(x)$ произвольной точки $x\in \Sigma$ выполняется
 \[
  \oord_x\Sigma \cdot \varepsilon \leq \H(\Sigma \cap B_\varepsilon(x)) = \oord_x \Sigma \cdot \varepsilon +o(\varepsilon).
 \]
 Заметим, что это уточняет константы регулярности по Альфорсу (см. свойства минимайзеров п.~\ref{j});
 \label{len1}
\item для произвольной точки $x\in \Sigma$ выполняется $\oord_x\Sigma=\oordball_x\Sigma$; 
\label{oo}
\item множество $\Sigma$ в окрестности произвольной $x \in G_\Sigma$ является графиком некоторой функции %(для краткости будем называть такую функцию "соответствующей"). 
Если точка $x \in G_\Sigma$ имеет два различных касательных луча, угол между которыми меньше $\pi$, то $\Sigma$
%(как функция) 
локально нестрого выпукла в окрестности точки $x$ (выпукла внутрь меньшего угла). В таком случае соответствующая функция нестрого выпукла, то есть, в частности,
%$\Sigma$ в окрестности $x$ является графиком нестрого выпуклой функции, то есть, в частности, функции, которая 
%Это, в частности означает, что соответствующая ей функция 
почти всюду имеет вторую производную;
\label{conv_}
\item если (содержащаяся в $\Sigma$) инъективная кривая с концом в точке $x$ не является нестрого выпуклой в её окрестности, то 
\label{nevv}
\begin{enumerate}
\item если она имеет кривизну, то кривизна по модулю не превосходит $1/r$ (если соответствующая данной кривой функция имеет в точке $x$ вторую производную, то она по модулю не превосходит $1/r$);
\item её односторонние касательные сходятся к односторонней касательной в точке $x$ (соответствующая данной кривой функция имеет непрерывную первую производную в точке $x$);
\label{ggg}
\item если существует другая инъективная кривая с концом в $x$, то  ее кривизна, в случае наличия, по модулю не превосходит $1/r$, а её односторонние касательные сходятся к односторонней касательной в точке $x$. При этом односторонние касательные к обеим инъективным кривым образуют прямую (то есть, функция, соответствующая $\Sigma$, имеет непрерывную производную в $x$); 
\item в достаточно малой окрестности $B_{\varepsilon}(x)$  выполняется
 \[
\oord_x\Sigma \cdot \varepsilon  \leq \H(\Sigma \cap B_\varepsilon(x)) \leq \oord_x\Sigma \cdot \varepsilon +O(\varepsilon^2).
 \]
 \label{len2}
\end{enumerate}
\end{enumerate}
\label{persp}
\end{theorem2}
\begin{proof}

Докажем пункт~\ref{f}. Из доказательства Теоремы~\ref{mainT1}  следует, что
каждая такая дуга либо является отрезком, либо содержится в псевдоконусе с вершиной в $x$ и энергетическим ребром в качестве оси. В первом случае утверждение пункта очевидно, а во втором следует из леммы~\ref{zapred}.
%\end{proof}
%леммы~\ref{eva} ы~\ref{uggi}
Покажем верность пункта~\ref{len1}. Множество $\Sigma \setminus \{x\}$ имеет $\oord_x \Sigma \leq 3$ компонент связности. Каждая из компонент связности, ввиду Теоремы~\ref{mainT1} имеет в точке $x$ касательную, а значит ввиду замечания~\ref{len0}, в достаточно малом шаре $B_\varepsilon(x)$ имеет длину $\varepsilon+ o(\varepsilon)$. 

Таким образом
\[
\H(\Sigma \cap B_\varepsilon(x)) =\oord_x \Sigma \varepsilon +o(\varepsilon).
\]
 Неравенство $\H(\Sigma \cap B_\varepsilon(x)) $ напрямую следует из неравенства коплощади

Покажем верность пункта~\ref{oo}. Предположим противное, то есть, ввиду замечания~\ref{rem_ord}, что $\oordball_x\Sigma >\oord_x\Sigma $.
В таком случае для достаточно малого $\varepsilon$
\[
\H(\Sigma \cap B_\varepsilon(x)) \geq \oordball_x \Sigma \varepsilon \geq (\oord_x \Sigma +1) \varepsilon,
\]
что противоречит утверждению пункта~\ref{len1}.

Докажем пункт~\ref{conv_}. Утверждение интересно только для $x\in E_\Sigma$. В таком случае хотя бы одна из двух касательных является энергетическим ребром, при этом ребро направлено в одну сторону. Рассмотрим дугу $\breve{sx}$, являющуюся замыканием компоненты связности $\Sigma \cap B_\varepsilon(x) \setminus \{x\}$ для достаточно малого $\varepsilon$, для которой данное энергетическое ребро является касательной в точке $x$. Не умаляя общности, будем полагать это ребро совпадающим с отрицательной частью оси абсцисс и будем полагать его направленным вверх. Будем также полагать, что для всех энергетических точек, принадлежащих $\breve{sx}$, соответствующие им точки находятся в верхней полуплоскости (это возможно ввиду показанного в лемме~\ref{Losiu}). В таком случае не существует двух точек $z_1, z_2 \in \breve{]sx[} $ таких, что поддуга $\breve{sx}$, их соединяющая, находится ниже соединяющего их отрезка: в противном случае замена дуги на отрезок уменьшило бы длину, без ущерба для связности и энергии. Несложно заметить, что данное свойство влечет нестрогую выпуклость вверх дуги $\breve{sx}$. Также мы показали, что $\breve{sx}$ можно рассматривать как график нестрого выпуклой функции.

Перейдем к пункту~\ref{nevv}: как было показано выше точка $x$ должна принадлежать множеству $E_\Sigma$, причем иметь энергетическое ребро, направленное в две стороны. В таком случае найдутся такие точки $y_1$, $y_2$, что прямая $(y_1y_2)$ перпендикулярна энергетическому ребру, \[|y_1x|=r=|xy_2|\] и \[B_r(y_1) \cap \Sigma =\emptyset = B_r(y_2)\cap \Sigma.\]
Отсюда тривиально следуют все утверждения пункта.
%\begin{remark}
%Доказательство  пунктов~\ref{len1} и~\ref{len2} можно было бы провести и аналитически, сопоставив кривой график функции $f$, точке $x$ начало координат, а касательной к кривой в точке $x$ --- ось абсцисс. Тогда $f(0)=0=f'(0)$. В случае~\ref{len2} кривую также пришлось бы сгладить, после чего заметить ограниченность модуля второй производной гладкой функции, приближающей $f$, числом $1/r$. 
%\end{remark}

\end{proof}
%Доказательства Теоремы~\ref{persp} 
%можно найти в разделе~\ref{prf}, 
%и объяснение, как методами данной статьи получать другие локальные утверждения можно найти в разделе~\ref{per}.
%Доказаны также некоторые еще утверждения про выпуклость %множества $\Sigma$ (см Леммой~\ref{main_ld}).


На самом деле, мы доказали даже более сильный результат, поскольку в доказательствах Теорем~\ref{mainT1} и~\ref{persp}  использовались только локальные аргументы, и поэтому его можно провести и для определенного ниже локального минимайзера.

\begin{definition}
Для заданного компактного множества $M \subset \R^2$ и числа $r>0$ локальным минимайзером функционала максимального расстояния будем называть такое связное замкнутое множество $\Sigma \subset \R^2$, что $F_M(\Sigma)\leq r$ и существует такое $\varepsilon>0$, что для произвольного замкнутого связного $\Sigma'$ такого, что $F_M(\Sigma')\leq r$ и $\diam \Sigma \triangle  \Sigma' < \varepsilon$ выполняется $\H(\Sigma)\leq \H(\Sigma')$.
\end{definition}

\begin{theorem2}
Пусть $\Sigma$ --- локальный минимайзер максимального расстояния.  Тогда выполняются все утверждения Теорем~\ref{mainT1} и~\ref{persp}.
%\begin{itemize}
%\item[(i)] множество $\Sigma$ является объединением конечного числа инъективных кривых;
%\item[(ii)] угол между любыми двумя касательными лучами в произвольной точке $x \in \Sigma$ не меньше $2 \pi/3$.
%\end{itemize}
%\label{mainT2}
\end{theorem2}

%\begin{corollary}
%Из Теоремы~\ref{mainT1} следует конечность числа точек порядка $3$ в (локальном) минимайзере максимального расстояния.
%\end{corollary}






%Покажем  верность Теоремы~\ref{persp}.


Поговорим о том, как получать иные утверждения о локальном поведении $\Sigma$. Оно интересует нас только в окрестностях точек из множества $E_\Sigma$. Ясно, что точки $E_\Sigma$ бывают следующих типов:
%\begin{enumerate}
%\item точки ветвления $x\in S_\Sigma$ степени $3$. Таких точек конечное число, поэтому при исследовании окрестностей точек $x\in %E_\Sigma$ можно считать, что их не существует.
%\item точки $x\in S_\Sigma$ степени $2$. Касательная в этих точках не меняется.
%\item точки $x\in X_\Sigma$ степени два такие, что существуют две окружности с центрами в $y_1,y_2$ такие, что $|y_1y_2|=2r$ и %$B_r(y_1)\cap \Sigma=\emptyset=B_r(y_2)\cap \Sigma$. В этом случае в точке $x$ касательная не меняется.
%\item Более интересные точки:
\begin{itemize}
%\item [(a)] точки $x\in X_\Sigma$ степени два такие, что в них $\Sigma$ имеет два разных отрезка с углом, не равным $\pi$; 
\item [(i)] точки $x\in E_\Sigma$ такие, что не существует двух окружностей с центрами в $y_1,y_2$ таких, что $|y_1y_2|=2r$ и $B_r(y_1)\cap \Sigma=\emptyset=B_r(y_2)\cap \Sigma$. Тогда $\Sigma$ в окрестности точки $x$ (нестрого) выпукла. % (однако хотя бы одна окружность $B_r(y)$, такая что $B_r(y)\cap\Sigma=\emptyset$ существует и ее расположение задает направление выпуклости). 
А значит, имеет субградиент, а также почти всюду выпукла и являются графиком функции, которая почти всюду %(но не обязательно в $x$)
имеет производную, которая монотонна;
\item [(ii)] точки $x\in E_\Sigma$ такие, что существуют две окружности с центрами в $y_1,y_2$, такие что $|y_1y_2|=2r$ и $B_r(y_1)\cap \Sigma=\emptyset=B_r(y_2)\cap \Sigma$. Тогда $\Sigma$ является графиком функции, которая имеет непрерывную производную в точке $x$. А если она имеет вторую производную, то та ограничена по модулю величиной $1/r$. 
\end{itemize}
%\end{enumerate}
%При этом точки типа (ii) являются пределом либо точек степени (ii), либо точек типа (i) или (a), где пустые окружности расположены по разную сторону от кривой. При этом выпуклость может меняться только в точках типа (ii), либо (в некотором смысле) в таких точках типа (i), что одна из кривых --- прямолинейный отрезок.

Если какая-то дуга минимайзера (c концом в $x$) целиком состоит из точек типа (i), то она наследует свойства некоторого подмножества множества $M$: утверждается, что множество $M$ тогда должно иметь кривую (или счетный набор кривых), полученную из данной дуги отступлением по внешней (если считать дугу границей выпуклой фигуры) нормали на $r$ во всех точках, где нормаль единственна (то есть в почти всех точках дуги). В частности, если дуга была непрерывно дифференцируемой, то ей соответствует дуга множества $M$. Причем данная дуга $\Sigma$ тогда должна быть дважды дифференцируемой, соответствующая ей дуга множества $M$ также должна быть дважды дифференцируемой, причем её вторая производная должна не превосходить $1/r$. Если она строго меньше $1/r$, то есть минимальный радиус кривизны дуги $M$ больше $r$, то тогда минимальный радиус кривизны дуги $\Sigma$ в точности равен разности между минимальным радиусом кривизны дуги $M$ и числом $r$. Доказательство данного факта мы приводить не будем, оно является достаточно очевидным следствием основного свойства энергетических точек. 

Если какая-то дуга целиком состоит из точек типа (ii), то она является непрерывно дифференцируемой. Тогда множество $M$ содержит две дуги полученных из данной дуги $\Sigma$ отступами по обеим нормалям на $r$. Несложно заметить, что тогда исходная дуга является дважды дифференцируемой и значит её вторая производная по модулю ограничена величиной $1/r$. При этом радиусы кривизны кривых $M$ отличаются от её радиусов кривизны в каждой точке на $r$.

Таким образом, получается что точки всех видов обладают рядом полезных свойств, комбинируя которые можно получать новые свойства $\Sigma$ или отвечать на вопрос, может ли то или иное множество быть минимайзером (отвечать отрицательно или конструктивно строить множество $M$, для которого данное множество может быть минимайзером). В частности --- графики элементарных функций, поскольку они (кроме графиков константы) обязаны состоять только из точек типа (i) и (ii).

\begin{example}
Может ли кривая, являющаяся графиком функции $f(x)= x^2\sin(\frac{1}{x})$ в окрестности нуля быть минимайзером для некоторого множества $M$?
\end{example}
\begin{proof}
Заметим, что точка $0$ --- точка типа (ii). Но производная функции $f$ не является непрерывной в нуле и значит график данной функции не может быть минимайзером. 
\end{proof}

\begin{example}
Может ли кривая, являющаяся графиком функции $f(x)= x^2 \sin \left (\frac{1}{\sqrt{x}} \right)$ в окрестности нуля быть минимайзером для некоторого множества $M$?
\end{example}
\begin{proof}
Заметим, что точка $0$ --- точка типа (ii). Теперь производная $f$ непрерывна в нуле. Поскольку для каждой точки $x\neq 0$ вторая производная существует, непрерывна и ее значение по модулю стремится к бесконечности при приближении к нулю и, значит, можно считать, что она больше, чем $1/r$. Тогда каждая точка, кроме $0$ может быть только типа (i). Но знак второй производной все время меняется и, значит, существует стремящаяся к нулю последовательность точек, в которых кривая меняет выпуклость. Ввиду отсутствия прямолинейных отрезков получили противоречие.
\end{proof}
%а выпуклость может меняться?



%Покажем верность правых частей в неравенствах пунктов~\ref{len1} и~\ref{len2}. Для этого достаточно показать, что %длина каждой из кривой


%Осталось доказать пункты~\ref{len1} и~\ref{len2}. Левые части следуют из неравенства ко-площади Предположим, это не так и длина какой-то из кривых
%ой еще про орд равно ордболл


%точки первого и второго типа
%пример: рассказ почему x^2\sin(\sqrt{x}) не подходит, хотя казалось бы а ой нет она же гладкая вне нуля и значит вт произв дб ограничены а они нет

==> ⥪�騩 ���᪨� ⥪�� (in english)/parts/trash.tex <==


Let $Q_1$ and $Q_5$ be such cusps with vertices at $L_1$ and $L_5$ and axes almost parallel to $o_rho(\bar x)$ that 

Let $S$ be the point of intersection $\partial B_r(y(L_1))$ and $\partial B_r(y(L_3))$. Let $A'$ be an area bounded by $[L_1,L_5]$, $\breve{L_1S}, $\breve{L_5S}$ where the arcs are the arcs of circumferences $\partial B_r(y(L_1))$ and $\partial B_r(y(L_3))$. And let $A$ be the union of $A'$ and its reflection regarding to $L_1L_5$. Thus $A$ is a union of two cusps $Q_1\in \mathbb{Q_{|L_1S|}}^{L_5,L_1}$ and $Q_5\in \mathbb{Q_{|L_5S|}}^{L_1,L_5}$. Then sets $S^{Q_1}$ and $S^{Q_5}$ defined at the proof of lemma~\ref{angles2} are such that $\H(S^{Q_1})=o(|L_1S|)$, $\overline{B_r(Q_1)}\subset \overline{B_r(S^{Q_1})}$
URURU


Let us construct a 


Now look at the set $ \Sigma \setminus ([L_2L_3] \cup [L_3L_4]) \cup [L_2L_4]\cup S^{[L_1L_5]}$, where $S^{[L_1L_5]}$ is defined in the proof of lemma~\ref{angles2}.



  
 Тогда множество $ \Sigma \setminus ([L_2L_3] \cup [L_3L_4]) \cup [L_2L_4]\cup S^{[L_1L_5]}$ лучше $\Sigma$: является связным (поскольку все внутренние точки исходной ломаной --- степени два), обладает меньшей длиной и не большей энергией. Противоречие с оптимальностью $\Sigma$ (см. рис~\ref{fig:dvapo}).



Предположим противное, то есть (ввиду Леммы~\ref{alm} п.~\ref{__2} для $c= \bar c/ 10$) что для сколь угодно малого $\rho > 0$ существует такая ломаная $L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\rho}$, что все углы $\angle((L_iL_{i+1}),(ix))> \bar{c}/2$ при $i=1,2,3,4$. 
Будем считать $(ix)$ осью абсцисс, а $\bar{c}$ достаточно малым. Не умаляя общности, точкам $L_1$, $L_3$, $L_5$ соответствуют верхние точки множества $M$, а точкам $L_2, L_4$ --- нижние: ввиду пункта~\ref{1145} доказательства Леммы~\ref{Losiu} и неравенства $\angle L_{i-1}L_{i}L_{i+1} \leq \pi-\bar{c}$, $i=2,3,4$ двум подряд идущим точкам не могут соответствовать одновременно верхние или нижние точки.
 Заметим теперь, что отношения между отрезками ломаной линейные (то есть отношение оценивается сверху и снизу константой, зависящей от $\bar{c}$), и замена ломаной на отрезки $L_1-L_2-L_4-L_5$ уменьшит длину на величину, линейно зависящую от $[L_1L_2]$:
 поскольку $L_3 \notin B_r(y(L_1))$ выполняется 
 \[
 |Pr_{(y(L_1)L_1)}[L_2L_3]|<|Pr_{(y(L_1)L_1)}[L_1L_2]|+o(|L_1L_3|).
 \label{1111}
 \]
  Поскольку 
  \[
  |\angle (y(L_1)L_1), (ix])-\pi/2| =o_\rho(1)
  \]
 выполняется 
 \[
 |L_2L_3|_y<|L_1L_2|_y+o(|L_1L_2|+|L_2L_3|),
 \]
 где $|\cdot |_y$ означает длину проекции на прямую, перпендикулярную $(ix)$. Тогда
 \[
 |L_2L_3|\sin \frac{ \bar{c}}{2}<|L_1L_2|+o(|L_1L_2|+|L_2L_3|),
 \]
 то есть
 \[
 |L_2L_3|< \frac{1}{\sin \frac{ \bar{c}}{2}}|L_1L_2|+o(|L_1L_2|+|L_2L_3|). 
 \]
%Тогда для достаточно малого $\rho$ выполняется

 Аналогично, поскольку  $L_3 \notin B_r(y(L_1))$ и $|\angle (y(L_3)L_3), (ix])-\pi/2| =o_\rho(1)$ выполняется
  \[
 [L_2L_1]<\frac{1}{\sin \frac{ \bar{c}}{2}}|L_3L_2|+o(|L_1L_2|+|L_2L_3|). 
 \]
 В таком случае
 \[
\sin\frac{ \bar{c}}{2}- \frac{o(|L_1L_2|+|L_2L_3|)}{|L_3L_2|}\leq  \frac{|L_2L_3|}{|L_1L_2|}\leq \frac{1}{\sin \frac{ \bar{c}}{2}}+\frac{o(|L_1L_2|+|L_2L_3|)}{|L_1L_2|},
 \]
 а значит, для достаточно малого $\rho$ верно
 \[
\frac{\bar c}{3} < \sin \frac{ \bar{c}}{2}- \frac{o(|L_2L_3|(1+\frac{1}{\sin\frac{ \bar{c}}{2}}|L_1L_2|+o_\rho(1)))}{|L_3L_2|}\leq  \frac{|L_2L_3|}{|L_1L_2|}\leq \frac{1}{\sin \frac{ \bar{c}}{2}}+\frac{o(|L_1L_2|(1+ \frac{1}{\sin \frac{ \bar{c}}{2}}+o_\rho(1)))}{|L_1L_2|}< \frac{3}{\bar{c}}.
 \]
 
  %\[[L_2L_3]_y>|L_1L_2|_y-|L_1L_3| o_{\varepsilon(c)}(1)\]
 %|L_1L_2|-\bar{\varepsilon}^2,\]
  %где нижний индекс $y$ означает проекцию на ось абсцисс. То есть $|L_2L_3|>\sin c |L_1L_2|-o_{\bar{\varepsilon}}(1)|L_1L_3|$.
% И наоборот, $|L_1L_2|>\sin \bar{c} |L_2L_3|-o_{\bar{\varepsilon}}(1)|L_1L_3|$. 
 %Из этого очевидным образом следует существование $c_1, c_2>0$ таких, что $c_2|L_2L_3|\geq |L_1L_2| \geq c_1|L_1L_3|$.   
 Аналогично и для остальных $L_i$. 
 
 Замена ломаной $L_1-L_2-L_3-L_4-L_5$ на $L_1-L_2-L_4-L_5$ уменьшит ее длину не меньше, чем на величину, линейно зависящую от $|L_1L_2|$, поскольку $\angle L_2L_3L_4 \leq \pi-\bar{c}$ (а значит $\cos \angle L_2L_3L_4 \geq  -\cos \bar{c}$):
 \begin{multline*}
 |L_2L_3|+|L_3L_4|-|L_2L_4|=\frac{(|L_2L_3|+|L_3L_4|)^2-|L_2L_4|^2}{|L_2L_3|+|L_3L_4|+|L_2L_4|}>\\
 > \frac{2|L_2L_3||L_3L_4| (1+ \cos \angle L_2L_3L_4)}{2(|L_2L_3|+|L_3L_4|)}\geq
 \frac{|L_3L_4|(1- \cos \bar{c})}{ \left (1+\frac{|L_3L_4|}{|L_2L_3|} \right)}\geq  \frac{(\frac{\bar{c}}{3})^3}{(1+\frac{3}{\bar{c}})}|L_1L_2|.
\end{multline*}
 
 
 
% \[
% |L_2L_3|+|L_3L_4|-|L_2L_4|\geq  |L_2L_3|(1+\frac{c}{3}-\frac{1}{\sin c})>|L_2L_3|(1+\frac 2 c),
 %\]
 %поскольку 
 %\[
 %|L_2L_4|=\sin \angle L_2L_3L_4 \frac{|L_2L_3|}{\sin L_2L_4 L_3}\leq  \frac{|L_2L_3|}{\sin L_2L_4 L_3} \leq  \frac{|L_2L_3|}{\sin (\pi-c)}= \frac{|L_2L_3|}{\sin c}.
 %\]
 %ой ОЙОЙ ТУТ НЕ ТАК
 
% \begin{multline*}
 %|L_2L_3|+|L_3L_4|-\sqrt{ |L_2L_3|^2+|L_3L_4|^2+2 %|L_2L_3||L_3L_4|\cos (2c) }\geq \\
%|L_1L_2| \left(\sin c+\sin^2 c-\sqrt{\frac{1}{\sin^2 c}+\frac{1}{\sin^4 c}+2\frac{\cos (2c)}{\sin^3 c}})+o_{\varepsilon(c)}(1|L_1L_2| \right),
% \end{multline*}
%Таким образом замена уменьшает длину множества на величину, линейно зависящую от $|L_1L_2|$.
%\input{pictures/dvapo}
%Обозначим точки $L_6 \defeq [L_1y(L_3)] \cap \partial B_r(y(L_3))$ и $L_7 \defeq [L_5y(L_3)] %\cap \partial B_r(y(L_3))$ где $y(L_3)$ произвольная соответствующая $L_3$ точка. Тогда %$$B_r([L_1L_6]) \cup B_r([L_5L_7]) \supset B_r([L_1L_3]) \cup B_r([L_3L_5]).$$ и %$\H([L_1L_6]) \cup B_r([L_5L_7]))=o_{[L_1L_2]}(1)$ (это следует из теоремы Пифагора и  %пункта~\ref{1145} доказательства Леммы~\ref{Losiu}). Тогда можно заменить ломаную  %$L_1-L_2-L_3-L_4-L_5$ на $L_6-L_1-L_2-L_4-L_5-L_7$ и получить противоречие с оптимальностью %$\Sigma$ (см. рис~\ref{fig:dvapo}).
%А значит
%\[
%\H([L_1L_2]\cup [L_2L_4]\cup[L_4L_5]\cup S^{[L_1L_5]})\leq \H(L_1-L_2-L_3-L_4-L_5)-|L_2L_3|(1+\frac 2 c)+o(|L_1L_5|)<\H(L_1-L_2-L_3-L_4-L_5).
%\]
Тогда множество $ \Sigma \setminus ([L_2L_3] \cup [L_3L_4]) \cup [L_2L_4]\cup S^{[L_1L_5]}$ лучше $\Sigma$: является связным (поскольку все внутренние точки исходной ломаной --- степени два), обладает меньшей длиной и не большей энергией. Противоречие с оптимальностью $\Sigma$ (см. рис~\ref{fig:dvapo}).
%ПОМЕНЯТЬ РИСУНОК ИЛИ ВЕРНУТЬ ЗАКОМЕНЧЕННОЕ



\[ 
\H(Pr_{(a_0x_0]}(\sigma \cap B_{\rho_0}(x_0))) \geq \cos (\angle z_0x_0a_0) |z_0 x_0|\geq 
\]
Herewith $\angle ((ax], (a_0x_0])=o_{\rho_2}(1)$, а значит, при достаточно малом $\rho_2$, все односторонние касательные к $\sigma \cap B_{\rho_0}(x_0)$ имеют угол с $(a_0x_0]$, больший $1/20$.
Тогда
\[
\H(\sigma \cap B_{\rho_0}(x_0)) \geq \frac{Pr_{(a_0x_0]}(\sigma \cap B_{\rho_0}(x_0))}{\cos \frac{1}{10}}\geq \frac{\cos (\angle  z_0x_0a_0)}{\cos \frac{1}{10}}|z_0 x_0|=\frac{\cos (o_{\rho_0}(1))}{\cos \frac{1}{10}}\rho_0.
\]
С другой стороны, поскольку ребро $(a_0x_0]$ направлено в обе стороны, выполняется $\H(\sigma \cap B_{\rho_0}(x_0))=\rho_0+o_{\rho_0}(1)$. Противоречие для достаточно малого $\rho_0$.


Не умаляя общности будем считать, что ребро $(ax]$ направлено в одну сторону, поскольку в противном случае применим пункт~\ref{A} (см замечание~\ref{remA}).
Пусть $\varepsilon>0$ такое, что $\sharp (\partial B_\varepsilon(x)\cap \Sigma)=\oordball_x\Sigma \leq 3$. И пусть $s \in \partial B_\varepsilon(x)$ такая, что путь из $s$ в $x$ лежит в $\overline{B_\varepsilon(x)}$.

Рассмотрим величину поворота пути: $|\turn(\breve{sx})|<2\pi$. Аналогично рассуждениям в предыдущем пункте заметим, что конечность величины поворота и наличие в компоненте связности энергетических точек только одного ребра, причем направленного в одну сторону, влечет конечность числа точек ветвления на пути из $s$ в $x$. Таким образом можно выбрать $\varepsilon>0$ таким, что $\breve{sx}$ не содержит точек ветвления.

Тогда ввиду Леммы~\ref{dug_ok}  $\breve{sx}$  содержится внутри некоторого псевдоконуса.

%Пусть инъективная функция $f: [0;1] \rightarrow \R^2$ параметризует $\breve{[sx]}$. Множество $\breve{[sx]} \cap G_\Sigma$ содержится в псевдоконусе $Q_{\rho}^{a,x}$. Будем также считать, что это псевдоконус имеет следующий вид: $Q^{a,x}_{\varepsilon} \defeq \bigcup_{k=1}^{\infty} \left( Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) \right)$ для некоторых сходящихся к нулю монотонных последовательностей неотрицательных чисел $\{s_k\}$ и $\{\rho_k\}$, где $\rho_1=\varepsilon$ (см Лемму~\ref{con}). Будем считать выбранные последовательности минимальными по включению. Пусть точки $c,d \in [0;1]$ такие, что $f([c,d])\cap G_\Sigma=f(c) \cup f(d)$. Тогда, ввиду отсутствия на дуге $\breve{[sx]}$ точек ветвления, выполняется $f([c,d])=[f(c),f(d)]$. В таком случае, если $f(c) \in Q(\rho_{k-1},s_{k-1},x,a) \setminus B_{\rho_{k}}(x) $, $f(d) \in Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) $, то выполняется $[f(c);f(d)] \subset  Q(\rho_{k-1},s_{k-1},x,a) \setminus B_{\rho_{k+1}}(x)$. А значит, 
%\[
%\breve{[sx]}=f([0;1]) \subset \bar{Q}^{a,x}_{\varepsilon} \defeq \bigcup_{k=1}^{\infty} \left(Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+2}}(x) \right).
%\]
%Тогда к $\breve{[sx]}$ применим пункт~\ref{A}.
%МОЖЕТ НАДО ВЕРНУТЬ
%\end{proof}

усть $\Sigma'$ --- замыкание компоненты связности $\Sigma \setminus \{x\}$ и пусть $\Sigma'$ содержит бесконечную последовательность энергетических точек ребра $(ax]$, сходящуюся к $x$. Пусть кроме того $\Sigma' \cap \overline{B_{\rho}(x)}$ не содержит иных энергетических точек для некоторого $\rho>0$. Тогда $\Sigma' \cap \overline{B_{\rho}(x)}$ содержит конечное число точек ветвления.  
%То есть найдется такое $\rho_1>0$, что множество $\overline{B_{\rho_1}(x)} \cap \Sigma'$ является дугой. 
Кроме того найдется такое $\rho_1>0$ и псевдоконус $Q_1 \in Q^{a,x}_{\rho_1}$, что $\Sigma' \cap \overline{B_{\rho_1}(x)}\subset Q_1$. %При этом прямые, содержащие односторонние касательные к $\Sigma $ в энергетической точке $\bar x$ ребра $(ix]$, стремятся к $(ix)$ при $\bar x \rightarrow x$, $i=a,b$.


Для любой точки $\bar{x} \in G_\Sigma \cap  \Sigma' \cap U \setminus \{ x\}$ касательные лучи к $\bar x$ параллельны ближайшему к ней энергетическому ребру $(ix]$ с точностью до $\alpha/100$.

Докажем утверждение шага от противного: пусть, не умаляя общности, точка $x^a_1 \subset Q^{a,x}_\rho \cap U \cap \Sigma' \cap X_\Sigma$ имеет порядок два. 
Пусть $[x^a_1;t]$ --- максимальный по включению  отрезок, содержащийся на пути из $x^a_1$ в $x$. Тогда, по предположению и ввиду следствия~\ref{sm_an},
\[
\alpha/100< \angle((ax),(x^a_1t)) \leq \pi/6+\alpha/100.  
\]
Несложно заметить, что $\angle ((x^a_1t],(ax])= \angle((ax),(x^a_1t))$ (а не $\pi-\angle((ax),(x^a_1x))$) поскольку в противном случае любой путь, начинающийся с $x^a_1-s$, где $[x^a_1s]$ --- второй максимальный отрезок инцидентный $x$, находится внутри области, ограниченной путем из $x^a_1$ в $x$ и двумя пустыми шарами с радиусом $r$ и с центрами в точке, соответствующей $x^a_1$, и в точке сгущения точек, соответствующих энергетическим точкам ребра $(ax]$. В таком случае такой путь не может содержать энергетических точек ребра $(bx]$, а значит концевыми точками для него могут быть только энергетические точки ребра $(ax]$ степени $1$, ввиду леммы~\ref{alm} принадлежащие $X_\Sigma$. Но путь, начинающийся с $x^a_1-s$ и в точках ветвления продолжающийся не тем отрезком, который является почти перпендикулярным $(ax]$, 
%(нетрудно заметить, что всегда найдется два направления, имеющих с ребром угол, не больший $\pi/6+\alpha/100$), 
не будет содержать энергетических точек ребра $(ax]$ степени $1$ (а также точек $\partial U$, точки $x$ и энергетических точек ребра $(bx]$ степени $1$), а значит никогда не закончится.


==> ⥪�騩 ���᪨� ⥪�� (in english)/pictures/trash/4proofs.tex <==
\section {Доказательство основной Леммы и Теоремы~\ref{persp}} \label{prf}

\begin{proof}[Доказательство Леммы~\ref{main_l}]
Пусть $\rho_0>0$ достаточно мало. Точка $x\in E_\Sigma$ имеет одно или два энергетических ребра. Пункты доказательства c 1. по 8. содержат утверждения для одного ребра, поэтому относятся ко всем утверждениям Леммы сразу.  %СЕМЬ ИЛИ ВОСЕМЬ
После того, как первые восемь пунктов будут доказаны, мы будем предполагать, что у точки $x$, имеющей два энергетических ребра, порядок $\oord_x \Sigma = 1$. После того, как этот случай будет исключен, будут последовательно разобраны все случаи Леммы, не исключая также и случай энергетического ребра, направленного сразу в две стороны. 

Все дальнейшие рассуждения будут проводиться в множестве $\Sigma \cap B_{\rho_0}(x)$, а все утверждения будут доказаны для $\Sigma \cap B_{\rho}(x)$ для достаточно малого $\rho< \rho_0$, где ограничения сверху на $\rho$ будут появляться в процессе доказательства. 
%, где $\rho<\rho_0$, а $\rho_0>0$ --- достаточно малое число. 
Как было показано в Утверждении~\ref{edgeangle}, все энергетические точки множества $\Sigma \cap B_{\rho_0}(x)$ содержатся в объединении двух псевдоконусов $U^a(\rho_0)$ и $U^b(\rho_0)$ с биссектрисами $(ax]$ и $(bx]$ соответственно и раствором $\alpha(\rho_0)$ (в дальнейшем $\alpha$) (или внутри одного псевдоконуса $U^a(\rho_0)$, если $x$ имела ровно одно энергетическое ребро $(ax]$).
Поскольку $\rho_0$ достаточно мало, выполняется $U^a(\rho_0) \cap U^b(\rho_0) =x$.

Выберем также произвольные (бесконечные) последовательности энергетических точек $\{x^a_k\} \subset U^a(\rho_0) \cap G_\Sigma$ и $\{x^b_k\} \subset U^b(\rho_0) \cap G_\Sigma$ такие, что
$x^i_k \xrightarrow{}x$ и $(x^i_k x]\xrightarrow{}(ix]$, где буква $i$ означает $a$ или $b$ (или одну последовательность, если $x$ имело ровно одно энергетическое ребро $(ax]$). В процессе доказательства мы неоднократно, без перенумерации, будем переходить к подпоследовательностям $\left\{x^i_k \right \}$. При этом выбор последовательности и переход к подпоследовательностям устроены таким образом, что для достаточно малого $\rho_0$ все доказанные для $x^i_k$ точные (не содержащие значка $o$-малое или слова ``почти'') утверждения верны для произвольной энергетической точки из $B_{\rho}(x)\setminus x$. 



Пусть $\rho_0 \geq \rho(k) \xrightarrow{}0$ при $k \xrightarrow{}\infty$. Например, перейдя к подпоследовательности, можно выбрать монотонную функцию, в целых точках совпадающую с $\rho(k) \defeq |x^i_kx|$.
Слово ``почти''\ означает ``с точностью до величины $o_\rho(1)$'', то есть с точностью до величины, стремящейся к нулю при $\rho \xrightarrow{}0$ (а значит и при $k \xrightarrow{}\infty$).

\begin{enumerate}

\item Раствор дуги, покрываемой $x^i_k$, $\rho$-узок, то есть составляет $o_\rho(1)$. 
То есть все такие точки $y^i_k \in M$, что $|x^i_k y^i_k|=r$ и $B_r(y^i_k) \cap \Sigma = \emptyset$, удовлетворяют условию 
\[
\left|\frac{\pi}{2}-\angle ((ix), (y^i_kx^i_k))\right| = o_\rho (1)
\]
или, иначе говоря, для произвольного $c>0$ найдется такой номер $N$, что для каждого номера $k>N$ выполняется  
\[
\left|\frac{\pi}{2}-\angle ((ix), (y^i_kx^i_k))\right|<c.
\]
\label{angles}

\begin{proof}
Предположим противное. То есть можно выбрать подпоследовательность точек $\{ x^i_k\}$, соответствующих им точек $\{y^i_k\}$ и число $c>0$ такие, что 
\begin{equation}
\left|\frac{\pi}{2}-\angle ((ix),(y^i_kx^i_k))\right| > c.
\label{losloh}
\end{equation}
Но тогда для любой предельной точки $y^i$ множества $\{y^i_k\}$ верно, что $B_r(y^i) \cap \Sigma =\emptyset$, $|y^ix|=r$ и $|\frac{\pi}{2}-\angle ixy^i| \geq c$.
Но $\frac{\pi}{2}-\angle i x y^i \geq c$ противоречит определению ребра $(ix]$, поскольку в таком случае $B_\varepsilon(x^i_k) \cap U^i(\rho_0)\setminus B_r(y^i) =\emptyset$ для достаточно малого $\varepsilon>0$. А  $\angle i x y^i-\frac{\pi}{2} \geq c$, как несложно заметить, влечет
$\angle x^i_lxy^i \geq \frac{\pi}{2} + \frac{c}{2}$, для достаточно большого номера $l$.
А значит, не умаляя общности, $\angle x^i_lxy^i_l \geq \frac{\pi}{2} + \frac{c}{4}$ и $\angle x_l x_m y_l \geq \frac{\pi}{2} + \frac{c}{8}$ для достаточно большого номера $m>l$.
Но тогда $|x^i_my^i_l|<|x^i_ly^i_l|=r$, а значит $B_r(y^i_l)\cap \Sigma \neq \emptyset$. Полученное противоречие завершает доказательство пункта.

В частности, формула~\ref{losloh} и п.~\ref{perp_edge} Замечания~\ref{emptyball} влекут
\begin{corollary}
Энергетические ребра точек $x^i_k$ почти параллельны энергетическому ребру $(ix]$. 
\label{edges}
\end{corollary}

\end{proof}
\begin{remark}
В случае энергетического ребра, направленного сразу в две стороны, предлагается по отдельности провести рассуждение для двух подпоследовательностей точек $x^i_k$ таких, что внутри одной подпоследовательности точки $y^i_k$ расположены в одной полуплоскости относительно $(ix)$. Две подпоследовательности могут иметь общие точки.
\end{remark}

\item Зафиксируем произвольную точку $x^i_k$. Тогда существует такое $\varepsilon_k>0$, что для $0<\varepsilon <\varepsilon_k$ и такой точки $w \in \partial B_{\varepsilon}(x^i_k)$, что луч $[wx^i_k)$ почти параллелен $(ix]$ (то есть $\angle((ix)(wx^i_k))=o_\rho(1)$), верно, что существует такое связное множество $S \ni w$, что 
%\[
%M \cap B_r(\Sigma \cap B_\varepsilon(x^i_k)) \subset B_r(S)
%]
\[
F_M(\Sigma \setminus B_\varepsilon(x^i_k) \cup S) \leq F_M(\Sigma)
\]
и $\H(S)=o_\varepsilon(1)+\varepsilon o_\rho(1)$. 
В частности, это верно для $w=x^i_k$.
\label{Losiu}

\begin{proof}
Пусть $\{ \varepsilon_l \}$ --- сходящаяся к нулю последовательность, такая что для произвольных номеров $l$ и $m$ выполняется $B_{\varepsilon_l}(x^i_l)\cap B_{\varepsilon_m}(x^i_m)=\emptyset$ (очевидно, такие $\varepsilon$ можно выбрать для любой сходящейся нестабилизирующейся последовательности $\{ x^i_k \}$). Кроме того, уменьшим, при необходимости числа $\varepsilon_k$ так, чтобы выполнялось
\begin{equation}
\frac{\varepsilon_k}{|x^i_kx|} \xrightarrow[k \xrightarrow{} \infty]{} 0.
\label{y}
\end{equation}
Для произвольного номера $l$ определим множество 
$$U^i_l \defeq \{y\in M | \dist(y, \overline{B_{\varepsilon_l}(x^i_l)})\leq r, \dist(y, \Sigma \setminus \overline{B_{\varepsilon_l}(x^i_l)})> r \}.$$
Заметим, что тогда 
\begin{equation}
F_{M \setminus U^i_l}(\Sigma \setminus B_{\varepsilon_l}(x^i_l)) \leq r. 
\label{0}
\end{equation}

Пусть $\{u_l\}$ --- произвольная последовательность точек $u_l \in U^i_l$, а $\{v_l\}$ --- такая последовательность точек, что $v_l \in B_{\varepsilon_l}(x^i_l)$ и $|u_lv_l| \leq r$. Тогда покажем, что 
\begin{equation}
\left |\angle((u_lv_l),(ix))-\frac{\pi}{2} \right|=o_\rho(1).
\label{1}
\end{equation}

Предположим, что формула~(\ref{1}) неверна, тогда найдется такое $c>0$, что $|\angle((u_lv_l),(ix))-\frac{\pi}{2}|>2c$. 

Пусть существует такая подпоследовательность, что $\angle((u_lv_l],(ix])-\frac{\pi}{2}>2c$. Несложно заметить, ввиду условия~\ref{y}, что $|\angle((ix),(v_lx))|=o_\rho(1)$, а значит, не умаляя общности, и ввиду определения ребра, можно считать что существует такая подпоследовательность, что $\angle u_l v_l x < \frac{\pi}{2} - c$ для каждого $l$. Поскольку последовательность $v_m$ сходится к точке $x$, можно выбрать такое достаточно большое $l$, что $\angle v_l u_l x < \frac{c}{4}$. Для этого $l$ можно выбрать такое, достаточно большое $m>l$, что $\angle v_l u_l v_m < \frac{c}{2}$ и $\angle u_l v_l v_m < \frac{\pi}{2} - \frac{c}{2}$. Тогда $|v_mu_l|<|v_lu_l|\leq r$, что невозможно ввиду определения множества $U^i_l$.

Значит, для достаточно большого $l$ выполняется неравенство 
$$\angle((u_lv_l],(ix]) < \frac{\pi}{2}-2c.$$ 
Тогда $\dist(u_l,(ix))\leq \sin (\frac{\pi}{2} - c)r$ для достаточно большого номера $l$. Но тогда $B_r(u_l)\cap (ix]$ является подмножеством хорды $\partial B_r(u_l)$. Тогда для достаточно большого номера $m>l$ верно $B_{\varepsilon_m}(v_m) \subset B_r(u_l)$. Что противоречит определению множества $U^i_l$. Таким образом, формула~(\ref{1}) доказана.


Отныне будем считать, не умаляя общности, что все множества $U^i_l$ лежат в одной полуплоскости относительно прямой $(ix)$. Это верно, за исключением конечного числа множеств, во всех случаях кроме ребра $(ix]$, направленного в две стороны. Но в таком случае все рассуждения можно провести для двух наборов множеств, каждый из которых лежит по одну сторону $(ix)$.

Покажем теперь, что для произвольного набора точек $w_l \in B_{\varepsilon_l}(x^i_l)$, в том числе для $w_l=x^i_l$, выполняется
\begin{equation}
\left |\angle ((u_l,w_l),(ix]) - \frac{\pi}{2} \right |=o_{\rho}(1).
\label{2}
\end{equation}
Посмотрим на треугольник $\triangle u_l v_l w_l$: сторона $|v_lu_l|\geq r-|u_l u_{l+1}|=r-o_{\rho}(1)$ ввиду фундаментальности $\{u_l\}$, сторона $|v_l w_l|\leq 2\varepsilon_l$, таким образом по теореме синусов $\sin \angle v_lu_lw_l = o_{\rho}(1)$. Тогда и $\angle v_lu_lw_l=o_{\rho}(1)$, а значит $\angle ((u_l,w_l),(ix]) = \angle((u_lv_l),(ix])+o_\rho(1)$, что влечет $|\angle ((u_l,w_l),(ix]) - \frac{\pi}{2}|=o_{\rho}(1)$. Таким образом, формула~(\ref{2}) доказана.

Покажем теперь, что 
\begin{equation}
\angle((v_lx^i_l),(ix])=o_\rho(1)
\label{3}
\end{equation}
(в частности, при $v_l = x^i_l$ данный угол будем считать нулевым).
Посмотрим на $\triangle u_lv_l x^i_l$. 
Пусть $y^i_k$ --- произвольная точка, удовлетворяющая условиям, перечисленным в  пункте~\ref{angles} (то есть $y^i_k \in M$, $|x^i_l y^i_l|=r$ и $B_r(y^i_k) \cap \Sigma = \emptyset$). Тогда, ввиду пункта~\ref{angles} ясно, что для произвольной точки $v^l \in \Sigma \cap B_{\varepsilon_l}(x^i_l) \setminus \{ x^i_l\}$ либо $\angle v^l x^i_l y^i_l=o_\rho(1)$, либо  $\angle v^l x^i_l y^i_l>\frac{\pi}{2}$. Пусть предположение неверно, то есть найдется такое $c>0$, что $\angle((v_lx^i_l),(ix])>c$ для каждого $l$. Тогда, для $v_l \neq x^i_l$ верно  $\angle v_l x^i_l y^i_l>\frac{\pi}{2}$, а значит $\angle v_l x^i_l y^i_l \geq \frac{\pi}{2} +c$. Тогда для достаточно малого $\rho_0$ можно считать $\angle v_l x^i_l u_l \geq \frac{\pi}{2} + \frac{c}{2}$. Тогда $|x^i_lu_l|\leq \cos(\frac{\pi}{2} + \frac{c}{2})|v_lu_l|\leq r(1 - \frac{c^2}{3})$. Тогда для предельной точки $\hat u=\lim\limits_{l \xrightarrow{} \infty} u_l$ верно, что $|x \hat u|\leq r(1 - \frac{c^2}{3})$, что не может быть правдой, поскольку по определению $U^i_l$ верно
$||x^i_lu_l|-r|\leq \varepsilon_l+\varepsilon_{l+1} +|x^i_lx^i_{l+1}|$, а значит $|x \hat u|=r$. Полученное противоречие завершает доказательство формулы~(\ref{3}).


Пусть теперь $w$ из условия доказываемого пункта, а $u$ --- самая дальняя от неё точка множества $U^i_k$. 
Пусть $v \in B_{\varepsilon_k}(x^i_k)$ такая, что $|vu| \leq r$. Покажем, что $|wu|=r+\varepsilon o_\rho(1)+o_\varepsilon(1)$. Для этого нам придется сначала показать, что $|x^i_ku|=r+\varepsilon o_\rho(1)+o_\varepsilon(1)$.

Ввиду формул~(\ref{1}) и (\ref{3}) несложно заметить, что
\begin{equation*}
\left |\angle uvx^i_k - \frac{\pi}{2} \right |=o_\rho(1).
%\label{4}
\end{equation*}
При этом $|x^i_kv|\leq \varepsilon$ и $|vu|\leq r$.
Тогда по теореме косинусов для $\triangle x^i_kvu$
\begin{equation}
|x^i_ku|=\sqrt{|x^i_kv|^2+|uv|^2-2|x^i_ku||uv|\cos \angle uvx^i_k}=  \sqrt{\varepsilon^2 + r^2 + \varepsilon o_\rho(1)}=r+\varepsilon o_\rho(1)+o_\varepsilon(1).
\label{5}
\end{equation}


Ввиду формулы~(\ref{2}) для $l=k$, $w_l=x^i_k$ и условия $\angle((ix)(wx^i_k))=o_\rho(1)$ несложно заметить, что
\begin{equation*}
\left |\angle wx^i_ku - \frac{\pi}{2} \right |=o_\rho(1).
%\label{6}
\end{equation*}
При этом $|x^i_kw|\leq \varepsilon$ и, ввиду~(\ref{5}), $|x^i_ku|\leq r+\varepsilon o_\rho(1)+o_\varepsilon(1)$.
Тогда по теореме косинусов для треугольника $\triangle x^i_kwu$  
\begin{multline*}
|wu|=\sqrt{|x^i_kw|^2+|x^i_ku|^2-2|x^i_kw||x^i_ku|\cos \angle  wx^i_ku}= \\
= \sqrt{\varepsilon^2+(r+\varepsilon o_\rho(1)+o_\varepsilon(1))^2+\varepsilon o_\rho(1)(r+\varepsilon o_\rho(1)+o_\varepsilon(1))}=r+\varepsilon o_\rho(1)+o_\varepsilon(1).
\end{multline*}

А значит $U^i_k \subset \overline{B_{r+\varepsilon o_\rho(1)+o_\varepsilon(1)}(w)}$. С другой стороны, ввиду формулы~(\ref{2}) можно говорить, что множество $U^i_k$ содержится в углу с вершиной $w$ и с раствором $o_\rho(1)$. Не умаляя общности, положим луч $[wu)$ биссектрисой данного угла и назовем этот угол $\Lambda^i_k$.
Тогда 
\[
U^i_k \subset B_{|wu|}(w) \cap \Lambda^i_k.
\]
Обозначим за $G$ один из двух концов дуги $\partial B_{|wu|}(w) \cap \Lambda^i_k$. Пусть $T \in [wu]$ --- такая точка, что $|TG|=r$. Несложно заметить, что 
\[
\overline{B_r([wT])} \supset \overline{B_{|wu|}(w) \cap \Lambda^i_k} \supset U^i_k. 
\]
Таким образом, ввиду формулы~(\ref{0}), осталось показать, что длина множества $|wT|=\varepsilon o_\rho(1)+o_\varepsilon(1)$ и тогда искомое множество $S \defeq [wT]$ будет найдено.

Пусть $\phi \defeq \angle Gwu$ (то есть $\phi=o_\rho(1)$), $\psi \defeq \angle GTu$ и $h\defeq|wu|-r$ (то есть $h=\varepsilon o_\rho(1)+o_\varepsilon(1)$). Тогда
\[
\begin{array}{ccc}
    \sin \psi &=& (1+\frac{h}{r}) \sin \phi;  \\
    \sin \psi -\sin \phi &=& \varepsilon o_\rho(1)+o_\varepsilon(1);\\
    \psi - \phi &=& \varepsilon o_\rho(1)+o_\varepsilon(1);\\
    \cos \phi -\cos \psi = -2\sin \left (\frac{\phi + \psi}{2} \right)\sin \left (\frac{\phi - \psi}{2} \right) &=& \varepsilon o_\rho(1)+o_\varepsilon(1).\\
\end{array}
\]
Тогда 
\[
    |wT| = |wu| - |Tu| = r\left(\left(1 + \frac{h}{r}\right)\cos \phi - \cos \psi\right ) =\varepsilon o_\rho(1)+o_\varepsilon(1).
\]

Таким образом, множество $S \defeq [wT]$ удовлетворяет всем заявленным условиям.
\end{proof}

\item Для произвольной точки $x^i_k$ ее круговой порядок $\oordball_{x^i_k}\Sigma$ не превосходит двух.
Из этого, благодаря Замечанию~\ref{rem_ord}, следует $\oord_{x^i_k}\Sigma \leq 2$.
\label{ordball}

\begin{proof}
Пусть $n \defeq \oordball_{x^i_k}\Sigma$ и пусть $\varepsilon>0$ достаточно малое число такое, что 
\[
\sharp (\partial B_{\varepsilon}(x^i_k) \cap \Sigma) = n. 
\]
%сослаться  на формулу коплощади
Тогда, согласно формуле коплощади $\H(B_\varepsilon(x^i_k)\cap \Sigma) \geq n \varepsilon$. Предположим, что $n > 2$. Поскольку все эти $n$ точек располагаются на дуге окружности $\partial B_{\varepsilon_l}(x^i_k)$ размера $\pi+o(\varepsilon)$, нетрудно заметить, что штейнеровское дерево $St$, соединяющие все эти $n$ точек и точку $x^i_k$, имеет такую длину, что $n \varepsilon - \H(St)=c_n\varepsilon \geq c_3$, где $c_3$ --- положительная константа, которую можно посчитать. 
Применив пункт~\ref{Losiu} для $w=x^i_k$, получим множество $S$, такое что для достаточно малых $\rho_0$ и $\varepsilon$  величина $\H(S)$ строго меньше $n \varepsilon - \H(St)$. Таким образом, замена $\Sigma$ на $\Sigma \setminus B_\varepsilon(x^i_k) \cup St \cup S$ уменьшает длину, не увеличивает энергию и сохраняет связность. Противоречие. 
\end{proof}

\item В случае, если  $\oord_{x^i_k} \Sigma =1$, точка $x^i_k$ принадлежит множеству $X_\Sigma$.
\label{discr}

\begin{proof}
Предположим противное: пусть точка $x^i_k$ принадлежит множеству $E_\Sigma$. Тогда существует последовательность энергетических точек $\{x'_l\}$, сходящихся к $x^i_k$. Энергетическое ребро или ребра, к которым они сходятся, должны лежать на прямой, почти параллельной $(ix]$ ввиду Замечания~\ref{edges}.  

Ввиду пункта~\ref{ordball} достаточно разобрать только следующие случаи:
\begin{itemize}
\item[(a)] Случай $\oordball_{x^i_k}\Sigma=1$.
Пусть $\varepsilon_0(k)>0$ достаточно мало, а $\varepsilon_l>0$ последовательность стремящихся к нулю чисел, меньших $\varepsilon_0(k)$ таких, что $\sharp (\partial B_{\varepsilon_l}(x^i_k) \cap \Sigma )=1$. Обозначим $s^l\defeq \partial B_{\varepsilon_l}(x^i_k) \cap \Sigma$. Тогда $(s^lx^i_k)$ почти перпендикулярно $(ix)$. Предположим, что это не так, то есть существуют константа $c>0$ и последовальность $K \subset \mathbb{N}$ такие, что для любого $k \in K$ существует сколь угодно большой номер $l$, такой что выполняется неравенство $|\angle ((s^lx^i_k), (ix))-\frac{\pi}{2}| > c$.
 
Пусть тогда $w$ --- основание перпендикуляра, опущенного из $s^l$ на прямую, параллельную $(ix)$ и проходящую через $x^i_k$: $(wx^i_k)\ ||\ (ix)$ и $(ws^l) \perp (ix)$. Тогда определим множество $S \ni w$  как в пункте~\ref{Losiu}. При этом длина этого множества $\H(S)=o_{\varepsilon_l}(1)+o_\rho(1)\varepsilon_l$, поскольку $|wx^i_k|= \cos \angle ([s^lx^i_k],(ix]) \cdot |s^lx^i_k|< \varepsilon_l$. В то же время $|ws^l|=\sin \angle([s^lx^i_k],(ix]) \cdot |s^lx^i_k| < (1 - \frac{c^2}{2}) \varepsilon_l$ и $\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq \varepsilon_l$. Таким образом, 
\[
\H(\Sigma \setminus  B_{\varepsilon_l}(x^i_k) \cup [s^lw] \cup S)\leq \H(\Sigma)-\varepsilon_l+\left(1-\frac{c^2}{2}\right)\varepsilon_l+o_{\varepsilon_l}(1)+o_\rho(1)\varepsilon_l<\H(\Sigma).
\]

То есть связное множество $\Sigma \setminus [s^lx^i_k] \cup [s^lw] \cup S$ будет иметь длину  меньше, а энергию не больше, чем $\Sigma$. Получили противоречие с оптимальностью $\Sigma$, то есть предположение о неперпендикулярности было неверным. То есть $(s^lx^i_k)$ почти перпендикулярно $(ix)$:
\begin{equation}
\left|\angle ((s^lx^i_k), (ix))-\frac{\pi}{2}\right| =o_\rho(1).
\label{99}
\end{equation}
Заметим теперь, что для каждого $\varepsilon_l$ верно
\begin{equation}
\H(B_{\varepsilon_l}(x^i_k)\cap \Sigma)=\varepsilon_l+o_{\varepsilon_l}(1)+o_\rho(1)\varepsilon.
\label{100}
\end{equation}

Формула~\eqref{100} верна ввиду пункта~\ref{Losiu}: в противном случае можно было бы заменить $\Sigma$ на связное множество $\Sigma \setminus B_{\varepsilon_l}(x^i_k) \cup [x^i_ks^l]\cup S$, где $S$ определено в пункте~\ref{Losiu} при $w=x^i_k$, и получить противоречие с оптимальностью $\Sigma$. 

Можно считать, что 
\begin{equation}
\H(B_{\varepsilon_l}(x^i_k)\cap \Sigma)<\varepsilon_l \left(1+\frac{1}{18}\right).
\label{101}
\end{equation}
Теперь заметим, что можно считать, что 
\begin{equation}
\frac{\varepsilon_l}{\varepsilon_{l+1}}\leq \frac{18}{17}.
\label{103}
\end{equation}
Пусть не так, тогда найдется $\varepsilon_l$ такой, что $\sharp ( \partial B_{\varepsilon_l}(x^i_k)\cap \Sigma)\geq 2$ для каждого $\varepsilon \in [\frac{17\varepsilon_l}{18},\varepsilon_l[$. Но тогда, ввиду неравенства коплощади
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k))\geq \H(\Sigma \cap B_{\frac{17\varepsilon_l}{18}}(x^i_k)) +\H(\Sigma \cap (B_{\varepsilon_l}(x^i_k) \setminus  B_{\frac{17\varepsilon_l}{18}}(x^i_k))\geq \varepsilon_l \left (1+\frac{1}{18} \right),
\]
что противоречит~\eqref{101}.
Ввиду наличия у $x^i_k$ ребра, существования последовательности $\{ s_l \}$ и единичного порядка $\oord{x^i_k}(\Sigma)=1$ существует также сходящаяся к $x^i_k$ последовательность точек $\{ u_l\}\subset \Sigma$ таких, что $\angle((u_lx^i_k),(ix)) = \frac{\pi}{4}$.

Рассмотрим произвольную такую точку $u_m$. Выберем такой номер $l$, что 
\begin{equation}
0<\varepsilon_l-|x^i_ku_m|\leq \frac{1}{18}\varepsilon_l.
\label{104}
\end{equation}
Такое $\varepsilon_l$ существует ввиду формулы~\eqref{103}. Заметим также, что ввиду~\eqref{99} выполняется
\[
\sharp (\partial B_{|x^i_k u_m|}(x^i_k)\cap \Sigma) \geq 2.
\] 
Кроме того, 
\begin{equation}
d \defeq \dist(u_m, Q_a\cup Q_b \cup Q)\geq \frac{\sqrt{2}}{2}|x^i_ku_m|-o_\rho(1)\varepsilon> \frac{1}{\sqrt{3}}|x^i_ku_m|,
%\label{105}
\end{equation}
где $Q$ --- область возможного расположения точек $s_l$ (угол с вершиной в $x^i_k$, раствором $o_\rho(1)$ и перпендикуляром к $(ix)$ в качестве биссектрисы).
Пусть $q$ ---  компонента связности $\Sigma \cap Q$, содержащая $u_m$. Пусть теперь $c$ --- длина проекции $q$ на ближайшую к $u_m$ сторону угла $Q$ (то есть на луч с вершиной в $x^i_k$, имеющий угол $\frac{\pi}{2}-o_\rho(1)$ с прямой $(ix)$). Тогда
%а $var(c)$ величина проекции на эту координату. Тогда
\[
\H(q)\geq \frac{c+d}{2}.
\]
Тогда 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq \varepsilon_l-c+\frac{c+d}{2}.
\]
С другой стороны, по неравенству коплощади 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq \varepsilon_l+c.
\]
А значит верно и неравенство с полусуммой:
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq \varepsilon_l+\frac{c+d}{4}>\varepsilon_l+\frac{d}{4}>\varepsilon_l+ \frac{|x^i_ku_m|}{4\sqrt{3}}.
\]

Тогда, ввиду~\eqref{104}, 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k))>\varepsilon_l \left(1+\frac{17}{72\sqrt{3}}\right).
\]
Полученное противоречие с~\eqref{101} завершает доказательство случая.
\item [(б)] Случай $\oordball_{x^i_k}\Sigma=2$.
Пусть $\varepsilon_0(k)>0$ достаточно мало, а $\varepsilon_l>0$ последовательность чисел, меньших $\varepsilon_0(k)$ таких, что $\sharp (\partial B_{\varepsilon_l}(x^i_k) \cap \Sigma )=2$. Обозначим  $s^l, t^l \defeq \partial B_{\varepsilon_l}(x^i_k) \cap \Sigma$. Ясно, что угол $\angle s^lx^i_kt^l > \frac{2\pi}{3} - o_\rho(1)$ (в противном случае замена $\Sigma \setminus B_\varepsilon(x^i_k) \cup St(s^l,t^l,x^i_k)$, где $S \ni x^i_k$ --- множество, определенное в пункте~\ref{Losiu} для точки $w=x^i_k$, а $St(s^l,t^l,x^i_k)$ --- дерево Штейнера, соединяющее точки $s^l$,$t^l$ и $x^i_k$, имело бы не большую энергию и строго меньшую длину, чем множество $\Sigma$). 

То есть
\begin{equation}
\angle ((s^lx^i_k), (t^lx^i_k))\geq \frac{2\pi}{3}.
\label{990}
\end{equation}
Заметим теперь, что для каждого $\varepsilon_l$ верно
\begin{equation}
\H(B_{\varepsilon_l}(x^i_k)\cap \Sigma)=2\varepsilon_l+o_{\varepsilon_l}(1)+o_\rho(1)\varepsilon.
\label{1000}
\end{equation}
Формула~\eqref{1000} верна ввиду пункта~\ref{Losiu}: в противном случае, можно было бы заменить $\Sigma$ на связное множество $\Sigma \setminus B_{\varepsilon_l}(x^i_k) \cup [x^i_ks^l]\cup S$, где $S$ определено в пункте~\ref{Losiu} при $w=x^i_k$, и получить противоречие с оптимальностью $\Sigma$. 
Можно считать, что 
\begin{equation}
\H(B_{\varepsilon_l}(x^i_k)\cap \Sigma)<2\varepsilon_l \left (1+\frac{1}{36}\right).
\label{1010}
\end{equation}


Теперь заметим, что можно считать, что 
\begin{equation}
\frac{\varepsilon_l}{\varepsilon_{l+1}}\leq \frac{18}{17}.
\label{1030}
\end{equation}
Пусть не так, тогда найдется $\varepsilon_l$ такое, что $\sharp \left( \partial B_{\varepsilon_l}(x^i_k)\cap \Sigma
\right) \geq 3$ для каждого $\varepsilon \in [\frac{17\varepsilon_l}{18},\varepsilon_l[$. Но тогда, ввиду неравенства коплощади
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k))\geq \H(\Sigma \cap B_{\frac{17\varepsilon_l}{18}}(x^i_k)) +\H(\Sigma \cap (B_{\varepsilon_l}(x^i_k) \setminus  B_{\frac{17\varepsilon_l}{18}}(x^i_k))\geq 2\varepsilon_l\left(1+\frac{1}{36}\right),
\]
что противоречит (\ref{1010}).
Ввиду наличия последовательностей $\left\{s^l\right\}$, $\left \{t^l\right \}$ и единичного порядка $\oord_{x^i_k}(\Sigma)=1$ существует также сходящаяся к $x^i_k$ последовательность точек $\{ u_l\}$ таких, что $\angle((u_lx^i_k),(ix))=\frac{\pi}{2}$.

Рассмотрим произвольную такую точку $u_m$. Выберем такой номер $l$, что 
\begin{equation}
0<\varepsilon_l-|x^i_ku_m|\leq \frac{1}{18}\varepsilon_l.
\label{1040}
\end{equation}
Такое $\varepsilon_l$ существует ввиду формулы~\eqref{1030}. Заметим также, что ввиду~\eqref{990} выполняется
\[
\sharp (\partial B_{|x^i_k u_m|}(x^i_k)\cap \Sigma) \geq 3.
\] 
Кроме того, 
\begin{equation}
d \defeq \dist(u_m, Q)\geq \frac{1}{2}|x^i_ku_m|-o_\rho(1)\varepsilon> \frac{1}{3}|x^i_ku_m|,
\label{1050}
\end{equation}
где $Q$ --- область возможного расположения точек $s^l, t^l$ (множество $Q$ не пересекается с углом с вершиной в $x^i_k$, раствором $\frac{\pi}{3} - o_\rho(1)$ и перпендикуляром к $(ix)$ в качестве биссектрисы).
Пусть $q$ --- компонента связности $\Sigma \setminus Q$, содержащая $u_m$. Пусть теперь $c$ --- длина проекции $q$ на ту сторону $Q$, чье пересечение с $q$ не пусто, тогда
%а $var(c)$ величина проекции на эту координату. Тогда
\[
\H(q)\geq \frac{c+d}{2}.
\]
Тогда 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq 2\varepsilon_l-2c+\frac{c+d}{2}.
\]
С другой стороны, по неравенству коплощади 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq 2\varepsilon_l+c.
\]
А значит верно и такое неравенство:
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq
\frac{2}{5}\left(2\varepsilon_l-2c+\frac{c+d}{2}\right)+\frac{3}{5}\left(2\varepsilon_l+c \right)\geq 2\varepsilon_l+\frac{d}{5}.
\]
Тогда, ввиду~\eqref{1050},
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k)) \geq 2\varepsilon_l+\frac{|x^i_ku_m|}{15}.
\]
Но тогда, ввиду~\eqref{1040}, 
\[
\H(\Sigma \cap B_{\varepsilon_l}(x^i_k))>2\varepsilon_l \left( 1+\frac{17}{540} \right).
\]
Полученное противоречие с~\eqref{1010} завершает доказательство пункта.
\end{itemize}

\end{proof}
\item В случае, если  $\oord_{x^i_k} \Sigma = 1$, отрезок, входящий в  $x^i_k$, будет почти перпендекулярно ребру $(ix]$.
\label{perp_edge2}

\begin{proof}
Сперва поясним корректность формулировки. Ввиду пункта~\ref{discr} точка $x^i_k \in X_\Sigma$.  Ввиду Утверждения~\ref{discr_str} можно выбрать такое $\varepsilon > 0$, что $\Sigma \cap B_{\varepsilon}(x^i_k)$ совпадает с отрезком $[sx^i_k]$, где $s \in \partial B_{\varepsilon}(x^i_k)$. Утверждается, что тогда ребро $[sx^i_k] \subset \Sigma$ будет почти перпендекулярно ребру $(ix]$, то есть $|\frac{\pi}{2} - \angle ([sx^i_k],(ix])|=o_\rho(1)$.

Мы видим, что $\oordball_{x^i_k} \Sigma = 1$, а значит нам нужно лишь повторить доказательство случая (а) из пункта~\ref{discr} (в качестве $s^l$ можно брать произвольную точку $\Sigma \cap B_\varepsilon(x^i)$).
\end{proof}


\item  Пусть $\oord_{x^i_k} \Sigma =2$ и $x^i_k \in X_\Sigma$, тогда, согласно Утверждению~\ref{discr_str}, существует такое $\varepsilon$, что $\Sigma \cap \overline{B_{\varepsilon}(x^i_k)}=[sx^i_k] \sqcup [tx^i_k]$, причем угол 
$\angle sx^i_kt \geq \frac{2\pi}{3}$. Утверждается, что тогда
\[
\angle((sx^i_k], (ix))=\angle( (ix),(tx^i_k] )+ o_\rho(1).
\]

\label{ugli}

\begin{corollary}

В частности, тогда

\[
\angle((sx^i_k], (ix))=\angle( (ix),(tx^i_k] )+ o_\rho(1)\leq \frac{\pi}{6}.
\] 

\end{corollary}

\begin{proof}
Предположим противное: не умаляя общности, найдется число $c_1>0$, такое что 
\[
\eta \defeq \angle((sx^i_k], (ix))-\angle( (ix),(tx^i_k]) \geq c_1.
\]
Пусть $l$ --- прямая, проходящая через точку $x^i_k$ и параллельная $(ix)$. Отразим отрезок $[tx^i_k]$ относительно $l$. Пусть $t'$ --- образ точки $t$ при этом отображении. Тогда $|t'x^i_k|=\varepsilon$ и
\[
|sx^i_k|+|tx^i_k|=|sx^i_k|+|t'x^i_k|=2\varepsilon.
\]
В то же время по теореме косинусов для $\Delta sx^i_kt'$
\[
|st'|^2 = |sx^i_k|^2+|x^i_kt'|^2-2|sx^i_k||x^i_kt'|\cos \angle sx^i_kt'=2\varepsilon^2(1-\cos \eta),
\]
поскольку $\angle sx^i_kt'=\pi+\angle((tx^i_k], (ix))-\angle( (ix),(sx^i_k])=\pi-\eta$.
Таким образом,
\[
|sx^i_k|+|t'x^i_k|-|st'| > c_2\varepsilon,
\]
где $c_2 > 0$ константа, зависящая только от $\eta$.

Пусть теперь точка $d \defeq [st']\cap l$. Тогда $\angle((sd], (ix))=\angle( (ix),(td])$ и 
%\begin{equation*}
\[(|sx^i_k|+|tx^i_k|)-(|sd|+|dt|)= 2\varepsilon - |st'|>c_2\varepsilon.\]
%\end{equation*}

Пусть $S \ni d$ --- множество, определенное в пункте~\ref{Losiu}. Тогда $\H(S)=o_\varepsilon(1)+o_\rho(1)\varepsilon$.
А значит связное множество $\Sigma \setminus ([sx^i_k]\cup[tx^i_k]) \cup S \cup [sd] \cup [td]$ при достаточно малых $\rho$ и $\varepsilon$ будет лучше $\Sigma$, поскольку имеет не большую энергию и длину, не превосходящую $\H(\Sigma)-c_2\varepsilon+ o_\rho(1)\varepsilon+o(\varepsilon)$. Полученное противоречие с оптимальностью $\Sigma$ завершает доказательство пункта.
\end{proof}

%небольшие проблемы с аккуратностью про конусы
%и надо поменять формулировку: что совпадает с дугами (и про концы дуг сказать)
\item Пусть  $\oord_{x^i_k} \Sigma =2$ и $x^i_k \in E_\Sigma$, тогда
%, согласно Лемме~\ref{ord_arcs}, 
существует такое $\varepsilon$, что $\Sigma \cap \overline{B_{\varepsilon}(x^i_k)}$ содержит две дуги $\breve{[sx^i_k]}$ и $\breve{[tx^i_k]}$, пересекающиеся только по точке $x^i_k$. Докажем, что эти дуги содержатся в узких  псевдоконусах с биссектрисами, $o_\rho(1)$-почти образующими развернутый угол и $o_\rho(1)$-почти параллельными $(ix]$ и с раствором $\gamma(\rho) = o_\rho(1)$.


\label{arc_par}
\begin{proof}
Напомним, что $x^i_k$ имеет одно или два энергетических ребра, причем они почти параллельны $(ix)$. Пусть $Q = Q_1 \cup Q_2$ --- объединение двух узких  псевдоконусов  с биссектрисами почти параллельными $(ix]$ и
$G_\Sigma \cap B_{\varepsilon}(x^i_k) \subset Q$. Оно существует ввиду Утверждения~\ref{edgeangle}. Не умаляя общности, ввиду пункта~\ref{ordball} будем считать $\varepsilon>0$ таким, что $\sharp(\Sigma \cap \partial B_\varepsilon(x^i_k)) \leq 2$.
 
Если хотя бы одно из двух ребер $x^i_k$ направлено в две стороны, пункт тривиален ввиду Утверждения~\ref{star}. Таким образом, можно считать, что каждое ребро направлено в одну сторону. Угол между ребрами, не содержащий точек $y^i_k$, соответствующих энергетическим точкам из $Q$, будем называть внутренним. Величина его не превосходит $\pi$.
 
Пусть $(qx^i_k]$ --- луч, не совпадающий ни с одним ребром $x^i_k$. Покажем, что тогда либо число пересечений $\sharp \left(\Sigma \cap B_{\varepsilon}(x^i_k) \cap (qx^i_k] \right)$ конечно, либо $\Sigma$ содержит отрезок этого луча ненулевой длины c концом в $x^i_k$. Во втором случае, не умаляя общности, будем рассматривать $\varepsilon$, не превосходящий длину этого отрезка. 

Пусть не реализовался ни один из двух случаев и множество $\Sigma \cap B_{\varepsilon}(x^i_k) \cap (qx^i_k]$ содержит бесконечное число точек. Заметим, что любая точка из множества $\Sigma \cap B_{\varepsilon}(x^i_k) \cap (qx^i_k]$ не энергетическая и, значит, является центром отрезка или правильной треноги, а множество $\Sigma \cap B_{\varepsilon}(x^i_k) \setminus Q$ является штейнеровским лесом. 

Пусть $L$ обозначает ту часть внутреннего угла, которая ограничена $(qx^i_k]$ и перпендикуляром к $(ix)$, проходящим через $x^i_k$ (если луч $(qx^i_k]$ не перпендикулярен $(ix)$). Тогда $S := L\setminus Q \cap \overline{B_\varepsilon (x^i_k)}\cap \Sigma$ является штейнеровским лесом, причем все точки $\partial S$ (число которых бесконечно), за исключением конечного числа принадлежащих $(\partial B_\varepsilon (x^i_k) \cap L \setminus Q)\cap \Sigma$, лежат на $(qx^i_k]$ или на перпендикуляре. Тогда ввиду Леммы~\ref{St_l} число концевых точек леса $\partial S$, принадлежащих перпендикуляру, бесконечно, а значит найдется сходящаяся к $x^i_k$ бесконечная последовательность точек $\{u_l\}$ таких, что $\angle((u_l,x^i_k)(ix))=\pi/2$ для каждого номера $l$. Однако существование такой последовательности приводит к противоречию, как было показано в случае (б) пункта ~\ref{discr}.


%Поскольку луч $(qx^i_k]$ произвольный, из этого сразу будет следовать конечность 
Покажем, что число пересечений $\Sigma$ и внутренней (то есть лежащей во внутреннем углу) границы произвольного псевдоконуса $q_{inn}$ конечно. 

Предположим противное, то есть что множество $\left(\Sigma \cap B_{\varepsilon}(x^i_k) \cap q_{inn} \right)$ бесконечно. Пусть при этом $\varepsilon>0$ такое, что $\sharp(\partial B_\varepsilon(x^i_k) \cap \Sigma) =2$. Выберем луч $(qx^i_k]$ так, чтобы в шаре $B_\varepsilon(x^i_k)$  он не пересекался с $Q$ %и чтобы $\Lambda$ (фигура, ограниченная  $q_{inn}$, $(qx^i_k]$ и $\partial B_\varepsilon(x^i_k)$), была такова, что $\sharp (\overline{\Lambda} \cap \Sigma \cap \partial B_\varepsilon(x^i_k)) \leq 2$.
и не содержал точек $\Sigma$ (возможно, $\varepsilon$ пришлось заменить на меньший радиус, сохраняя условие $\sharp(\partial B_\varepsilon(x^i_k) \cap \Sigma) =2$).  

Заметим, что $\Lambda \setminus q_{inn}$ не содержит энергетических, а значит и концевых точек $\Sigma$. Пусть теперь $W$ --- гладкая кривая между $q_{inn}$ и $(qx^i_k]$, то есть такая кривая, пересечением которой и произвольной окружности с центром в $x^i_k$ и радиусом $\varepsilon'<\varepsilon$, является точка, принадлежащая внутренности дуги с концами в точках $q_{inn}$ и $(qx^i_k]$. Потребуем кроме того, чтобы ребро $x^i_k$ было односторонней касательной к $W$. Если $\sharp (\Sigma \cap W)$ конечно, переопределим псевдоконус, заменив $q_{inn}$ на $W$. Предположим, что это множество бесконечно. Пусть $\Lambda$ --- фигура, ограниченная  $W$, $(qx^i_k]$ и $\partial B_\varepsilon(x^i_k)$. По нашему предположению $\partial \Lambda \cap \Sigma$ не содержит точек на  $(qx^i_k]$, содержит не более двух точек на $\partial B_\varepsilon(x^i_k)$ и бесконечно много точек на $W$. Заметим, что изменение наклона касательной к $W$ внутри $B_\varepsilon(x)$ зависит от $\varepsilon$ и сколь угодно мало. Обозначим его за $\xi_1$. Пусть $ \varepsilon_1<\varepsilon$ достаточно мало. За $\xi_2$ обозначим максимальный угол, под которым дуга $\Lambda \cap \partial  B_\varepsilon(x^i_k)$ видна из $\Lambda \cap B_{ \varepsilon_1}$
%$\angle ix^i_kq$, соответствующий изменению касательной к $\partial B_\varepsilon(x^i_k) \cap \overline \Lambda$.
 Покажем, что в области $\Lambda \cap B_{ \varepsilon_1}(x^i_k)$ нет точек ветвления $\Sigma$. Предположим противное: пусть точка ветвления существует. Продолжим исходящие из неё ребра лучами и заметим, что один из лучей пересек $\partial \Lambda \cap (qx^i_k]$, поскольку $\xi_1+\xi_2+\pi<4\pi/3$. Но  это означает, что и $\Sigma \cap \Lambda \cap (qx^i_k] \neq \emptyset$, поскольку $\Lambda \cap \Sigma \subset S_\Sigma$. Полученное противоречие показывает, что $\Sigma \cap \Lambda \cap B_{ \varepsilon_1}(x^i_k)$ состоит из отрезков, соединяющих точки, лежащие на $W$. Ясно, что последовательное соединение счетного числа точек $\{z_l\}\subset W$, имеющих единственную точку сгущения $x^i_k$ дает возможную границу псевдоконуса (поскольку $\angle((z_l z_{l+1}), (ix^i_k])$ стремится к нулю, а значит для $z\in[z_l z_{l+1}]$ угол $\angle zx^i_ki \leq z_lx^i_ki \rightarrow 0$, и другие условия на границу псевдоконуса также выполнены). Но тогда можно выбрать такой псевдоконус $Q$ (переопределив $\varepsilon \defeq \varepsilon_1$), что все точки $\{z_l\} \subset \Int(Q)$.

%МОЖЕТ БЫТЬ НАДО НАПИСАТЬ ЭТО ВСЕ КАК ОБЩЕЕ УТВЕРЖДЕНИЕ ПРО ПСЕВДОКОНУС, А ТУТ ПРОСТО СОСЛАТЬСЯ

% Применив Следствие~\ref{1} к штейнеровскому лесу, образованного пересечением $\Sigma$ и областью, ограниченной $%\partial W$, $\partial B_\varepsilon'(x^i_k)$, получим, что  число пересечений $\left(\Sigma \cap U \cap \partial W \right)$ %конечно, и переопределим псевдоконус, заменив границу $Q_{inn}$ кривой $W$.

Таким образом, можно считать $\varepsilon>0$ настолько малым, что пересечение $\Sigma \cap B_\varepsilon(x^i_k) \cap \partial Q =\emptyset$, а значит каждая из двух дуг $\breve{[sx^i_k]}$ и $\breve{[tx^i_k]}$ либо содержится в конусе $Q_1$ или $Q_2$, либо совпадает с отрезком внутри множества $B_{\varepsilon}(x^i_k) \setminus (Q_1 \cup Q_2)$. Если дуга содержится в псевдоконусе $Q_i$ ($i=1,2$), то она имеет одностороннюю касательную, а значит к ней применима Лемма~\ref{angles2}. Поскольку $x^i_k \in E_\Sigma$, она имеет хотя бы одно энергетическое ребро, а значит, ввиду определения ребра и условия на $\varepsilon$, хотя бы одна из дуг должна содержаться в каком-либо псевдоконусе. Не умаляя общности, $\breve{[sx^i_k]} \subset Q_1$. Тогда ввиду Леммы~\ref{angles2} вторая дуга $\breve{[tx^i_k]}$ не может содержаться в том же псевдоконусе. Пусть $\breve{[tx^i_k]}$ не содержится в псевдоконусе $Q_2$. Тогда она является отрезком, причем $\breve{[tx^i_k]}=[tx^i_k]\subset B_\varepsilon(x^i_k)\setminus Q$. Предположим, что этот отрезок не является $o_\rho(1)$-почти параллельным $(ix)$, то есть 
\[
|\angle(s_{\bar{\varepsilon}}x^i_k),(ix))-\angle(t_{\bar{\varepsilon}}x^i_k),(ix))|>c_1,
\]
 где $s_{\bar{\varepsilon}} \defeq \breve{[sx^i_k]} \cap \partial B_{\bar{\varepsilon}}(x^i_k)$, $t_{\bar{\varepsilon}} \defeq [tx^i_k] \cap \partial B_{\bar{\varepsilon}}(x^i_k)$, $0<\bar{\varepsilon}<\varepsilon$, а $c_1>0$ является константой, не зависящей от $\bar{\varepsilon}$ и $\rho$. Тогда, как было показано в пункте~\ref{ugli}
 \[
 |s_{\bar{\varepsilon}}x^i_k|+|t_{\bar{\varepsilon}}x^i_k|-|s_{\bar{\varepsilon}}d|-|t_{\bar{\varepsilon}}d| > c_2 \bar \varepsilon,
 \]
 где $d \in B_{\bar{\varepsilon}}(x^i_k)$ такая точка, что $\angle(s_{\bar{\varepsilon}}x^i_k),(ix))=\angle(t_{\bar{\varepsilon}}x^i_k),(ix))$, а прямая $(dx^i_k)$ параллельна $ix$; а положительная константа $c_2$ зависит только от $c_1$. Тогда замена множества $\Sigma$ на связное множество $\Sigma \setminus B_{\bar{\varepsilon}}(x^i_k) \cup [s_{\bar{\varepsilon}}d] \cup [t_{\bar{\varepsilon}}d] \cup S$, где $S$ определено в пункте~\ref{Losiu} при $w=d$ и для шара $B_{\bar{\varepsilon}}(x^i_k)$, демонстрирует противоречие с оптимальностью $\Sigma$. Таким образом, $\breve{[tx^i_k]}$ содержится в псевдоконусе $Q_2$, либо является отрезком, принадлежащим прямой  $o_\rho(1)$-почти параллельным $(ix)$. В этом случае переопределим $Q_2$ как произвольный псевдоконус с биссектрисой $[x^i_kt)$,  и утверждение пункта будет доказано.
\end{proof} 
 \begin{remark}
 Мы также доказали, что $\Sigma \cap B_\varepsilon(x^i_k) \setminus Q =\emptyset$.
 \end{remark}
 \begin{remark}
 Заметим также, то угол между ребрами, содержащий соответствующую $x^i_k$ точку $y^i$, не может быть меньше $\pi$ (если покрытые $x^i_k$ точки есть в обеих полуплоскостях, то угол между ребрами составляет ровно $\pi$).
 \label{rovno}
 \end{remark}


\begin{remark}
Поскольку $\Sigma$ не содержит циклов и имеет конечную длину, между любыми точками $x_1, x_2 \in \Sigma$ существует единственный несамопересекающийся путь. В дальнейшем мы будем опускать формальности и просто писать ``путь из $x_1$ в $x_2$''.
\end{remark}

\item В окрестности произвольной $x^i_k$ конечное число точек ветвления.
\label{fsinite}
\begin{proof}
Случай $x^i_k \in X_\Sigma \cup S_\Sigma$ тривиален; согласно пункту~\ref{discr} точка $x^i_k \in E_\Sigma$ имеет порядок $2$.
Тогда, ввиду пункта~\ref{arc_par}, найдется такое, сколь угодно малое, $\varepsilon>0$, что:
\begin{itemize}
\item $B_\varepsilon(x^i_k) \cap \Sigma \supset \breve{[sx^i_k]}\cup \breve{[tx^i_k]}$,
\item $\{s, t \}= \partial B_\varepsilon(x^i_k) \cap \Sigma$,
\item $\breve{[sx^i_k]} \subset Q_1$, $\breve{[tx^i_k]} \subset Q_2$ где $Q_1$, $Q_2$ --- псевдоконусы с ребрами $x^i_k$ (которые почти параллельны $(ix)$) в качестве биссектрис.
\item $B_\varepsilon(x^i_k) \cap \Sigma \setminus Q_1 \setminus Q_2$ пусто.  
\end{itemize}
%Пусть предположене пункта неверно, тогда, не умаляя общности, %$\breve{[sxi_k]} \subset Q_1$, где $Q_1$ псевдоконус, %содержащий бесконечное число точек ветвления. 

Предположим, что дуга $\breve{[sx^i_k]}$ содержит бесконечное число точек ветвления. 

Разберем два случая:
\begin{itemize}
\item[(А)] пусть ребро, совпадающее с биссектрисой $Q_1$, направлено в одну сторону.

Заметим, что в этом случае шар $B_\varepsilon(x^i_k)$ разбит дугами на две половины, одна из которых не может содержать энергетических точек (не умаляя общности, назовем её ``верхней'', а дугу $[sx^i_k]$ ``левой'').

Рассмотрим такую точку ветвления $D_2$ на дуге $\breve{[sx^i_k]}$, что на пути из $D_2$ в $x^i_k$ бесконечно точек ветвления, а на пути из $s$ в $D_2$ достаточно много точек ветвления. Из точки $D_2$ выходит три отрезка $[D_1D_2]$, $[D_2D_3]$ и $[D_2C]$ с попарными углами $2\pi/3$. Не умаляя общности, путь $D_1-D_2-D_3$ подмножество пути из $s$ в $x^i_k$. Заметим, что ввиду условий на $[sx^i_k]$ верно
 \[
| \turn (D_1-D_2-D_3-\dots -x^i_k)| \leq |\turn ([sx^i_k])| \leq 2\pi,
 \]
 где $\turn$ обозначает изменение направления касательной вдоль дуги. Поскольку касательная есть в почти всех точках, то будем воспринимать $\turn(\breve{[sx^i_k]})$ верхний предел (супремум) по всем последовательностям точек кривой:
 \[
 \turn(\breve{[sx^i_k]})=\sup_{n\in \N, s\preceq t_1 \prec \dots \prec t_n \preceq x^i_k} \sum_{i=2}^{n} |t^i-t^{i-1}|,
 \]
 где $t^i \in [-\pi,\pi]$ означает наклон касательной к кривой $\breve{[sx^i_k]}$ в точке $t_i$, а ${t_1,\dots, t_n}$ --- разбиение кривой $\breve{[sx^i_k]}$ в порядке, соответствующем параметризации, при которой $s$ --- начало кривой, а $x^i_k$ --- конец, такое, что в каждой точке $t_i$ кривая $\breve{[sx^i_k]}$ имеет касательную. Заметим, что направление угла $\angle D_1D_2D_3=2\pi/3$ определяется однозначно: в выбранных обозначениях угол направлен против часовой стрелки, то есть $\turn=\pi/3$. Это так, поскольку путь, начавшийся с отрезка $[D_2C]$ должен закончиться энергетической точкой, а значит идти в верхнюю  половину шара $B_\varepsilon(x^i_k)$.
Рассмотрим теперь путь  из $D_1$ в $x^i_k$. Начав с отрезка $[D_2D_3]$, путь движется по прямой вплоть до первой точки ветвления или энергетической точки. Из пункта~\ref{arc_par}, Замечания~\ref{rovno} и того, что ребра направлены только в одну сторону следует, что угол направления касательной в энергетических точках меняется в ту же сторону (то есть $\turn$ положительный). При этом в каждой точке ветвления путь поворачивает на $\pi/3$ против часовой стрелки, то есть поворот $\turn$ увеличивается на $\pi/3$. Таким образом, показано, что $\turn ([sx^i_k]) =\infty$. Противоречие.
(Иначе говоря, бесконечно закручивающаяся кривая, принадлежащая псевдоконусу, не может иметь пределом его вершину.)

% из множества $X_\Sigma$ или $E_\Sigma$, в которых  меняется направление односторонней касательной: Однако, как было показано  в пункте~\ref{arc_par}, если и меняется, то в ту же сторону (угол между односторонними касательными изменился не больше, чем на $\pi/3$). В то же время как следует из утверждения пункта~\ref{arc_par} и замечания~\ref{rovno} если в точке из множества $E_\Sigma$ направление односторонней касательной почти не меняется, а если и изменяется, то в ту же сторону. Встретив же точку ветвления, мы обязаны повернуть на $\pi/3$ в ту же сторону.  Таким образом путь из $D_1$ в $x^i_k$ бесконечно ``закручивается''(иначе говоря $turn(\breve{[sx^i_k}=\infty)$). Но, поскольку он при этом содержится в псевдоконусе $Q$, точка $x^i_k$ не может быть его пределом. Противоречие. 
 
\item[(Б)] пусть ребро, совпадающее с биссектрисой $Q_1$, направлено в обе стороны.

Несложно понять, что $\oordball x^i_k=1$ и можно считать достаточно малое $\delta$ таким, что $\sharp (\Sigma \cap \partial B_{\delta}(x^i_k)\cap Q_1) =1$ (в противном случае ввиду неравества коплощади можно было бы уменьшить длину $\Sigma$ (заменив $\Sigma \cap Q_1 \cap B_{\delta}(x^i_k)\cap Q_1$ на множество с длиной $\delta +o(\delta)$)).
В данном пункте ``почти'' будет означать ``с точностью до $o_\delta(1)$''. Биссектрису $Q_1$ будем обозначать $(qx^i_k]$. Все доказанные для $x$ и $\rho$ утверждения верны и для $x^i_k$ и $\delta$.

Поскольку количество точек ветвления в $Q_1$ бесконечно, бесконечно и количество концевых точек. Пусть $W$ --- концевая точка. Ей соответствует точка $y_W \in M$ такая, что $|wy_W|=r$ и $B_r(y_W) \cap \Sigma =\emptyset$. Условно будем говорить, что точки из множества $M$, соответствующие концевым точкам из $Q_1$ могут располагаться ``сверху'' или ``снизу'' (полагаем прямую $(qx^i_k]$ горизонтальной). Точка $y_W$, не умаляя общности, располагается ``сверху''. Также, не умаляя общности, полагаем точку $x^i_k$ находящейся ``справа'' от точки $W$.
%\input{pictures/9netputi}
Из точки $W$ выходит отрезок $[WD_1]\subset \Sigma$, почти перпендикулярный $(qx^i_k]$, где $D_1$ --- точка ветвления: из-за условия почти-перпендикулярности $D_1$ не может быть точкой из $X_\Sigma$ степени $2$ или точкой из $E_\Sigma$ (см. пункты~\ref{discr}, ~\ref{arc_par}  и следствие из пункта~\ref{ugli}). Ясно, что путь $L$ из $D_1$ в $x^i_k$ начинается с отрезка $[D_1D_2]$, направленного в сторону $x^i_k$: в противном случае, если бы путь $L$ начинался с отрезка $[D_1D_{-2}]$, направленного от $x^i_k$, то, ввиду условия  $B_r(y_W) \cap \Sigma =\emptyset$ (и ввиду дугообразной связности, из-за которой путь $L$ должен существовать в достаточно малой окрестности $x^i_k$, а значит не может иметь диаметр, больший $r$), он ``отрезал'' бы путь $P$, начинающийся со второго отрезка $[D_1D_{2}]$ и в каждой точке ветвления поворачивающий ''вниз'', от находящихся ``снизу'' точек множества $M$: то есть либо пути $L$ и $P$ должны пересечься, либо пустая окружность радиуса $r$, касающаяся энергетической точки, которой заканчивается путь $P$, должна пересекать путь $L$, что также невозможно (см. рис.~\ref{fig:netputi}). 

\input{pictures/dvap}
Точка $D_2$ может быть точкой степени $2$ или $3$, в любом случае путь $L$ продолжается отрезком $[D_2D_3]$, направленным ``вправо'' (и ввиду утверждения пункта~\ref{ugli} имеющим относительно $(qx^i_k]$ угол почти $\pi/6$): если бы он продолжался отрезком $[D_2D_{-3}]$, направленным вниз,  то существовал бы путь, выходящий из $D_{-3}$ и поворачивающий на каждом шагу ``налево''. Наличие аналогичного пути из $D_{-2}$  влечет противоречие с выбором $\delta$ (оба пути не могут закончиться энергетической точкой степени $1$, поскольку все составляющие их отрезки имеют угол с $(qx^i_k]$ почти $\pi/6$. То есть каждый из путей должен пересечь $\partial B_{\delta} (x^i_k)$ (см. рис.~\ref{fig:dvap})).

Далее можно повторять те же рассуждения с точностью до симметрии относительно $(qx^i_k]$ и взяв точку $D_{-3}$ (в случае её наличия) в качестве точки $W$. В случае же ее отсутствия, точка $D_2$ будет выступать в роли отрезка $[WD_1]$, поскольку входящие в нее отрезки имеют угол почти $\pi/6$ с $(qx^i_k]$.

То есть путь $L$ содержит отрезок $[D_2D_3]$, где $D_3$ либо точка ветвления, либо точка степени $2$. Несложно заметить, что в первом случае $\Sigma$ содержит отрезок $[D_3G]$, где $G$ концевая точка (иначе существовал бы начавшийся в $G$ и не заканчивающийся энергетической точкой путь, в каждой точке ветвления, поворачивающий от точки $x^i_k$). Во втором случае, как следует из пункта~\ref{ugli}, $L$ продолжается отрезком $[D_3D_4]$, имеющим почти такой же угол с $(qx^i_k]$, что и $(D_2D_3)$ (то есть отличающийся от $\pi/6$ на величину $o_\delta(1)$). То есть точка $D_4$ может быть либо точкой ветвления, либо точкой степени $2$ (причем в таком случае она должна принадлежать $X_\Sigma$) и т.д. 

Заметим, что путь $L$ не может содержать ломаную $L_1-L_2-L_3-L_4-L_5$, где все точки $L_i$ имеют степень $2$, а углы $\angle (L_iL_{i+1}), (ix)), \angle (L_iL_{i-1}), (ix))  \geq  \pi/7$. Поскольку данное утверждение потребуется нам за пределами пункта, сформулируем его в более общем виде:
\begin{proposition}
Пусть $\bar x \in E_\Sigma$ и существуют такие точки $y_1, y_2$, что $|y_1y_2|=2r$, $|y_1\bar x|=r =|y_2 \bar x|$ и $B_r(y_1)\cap \Sigma = B_r(y_2)\cap \Sigma =\emptyset $. Пусть, кроме того $\bar{\varepsilon}>0$ такой, что $B_\varepsilon(\bar{x}) \cap \Sigma$ является дугой. Тогда для произвольного $c>0$ найдется $\varepsilon(c)>0$ такой, что все односторонние касательные к точкам $B_{\bar \varepsilon}(\bar{x}) \cap \Sigma$ имеют угол с прямой $(y_1y_2)$ находящийся в промежутке $[\pi/2-2c, \pi/2]$.
\label{zapred}
\end{proposition}

\begin{proof}
Предположим противное, то есть что существует последовательность точек, в которых односторонняя касательная имеют угол с $(y_1y_2)$ вне указанного промежутка. Ввиду утверждения пункта~\ref{arc_par} (для $\bar{x}$ в качестве $x$ и энергетических точек из этой последовательности в качестве точек $x^i_k$) достаточно рассматривать только точки из множества $X_\Sigma \sqcup S_\Sigma$. Поскольку в точках $S_\Sigma$ направление касательной не меняется ясно, что найдется сходящаяся к $\bar{x}$ последовательность точек из $X_\Sigma$ таких, что хотя бы один из двух входящих в точку отрезков имеет угол с $(y_1y_2)$, меньший $\pi/2-2c$. Пусть $L_1$ такая точка, достаточно близкая к $\bar{x}$. Ввиду утверждения пункта~\ref{ugli}, можно считать, что оба входящих в $L_1$ отрезка имеют угол с $(y_1y_2)$, меньший $\pi/2-9/5c$. Тогда отрезок, лежащий на пути из $L_1$ в $\bar{x}$ обязательно заканчивается точкой $L_2 \in X_\Sigma$. Но отрезок, выходящий из $L_2$ должен иметь угол с $(y_1y_2)$, меньший $\pi/2-8/5c$ и заканчиваться точкой $L_3 \in X_\Sigma$. Ясно, что таким образом для любого, сколь угодно малого $\varepsilon$ существует такая ломаная $L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\bar{\varepsilon}}$, что все углы $\angle((L_iL_{i+1}),(Y_1y_2))<\pi/2-c$ при $i=1,2,3,4$. 
Не умаляя общности будем считать $(y_1y_2)$ осью ординат, а точку $\bar{x}$ началом координат. Не умаляя общности, точкам $L_1$, $L_2$, $L_3$ соответствуют верхние точки множества $M$, а точкам $L_2, L_4$ --- нижние: ввиду утверждения пункта~\ref{angles} и неравенства $\angle L_{i-1}L_{i}L_{i+1} \leq \pi-2c, i=2,3,4$ двум подряд идущим точкам не могут соответствовать одновременно верхние или нижние точки.
 Заметим теперь, что отношения между отрезками ломаной линейные, и замена ломаной на отрезки $L_1-L_2-L_4-L_5$ уменьшит длину на величину, линейно зависящую от $[L_1L_2]$. 

Строго говоря, поскольку $B_r(y_{L_{i+1}})\cap [L_{i-1}L_{i}]=\emptyset = B_r(y_{L_{i-1}})\cap [L_{i}L_{i+1}]$, где $y_{L_j} \in M$ соответствует $L_j$, $j= 1 \dots 5$, $i=2,3,4$ и ввиду пункта~\ref{angles}, выполняется \[[L_2L_3]_y>|L_1L_2|_y-|L_1L_3| o_{\bar{\varepsilon}}(1)\]
 %|L_1L_2|-\bar{\varepsilon}^2,\]
  где нижний индекс $y$ означает проекцию на $(y_1y_2)$. То есть $|L_2L_3|>\sin c |L_1L_2|-o_{\bar{\varepsilon}}(1)|L_1L_3|$.
 И наоборот, $|L_1L_2|>\sin c |L_2L_3|-o_{\bar{\varepsilon}}(1)|L_1L_3|$. 
 %Из этого очевидным образом следует существование $c_1, c_2>0$ таких, что $c_2|L_2L_3|\geq |L_1L_2| \geq c_1|L_1L_3|$.   
 Аналогично и для остальных $L_i$. Замена ломаной на $L_1-L_2-L_4-L_5$ уменьшит ее длину не меньше, чем на
 \begin{multline*}
 |L_2L_3|+|L_3L_4|-\sqrt{ |L_2L_3|^2+|L_3L_4|^2+2 |L_2L_3||L_3L_4|\cos (2c) }\geq \\
|L_1L_2| \left(\sin c+\sin^2 c-\sqrt{\frac{1}{\sin^2 c}+\frac{1}{\sin^4 c}+2\frac{\cos (2c)}{\sin^3 c}})+o_{\bar{\varepsilon}}(1|L_1L_2| \right),
 \end{multline*}
то есть замена, действительно, уменьшает длину на величину, линейно зависящую от $|L_1L_2|$.
\input{pictures/dvapo}
Кроме того, несложно понять (как обычно используя пункт~\ref{angles}), что существуют
% отрезки $[L_1L_{6}]$ и $[L_5L_7]$
точки $L_6$ и $L_7$  такие, что $$B_r([L_1L_6]) \cup B_r([L_5L_7]) \supset B_r([L_1L_3]) \cup B_r([L_3L_5]).$$ Причем эти отрезки имеют длину $o_{[L_1L_2]}(1)$. 

 Тогда можно заменить ломаную  $L_1-L_2-L_3-L_4-L_5$ на $L_6-L_1-L_2-L_4-L_5-L_7$ и получить противоречие с оптимальностью $\Sigma$ (см. рис~\ref{fig:dvapo}).
 \end{proof}

%тут уруру конечно ужасно лень аккуратно писать но в общем выпуклости у нас нет, но зато есть почти выпуклость из-за того что окружности для L_1 и L_5 всё выгрызли и L_3 не могла высоко подпрыгнуть
Вернемся к пути $L$. Теперь ясно, что он является ломаной с узлами в точках ветвления и энергетических точках степени $2$. Причем последние не могут встречаться более четырех раз подряд, если их угол с осью абсцисс достаточно велик. А из узлов в точках ветвления отходят (не принадлежащие $L$) отрезки, почти перпендикулярные $(ix)$. Тогда все отрезки ломаной $L$ имеют угол с $(ix)$, больший, чем $\pi/7$ (поскольку в отрезках, выходящих из точек ветвления угол почти $\pi/6$, а в точках степени два угол падения почти равен углу отражения, причем погрешность не накапливается, поскольку не может быть больше четырех точек ветвления подряд). 

Но тогда длина пути $L$ составляет не меньше, чем
\[
Pr_{(ix)}(L) \left (1+\tg \frac{\pi}{7} \right )=\delta \left (1+\tg \frac{\pi}{7} \right),
\]
где $Pr_{(ix)}(L)$ ---  проекция пути $L$ на прямую $(ix)$.
С другой стороны из условий на $Q$ следует, что длина $\Sigma \cap B_{\delta}(x^i_k)\cap Q$, а значит и длина пути $L$, не превосходит $\delta+o(\delta)$. Полученное противоречие завершает доказательство пункта.
\end{itemize}





\end{proof}

\begin{remark}
Заметим, что в пункте~\ref{fsinite} доказано утверждение о конечности точек ветвления на дуге $\breve{[sx]}$ для произвольной точки $x \in E_\Sigma$ в случае если $\breve{[sx]}$ лежит в каком либо псевдоконусе $Q$ и $\Sigma \cap \partial Q =\emptyset.$
\label{rfinite}
\end{remark}

\item Покажем, что компонента связности $\Sigma \cap B_\rho(x) \setminus \{x\}$ содержит бесконечное число энергетических точек не более чем одного энергетического ребра (иначе говоря, находящихся не более чем в одном псевдоконусе).
\label{rozo4ki}

\begin{remark}
В доказательстве данного пункта в случае $\oord_x \Sigma =1$ компоненту связности множества $\Sigma \cap B_\rho(x) \setminus \{x\}$ можно считать совпадающей с данным множеством.
\end{remark}

В доказательстве данного пункта рассматриваются только точки принадлежащие данной компоненте. Для простоты записи будем считать, что рассматривается ситуация $\oord_x \Sigma =1$.

\begin{proof}
Предположим противное утверждению пункта~\ref{rozo4ki}.
\begin{enumerate}


\item Точка $x^i_k \in X_\Sigma$ не может иметь порядок $2$. 
\label{9}
\begin{proof}
Пусть $x$ имеет два ребра $(ax]$ и $(bx]$, $\alpha \in]0, \pi]$ --- угол между этими лучами, $\rho>0$ достаточно мало и $\sharp(\partial B_\rho(x) \cap \Sigma) \leq 3$ (корректно ввиду Замечания~\ref{ord_en}), $Q^a$, $Q^b$ --- псевдоконусы с ребами в качестве биссектрис, содержащие все энергетические точки этих ребер (в достаточно малой окрестности $B_\rho(x)$). Меньший угол между ребрами называется внутренним (а если оба угла равны $\pi$, то внутренним называется угол, не содержащий точку $y \in M$, соответствующую точке $x$: можно считать, что ребра направлены в одну сторону, иначе утверждение пункта тривиально).


Не умаляя общности, $i=a$. Предположим противное утверждению пункта: пусть точка $x^a_k \in X_\Sigma$ имеет степень два. Воспользуемся пунктом~\ref{ugli} и обозначим, с точностью до $o_\rho(1)$, угол между входящими в $x^a_k$ отрезками и ребром $(ax]$ за $\delta$.
Выполняется неравенство $\delta \leq \frac{\pi}{6} + o_\rho(1)$. 

Обозначим за $[x^a_k t]$ тот отрезок из $x^a_k$, который направлен к $x$. Возможны два варианта:


\begin{itemize}
\item Отрезок $[x^a_k t]$ заканчивается точкой ветвления. Если $t$ соединена со следующей энергетической точкой того же ребра $[ax]$ (то есть лежащего в криволинейном  псевдоконусе этого ребра, определенном в Утверждении~\ref{edgeangle}), то угол между $(tx^a_{k+1})$ и $(ax)$ будет равен $\frac{\pi}{3} - \delta \leq \frac{\pi}{6} + o_\rho(1)$. В таком случае, $\delta = \frac{\pi}{6} + o_\rho(1)$ (как изображено на Рис.~\ref{norm1}). 
Если точка $t$ не соединена с $x^a_{k+1}$, то она соединена с точкой ветвления $C$ такой, что отрезок $[tC]$ направлен от ребра $(bx]$ (как изображено на Рис.~\ref{norm11}). Тогда путь, начинающийся с отрезков $[x^a_k t]$ и $[tC]$ и продолжающийся поворотами в ту же сторону сможет закончиться только если $C$ соединена с $x^a_{k+1}$. 
\begin{remark}
Здесь и в дальнейшем доказательстве пункта~\ref{rozo4ki} можно считать, что ни один рассматриваемый путь не может закончиться на $\partial B_\rho(x)$ (поскольку число пересечений $\partial B_\rho (x) \cap \Sigma$ конечно и значит можно выбрать $\rho>0$ так, чтобы это было верно).
\end{remark}
В этом случае угол между отрезком $[Cx^a_{k+1}]$, и ребром $(ax]$ будет равен $\frac{\pi}{3} +\delta$. Значит, точка $x^a_{k+1}$ имеет порядок один. Но в этом случае указанный угол должен совпадать с $\frac{\pi}{2}+o_\rho(1)$, поэтому все равно $\delta = \frac{\pi}{6} +o_\rho(1)$.
%\input{pictures/norm1}

Оставшийся отрезок точки $t$ (обозначим его за $[tD]$) имеет угол 
$$\frac{2\pi}{3} - \delta - \alpha = \frac{\pi}{2}-\alpha + o_\rho (1)$$
 со вторым ребром $(bx]$. То есть если $J \defeq [tD) \cap (bx]$, то $\angle tJx =\frac{\pi}{2} -\alpha +  o_\rho (1)$. Тогда точка $D$ не может быть энергетической точкой степени один или точкой из $E_\Sigma$ степени два. Энергетической точкой из $X_\Sigma$ степени два или точкой ветвления она также не может быть, потому что тогда найдется бесконечный путь, начинающийся с $[sx^a_k], [x^a_{k}t], [tD], \dots$, где
$[sx^a_k]$ --- отрезок, входящий в $x^a_k$, а поворот на каждом шаге не меньше $\frac{2\pi}{3}$. Противоречие.

%\input{pictures/norm11}

\item Точка $t$ является энергетической точкой ребра $(bx]$, то есть совпадает с точкой $x^b_l$.

Тогда $x^b_l$ должна быть степени два (иначе нет пути из $x^a_k$ в $x$) и принадлежать множеству $X_\Sigma$, т.к. $\angle((x^a_kx^l_b],(bx])=\alpha+\delta+o_\rho(1) \neq o_\rho(1)$. Ситуация $\angle((x^a_kx^l_b],(bx])=\pi+o_\rho(1)$ также невозможна ввиду наличия окружностей $B_r(x^a_k)$, $B_r(y_l^b)$ и $B_r(y)$, не пересекающихся с $\Sigma$.


 %$B_{\min(|xx^b_{l}|, |xx^a_{k}|)}(x) \cap \Sigma$, связности). 
Но тогда есть отрезок $[x^b_l d] \subset \Sigma$, выходящий из  $x^b_l$ с углом $\angle xx^b_ld = \angle bx^b_lx^a_k +  o_\rho (1)$.
%= \pi-\delta -\alpha$.  
Разберем ситуацию, когда он не разветвился, а также воткнулся в энергетическую точку $x^a_{k+1}$ первого ребра. Пусть и новый отрезок не разветвился и $[x^a_{k+1}x^b_{l+1}] \subset \Sigma$, где $x^b_{l+1}$ --- энергетическая точка второго ребра. И так далее. Несложно заметить, что тогда углы падения и отражения будут увеличиваться c каждым шагом на $\alpha + o_\rho (1)$ (как изображено на Рис.~\ref{norm2}).
Но они не должны превосходить $\frac{\pi}{6}$. Ситуация, когда какой-то из отрезков уже разветвился разобрана выше. Противоречие. 

%\input{pictures/norm2}

\end{itemize}
\end{proof}
\item Все точки $x^i_k$ принадлежат множеству $X_\Sigma$.

\begin{proof}
Предположим, что найдется точка $x^a_k$ из $E_\Sigma$. Тогда, согласно пункту~\ref{discr}, $\oord_{x^a_k}\Sigma = 2$, тогда, ввиду пункта~\ref{arc_par},  в $x^a_k$ входят две дуги, локально почти параллельные $(ax]$. Посмотрим на путь в $\Sigma$ от $x^a_k$ к $x$. Покажем, что он не может содержать точки ветвления до выхода из псевдоконуса $Q^a$. Предположим противное и обозначим за $A$ первую точку ветвления на пути (такая точка существует ввиду утверждения пункта~\ref{fsinite}). Тогда $A \in S_\Sigma$. И пусть --- $B$ последняя энергетическая точка на пути из $x^a_k$ в $A$ (может совпадать с $x^a_k$). Тогда путь из $B$ в $A$ является отрезком, причем, ввиду доказанного в пункте~\ref{arc_par}, отрезок $[BA]$ почти параллелен лучу $(ax]$.

Рассмотрим путь, начинающийся с отрезка $[BA]$ и продолжающийся отрезком $[AC]$, направленным от ребра $(bx]$, то есть его угол с ребром $(ax]$ составляет $\frac{\pi}{3}$. 
Ясно, что $C$ не может быть энергетической точкой степени один, поскольку это противоречит пункту~\ref{perp_edge2} и не может быть энергетической точкой степени два, поскольку это противоречит пункту~\ref{arc_par}, а значит $C$ --- точка ветвления. Повернем в точке $C$ в ту же сторону, что и в точке $A$. Угол нового отрезка с ребром $(ax]$ также составляет почти $\frac{\pi}{3}$. Рассматриваемый нами путь, в котором мы в каждом узле поворачиваем  от ребра $(bx]$, никогда не закончится (поскольку число пересечений $\partial B_\rho (x) \cap \Sigma$ конечно и значит можно выбрать $\rho>0$ таким, чтобы считать, что ни один путь не мог закончиться на $\partial B_\rho(x)$). Полученное противоречие влечет отсутствие точки ветвления на пути $x^i_k$ в $x$ до выхода из псевдоконуса $Q^a$. Пусть такой выход произошел (в противном случае несложно получить противоречие с условием $\oord_x \Sigma = 1$) и $G$ --- первая точка на пути из $x^a_k$ в $x$ такая, что $G\in \partial Q^a$ и 
\[
\forall \delta>0 \qquad (\Sigma \cap B_\delta(G)\cap Q^a \neq \emptyset)   \wedge (\Sigma \cap B_\delta(G)\setminus Q^a \neq \emptyset ). 
\]
Тогда путь продолжается отрезком $[GH]$, где $H\in Q^b$ и $\angle ((GH], (bx])=\alpha+o(\rho)$. Ясно, что точку $H$ можно считать точкой ветвления. Тогда от нее в сторону ребра $(ax]$ выходит отрезок $[HS]$ с углом $\angle ((HS], (ax])=\pi/3$. Но путь, начавшийся с отрезка $[HS]$ и содержащий только отрезки, имеющие угол с $(ax]$ почти $\pi/3$, никогда не закончится. Противоречие.
\end{proof}

%Заметим, что из доказанного следует, что все энергетические точки множества $G_\Sigma \cap B_{\rho}(x) \setminus x$ %изолированные, а значит можно выбрать последовательности $\{ x^i_k\}$ так, чтобы они содержали все точки %энергетические точки множества $G_\Sigma \cap B_{\rho}(x) \setminus x$, а также чтобы для последовательных точек %выполнялось неравенство $\dist (x, x^i_k) > \dist (x, x^i_{k+1})$.



%\end{proof}

\item Таким образом, $\Sigma$ --- локально минимальное штейнеровское дерево, без вершин степени $2$. Это означает, что отрезки $\Sigma$ могут быть только шести направлений. Но поскольку $\Sigma$ содержит отрезки, $o_\rho(1)$-почти перпендикулярные обоим ребрам $(ax]$ и $(bx]$, угол $\alpha = \angle axb$ может составлять только $\frac{\pi}{3}$ или $\frac{2\pi}{3}$.
%\end{enumerate}
\begin{itemize}


\item Пусть $\alpha := \frac{\pi}{3}$. Нарисуем розу ветров (см. определение~\ref{roza_v}), среди лучей которой есть перпендикуляры к обоим ребрам $x$. При этом, если расположить центр розы ветров во внутреннем угле $x$, то на лучах, перпендикулярных $(ax]$ ($(bx]$) и направленных к $(ax]$ ($(bx]$) стоит число $1$ (данная роза ветров изображена на Рисунке~\ref{fig:roza1}). 
 Выберем также достаточно малое $\rho_1<\rho$ так, чтобы $\sharp(\Sigma \cap \partial(B_{\rho_1}(x)))\leq 3$.

Тогда с одной стороны, ввиду Замечания~\ref{main_rose_property2}, сумма всех чисел во всех вершинах штейнеровского леса $\Sigma \cap (\overline{B_\rho(x)}\setminus B_{\rho_1}(x))$, равна $0$.

А с другой стороны, поскольку $\sharp(\Sigma \cap (\partial(B_\rho(x))\cup \partial(B_{\rho_1}(x)))\leq 6$, сумма сколь угодно велика, поскольку содержит бесконечно много положительных слагаемых и не больше шести отрицательных.
% присвоим каждой концевой вершине дерева число, соответствующее одному из шести направлений, и замет%им, что у любого локально минимального штейнеровского дерева сумма направлений будет нулевой. 
%Выберем такую малую окрестность $U(x)$, что $\sharp (\partial U(x) \cap \Sigma) = 1$, сопоставим обоим направлениям, %перпендикулярным $(ax]$ и $(bx]$ число $1$, и заметим, что можно выбрать такую окрестность $V(x)\subset U(x)$, что $%\sharp (\partial V(x) \cap \Sigma) = 1$ и что сумма направлений поддерева $\Sigma \cap (U(x)\setminus V(x))$ будет сколь %угодно велика, поскольку содержит много вершин положительных направлений и не больше двух отрицательных.  

%\input{pictures/roza1}

\item Пусть $\alpha := \frac{2\pi}{3}$. Повторим рассуждение из предыдущего пункта, взяв другую розу ветров (которая изображена на Рисунке~\ref{fig:roza2}: на луче, перпендикулярном $(ax]$ и направленном к нему, поставим $1$, а на луче, перпендикулярном $(bx]$ и направленном к нему, поставим $2$).

\input{pictures/roza2}
\end{itemize}
\end{enumerate}

Полученное противоречие завершает доказательство пункта.

\end{proof}

\item Завершение доказательства Леммы.
\label{finfin}
\begin{proof}
Поскольку $x\in E_\Sigma$ и ввиду Замечания~\ref{emptyball} пункта~\ref{netri} возможно два варианта:
\begin{enumerate}
    \item $x$ имеет одно энергетическое ребро
    Пусть $\rho$ такое, что $\sharp( \partial B_\rho(x) \cap \Sigma) \leq 3$, что возможно ввиду Замечания~\ref{ord_en}. Тогда посмотрим на замыкание множества $\Sigma \setminus Q$, где $Q$ --- псевдоконус энергетического ребра. Все концевые точки этого множества, кроме не более, чем $\oord_x \Sigma$, располагаются на $\partial Q$. Несложно заметить, что в таком случае можно считать, что $\sharp(\Sigma \cap \partial Q \cap  B_\rho(x)) <\infty$. Но тогда, не умаляя общности, можно считать $\Sigma \cap \partial Q \cap B_\rho(x)=\emptyset$. Тогда ввиду пункта~\ref{fsinite} и Замечания~\ref{rfinite} число точек ветвления в множестве $\Sigma \cap Q \cap  B_\rho(x)$ конечно. Конечно и число точек ветвления в множестве $\Sigma \cap  B_\rho(x) \setminus Q$, ввиду конечности числа концевых точек. Тогда, не умаляя общности, в множестве $\Sigma \cap B_\rho(x)$ нет точек ветвления и оно является объединением дуги $\breve{[qx]}$, лежащей в $Q$ и отрезков с одним концом в $x$ и другим на $\partial B_\rho (x)$. Поскольку биссектриса псевдоконуса $Q$ является односторонней касательной для $\breve{[qx]}\subset Q$, применима Лемма~\ref{angles2} и, значит, отрезок может быть только один, причем его угол с односторонней касательной $\breve{[qx]}$ составляет хотя бы $2\pi/3$. 
    Таким образом, в данном случае $\overline{B_\rho(x)} \cap \Sigma =\breve {qx} \cup [wx]$ или $\overline{B_\rho(x)} \cap \Sigma =\breve {qx}$, причем дуга $\breve{[qx]}$ имеет одностороннюю касательную и, в первом случае, ее угол с $[wx]$ составляет хотя бы $2\pi/3$.
    \item $x$ имеет два энергетических ребра.
        \begin{enumerate}
            \item[i] Хотя бы одно ребро направлено в обе стороны.
            В этом случае $\Sigma \cap B_\rho(x)$ является объединением двух множеств, каждое из которых содержится в каком-либо псевдоконусе с вершиной в $x$. Тогда к каждому из множеств можно применить пункт~\ref{fsinite} и Замечание~\ref{rfinite}. Таким образом, можно, считать, что множество $\Sigma \cap B_\rho(x)$ является объединением двух дуг, имеющих односторонние касательные с углом $\pi$ между этими касательными.
            \item[ii] Каждое ребро направлено в одну сторону. 
            Обозначим ребра $(ax]$ и $(bx]$, а соответствующие псевдоконусы за $Q^a$ и $Q^b$ (в процессе доказательства мы будем корректировать выбор псевдоконусов, не изменяя обозначений). Ввиду $\oord_x \Sigma < \infty$ и ввиду определения энергетического ребра, существует компонента связности $\Sigma \cap B_\rho(x)\setminus \{x\}$, содержащая бесконечное число энергетических точек ребра $(ax[$ (энергетических точек, принадлежащих псевдоконусу $Q^a$). Ввиду пункта~\ref{rozo4ki} можно так же считать, что эта компонента связности не содержит энергетических точек ребра $(bx]$ (энергетических точек, принадлежащих псевдоконусу $Q^b$). Повторяя рассуждения случая[А] доказательства пункта~\ref{fsinite} несложно убедиться, что тогда указанная компонента связности содержит не более, чем конечное число точек ветвления. А значит, можно считать, что не содержит точек ветвления вообще. Аналогичное верно для компоненты связности $\Sigma \cap B_\rho(x)\setminus \{x\}$, содержащей бесконечное число энергетических точек ребра $(bx[$ (энергетических точек, принадлежащих псевдоконусу $Q^b$). Таким образом, каждая из этих компонент связности является дугой, содержащей либо энергетические точки (принадлежащие соответствующему псевдоконусу), либо точки из $S_\Sigma$, являющиеся серединой отрезка. Несложно заметить, что тогда, ввиду определения энергетических ребер, каждая из указанных дуг содержится в некотором псевдоконусе энергетического ребра.
            
            Тогда энергетические ребра являются односторонними касательными указанных дуг, а значит к указанным дугам применима Лемма~\ref{angles2}. Тогда ясно, что угол между энергетическими ребрами $(ax]$ и $(bx]$ составляет хотя бы $2\pi/3$. Также несложно заметить, что $\Sigma \cap B_\rho(x)$ является объединением этих дуг (обозначим их $\breve{[qx]}$, $\breve{[sx]}$). В противном случае рассмотрим $\Sigma' \defeq \Sigma \setminus (\breve{[qx]} \cup \breve{[sx]})$. Тогда 
            \[
            \oord_x \Sigma'=\oord_x\Sigma -2 \leq 1
            \]
            (последнее неравенство верно ввиду Леммы~\ref{ord_en} и Замечания~\ref{rem_ord}).
            Если $\oord_x\Sigma'=1$, то существует дуга $\breve{[fx]} \subset B_\rho(x)$. Она, очевидно, не содержит точек ветвления и энергетических точек, кроме $x$, а значит является отрезком. Но тогда к ней применима Лемма~\ref{angles2} и, значит, дуга $\breve{[fx]}$ не может принадлежать $\Sigma$ одновременно с $\breve{[qx]}$ и $\breve{[sx]}$. То есть $\oord_x\Sigma'=0$, а значит найдется такая окрестность $U \ni x$, что $\Sigma' \cap \partial U=\emptyset$. Ввиду связности $\Sigma'$ найдется такой $\bar{\rho}>0$, что $\Sigma' \cap B_{\bar{\rho}}(x)=\emptyset$, то есть 
            \[
            \Sigma \cap B_{\bar{\rho}}(x)=\breve{[sx]}\cup \breve{[qx]}.
            \]
  
      \end{enumerate}
    
\end{enumerate}
\end{proof}
 
\end{enumerate}

\end{proof}

Таким образом, основная Лемма~\ref{main_l} доказана. 

%\begin{proof}
%\end{proof}



%завершает доказательство Теоремы~\ref{mainT1}.

